A stable added-mass partitioned (AMP) algorithm for elastic solids and incompressible flow: model problem analysis

A stable added-mass partitioned (AMP) algorithm is developed for fluid-structure interaction (FSI) problems involving viscous incompressible flow and compressible elastic-solids. The AMP scheme remains stable and second-order accurate even when added-mass and added-damping effects are large. The fluid is updated with an implicit-explicit (IMEX) fractional-step scheme whereby the velocity is advanced in one step, treating the viscous terms implicitly, and the pressure is computed in a second step. The AMP interface conditions for the fluid arise from the outgoing characteristic variables in the solid and are partitioned into a Robin (mixed) interface condition for the pressure, and interface conditions for the velocity. The latter conditions include an impedance-weighted average between fluid and solid velocities using a fluid impedance of a special form. A similar impedance-weighted average is used to define interface values for the solid. The fluid impedance is defined using material and discretization parameters and follows from a careful analysis of the discretization of the governing equations and coupling conditions near the interface. A normal mode analysis is performed to show that the AMP scheme is stable for a few carefully-selected model problems. Two extensions of the analysis in Banks et al. are considered, including a first-order accurate discretization of a viscous model problem and a second-order accurate discretization of an inviscid model problem. The AMP algorithm is shown to be stable for any ratio of solid and fluid densities, including when added-mass effects are large. The algorithm is verified for accuracy and stability for a set of new exact benchmark solutions where finite interface deformations are permitted. The AMP scheme is found to be stable and second-order accurate even for very difficult cases of very light solids.

==> tables/ElasticPistonConvergenceOld.tex <==
\begin{table}[H]
\caption{\label{fig:ElasticPistonConvergence}Elastic piston convergence tables for $\rhos/\rho = 10^3,\, \rhos/\rho=1,$ and $\rhos/\rho=10^{-3}.$
The parameters were chosen to be 
$\bar{H} = \frac{1}{2},\, H = 1,\, \mus=\lambdas=\rhos,\, \mu =0.01.$
The final time is $t_{\rm final} = 0.3.$}
\begin{center}
\begin{tabular}{c}
Heavy solid: $\rhos/\rho = 10^3$
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  5.0e-04 &      &  3.6e-05 &      &  3.9e-06 &      &  2.5e-05 &      &  2.2e-02 &     \\
1/ 40 &   105 &  8.9e-05 &  5.7 &  6.4e-06 &  5.6 &  1.1e-06 &  3.4 &  5.0e-06 &  4.9 &  3.5e-03 &  6.2 \\
1/ 80 &   208 &  1.4e-05 &  6.3 &  1.2e-06 &  5.5 &  3.1e-07 &  3.6 &  1.0e-06 &  4.8 &  7.0e-04 &  5.0 \\
1/160 &   416 &  1.8e-06 &  7.9 &  2.4e-07 &  4.9 &  8.0e-08 &  3.9 &  2.3e-07 &  4.5 &  1.8e-04 &  3.8 \\
\hline
\\
\end{tabular}

\begin{tabular}{c}
Medium solid: $\rhos/\rho = 1$
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  6.6e-05 &      &  6.0e-06 &      &  6.3e-06 &      &  1.7e-05 &      &  5.8e-05 &     \\
1/ 40 &   105 &  1.3e-05 &  5.1 &  5.6e-07 & 10.7 &  1.7e-06 &  3.6 &  2.1e-06 &  7.9 &  1.1e-05 &  5.4 \\
1/ 80 &   208 &  2.7e-06 &  4.9 &  4.4e-08 & 12.6 &  4.5e-07 &  3.9 &  2.7e-07 &  7.9 &  2.1e-06 &  5.2 \\
1/160 &   416 &  5.8e-07 &  4.6 &  8.5e-09 &  5.2 &  1.1e-07 &  4.0 &  4.4e-08 &  6.0 &  4.4e-07 &  4.8 \\
\hline
\\
\end{tabular}

% \caption{\label{fig:ElasticPistonConvergence}Convergence for elastic piston.\das{Placeholder for light solid $\rhos/\rho = 10^{-3}.$}}
\begin{tabular}{c}
Light solid: $\rhos/\rho = 10^{-3}$
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  9.2e-06 &      &  4.2e-06 &      &  7.8e-06 &      &  5.0e-06 &      &  4.3e-08 &     \\
1/ 40 &   105 &  2.3e-06 &  4.0 &  1.1e-06 &  3.9 &  1.9e-06 &  4.1 &  1.1e-06 &  4.6 &  1.0e-08 &  4.4 \\
1/ 80 &   208 &  5.9e-07 &  3.9 &  2.8e-07 &  3.9 &  4.8e-07 &  4.0 &  2.8e-07 &  3.8 &  2.2e-09 &  4.5 \\
1/160 &   416 &  1.5e-07 &  4.0 &  6.9e-08 &  4.0 &  1.2e-07 &  4.1 &  7.3e-08 &  3.9 &  5.0e-10 &  4.3 \\
\hline
\end{tabular}
\end{center}
\end{table}




% \begin{table}[H]
% \caption{\label{fig:ElasticPistonConvergenceHeavy}\das{Placeholder for heavy solid $\rhos/\rho = 10^3.$}}
% \begin{center}
% \begin{tabular}{ccccccccccc}
% \hline
% $h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
% \hline
% 1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
% 1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
% 1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
% 1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[H]
% \caption{\label{fig:ElasticPistonConvergenceMedium}Convergence for elastic piston.$\bar{H} = \frac{1}{2},\, H = 1,\, \rho = 1,\, \bar{\rho} = 1,\, \bar{\mu} = 10,\,
% \mu = .02.$ \das{Placeholder for medium solid $\rhos/\rho = 1.$} }
% \begin{center}
% \begin{tabular}{ccccccccccc}
% \hline
% $h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
% \hline
% 1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
% 1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
% 1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
% 1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[H]
% \caption{\label{fig:ElasticPistonConvergence}Convergence for elastic piston.\das{Placeholder for light solid $\rhos/\rho = 10^{-3}.$}}
% \begin{center}
% \begin{tabular}{ccccccccccc}
% \hline
% $h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
% \hline
% 1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
% 1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
% 1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
% 1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}


==> tables/ShearSolutionConvergenceOld.tex <==
\begin{table}[H]
\caption{\label{fig:ShearSolutionConvergence}Shear solution convergence tables for $\rhos/\rho = 10^3,\, \rhos/\rho=1,$ and $\rhos/\rho=10^{-3}.$
The parameters were chosen to be
$\bar{H} = \frac{1}{2}, H = 1, \rho = 1, \rhos = \mus = \lambdas = \mu$.
The final time is $t_{\rm final} = 0.3.$ }
\begin{center}
\begin{tabular}{c}
Heavy solid: $\rhos/\rho = 10^3$ 
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  5.9e-12 &      &  4.5e-04 &      &  1.9e-04 &      &  5.1e-04 &      &  9.8e-01 &     \\
1/ 40 &   105 &  1.2e-11 &  0.5 &  1.1e-04 &  4.0 &  4.6e-05 &  4.2 &  1.4e-04 &  3.6 &  2.6e-01 &  3.8 \\
1/ 80 &   208 &  3.2e-12 &  3.8 &  2.8e-05 &  4.0 &  1.1e-05 &  4.1 &  3.8e-05 &  3.7 &  6.5e-02 &  3.9 \\
1/160 &   416 &  7.0e-12 &  0.5 &  6.9e-06 &  4.0 &  2.8e-06 &  4.0 &  9.9e-06 &  3.8 &  1.6e-02 &  4.0 \\
\hline
\\
\end{tabular}

\begin{tabular}{c}
Medium solid: $\rhos/\rho = 1$ 
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  3.1e-16 &      &  1.4e-05 &      &  2.9e-06 &      &  1.1e-05 &      &  4.8e-05 &     \\
1/ 40 &   105 &  8.3e-16 &  0.4 &  3.3e-06 &  4.1 &  5.8e-07 &  5.0 &  2.0e-06 &  5.6 &  1.1e-05 &  4.2 \\
1/ 80 &   208 &  1.5e-15 &  0.6 &  8.1e-07 &  4.1 &  1.3e-07 &  4.5 &  4.8e-07 &  4.2 &  2.8e-06 &  4.0 \\
1/160 &   416 &  2.2e-15 &  0.7 &  2.0e-07 &  4.0 &  3.0e-08 &  4.3 &  1.2e-07 &  3.8 &  7.1e-07 &  4.0 \\
\hline
\\
\end{tabular}

\begin{tabular}{c}
Light solid: $\rhos/\rho = 10^{-3}$ 
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  2.9e-18 &      &  4.9e-05 &      &  7.5e-06 &      &  4.9e-05 &      &  5.0e-08 &     \\
1/ 40 &   105 &  3.4e-18 &  0.8 &  2.2e-05 &  2.3 &  3.7e-06 &  2.0 &  2.2e-05 &  2.3 &  2.2e-08 &  2.3 \\
1/ 80 &   208 &  5.9e-18 &  0.6 &  6.5e-06 &  3.3 &  1.2e-06 &  2.9 &  6.5e-06 &  3.3 &  6.5e-09 &  3.3 \\
1/160 &   416 &  9.6e-18 &  0.6 &  1.7e-06 &  3.9 &  3.4e-07 &  3.7 &  1.7e-06 &  3.9 &  1.7e-09 &  3.9 \\
\hline
\end{tabular}

\end{center}
\end{table}


==> texFiles/algorithm.tex <==
\section{The AMP algorithm} \label{sec:algorithm}

\input ../texFiles/ampAlg

In this section, the AMP interface conditions and time stepping algorithm are described.
Since the AMP interface conditions are derived in \cite{fibr2019}, 
we will briefly summarize the details.
Algorithm~\ref{alg:ampAlgorithm} lists the key steps for a 
fractional step predictor-corrector scheme with the AMP interface conditions.
This algorithm advances the solution from time step $t^n$ to $t^{n+1}$.
Difference operators such as $\grad_h$ and $\Delta_h$ represent discrete approximations
to their continuous counterpart. For the scheme used in this paper, second order 
finite differences are used in space.  \dws{[Making a note to be careful about stating what
discretizations we actually ``use'' in this paper.]}
The fluid domain is discretized into interior points $\iv \in \OmegaFh,$
boundary points $\iv \in \partial \OmegaFh,$ and interface points $\iv \in \GammaIfh.$
Similarly, the solid domain is discretized into interior points $\isv \in \OmegaSh,$
boundary points $\isv \in \partial \OmegaSh,$ and interface points $\isv \in \GammaIsh.$


The predictor consists of steps 1--5 and the corrector consists of steps 6--9.
During step 1, the solid displacement is predicted using a Lax-Wendroff type 
scheme and the solid velocity and stress are advanced using a Godunov type scheme.
In the scheme,
$\Qsv$ represents a state vector containing components of the solid velocity and stress,
$\Fsv_{m, \; \isv}^\pm$ represents the upwind fluxes corresponding to the 
$\xs_m$ coordinate direction, and $\Hsv_{\isv}^n$ represents the contribution from the body force.
In step 2, the solid displacement is used to compute the deformed fluid grid at time
$t^{n+1}.$
The fluid velocity is predicted in step 3. 
$\Nvh$ and $\Lvh$ represent grid operators associated with the explicit and implicit terms 
in the velocity update, respectively, given by
\ba
\Nvh(\vv_\iv,p_\iv) = - \bigl( (\vv_\iv - \dot{\xv}_\iv) \cdot \Grad \bigr) \vv_\iv 
- \frac{1}{\rho} \Grad \,p_\iv ,\qquad
\Lvh(\vv_\iv) = \nu \Delta_h \vv_\iv.
\ea
%
Here, $\dot{\xv}_\iv$ is the velocity of the grid. 
The explicit terms are advanced using an Adams-Bashforth scheme and the implicit terms
are advanced using Crank-Nicholson.
The interface equations used to obtain the boundary and ghost points make use of an 
predicted velocity, obtained from 
\ba
\Vv\sp{p}_h(\vv_\iv\sp{(p)}) \eqdef \vv_\iv^n + \frac{\dt}{2}\left(3\Nvh(\vv_\iv^ n,p_\iv^ n) - \Nvh(\vv_\iv^{n-1},p_\iv^{n-1})\right)
+ \frac{\dt}{2}\Big(\Lvh(\vv_\iv^{(p)}) + \Lvh(\vv_\iv^ n)\Big). \label{eq:veDef}
\ea
The fluid impedance, $\zf$, appears in this condition and is defined to be
\begin{align}
\zf = \rho v_f, \qquad v_f = \frac{2 \nu}{h} + \frac{h}{\dt },
\label{eq:zfAlgorithm}
\end{align}
%
where $h$ is taken to be the minimum grid spacing in the fluid.
The fluid impedance is derived in Section \ref{sec:monolithic} by analyzing a monolithic 
scheme applied to a simplified model problem.
\dws{[My vote would be not to give the algorithmic details that are used for the implementation
in FIBR, but rather give a higher-level description using ``function-type'' calls.  In this way
we can use the high-level description as a basis for the various implementations of the AMP algorithm
for the model problems, and also say that the full implementation for 2D with moving grids and
such is done in FIBR.  This approach also avoids the need for discussing the form for $z_f$ at this stage.]}
In step 4, the predicted pressure is obtained.
The last step of the predictor is step 5, where the interface velocity and traction 
are taken to be impedance weighted averages of the predicted interface values from the 
fluid and solid.
These interface values overwrite the values of the solid on the boundary. 
The fluid impedance is defined in equation \eqref{eq:zfAlgorithm}.
The corrector steps essentially mirror the predictor steps. 
One difference occurs in step 7, where the explicit terms in the fluid velocity 
update is corrected using an Adams-Moulton corrector.
Additionally in step 9, the solid velocity and traction are set equal to the 
current fluid values, so the fluid and solid interface values agree at the end of 
the corrector step.

% % ================================ ALGORITHM ============================================
% {
%     \def\alignspace{\hspace{1.2em}}
% \begin{algorithm}\caption{\rm Added-mass partitioned (AMP) scheme \das{make sure this agrees}
% \label{alg:ampAlgorithm}}\scriptsize
% \medskip
% \[
% \begin{array}{l}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hbox{// \textsl{Predictor steps}}\smallskip\\
% 1.\text{ Predict solid:}\\ 
% \alignspace 
% \begin{cases}
% \Usv_\isv^{(p)} = \Usv_\isv^n
% + \dt \Vsv_\isv^n
% + \frac{\dt^2}{2} \left(\Grads \cdot \Sigmasv_\isv^n - \bsv_\isv^n \right), 
% & \qquad \isv \in \OmegaSh. \\
% \Qsv_\isv^{(p)} = \Qsv_\isv^n 
% - \dt \sum_{m=1}^3 \frac{1}{\dxs_m} 
% \left( \Fsv_{m, \; \isv}^+ - \Fsv_{m, \; \isv}^- \right)
% + \dt \Hsv_{\isv}^n, & \qquad \isv \in \OmegaSh, \\
% \text{Solid boundary conditions on }\partial\OmegaSh\backslash\GammaIsh
% \end{cases} 
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \hbox{// \textsl{comment}}\smallskip\\
% 2.\text{ Predict fluid grid motion using $\Usv_\isv^{(p)}$ for $\isv \in \GammaIsh$.}
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \hbox{// \textsl{comment}}\smallskip\\
% 3.\text{ Predict fluid velocity:}\\ 
% \alignspace 
% \begin{cases}
% \vv_\iv^{(p)} = \vv_\iv^n + \frac{\dt}{2}\left(3\Nvh(\vv_\iv\sp n,p_\iv\sp n) - \Nvh(\vv_\iv\sp{n-1},p_\iv\sp{n-1})\right)
% + \frac{\dt}{2}\left(\Lvh(\vv_\iv\sp{(p)}) + \Lvh(\vv_\iv\sp n)\right),
%    & \qquad \iv \in \OmegaFh\backslash\GammaIfh, \\
%  \tnv_m^T \tauv_{\iv}^{(p)} \nv + \zs \tnv_m^T \vv_\iv^{(p)} =
%  \tnv_m^T \Sigmasv_\isv^{(p)} \nv
% + \zs \tnv_m^T \Vsv_{\isv}^{(p)}
% ,  \qquad m = 1,2,
%  & \qquad\iv \in \GammaIfh, \; \isv \in \GammaIsh,  \\
% \Grad\cdot\vv_\iv\sp{(p)}=0,
%  & \qquad \iv \in \GammaIfh, \\
%  \nv^T\vv_\iv^{(p)}=\f{\hat{\zf}}{\hat{\zf}+\zp}\nv^T\vv_\iv^{(e)}+ \f{\zp}{\hat{\zf}+\zp}\nv^T\vsv_\isv^{(p)}, \qquad \phantom{m = 1,2,} & \qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh, \\
% %
% \tnv_m^T\vv_\iv^{(p)}=\tnv_m^T\vv_\iv^{(e)},  \qquad m = 1,2, & \qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh, \\
% \text{Velocity boundary conditions on $\partial \OmegaFh \backslash \GammaIfh$.}
% \end{cases}
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \hbox{// \textsl{comment}}\smallskip\\
% 4.\text{ Predict fluid pressure:}\\ 
% \alignspace 
% \begin{cases}
% \Delta_h p_\iv^{(p)} = -\rho \Grad \vv_\iv^{(p)} : \left(\Grad \vv_\iv^{(p)}  \right)^T,
% &\qquad \iv \in \OmegaFh, \\
% -p_\iv^{(p)}
% -\frac{\zp \dt}{\rho} (\nv\cdot\Grad) p_\iv^{(p)}
% = 
% \nv^T \left(\Sigmasv_\isv^{(p)} \nv - \tauv_\iv^{(p)} \nv\right) 
% + \zp \dt
%  \nv^T \left(\nu \Grad \curl \Grad \curl \vv_\iv^{(p)} + (\vsv_t)_\isv^{(p)}\right), &\qquad \iv \in \GammaIFh, \\
% \text{Pressure boundary conditions on $\partial \OmegaFh \backslash \GammaIfh$.}
% \end{cases}
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \hbox{// \textsl{comment}}\smallskip\\
% 5.\text{ Predict solid interface:}\\ 
% \alignspace 
% \begin{cases}
% \nv^T \Vsv_\isv^I = \frac{\zf}{\zf+\zp} \nv^T \vv_\iv^{(p)}
%      + \frac{\zp}{\zf+\zp} \nv^T \Vsv_\isv^{(p)} 
%      + { \f{1}{\zf+\zp}\Big( \nv^T\Sigmasv^{(p)}_\iv\nv - \nv^T\Sigmav^{(p)}_\iv\nv \Big)},
%      &\qquad \isv \in \GammaIsh, \iv \in \GammaIfh,\\
% %
% \tv_m^T \Vsv_\isv^I = \frac{\zf}{\zf+\zs} \tv_m^T \vv_\iv^{(p)}
%      + \frac{\zs}{\zf+\zs} \tv_m^T \Vsv_\isv^{(p)}
%      + { \f{1}{\zf+\zs}\Big( \tv_m^T\Sigmasv^{(p)}_\iv\nv - \tv_m^T\Sigmav^{(p)}_\iv\nv \Big)},
%      &\qquad \isv \in \GammaIsh, \iv \in \GammaIfh,\\
% %
% \nv^T \Sigmasv^I_{\isv} \nv = \frac{\zf^{-1}}{\zf^{-1}+\zp^{-1}}\nv^T\Sigmav^{(p)}_\iv \nv
% + \frac{\zp^{-1}}{\zf^{-1}+\zp^{-1}} \nv^T\Sigmasv^{(p)} \nv
% + { \f{1}{\zf^{-1}+\zp^{-1}}\Big( \nv^T\vsv^{(p)}_\iv - \nv^T\vv^{(p)}_\iv \Big)},
%      &\qquad \isv \in \GammaIsh, \iv \in \GammaIfh. \\
% %
% \tv_m^T \Sigmasv^I_{\isv} \nv = \frac{\zf^{-1}}{\zf^{-1}+\zs^{-1}}\tv_m^T\Sigmav^{(p)}_\iv \nv
%     + \frac{\zs^{-1}}{\zf^{-1}+\zs^{-1}} \tv_m^T\Sigmasv^{(p)} \nv
%     + { \f{1}{\zf^{-1}+\zs^{-1}}\Big( \tv_m^T\vsv^{(p)}_\iv - \tv_m^T\vv^{(p)}_\iv \Big)},
%         &\qquad \isv \in \GammaIsh, \iv \in \GammaIfh.
% \end{cases}
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hbox{// \textsl{Corrector steps}}\smallskip\\
% 6.\text{ Correct fluid grid motion.}
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \hbox{// \textsl{comment}}\smallskip\\
% 7.\text{ Correct fluid velocity:} \\
% \alignspace 
% \begin{cases}
% \vv_\iv^{n+1} = \vv_\iv^n + \frac{\dt}{2}\left(\Nvh(\vv_\iv^{(p)},p_\iv^{(p)}) + \Nvh(\vv_\iv^{n},p_\iv^{n})\right)
% + \frac{\dt}{2}\left(\Lvh(\vv_\iv^{n+1}) + \Lvh(\vv_\iv^ n)\right),
% &\qquad    \iv \in \OmegaFh\backslash\GammaIfh, \\
%  \tnv_m^T \tauv_{\iv}^{n+1} \nv + \zs \tnv_m^T \vv_\iv^{n+1} =
%  \tnv_m^T \Sigmasv_\isv^{n+1} \nv
% + \zs \tnv_m^T \Vsv_{\isv}^{n+1}
% ,  \qquad m = 1,2,
%  & \qquad\iv \in \GammaIfh, \; \isv \in \GammaIsh,  \\
% \Grad\cdot\vv_\iv\sp{n+1}=0,
%  & \qquad \iv \in \GammaIfh, \\
%  \nv^T\vv_\iv^{n+1}=\f{\hat{\zf}}{\hat{\zf}+\zp}\nv^T\vv_\iv^{(e)}+ \f{\zp}{\hat{\zf}+\zp}\nv^T\vsv_\isv^{n+1} +{1\over\hat{\zf}+\zp}\nv^T\bigl((\sigmasv\nv)_\isv^{n+1}-(\sigmav\nv)_\iv^{(p)}\bigr),  & \qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh, \\
% %
% \tnv_m^T\vv_\iv^{n+1}=\tnv_m^T\vv_\iv^{(e)},  \qquad m = 1,2, & \qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh, \\
% \text{Velocity boundary conditions on $\partial \OmegaFh \backslash \GammaIfh$.}
% \end{cases}
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \hbox{// \textsl{comment}}\smallskip\\
% 8.\text{ Correct fluid pressure.}
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \hbox{// \textsl{comment}}\smallskip\\
% 9.\text{ Correct solid interface.}
% \medskip\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \end{array}
% \]
% \label{alg:ampRB}
% \end{algorithm}
% }



==> texFiles/exactSolutions.tex <==
\section{Exact solutions} 

\das{DAS: Are we putting the exact solutions in this paper???}
In this section, we discuss various exact solutions to the FSI problem.
These exact solutions are used to test and verify the AMP algorithm in
section \ref{sec:numericalResults}.

\subsection{Rectangular elastic piston} \label{sec:ElasticPiston}

%\input texFiles/rectangularGeometryNumericalResults

The geometry of the rectangular elastic piston is shown in figure
\ref{fig:rectangularModelProblemNumericalResults}.
We consider 1D longitudinal motions in the $y$ dimension. The horizontal fluid velocity, $v_1,$ 
solid displacement, $\us_1,$ and derivatives with respect to $x$ are all zero.
With this simplification, the vertical fluid velocity is equal to the interface velocity everywhere in the domain, $v_2 = v_2(t)$,
and the pressure is a time-dependent linear interpolant between the interface pressure, $p_I(t),$ and the specified boundary pressure at $y=H$, $p_0(t)$. 
The solid boundary at $y=-\Hs$ is held fixed so that $\us_2 = 0.$ The fluid and solid equations simplify to 
\begin{alignat}{2}
\dot{v}_{2}(t) &= - \frac{p_0(t) - p_I(t)}{\rho H} 
\bigg{/}\left(1 - \frac{y_{I}(t)}{H}\right), \quad &&y \in (y_I(t),H)
\label{eq:ElasticPistonMomentum} \\
\bar{u}_{2,tt} &= \bar{c}_p^2 \bar{u}_{2,\bar{y}\bar{y}}, \quad &&\ys \in (-\Hs,0)
\label{eq:LongitudinalWaveEquation}
\end{alignat}
%
where $y_I(t) = u_2(0,t)$ is the solid interface deformation. 
Equation \eqref{eq:ElasticPistonMomentum} implies that the (uniform) fluid velocity is driven by a pressure gradient 
and equation \eqref{eq:LongitudinalWaveEquation} is a longitudinal wave equation for the solid displacement.
The interface conditions are
\begin{align}
v_2(t) &= \dot{y}_I(t) \\
(\lambdas + 2 \mus) \us_{2,\bar{y}}(0,t) &= -p_I(t).
\end{align}
%
The fluid variables can be eliminated from equation \eqref{eq:ElasticPistonMomentum} 
to obtain a boundary condition at the interface for $\us.$
\begin{align}
\us_{tt}(0,t) = - \frac{p_0(t) + (\lambdas+2\mus)\us_\ys(0,t)}{\rho H} \bigg{/}
\left(1 - \frac{\us(0,t)}{H} \right)
\label{eq:NonlinearInterfaceCondition}
\end{align}
%
In general, the nonlinear initial-boundary value problem may not be solvable. When 
$\us(0,t)/H$ is small, an asymptotic solution may be obtained. Instead, we 
manufacture an exact solution by finding $p_0$
for a given solid displacement.
Let the solid displacement be given by
\begin{align}
\bar{u}_2(\ys,t) = F(t + (\ys+\Hs)/\cp ) -  F(t - (\ys+\Hs)/\cp),
\end{align}
% 
for any smooth function $F$.
This satisfies both the wave equation and the displacement boundary 
condition at $\ys=-\Hs$. 
% Given this solution, the interface quantities are computed
% \begin{align}
% y_I(t) &= A \sin(k\bar{H}) \cos(\bar{c}_p k t + \phi_0) \\
% v_{2,I}(t) &= -A \bar{c}_p k \sin(k\bar{H}) \sin(\bar{c}_p k t + \phi_0) \\
% p_I(t) = -\sigma_{22,I}(t) &=  
% - A (\bar{\lambda} + 2 \bar{\mu}) \bar{c}_p k
% \, \wdh{\cos(k\bar{H})} \cos(\bar{c}_p k t + \phi_0).
% \end{align}
% %
% Using \eqref{eq:NonlinearInterfaceCondition}, the pressure at $y=H$ is given by
% \begin{align}
% p_0(t) = p_I(t) - \rho H \dot{v}_{2,I}(t) \left(1 - \frac{y_I(t)}{H}\right)
% \end{align}
% %
% and the exact pressure is given by
% \begin{align}
% p(y,t) = p_0(t) - \frac{p_0(t) - p_I(t)}{H - y_I(t)} (H - y).
% \end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ramp function here:
Given this solution, the interface quantities are computed to be
\begin{align}
y_I(t) &= F(t + \Hs/\cp ) -  F(t - \Hs/\cp),  \\
% \dot{y}_{I}(t) &= \us_{2,t}(0,t) =  F'(t + \Hs/\cp ) -  F'(t - \Hs/\cp), \\
% \ddot{y}_{I}(t) &=  F''(t + \Hs/\cp ) -  F''(t - \Hs/\cp),\\
p_I(t) &= 
       -\f{\lambdas+2\mus}{\cp} \, \Big( F'(t + \Hs/\cp ) +  F'(t - \Hs/\cp) \Big).
\end{align}
%
Using \eqref{eq:NonlinearInterfaceCondition}, the $p_0(t)$ is given by
\begin{align}
p_0(t) = p_I(t) - \rho H \ddot{y}_{I}(t) \left(1 - \frac{y_I(t)}{H}\right) ,
\end{align}
%
and the exact pressure is given by
\begin{align}
p(y,t) = p_0(t) - \frac{p_0(t) - p_I(t)}{H - y_I(t)} (H - y).
\end{align}
%
The fluid velocity and solid stress are then given by
\begin{align}
v_2(y,t) &= \dot{y}_{I}(t), \\
    \sigmas_{22}(\ys,t) &= 
               \f{(\lambdas+2\mus)}{\cp} \, \Big( F'(t + (\ys+\Hs)/\cp ) +  F'(t - (\ys+\Hs)/\cp) \Big).
\end{align}
%
This solution is valid for any smooth $F$. We choose
\begin{align}
  & F(\xi) = \alpha \,\sin(2\pi k (\xi - \phi_0)),
\end{align}
%
It can be shown that the interface displacement at $t=0$ is given by
\begin{align}
   y_I(0) %&=  F(\Hs/\cp ) -  F(-\Hs/\cp) = \alpha \,
          %    \Big( \sin(2\pi k (\Hs/\cp - \phi_0)) - \sin(2\pi k (-\Hs/\cp - \phi_0))\Big) , \\ 
      &= 2 \alpha \, \sin(2 \pi k \Hs/\cp) \, \cos(2\pi k  \phi_0).
\end{align}
% 
We choose $\phi_0=1/(4 k)$ so the interface is initially undeformed. 


% \das{here we describe the ramp function, but it seems like we don't use a ramp function in code}
%
% This solution is valid for any smooth $F$. We choose
% \begin{align}
%   & F(\xi) = \alpha \, R(\xi) \,\sin(2\pi k (\xi - \phi_0)),
% \end{align}
% %
% where $R(\xi)$ is a ramp function that smoothly transitions from zero to one.
% A ramp function is used to avoid initialization issues with moving grids. The ramp 
% function is given by
% \begin{align}
% R(t) = 
% \begin{cases}
% 0, & t < 0\\
% (9+(-12+(3+t)t)t)t^3 & 0 \le t \le 1\\
% 1, & t > 1
% \end{cases}.
% \end{align}
% %
% This satisfies $R'(0) = R''(0) = R'(1) = R''(1) = 0,$ so the 
% velocity and acceleration are continuous.

% The {\tt rampOrder} defines the number of zero derivatives at the ramp interval ends. It is
% needed to have at least 2 zero derivatives 
% so the acceleration is continuous.
% We need to have the ramp function satisfy
% \[
%    F(\xi)=0 ~~\text{for}~~ \xi \le (\ys+\Hs)/\cp \le \Hs/\cp. 
% \] 
% With no ramp function, $R(\xi)=1$, the interface will be at $\ys=0$ at $t=0$ provided
% \begin{align}
%    \us_2(\ys,t) &=  F(\Hs/\cp ) -  F(-\Hs/\cp) = \alpha \,
%               \Big( \sin(2\pi k (\Hs/\cp - \phi_0)) - \sin(2\pi k (-\Hs/\cp - \phi_0))\Big) , \\ 
%       &= 2 \alpha \, \sin(2 \pi k \Hs/\cp) \, \cos(2\pi k  \phi_0).
% \end{align}
% % 
% and we can choose $\phi_0=1/(4 k)$. For a second-order accurate solution 
% we may need the ramp to have
% at least two, and maybe three?, or four ?, continuous derivatives, $R(0)=R'(0)=R''(0)=R'''(0)=R''''(0)=0$. 


% $r_a = -10, r_b = -9$

\subsection{Rectangular shear solution} \label{sec:ShearSolution}


The geometry of the rectangular shear solution is identical to that of the 
elastic piston and is shown in figure \ref{fig:rectangularModelProblemNumericalResults}.
We consider pure transverse motions in the fluid and solid.
The vertical fluid velocity, $v_2,$ solid displacement, $\us_2,$
and derivatives with respect to $x$ are all zero. Since there is no 
longitudinal displacement, (ie. $y_I(t) = 0$), the solid reference coordinate $\ys$ is 
equivalent to the physical coordinate $y.$
The equations simplify to
\begin{alignat}{2}
\rho v_{1,t} &= \mu v_{1,yy}, \quad &&y \in (0,H) 
\label{eq:HeatEquationFluid} \\
\us_{1,tt} &= \cs^2 \bar{u}_{1,yy}, \quad &&y \in (-\bar{H},0).
\label{eq:ShearWaveEquation}
\end{alignat}
%
Equation \eqref{eq:HeatEquationFluid} is a heat equation for the horizontal fluid velocity 
and equation \eqref{eq:ShearWaveEquation} is a shear wave equation for the horizontal solid displacement.
These equations can be solved by searching for solutions of the form
\begin{align}
v_1(y,t) = \hat{v}_1(y) e^{i \omega t}, \quad \us_1(y,t) = \hat{\us}_1(y) e^{i \omega t}. 
\end{align}
%
The equations are simplified to second order constant coefficient ODEs in $y$, given by
\begin{align}
\hat{v}_1'' + \lambda^2 \hat{v}_1 &= 0, \\
\hat{\us}_1'' + k_s^2 \hat{\us}_1 &= 0,
\end{align}
%
where
\begin{align}
\lambda^2 = - \frac{i \rho \omega}{\mu}, \quad k_s^2 = \frac{\omega^2}{\cs^2}.
\end{align}
%
The solutions are
\begin{align}
\hat{v}_1(y) &=  a_1 \sin(\lambda (H-y)) + a_2 \cos(\lambda (H-y)), \\
\hat{\us}_1(y) &= b_1 \sin(k_s (y+\Hs)) +b_2 \cos(k_s (y+\Hs)),
\end{align}
%
where $a_1,a_2,b_1,b_2$ are constants to be determined by the boundary conditions.
At the solid boundary, $y = -\Hs,$ the solid is fixed so that $\us_1 = 0$.
A no-slip boundary condition, $v_1 = 0$, is applied at the fluid boundary, $y = H.$
These two conditions imply that $a_2=b_2=0.$
The interface matching conditions are
\begin{alignat}{2}
v_1(0,t) &= \us_{1,t}(0,t),  \\
\mu v_{1,y}(0,t) &= \mus \us_{1,y}(0,t).
\end{alignat}
%
The interface conditions form a homogeneous system of equations for 
$a_1$ and $b_1,$ given by
\begin{align}
\left[\begin{array}{cc}
\sin(\lambda H) & -i \omega \sin(k_s \Hs) \\
-\mu \lambda  \cos(\lambda H) & -\mus k_s \cos(k_s \Hs)
\end{array}\right]
\left[\begin{array}{c}
a_1 \\ b_1
\end{array}\right]
= 0 \label{eq:ShearSolutionSystem}
\end{align}
%
In order for nontrivial solutions for $a_1$ and $b_1$ to exist, the system must be singular.
It can be shown that solutions exist when the following dispersion relation is satisfied.
\begin{align}
\frac{\mus}{\mu \omega} \tan(\lambda H) =-  \frac{i \lambda}{k_s} \tan(k_s \Hs) 
\end{align}
%
This is a condition on $\omega$.
There seems to infinitely many solutions where $\Re(\omega) > 0$
and $\Im(\omega) > 0.$ These solutions correspond to interface oscillations which damp in time. 
Equation \ref{eq:ShearSolutionSystem} can be used to find $a_1$ and $b_1$ up to a scale factor,
namely
\begin{align}
\frac{a_1}{b_1} = i \omega \frac{\sin(k_s \Hs)}{\sin(\lambda H)}.
\end{align}
%
An extra condition is needed to determine the constants uniquely. 
The initial interface displacement is chosen to be $\us_1(0,0) = \us_{\max},$
which gives
\begin{align}
b_1 = \frac{\us_{\max}}{\sin (k_s \Hs)}.
\end{align}


\subsection{Radial elastic piston} \label{sec:RadialElasticPiston}

The radial elastic piston is the analogous solution to the rectangular elastic piston in
polar coordinates. We first define the polar basis vectors to be
\begin{align}
\ev_r = 
\left[\begin{array}{c}
\cos(\theta) \\ \sin(\theta)
\end{array}\right], \quad
\ev_\theta = 
\left[\begin{array}{c}
-\sin(\theta) \\ \cos(\theta)
\end{array}\right].
\end{align}
%
Subscripts $r$ and $\theta$ will be used to denote components of a vector and tensor, (ie.
$\vv = v_r \ev_r + v_\theta \ev_\theta$
and 
$\sigmav = \sigma_{rr} \ev_r \ev_r^T 
+ \sigma_{r\theta} \ev_r \ev_\theta^T
+ \sigma_{\theta r} \ev_\theta \ev_r^T
+ \sigma_{\theta\theta} \ev_\theta \ev_\theta^T$).


\input texFiles/radialElasticPistonGeometry

The geometry of the radial elastic piston solution is shown in figure \ref{fig:radialElasticPistonGeometry}.
Axisymmetric radial motions of the fluid and solid are considered.
The circumferential components of the fluid velocity, $v_\theta,$ and solid displacement, $\us_\theta$, are zero.
Under this assumption, the fluid continuity equation \eqref{eq:fluidContinuity} reduces to 
\begin{align}
\frac{1}{r} \frac{\partial }{\partial r} (r v_r) = 0, \quad r \in (R_I(t),R_f),
\end{align}
%
where $R_I(t)$ is the radial location of the interface.
The solution for the radial component of the fluid velocity is of the form
\begin{align}
v_r(r,t) = \frac{1}{r} f(t)
\end{align}
%
where $f(t)$ is some function of time, determined by a boundary condition.
The radial component of the fluid momentum equation \eqref{eq:fluidMomentum} reduces to
\begin{align}
\frac{\partial p}{ \partial r} = 
\frac{\rho}{r^3} f(t)^2 
- \frac{\rho}{r} f'(t), \quad r \in (R_I(t),R_f).
\end{align}
%
This equation can be integrated to solve for the pressure,
\begin{align}
p(r,t) = g(t) - \frac{\rho}{2r^2} f(t)^2 - \rho f'(t) \log \left( \frac{r}{R_I(I)} \right),
\label{eq:radialPistonPressure}
\end{align}
%
where $g(t)$ is the constant of integration which will be determined by boundary condition on pressure at $r=R_f.$
The solid equations simplify to a wave equation for the radial component of displacement,
\begin{align}
\frac{\partial^2 \us_r}{\partial t^2} = 
\cp^2 \frac{\partial}{\partial \rs} 
\left(  \frac{1}{\rs} \frac{\partial (\rs \us_r)}{\partial \rs}\right), \quad \rs \in (0,R_I(0))
\label{eq:radialWaveEquation}
\end{align}
%
We require the solid displacement remain bounded at $\rs=0.$
Equations \eqref{eq:radialPistonPressure} and \eqref{eq:radialWaveEquation} are 
the counterpart in polar coordinates to equations \eqref{eq:ElasticPistonMomentum} and \eqref{eq:LongitudinalWaveEquation}, respectively.
The interface matching conditions are given by
\begin{align}
v_r(R_I(t),t) &= \vs_r(R,t), \\
 \sigma_{rr}(R_I(t),t) &= \sigmas_{rr}(R,t).
\end{align}
%
Instead of solving the general initial boundary value problem, 
we `choose' a form of solution for the solid and determine $f(t)$ and $g(t)$ so that the equations are satisfied.
We look for solutions where the solid displacement is sinusoidal in time.
\begin{align}
\us_r(\rs,t) = \hat{\us}(\rs) \sin(\cp k t)
\end{align}
%
After substituting into equation \eqref{eq:radialWaveEquation}, 
a Bessel equation for $\hat{\us}(\rs)$ is obtained.
\begin{align}
\rs^2 \hat{\us}'' + \rs \hat{\us}' + (k^2 \rs^2 - 1) \hat{\us} = 0
\end{align}
%
Both $J_1(k\rs)$ and $Y_1(k\rs)$ are solutions to this equation, but only $J_1(k\rs)$ remains bounded at $\rs=0,$
therefore the solution for the solid displacement is 
\begin{align}
\us_r(\rs,t) = \us_0 J_1(k\rs) \sin(\cp k t).
\end{align}
%
The solid velocity and stress are given by
\begin{align}
\vs_r(\rs,t) &= \cp k \us_0 J_1(k \rs) \cos(\cp k t) \\
\sigmas_{rr}(r,t) &= 
 u_0 \sin(\cp k t) \left[ \frac{\lambdas}{r} J_1(k \rs)
+ k (\lambdas+ 2 \mus) J_1'(k \rs)\right].
\end{align}
%
The velocity matching condition is used to obtain $f(t)$, given by
\begin{align}
f(t) =  R_I(t) \; \vs_r(R,t).
\end{align}
%
Using the definition of the fluid stress tensor in equation \eqref{eq:fluidStressTensor},
the fluid stress is given by
\begin{align}
\sigma_{rr}(r,t) = 
-g(t) + \frac{\rho}{2r^2} f(t)^2 + \rho f'(t) \log \left( \frac{r}{R_I(I)} \right)
- \frac{2 \mu}{r^2} f(t).
\end{align}
%
The stress matching condition is then used to obtain $g(t)$.
\begin{align}
g(t) = 
\frac{\rho}{2R_I(t)^2} f(t)^2 - \frac{2 \mu}{R_I(t)^2} f(t)
-\sigmas_{rr}(R,t)
\end{align}

\subsection{Radial shear solution} \label{sec:RadialShearSolution}

The geometry of the radial shear solution is identical to that of the elastic piston 
geometry shown in figure \ref{fig:radialElasticPistonGeometry}, except we consider 
the interface radius to be constant for all time, $R_I(t) = R.$
We consider axisymmetric circumferential motions of the fluid and solid.
The radial component of the fluid velocity, $v_r$, and solid displacement, $\us_r$, is zero.
Under these assumptions, the equations reduce to
\begin{alignat}{2}
\rho \frac{\partial v_\theta}{\partial t} &= 
\mu \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r v_\theta)}{\partial r}\right), \quad &&r \in (R,R_f)
\label{eq:radialHeatEquation} \\
\frac{\partial^2 \us_\theta}{\partial t^2} &= \cs^2 \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r \us_\theta)}{\partial r}\right), \quad &&r \in (0,R)
\label{eq:radialShearWaveEquation}
\end{alignat}
%
Equation \eqref{eq:radialHeatEquation} is a heat equation for the circumferential fluid velocity
and equation \eqref{eq:radialShearWaveEquation} is a wave equation for the circumferential 
solid displacement. These equations are analogous to equations \eqref{eq:HeatEquationFluid}
and \eqref{eq:ShearWaveEquation} obtained for the rectangular shear solution.
We search for solutions of the form
\begin{align}
v_\theta(r,t) = \hat{v}_\theta(r) e^{i \omega t}, \quad
\us_\theta(r,t) = \hat{\us}_\theta(r) e^{i \omega t}
\end{align}
%
The fluid and solid equations simplify to Bessel equations given by
\begin{align}
r^2 \hat{v}_\theta'' + r \hat{v}_\theta' + (\lambda^2 r^2 - 1) \hat{v}_\theta &= 0\\
r^2 \hat{\us}_\theta'' + r \hat{\us}_\theta' + (k_s^2 r^2 - 1) \hat{\us}_\theta &= 0 ,
\end{align}
%
where
\begin{align}
\lambda^2 = - \frac{i \rho \omega}{\mu}, \quad k_s^2 = \frac{\omega^2}{\cs^2}.
\end{align}
%
$\lambda$ and $k_s$ are the same constants that arise in the rectangular shear solution.
Define
% \begin{align}
% \hat{v}_\theta(r,t) &= a_1 (Y_1(\lambda R_f) J_1(\lambda r) - J_1(\lambda R_f) Y_1(\lambda r))
% + a_2 (Y_1(\lambda R_f) J_1(\lambda r) + J_1(\lambda R_f) Y_1(\lambda r)),\\
% \hat{\us}_\theta(r,t) &= b_1 J_1(k_s r) + b_2 Y_1(k_s r),
% \end{align}
\newcommand{\B}{B}
\newcommand{\C}{C}
\begin{align}
\B(\xi) = Y_1(\lambda R_f) J_1(\xi) - J_1(\lambda R_f) Y_1(\xi) \\
\C(\xi) = Y_1(\lambda R_f) J_1(\xi) + J_1(\lambda R_f) Y_1(\xi),
\end{align}
%
then the solutions for the transformed variables are
\begin{align}
\hat{v}_\theta(r,t) &= a_1 \B(\lambda r) + a_2 \C(\lambda r)\\
\hat{\us}_\theta(r,t) &= b_1 J_1(k_s r) + b_2 Y_1(k_s r),
\end{align}
%
where $a_1,a_2,b_1,b_2$ are constants to be determined by the boundary conditions.
At $r=0,$ we enforce that the solid solution is bounded. 
At the fluid boundary, $r=R_f$, a no-slip boundary condition is applied, $\hat{v}_\theta = 0.$
Due to these conditions, we must take $a_2=b_2=0.$

Two interface conditions are required. The interface position in Eulerian coordinates is given by
$\xv_I = R \ev_r + \us_\theta(R,t) \ev_\theta.$ Since $|\xv_I|^2 - R^2 = |\us_\theta(R,t)|^2$,
the radial coordinate of the interface increases when $|\us_\theta|$ is non-zero. 
We ignore this `warping' effect by considering the case when $\frac{|\us_\theta|}{R} \ll 1$.
The interface matching conditions are
\begin{align}
v_\theta(R,t) = \vs_\theta(R,t), \\
\sigma_{r\theta}(R,t) = \sigmas_{r\theta}(R,t) .
\end{align}
%
As in the rectangular shear case, the interface conditions 
form a homogeneous system of equations for $a_1$ and $b_1,$ given by
\begin{align}
\left[\begin{array}{cc}
\B(\lambda R) & - i \omega J_1(k_s R) \\
\mu \left(\lambda \B'(\lambda R) - \frac{\B(\lambda R)}{R} \right) & 
-\mus \left( k_s J_1'(k_s R) - \frac{J_1(k_s R)}{R}\right)
\end{array}\right]
\left[\begin{array}{c}
a_1 \\ b_1
\end{array}\right]
= 0. \label{eq:RadialShearSystem}
\end{align}
%
In order for nontrivial solutions for $a_1$ and $b_1$ to exist, the system must be singular.
It can be shown that solutions exist when the following dispersion relation is satisfied.
\begin{align}
\frac{\mus}{\omega \mu} \left(\frac{J_1'(k_s R)}{J_1(k_s R)} - \frac{1}{R k_s} \right)
= \frac{i \lambda}{k_s} \left(\frac{\B'(\lambda R)}{\B(\lambda R)} - \frac{1}{R \lambda} \right) 
\end{align}
%
This is a condition for $\omega.$
As in the case of the Cartesian shear solution, there are infinitely many solutions
corresponding to interface oscillations which damp in time.
Equation \eqref{eq:RadialShearSystem} can be used to determine the two constants up 
to a scale factor, namely
\begin{align}
\frac{a_1}{b_1} = i \omega \frac{J_1(k_s R)}{B(\lambda R)}.
\end{align}
%
The initial interface displacement, $\us_{\theta}(R,0) = \us_{\max},$ 
is then given as a final condition giving
\begin{align}
b_1 = \frac{\us_{\max}}{J_1(k_s r)}.
\end{align}
%
After obtaining the solution for the fluid velocity, the pressure can be obtained
by solving 
\begin{align}
- \frac{\rho}{r} v_\theta^2 + \frac{\partial p}{\partial r} &= 0 .
\end{align}
%
Since the radial component of momentum is zero, the centripetal force 
in the fluid must be balanced by the pressure gradient.
A final interface condition arises by setting $\sigma_{rr} = \sigmas_{rr}$ at the
interface. Since $\sigmas_{rr}=0$ and the only contribution to $\sigma_{rr}$
is from the fluid pressure, this interface condition becomes
\begin{align}
p(R,t) = 0.
\end{align}
%
The solution for the pressure is thus given by
\begin{align}
p(r,t) = \rho \int_R^r \frac{v_\theta(s,t)^2}{s} \; ds.
\end{align}


\subsection{Radial traveling wave solution} \label{sec:RadialTravelingWave}

\input texFiles/radialTravelingWaveGeometry
The geometry for the radial traveling wave solution is shown in figure \ref{fig:radialTravelingWaveGeometry}.
Consider small disturbance solutions to the fluid equations
\eqref{eq:fluidContinuity}--\eqref{eq:fluidMomentum}
of the form
\begin{align}
\vv(r,\theta,t) = 
\left(\hat{v}_r(r) \ev_r + \hat{v}_\theta(r) \ev_\theta\right)
e^{i (n \theta - \omega t)}, \quad 
p(r,\theta,t) = \hat{p}(r) e^{i (n \theta - \omega t)},
\end{align}
%
where $n\ge1$. We consider $|\hat{v}_r|^2$ and $|\hat{v}_\theta|^2$ to be small, therefore we will ignore 
convection terms.
Under these assumptions, the fluid equations reduce to
\begin{align}
\hat{p}'' 
+ \frac{1}{r} \hat{p}'
- \frac{n^2}{r^2} \hat{p} &= 0 \label{eq:eulerp}\\
r^2 \hat{v}_r'' + 3 r \hat{v}_r' + (\lambda^2 r^2 - n^2+1) \hat{v}_r
&= \frac{r^2}{\mu} \hat{p}' 
\label{eq:besselvr} \\
\hat{v}_\theta &= -\frac{1}{in} \left(\hat{v}_r + r \hat{v}_r' \right),
\label{eq:constraintvt}
\end{align}
%
with $\lambda^2 = - i \rho \omega / \mu$ as defined in the previous solutions.
Equation \eqref{eq:eulerp} 
is an Euler equation for $\hat{p}$ resulting from the pressure Poisson equation.
Equation \eqref{eq:besselvr} can be manipulated into a Bessel equation
for $\hat{v}_r$ with a forcing term.
Equation \eqref{eq:constraintvt} is a constraint on $\hat{v}_\theta$ resulting from the
continuity equation. The solution is
\begin{align}
\hat{p}(r) &= a_1 \left( \frac{r}{R} \right)^n + a_2 \left( \frac{r}{R}\right)^{-n} \\
\hat{v}_r(r) &= 
\frac{a_3}{r} J_n(\lambda r) + \frac{a_4}{r} Y_n(\lambda r) 
+ \frac{a_1}{r} \frac{n}{\mu \lambda^2} \left( \frac{r}{R} \right)^n
- \frac{a_2}{r} \frac{n}{\mu \lambda^2} \left( \frac{r}{R}\right)^{-n},
\end{align}
%
where $a_1,\,a_2,\,a_3,\,a_4,$ are constants determined by the boundary conditions. 
In order for the fluid solution to remain bounded at $r=0$, we must have $a_2=a_4=0.$
$\hat{v}_\theta$ can be obtained using equation \eqref{eq:constraintvt}.

For the solid, we use Helmholtz decomposition to find the solution.
We write the solid displacement as the sum of a divergence-free component and a 
curl-free component,
\begin{align}
\usv = \grad \phi + \grad \curl \Hv.
\end{align}
%
When substituting this into the solid equations 
\eqref{eq:solidDisplacement}--\eqref{eq:solidMomentum},
we find that $\phi$ and $\Hv$ must satisfy wave equations with speeds $\cp$
and $\cs$, respectively.
\begin{align}
\phi_{tt} &= \cp^2 \Delta \phi \label{eq:waveEquationPhi}\\
\Hv_{tt} &= \cs^2 \Delta \Hv. \label{eq:waveEquationH}
\end{align}
%
Since we are only considering 2D displacements, $\Hv = H \ev_3$.
We search for solutions of the form
\begin{align}
\phi(r,\theta,t) = \hat{\phi}(r) e^{i (n \theta - \omega t)}, \quad
H(r,\theta,t) = \hat{H}(r) e^{i (n \theta - \omega t)}
\end{align}
%
Equations \eqref{eq:waveEquationPhi}--\eqref{eq:waveEquationH} reduce to 
the following Bessel equations,
\begin{align}
r^2 \hat{\phi}'' + r \hat{\phi} + \left(\frac{\omega^2}{\cp^2} r^2 - n^2 \right) \hat{\phi}
&= 0 \\
r^2 \hat{H}'' + r \hat{H} + \left(\frac{\omega^2}{\cs^2} r^2 - n^2 \right) \hat{H}
&= 0,
\end{align}
%
of which the solutions are
\begin{align}
\hat{\phi}(r) &= b_1 J_n(k_p r) + b_2 Y_n(k_p r) \\
\hat{H}(r) &= b_3 J_n(k_s r) + b_4 Y_n(k_s r),
\end{align}
%
where
\begin{align}
k_p = \frac{\omega}{\cp}, \quad k_s = \frac{\omega}{\cs}.
\end{align}
%
The displacement can be obtained using
\begin{align}
\hat{\us}_r = \hat{\phi}' + \frac{in}{r} \hat{H}, \quad
\hat{\us}_\theta = \frac{in}{r} \hat{\phi} - \hat{H}'.
\end{align}

Eight boundary conditions in total are needed for this solution.
At the interface, $r=R,$ 
there are two dynamic conditions and two kinetic conditions, given by
\begin{align}
\hat{v}_r(R) = \hat{\vs}_r(R), \quad
\hat{v}_\theta(R) = \hat{\vs}_\theta(R), \quad
\hat{\sigma}_{rr}(R) = \hat{\sigmas}_{rr}(R), \quad
\hat{\sigma}_{r\theta}(R) = \hat{\sigmas}_{r\theta}(R).
\end{align}
%
At $r=R_s,$ we impose a free surface condition for the solid,
\begin{align}
\hat{\sigmas}_{rr}(R_s) = 0, \quad
\hat{\sigmas}_{r\theta}(R_s) = 0.
\end{align}
%
The six non-zero boundary conditions are organized into the following matrix equation
\begin{align}
\Mv(\omega) \av = 0,
\end{align}
%
where $\Mv(\omega) \in \Complex^{6 \times 6}$ and $\av = [a_1,a_3,b_1,b_2,b_3,b_4]^T.$
Non-trivial solutions exist when $\det \Mv(\omega) = 0.$ 
A nonlinear root solver can be used to find solutions for $\omega.$
We require $\Im(\omega) \le 0$ so the solution remains bounded in time. When 
$\omega$ is found, an initial condition is needed to determine
$\av$. For this paper we choose
$\sqrt{|\hat{\us}_r(R)|^2 + |\hat{\us}_\theta(R)|^2} = u_I,$ where $u_I$ is the initial
interface displacement.



==> texFiles/fractionalStepAnalysis.tex <==
\section{Fractional step analysis}

The AMP interface conditions couple the velocity and pressure. 
In this section, we motivate and analyze AMP conditions for the fractional step scheme.

\subsection{Model problem} 
We consider a Stokes fluid and an ``acoustic'' solid.
The ``acoustic'' solid is a special case of linear elasticity obtained by 
taking $\lambdas=-\mus$ and corresponds to pressure and shear waves traveling at the same speed.
The governing equations reduce to
\begin{align}
\partial_t \vv + \frac{1}{\rho} \grad p &= \nu \Delta \vv, \\
\Delta p &= 0, \\
\partial_t \vsv &= \frac{1}{\rhos} \grad \cdot \sigmasv, \\
\partial_t \sigmasv &= -\mus \left(\grad \cdot \vsv\right) \Iv 
+ \mus \left(\grad \vsv + \left(\grad \vsv\right)^T\right).
\end{align}
%
The equations are discretized in time and left continuous in space.
The temporal grid is defined as $t^n = n \dt,$ where $\dt$ is the time step.
For the fluid, backward Euler is used for the viscous terms and forward Euler is
used for the pressure terms. 
A backward Euler scheme is used to advance the solid variables.
The numerical scheme is
\begin{align}
\frac{\vv^{n+1} - \vv^{n}}{\dt}
+ \frac{1}{\rho} \grad p^n
&= \nu \Delta \vv^{n+1}, \label{eq:fluidMomentumFrac} \\
\Delta p^{n+1} &= 0 \label{eq:fluidPressureFrac}\\
\frac{\vsv^{n+1}-\vsv^n}{\dt} 
&= \frac{1}{\rhos} \grad \cdot \sigmasv^{n+1}, \label{eq:solidMomentumFrac}\\
\frac{\sigmasv^{n+1}-\sigmasv^n}{\dt}&= -\mus \left(\grad \cdot \vsv^{n+1}\right) \Iv 
+ \mus \left(\grad \vsv^{n+1} + \left(\grad \vsv^{n+1}\right)^T\right).
\label{eq:solidStressFrac}
\end{align}
%
These equations are difference-differential equations and require an initial condition,
interface conditions, and boundary conditions away from the interface.
Equations \eqref{eq:fluidMomentumFrac}--\eqref{eq:fluidPressureFrac} are 
three second-order elliptic equations for the two components of the fluid velocity and
pressure. 
The solid equations \eqref{eq:solidMomentumFrac}--\eqref{eq:solidStressFrac}
form five first-order equations for the two components of the solid velocity and 
three components of the solid stress. Two interface boundary conditions are required to 
set the two incoming characteristics.
The coupled AMP conditions for the fluid are
\begin{align}
-p^{n+1} + \nv^T \tauv^{n+1} \nv + \zp \nv^T \vv^{n+1} &= 
\nv^T \sigmasv^{(p)} \nv + \zp \nv^T \vsv^{(p)}, \label{eq:pressureUncoupled}\\
\tv^T \tauv^{n+1} \nv + \zs \tv_m^T \vv^{n+1} &=
\tv^T \sigmasv^{(p)} \nv + \zs \tv_m^T \vsv^{(p)}, \label{eq:tangentialVelocity}\\
\grad \cdot \vv^{n+1} &= 0 . \label{eq:div}
\end{align}
%
Here, $\sigmasv^{(p)}$ and $\vsv^{(p)}$ are predicted solid values. For the purposes of the
analysis, we will lag the solid variables by one time step (ie. 
$\sigmasv^{(p)} = \sigmasv^n$ and $\vsv^{(p)} = \vsv^n$).
The solid interface conditions are given by
\begin{align}
\nv^T \sigmasv^{n+1} \nv - \zp \nv^T \vsv^{n+1}
= \nv^T \sigmav^{n+1} \nv - \zp \nv^T \vv^{n+1}, \label{eq:solidInterfaceA}\\
\tv^T \sigmasv^{n+1} \nv - \zs \tv^T \vsv^{n+1}
= \tv^T \sigmav^{n+1} \nv - \zs \tv^T \vv^{n+1} \label{eq:solidInterfaceB}.
\end{align}
%
We now proceed to derive AMP conditions for the fractional step scheme.
This will be achieved by converting equation \eqref{eq:pressureUncoupled}
into a mixed condition for the pressure. When this is done, a new condition is introduced
which sets the normal component of velocity in the limiting case $\zp \rightarrow \infty.$
This new condition will replace equation \eqref{eq:div}.
In equation \eqref{eq:pressureUncoupled}, we apply a backward Euler type scheme to
$\vv^{n+1}$ and $\vsv^{(p)}.$
\begin{align}
\vv^{n+1} = \vv_I^{n} 
- \frac{\dt}{\rho} \grad p^{n+1}
+ \dt \nu \Delta \vv^{n+1},
\quad
\vsv^{(p)} = \vv_I^{n}
+ \dt \av_I^{n+1}.
\end{align}
%
Here, $\vv_I$ and $\av_I$ are the interface velocity and acceleration.
When substituted into \eqref{eq:pressureUncoupled}, $\vv_I$ cancels on both sides.
The condition becomes a Robin condition for the pressure, given by
\begin{align}
-p^{n+1} - \frac{\zp \dt}{\rho} \partial_n p^{n+1}
=\;& \nv^T \sigmasv^{n+1} \nv 
- \nv^T \tauv^{n+1} \nv + 2 \mu (\grad \cdot \vv^{n+1}) \nonumber \\
& + \zp \dt \nv^T \av_I^{n+1} 
+ \nu \zp \dt \nv^T \left(\grad \times \grad \times \vv^{n+1}\right).
\label{eq:pressureRobin}
\end{align}
%
We have made use of the vector identity,
$\Delta \vv^{n+1} = - \grad \times \grad \times \vv^{n+1}$, which is true when
$\grad \cdot \vv^{n+1} = 0$. Additionally, we used a special form of 
the viscous stress tensor. 
\begin{align}
\tauv = \mu \left[\begin{array}{cc}
2 \partial_x v_1 & \partial_x v_2 + \partial_y v_1 \\
\partial_x v_2 + \partial_y v_1 & 2 \partial_y v_2
\end{array}\right],
\quad
\tauv - 2 \mu (\grad \cdot \vv) \Iv
= \mu \left[\begin{array}{cc}
-2 \partial_y v_2 & \partial_x v_2 + \partial_y v_1 \\
\partial_x v_2 + \partial_y v_1 & -2 \partial_x v_1
\end{array}\right],
\end{align}
%
To see why this form is useful, consider the normal component of the viscous stress and
the divergence written in terms of normal and tangential derivatives.
\begin{align}
\frac{1}{\mu} \nv^T \tauv \nv &= 2 \nv^T (\nv \cdot \grad) \vv \\
\grad \cdot \vv &= \nv^T (\nv \cdot \grad) \vv + \tv^T (\tv \cdot \grad) \vv 
\end{align}
%
By combining these terms in a special way, the normal derivatives of the velocity vanish.
\begin{align}
\frac{1}{\mu} \nv^T \tauv \nv - 2 (\grad \cdot \vv) 
&= -2 \tv^T (\tv \cdot \grad) \vv
\end{align}
%
In addition to the pressure condition, a condition for the normal component of velocity is
needed. The proposed condition, analogous to equation \ref{eq:AMPinterfaceNormalVelocity}, is
\begin{align}
\nv^T \vv^{n+1} &= \beta \nv^T \vv^{(e)} + (1-\beta) \nv^T \vsv^{(p)},
\label{eq:impedanceWeightedAverage}
\end{align}
%
where $\beta \in [0,1]$ 
is a parameter which smooths together the limiting behavior for heavy and light solids. 
The amp scheme corresponds to the choice $\beta = \zf / (\zf + \bar{z}).$
The extrapolated fluid velocity is given by
\begin{align}
\vv^{(e)} = \vv^n - \frac{\dt }{\rho} \grad p^n - 
\dt \nu\left(\grad \times \grad \times \vv^{n+1}\right).
\end{align}
%
As before, the curl-curl identity is used to replace the Laplacian. 
When the solid is light ($\beta \sim 1$), the fluid velocity will take the value of the 
extrapolated velocity. When the solid is heavy ($\beta \sim 0$), the fluid velocity will
take the value of the predicted solid velocity.
% \begin{align}
% \nv^T \vv^{n+1} &= \nv^T \vv^n - \frac{\dt }{\rho} \partial_n p^n - 
% \dt \nu \nv^T \left(\grad \times \grad \times \vv^{n+1}\right), \quad \xv \in \Gamma \\
% \nv^T \vv^{n+1} &= \nv^T \vv^n - \frac{\dt }{\rho} \partial_n p^n - 
% \dt \nu \nv^T \Delta \vv^{n+1}, \quad \xv \in \Omega
% \end{align}

\subsection{Stability analysis}
We consider the simplified geometry shown in Figure~\ref{fig:rectangularModelProblem},
but with taking the fluid height to be infinite ($H\rightarrow\infty$).
The final boundary conditions require the solution to remain bounded 
as $|y| \rightarrow \infty.$
We will solve the equations with the ansatz,
\begin{align}
\qv^n(x,y) = \hat{\qv}(y) e^{i k_x x} A^n,
\end{align}
%
where $\qv^n$ represents each variable in the fluid and solid.
For convenience, the hats will be dropped. The fluid equations for the velocity reduce to the
following.
\begin{align}
\lambda v_1(y) + \frac{i k_x}{\rho A} p(y) &= \nu \left(-k_x^2 + \partial_y^2\right) v_1(y), \\
\lambda v_2(y) + \frac{1}{\rho A} \partial_y p(y) &= \nu \left(-k_x^2 + \partial_y^2\right) v_2(y)
\end{align}
%
Here, $\lambda = (A-1) / (A \dt).$ The pressure equation reduces to
\begin{align}
\left(-k_x^2 + \partial_y^2 \right) p(y) = 0.
\end{align}
%
The solution is
\begin{align}
v_1(y) &= 
\left((v_1)_I + \frac{i p_I k_x}{\lambda \rho A} \right) e^{-\alpha y}
- \frac{i p_I k_x}{\lambda \rho A} e^{-k_x y}, \\
v_2(y) &= 
\left((v_2)_I - \frac{p_I k_x}{\lambda \rho A} \right) e^{-\alpha y}
+ \frac{p_I k_x}{\lambda \rho A} e^{-k_x y}, \\
p(y) &= p_I e^{-k_x y} ,
\end{align}
%
where
\begin{align}
\alpha = \sqrt{k_x^2 + \frac{\lambda}{\nu}}.
\end{align}
%
In the solid, the equations reduce to
\begin{align}
\rhos \lambda \vs_1(y) &= i k_x \sigmas_{11}(y) + \partial_y \sigmas_{12}(y), \\
\rhos \lambda \vs_2(y) &= i k_x \sigmas_{12}(y) + \partial_y \sigmas_{22}(y), \\
\lambda \sigmas_{11}(y) &= i k_x \mus \vs_1(y) - \mus \partial_y \vs_{2}(y), 
\label{eq:s11} \\
\lambda \sigmas_{12}(y) &= i k_x \mus \vs_2(y) + \mus \partial_y \vs_{1}(y), \\
\lambda \sigmas_{22}(y) &= -i k_x \mus \vs_{1}(y) + \mus \partial_y \vs_{2}(y).
\label{eq:s22}
\end{align}
%
Equation \eqref{eq:s11} can be summed with \eqref{eq:s22} to obtain the following relation.
\begin{align}
\lambda (\sigmas_{11}(y) + \sigmas_{22}(y)) = 0.
\end{align}
%
Therefore, $\sigmas_{22}(y) = -\sigmas_{11}(y)$ for all time. Four of the five equations are
linearly independent, so we can rewrite the equations as
\begin{align}
\frac{\partial}{\partial y} \left[\begin{array}{c}
\vs_1(y) \\ \vs_2(y) \\ \sigmas_{11}(y) \\ \sigmas_{12}(y)
\end{array}\right]
= 
\left[\begin{array}{cccc}
0 & -i k_x & 0 & \lambda/\mus \\
i k_x & 0 & -\lambda/\mus & 0 \\
0 & - \rhos \lambda & 0 & i k_x \\
\rhos \lambda & 0 & -i k_x & 0
\end{array}\right]
\left[\begin{array}{c}
\vs_1(y) \\ \vs_2(y) \\ \sigmas_{11}(y) \\ \sigmas_{12}(y)
\end{array}\right].
\end{align}
%
The solution is
\begin{align}
\vs_1(y) &= (\vs_1)_I e^{\gamma y}, \\
\vs_2(y) &= (\vs_2)_I e^{\gamma y}, \\
\sigmas_{11}(y) &= \lambda \rhos 
\frac{i k_x (\vs_1)_I - \gamma (\vs_2)_I }{\gamma^2 - k_x^2} e^{\gamma y}, \\
\sigmas_{12}(y) &= \lambda \rhos 
\frac{i k_x (\vs_2)_I + \gamma (\vs_1)_I }{\gamma^2 - k_x^2} e^{\gamma y}, \\
\sigmas_{22}(y) &= - \sigmas_{11}(y),
\end{align}
%
where
\begin{align}
\gamma = \sqrt{k_x^2 + \frac{\lambda^2 \rhos}{\mus}}.
\end{align}

Due to the simplified geometry, the interface normal and tangent vectors are
$\nv = [0,-1]$ and $\tv = [1,0].$
The solutions for the fluid and solid variables are substituted into the 
fractional step AMP interface conditions,
given by equations \eqref{eq:tangentialVelocity}, \eqref{eq:impedanceWeightedAverage}, 
\eqref{eq:pressureRobin}, and \eqref{eq:solidInterfaceA}--\eqref{eq:solidInterfaceB}.
In the pressure condition, the interface acceleration is defined as
$\av_I^{n+1} = \lambda \vv^{n+1}$. These five boundary conditions form a homogeneous system of
equations for the unknowns, $\rv = [(v_1)_I, (v_2)_I, p_I, (\vs_1)_I, (\vs_2)_I]^T,$
\begin{align}
M(A) \rv = 0.
\end{align}
%
We are interested in nontrivial solutions, therefore we look for solutions,
$g(A) = \det(M(A)) = 0.$

There are three dimensionless parameters that appear in this analysis.
\das{We may want to choose a different letter for the density ratio, it conflicts with
the inviscid analysis.}
\begin{align}
M = \frac{\rho}{\rhos}, \quad
r = \nu \dt k_x^2, \quad
\sigma = \bar{c} \dt k_x
\end{align}
%
$M$ is a density ratio, 
$r$ is the viscous CFL number for the fluid, and $\sigma$ is the CFL number for the solid.
The impedance ratio, defined in the viscous analysis,
can be written in terms of the three parameters.
\begin{align}
Z = \frac{\zf}{\bar{z}} = \frac{\rho \nu k_x}{\bar{z}} = \nu \dt k_x^2 
\frac{\rho / \rhos}{\bar{c} \dt k_x } 
= \frac{r M }{\sigma}
\end{align}
%
We can then define the impedance weighted average parameter, $\beta,$ 
in terms of $Z$, $\beta = \frac{Z}{Z + 1}.$

Solutions for the amplification factor are the roots of the transcendental equation $g(A) = 0.$
The argument principle can be used to determine the number of unstable roots.
\begin{align}
\int_C \frac{g'(z)}{g(z)} \; dz
= 2 \pi i \left( n_{\text{roots}} - n_{\text{poles}} \right)
\end{align}
%
\newcommand{\e}{\epsilon}
There is a pole at $z=1.$ 
To determine the number of stable roots $|A| < 1$, 
we integrate over the unit circle with a `pimple' around the pole at
$z=1.$ The integration path is the union of the two curves, $z_1$ and $z_2$,
given by
\begin{alignat}{2}
z_1(\theta) &= e^{i \theta},\quad && \theta \in [a, 2 \pi - a],\\
z_2(\theta) &= 1 + \e e^{i \theta},\quad && \theta \in [-b, b].
\end{alignat}
%
The limits of the curves are defined by the roots of the following equation.
\begin{align}
1 + \e e^{i b} - e^{i a} = 0 
\end{align}
%
In order to determine the total number of roots,
we integrate around a large circle of radius, $R$.
\begin{align}
z = R e^{i \theta}
\end{align}
%
If the total number of roots is equivalent to the number of stable roots, then the scheme is 
stable. Otherwise the scheme is unstable. 
The parameters used for the root search were $\e = 10^{-2}$ and $R=10^3.$
Stability was assessed for 25 logarithmically spaced points in parameter space for $r$ and $M$ 
in the interval $[10^{-6}, 10^{6}].$
For each pair of parameters, 20 points for $\lx$ in the interval $[0.05,1]$ were checked.
Three choices for $\beta$ were tested: $\beta=Z / (Z+1)$ corresponds to the AMP impedance 
weighted average, $\beta = 1$ corresponds to using the extrapolated fluid velocity,
and $\beta = 0$ corresponds to using the solid velocity.
Figure \ref{fig:fractionalResults} shows the results of this computation.  
Only the option $\beta=Z / (Z+1)$ remains stable for the whole parameter search.
The option $\beta=1$ becomes unstable when $M$ is small or when the solid is light compared to 
the fluid.
On the other hand, the option $\beta=0$ becomes unstable when $M$ is larger 
or when the solid is heavy.
This agrees with the behavior observed in the TP and ATP schemes.
\das{For both $\beta=1$ and $\beta=0$, 
the problem seems to be stabilized by taking a larger $r$. My guess is that an increase in 
$r$ corresponds to increasing the wave number. In the inviscid analysis, the constant
wave number was generally the worst case mode.}

\begin{figure}[h]
\includegraphics[width=.5\textwidth]{fig/IWA}
\includegraphics[width=.5\textwidth]{fig/beta1}
\includegraphics[width=.5\textwidth]{fig/beta0}
\caption{Top left: $\beta = \frac{Z}{Z + 1}$. 
Top right: $\beta = 1$ (use fluid velocity).
Bottom left: $\beta = 0$ (use solid velocity).
The x-axis goes from heavy solids on the left to light solids on the right.
The y-axis goes from small time steps on the bottom to large time steps
on the top.
Recall that $Z = M r / \sigma$.
\label{fig:fractionalResults}
}
\end{figure}


==> texFiles/fractionalStepAnalysisOld.tex <==
\section{Fractional step analysis old}

The AMP interface conditions couple the velocity and pressure. 
In this section, we motivate and analyze AMP conditions for the fractional step scheme.

\subsection{Model problem} 
We consider a Stokes fluid and an ``acoustic'' solid.
The ``acoustic'' solid is a special case of linear elasticity obtained by 
taking $\lambdas=-\mus$ and corresponds to pressure and shear waves traveling at the same speed.
The governing equations reduce to
\begin{align}
\partial_t \vv + \frac{1}{\rho} \grad p &= \nu \Delta \vv, \\
\Delta p &= 0, \\
\partial_t \vsv &= \frac{1}{\rhos} \grad \cdot \sigmasv, \\
\partial_t \sigmasv &= -\mus \left(\grad \cdot \vsv\right) \Iv 
+ \mus \left(\grad \vsv + \left(\grad \vsv\right)^T\right).
\end{align}
%
The equations are discretized in time and left continuous in space.
The temporal grid is defined as $t^n = n \dt,$ where $\dt$ is the time step.
For the fluid, backward Euler is used for the viscous terms and forward Euler is
used for the pressure terms. 
A backward Euler scheme is used to advance the solid variables.
The numerical scheme is
\begin{align}
\frac{\vv^{n+1} - \vv^{n}}{\dt}
+ \frac{1}{\rho} \grad p^n
&= \nu \Delta \vv^{n+1}, \label{eq:fluidMomentumFrac} \\
\Delta p^{n+1} &= 0 \label{eq:fluidPressureFrac}\\
\frac{\vsv^{n+1}-\vsv^n}{\dt} 
&= \frac{1}{\rhos} \grad \cdot \sigmasv^{n+1}, \label{eq:solidMomentumFrac}\\
\frac{\sigmasv^{n+1}-\sigmasv^n}{\dt}&= -\mus \left(\grad \cdot \vsv^{n+1}\right) \Iv 
+ \mus \left(\grad \vsv^{n+1} + \left(\grad \vsv^{n+1}\right)^T\right).
\label{eq:solidStressFrac}
\end{align}
%
These equations are difference-differential equations and require an initial condition,
interface conditions, and boundary conditions away from the interface.
Equations \eqref{eq:fluidMomentumFrac}--\eqref{eq:fluidPressureFrac} are 
three second-order elliptic equations for the two components of the fluid velocity and
pressure. 
The solid equations \eqref{eq:solidMomentumFrac}--\eqref{eq:solidStressFrac}
form five first-order equations for the two components of the solid velocity and 
three components of the solid stress. Two interface boundary conditions are required to 
set the two incoming characteristics.
The coupled AMP conditions for the fluid are
\begin{align}
-p^{n+1} + \nv^T \tauv^{n+1} \nv + \zp \nv^T \vv^{n+1} &= 
\nv^T \sigmasv^{(p)} \nv + \zp \nv^T \vsv^{(p)}, \label{eq:pressureUncoupled}\\
\tv^T \tauv^{n+1} \nv + \zs \tv_m^T \vv^{n+1} &=
\tv^T \sigmasv^{(p)} \nv + \zs \tv_m^T \vsv^{(p)}, \label{eq:tangentialVelocity}\\
\grad \cdot \vv^{n+1} &= 0 . \label{eq:div}
\end{align}
%
Here, $\sigmasv^{(p)}$ and $\vsv^{(p)}$ are predicted solid values. For the purposes of the
analysis, we will lag the solid variables by one time step (ie. 
$\sigmasv^{(p)} = \sigmasv^n$ and $\vsv^{(p)} = \vsv^n$).
The solid interface conditions are given by
\begin{align}
\nv^T \sigmasv^{n+1} \nv - \zp \nv^T \vsv^{n+1}
= \nv^T \sigmav^{n+1} \nv - \zp \nv^T \vv^{n+1}, \label{eq:solidInterfaceA}\\
\tv^T \sigmasv^{n+1} \nv - \zs \tv^T \vsv^{n+1}
= \tv^T \sigmav^{n+1} \nv - \zs \tv^T \vv^{n+1} \label{eq:solidInterfaceB}.
\end{align}
%
We now proceed to derive AMP conditions for the fractional step scheme.
This will be achieved by converting equation \eqref{eq:pressureUncoupled}
into a mixed condition for the pressure. When this is done, a new condition is introduced
which sets the normal component of velocity in the limiting case $\zp \rightarrow \infty.$
This new condition will replace equation \eqref{eq:div}.
In equation \eqref{eq:pressureUncoupled}, we apply a backward Euler type scheme to
$\vv^{n+1}$ and $\vsv^{(p)}.$
\begin{align}
\vv^{n+1} = \vv_I^{n} 
- \frac{\dt}{\rho} \grad p^{n+1}
+ \dt \nu \Delta \vv^{n+1},
\quad
\vsv^{(p)} = \vv_I^{n}
+ \dt \av_I^{n+1}.
\end{align}
%
Here, $\vv_I$ and $\av_I$ are the interface velocity and acceleration.
When substituted into \eqref{eq:pressureUncoupled}, $\vv_I$ cancels on both sides.
The condition becomes a Robin condition for the pressure, given by
\begin{align}
-p^{n+1} - \frac{\zp \dt}{\rho} \partial_n p^{n+1}
=\;& \nv^T \sigmasv^{n+1} \nv 
- \nv^T \tauv^{n+1} \nv + 2 \mu (\grad \cdot \vv^{n+1}) \nonumber \\
& + \zp \dt \nv^T \av_I^{n+1} 
+ \nu \zp \dt \nv^T \left(\grad \times \grad \times \vv^{n+1}\right).
\label{eq:pressureRobin}
\end{align}
%
We have made use of the vector identity,
$\Delta \vv^{n+1} = - \grad \times \grad \times \vv^{n+1}$, which is true when
$\grad \cdot \vv^{n+1} = 0$. Additionally, we used a special form of 
the viscous stress tensor. 
\begin{align}
\tauv = \mu \left[\begin{array}{cc}
2 \partial_x v_1 & \partial_x v_2 + \partial_y v_1 \\
\partial_x v_2 + \partial_y v_1 & 2 \partial_y v_2
\end{array}\right],
\quad
\tauv - 2 \mu (\grad \cdot \vv) \Iv
= \mu \left[\begin{array}{cc}
-2 \partial_y v_2 & \partial_x v_2 + \partial_y v_1 \\
\partial_x v_2 + \partial_y v_1 & -2 \partial_x v_1
\end{array}\right],
\end{align}
%
To see why this form is useful, consider the normal component of the viscous stress and
the divergence written in terms of normal and tangential derivatives.
\begin{align}
\frac{1}{\mu} \nv^T \tauv \nv &= 2 \nv^T (\nv \cdot \grad) \vv \\
\grad \cdot \vv &= \nv^T (\nv \cdot \grad) \vv + \tv^T (\tv \cdot \grad) \vv 
\end{align}
%
By combining these terms in a special way, the normal derivatives of the velocity vanish.
\begin{align}
\frac{1}{\mu} \nv^T \tauv \nv - 2 (\grad \cdot \vv) 
&= -2 \tv^T (\tv \cdot \grad) \vv
\end{align}
%
In addition to the pressure condition, a condition for the normal component of velocity is
needed. The proposed condition, analogous to equation \ref{eq:AMPinterfaceNormalVelocity}, is
\begin{align}
\nv^T \vv^{n+1} &= \beta \nv^T \vv^{(e)} + (1-\beta) \nv^T \vsv^{(p)},
\label{eq:impedanceWeightedAverage}
\end{align}
%
where $\beta \in [0,1]$ 
is a parameter which smooths together the limiting behavior for heavy and light solids. 
The amp scheme corresponds to the choice $\beta = \zf / (\zf + \bar{z}).$
The extrapolated fluid velocity is given by
\begin{align}
\vv^{(e)} = \vv^n - \frac{\dt }{\rho} \grad p^n - 
\dt \nu\left(\grad \times \grad \times \vv^{n+1}\right).
\end{align}
%
As before, the curl-curl identity is used to replace the Laplacian. 
When the solid is light ($\beta \sim 1$), the fluid velocity will take the value of the 
extrapolated velocity. When the solid is heavy ($\beta \sim 0$), the fluid velocity will
take the value of the predicted solid velocity.
% \begin{align}
% \nv^T \vv^{n+1} &= \nv^T \vv^n - \frac{\dt }{\rho} \partial_n p^n - 
% \dt \nu \nv^T \left(\grad \times \grad \times \vv^{n+1}\right), \quad \xv \in \Gamma \\
% \nv^T \vv^{n+1} &= \nv^T \vv^n - \frac{\dt }{\rho} \partial_n p^n - 
% \dt \nu \nv^T \Delta \vv^{n+1}, \quad \xv \in \Omega
% \end{align}

\subsection{Stability analysis}
We consider the simplified geometry shown in Figure~\ref{fig:rectangularModelProblem},
but with taking the fluid height to be infinite ($H\rightarrow\infty$).
The final boundary conditions require the solution to remain bounded 
as $|y| \rightarrow \infty.$
We will solve the equations with the ansatz,
\begin{align}
\qv^n(x,y) = \hat{\qv}(y) e^{i k_x x} A^n,
\end{align}
%
where $\qv^n$ represents each variable in the fluid and solid.
For convenience, the hats will be dropped. The fluid equations for the velocity reduce to the
following.
\begin{align}
\lambda v_1(y) + \frac{i k_x}{\rho A} p(y) &= \nu \left(-k_x^2 + \partial_y^2\right) v_1(y), \\
\lambda v_2(y) + \frac{1}{\rho A} \partial_y p(y) &= \nu \left(-k_x^2 + \partial_y^2\right) v_2(y)
\end{align}
%
Here, $\lambda = (A-1) / (A \dt).$ The pressure equation reduces to
\begin{align}
\left(-k_x^2 + \partial_y^2 \right) p(y) = 0.
\end{align}
%
The solution is
\begin{align}
v_1(y) &= 
\left((v_1)_I + \frac{i p_I k_x}{\lambda \rho A} \right) e^{-\alpha y}
- \frac{i p_I k_x}{\lambda \rho A} e^{-k_x y}, \\
v_2(y) &= 
\left((v_2)_I - \frac{p_I k_x}{\lambda \rho A} \right) e^{-\alpha y}
+ \frac{p_I k_x}{\lambda \rho A} e^{-k_x y}, \\
p(y) &= p_I e^{-k_x y} ,
\end{align}
%
where
\begin{align}
\alpha = \sqrt{k_x^2 + \frac{\lambda}{\nu}}.
\end{align}
%
In the solid, the equations reduce to
\begin{align}
\rhos \lambda \vs_1(y) &= i k_x \sigmas_{11}(y) + \partial_y \sigmas_{12}(y), \\
\rhos \lambda \vs_2(y) &= i k_x \sigmas_{12}(y) + \partial_y \sigmas_{22}(y), \\
\lambda \sigmas_{11}(y) &= i k_x \mus \vs_1(y) - \mus \partial_y \vs_{2}(y), 
\label{eq:s11} \\
\lambda \sigmas_{12}(y) &= i k_x \mus \vs_2(y) + \mus \partial_y \vs_{1}(y), \\
\lambda \sigmas_{22}(y) &= -i k_x \mus \vs_{1}(y) + \mus \partial_y \vs_{2}(y).
\label{eq:s22}
\end{align}
%
Equation \eqref{eq:s11} can be summed with \eqref{eq:s22} to obtain the following relation.
\begin{align}
\lambda (\sigmas_{11}(y) + \sigmas_{22}(y)) = 0.
\end{align}
%
Therefore, $\sigmas_{22}(y) = -\sigmas_{11}(y)$ for all time. Four of the five equations are
linearly independent, so we can rewrite the equations as
\begin{align}
\frac{\partial}{\partial y} \left[\begin{array}{c}
\vs_1(y) \\ \vs_2(y) \\ \sigmas_{11}(y) \\ \sigmas_{12}(y)
\end{array}\right]
= 
\left[\begin{array}{cccc}
0 & -i k_x & 0 & \lambda/\mus \\
i k_x & 0 & -\lambda/\mus & 0 \\
0 & - \rhos \lambda & 0 & i k_x \\
\rhos \lambda & 0 & -i k_x & 0
\end{array}\right]
\left[\begin{array}{c}
\vs_1(y) \\ \vs_2(y) \\ \sigmas_{11}(y) \\ \sigmas_{12}(y)
\end{array}\right].
\end{align}
%
The solution is
\begin{align}
\vs_1(y) &= (\vs_1)_I e^{\gamma y}, \\
\vs_2(y) &= (\vs_2)_I e^{\gamma y}, \\
\sigmas_{11}(y) &= \lambda \rhos 
\frac{i k_x (\vs_1)_I - \gamma (\vs_2)_I }{\gamma^2 - k_x^2} e^{\gamma y}, \\
\sigmas_{12}(y) &= \lambda \rhos 
\frac{i k_x (\vs_2)_I + \gamma (\vs_1)_I }{\gamma^2 - k_x^2} e^{\gamma y}, \\
\sigmas_{22}(y) &= - \sigmas_{11}(y),
\end{align}
%
where
\begin{align}
\gamma = \sqrt{k_x^2 + \frac{\lambda^2 \rhos}{\mus}}.
\end{align}

Due to the simplified geometry, the interface normal and tangent vectors are
$\nv = [0,-1]$ and $\tv = [1,0].$
The solutions for the fluid and solid variables are substituted into the 
fractional step AMP interface conditions,
given by equations \eqref{eq:tangentialVelocity}, \eqref{eq:impedanceWeightedAverage}, 
\eqref{eq:pressureRobin}, and \eqref{eq:solidInterfaceA}--\eqref{eq:solidInterfaceB}.
In the pressure condition, the interface acceleration is defined as
$\av_I^{n+1} = \lambda \vv^{n+1}$. These five boundary conditions form a homogeneous system of
equations for the unknowns, $\rv = [(v_1)_I, (v_2)_I, p_I, (\vs_1)_I, (\vs_2)_I]^T,$
\begin{align}
M(A) \rv = 0.
\end{align}
%
We are interested in nontrivial solutions, therefore we look for solutions,
$g(A) = \det(M(A)) = 0.$

There are three dimensionless parameters that appear in this analysis.
\das{We may want to choose a different letter for the density ratio, it conflicts with
the inviscid analysis.}
\begin{align}
M = \frac{\rho}{\rhos}, \quad
r = \nu \dt k_x^2, \quad
\sigma = \bar{c} \dt k_x
\end{align}
%
$M$ is a density ratio, 
$r$ is the viscous CFL number for the fluid, and $\sigma$ is the CFL number for the solid.
The impedance ratio, defined in the viscous analysis,
can be written in terms of the three parameters.
\begin{align}
Z = \frac{\zf}{\bar{z}} = \frac{\rho \nu k_x}{\bar{z}} = \nu \dt k_x^2 
\frac{\rho / \rhos}{\bar{c} \dt k_x } 
= \frac{r M }{\sigma}
\end{align}
%
We can then define the impedance weighted average parameter, $\beta,$ 
in terms of $Z$, $\beta = \frac{Z}{Z + 1}.$

Solutions for the amplification factor are the roots of the transcendental equation $g(A) = 0.$
The argument principle can be used to determine the number of unstable roots.
\begin{align}
\int_C \frac{g'(z)}{g(z)} \; dz
= 2 \pi i \left( n_{\text{roots}} - n_{\text{poles}} \right)
\end{align}
%
\newcommand{\e}{\epsilon}
There is a pole at $z=1.$ 
To determine the number of stable roots $|A| < 1$, 
we integrate over the unit circle with a `pimple' around the pole at
$z=1.$ The integration path is the union of the two curves, $z_1$ and $z_2$,
given by
\begin{alignat}{2}
z_1(\theta) &= e^{i \theta},\quad && \theta \in [a, 2 \pi - a],\\
z_2(\theta) &= 1 + \e e^{i \theta},\quad && \theta \in [-b, b].
\end{alignat}
%
The limits of the curves are defined by the roots of the following equation.
\begin{align}
1 + \e e^{i b} - e^{i a} = 0 
\end{align}
%
In order to determine the total number of roots,
we integrate around a large circle of radius, $R$.
\begin{align}
z = R e^{i \theta}
\end{align}
%
If the total number of roots is equivalent to the number of stable roots, then the scheme is 
stable. Otherwise the scheme is unstable. 
The parameters used for the root search were $\e = 10^{-2}$ and $R=10^3.$
Stability was assessed for 25 logarithmically spaced points in parameter space for $r$ and $M$ 
in the interval $[10^{-6}, 10^{6}].$
For each pair of parameters, 20 points for $\lx$ in the interval $[0.05,1]$ were checked.
Three choices for $\beta$ were tested: $\beta=Z / (Z+1)$ corresponds to the AMP impedance 
weighted average, $\beta = 1$ corresponds to using the extrapolated fluid velocity,
and $\beta = 0$ corresponds to using the solid velocity.
Figure \ref{fig:fractionalResults} shows the results of this computation.  
Only the option $\beta=Z / (Z+1)$ remains stable for the whole parameter search.
The option $\beta=1$ becomes unstable when $M$ is small or when the solid is light compared to 
the fluid.
On the other hand, the option $\beta=0$ becomes unstable when $M$ is larger 
or when the solid is heavy.
This agrees with the behavior observed in the TP and ATP schemes.
\das{For both $\beta=1$ and $\beta=0$, 
the problem seems to be stabilized by taking a larger $r$. My guess is that an increase in 
$r$ corresponds to increasing the wave number. In the inviscid analysis, the constant
wave number was generally the worst case mode.}

\begin{figure}[h]
\includegraphics[width=.5\textwidth]{fig/IWA}
\includegraphics[width=.5\textwidth]{fig/beta1}
\includegraphics[width=.5\textwidth]{fig/beta0}
\caption{Top left: $\beta = \frac{Z}{Z + 1}$. 
Top right: $\beta = 1$ (use fluid velocity).
Bottom left: $\beta = 0$ (use solid velocity).
The x-axis goes from heavy solids on the left to light solids on the right.
The y-axis goes from small time steps on the bottom to large time steps
on the top.
Recall that $Z = M r / \sigma$.
\label{fig:fractionalResults}
}
\end{figure}


==> texFiles/governing.tex <==
\section{Governing equations and interface conditions} \label{sec:governingEquations}


We consider the coupled evolution of an incompressible fluid and a linear elastic solid. 
The fluid occupies the domain $\xv \in \OmegaF(t)$, where
$\xv=(x_1,x_2,x_3)$ is a vector of physical coordinates and $t$ is time. 
The velocity-pressure form of the INS equations is given by
\bse
\begin{alignat}{2}
\rho \vv_t + \rho (\vv \cdot \grad) \vv + \grad p &=
\mu \Delta \vv, \qquad &&\xv \in \OmegaF(t),
\label{eq:fluidMomentum} \\
\Delta p &= -\rho \grad \vv : \left(\grad \vv\right)^T, \qquad &&\xv \in \OmegaF(t),
\label{eq:pressurePoissonEquation}
\end{alignat}
\ese
%
where
\begin{align}
\grad \vv : \left(\grad \vv\right)^T \equiv 
\sum_{i=1}^3 \sum_{j=1}^3 \frac{\partial v_i}{\partial x_j} \frac{\partial v_j}{\partial x_i}.
\end{align}
%
where $\vv(\xv,t)$ is the velocity, $p(\xv,t)$ is the pressure,
$\rho$ is the (constant) density, and $\mu$ is the (constant) dynamic viscosity. 
The fluid stress tensor is given by
\begin{align}
\sigmav = - p \Iv + \tauv, 
\quad 
\tauv &= \mu \left(\grad \vv + \left(\grad \vv\right)^T \right),
\label{eq:fluidStressTensor} 
\end{align}
%
where $\Iv$ is the identity matrix and $\tauv(\xv,t)$ is
the viscous stress tensor.  
%
Here, components of the fluid velocity $\vv$ are denoted by $(v_1,v_2,v_3)$, and a similar notation is used for the components of tensors, e.g.~the components of $\sigmav$ are given by $\sigma_{mn}$ with $m,n=1$, 2, 3.
In the velocity-pressure form of the equations, an extra boundary condition is required and a suitable choice is to impose $\grad \cdot \vv = 0$ for $\xv\in\partial\OmegaF(t)$, see~\cite{splitStep2003}.

% solid eq
The equations for the solid are written in terms of the Lagrangian coordinate 
$\xsv=(\bar x_1,\bar x_2,\bar x_3)$ for
a reference configuration $\xsv \in \OmegaS$ at $t=0$.  
(An overbar is used here and elsewhere to denote
quantities belonging to the solid.)
The position of the solid in physical space is determined by the mapping
\begin{align}
\xv = \xsv + \usv(\xsv,t),
\label{eq:solidPhysicalCoordinates}
\end{align}
%
where $\usv(\xsv,t)$ is the displacement of the solid.
The Cauchy stress tensor $\sigmasv(\xsv,t)$ for a linearly-elastic solid is defined by
\begin{align}
\sigmasv &= \lambdas (\grads \cdot \usv) \Iv 
+ \mus \left(\grads \usv + \left(\grads \usv\right)^T\right),
\label{eq:solidStressTensor}
\end{align}
%
where $\lambdas$ and $\mus$ are Lam\'e parameters (taken to be constants).
Following the approach described in~\cite{smog}, the solid equations are treated as a 
first order system of PDEs in time and space, given by
\bse
\begin{alignat}{2}
\usv_t &= \vsv, \qquad &&\xvs \in \OmegaS ,
\label{eq:solidDisplacement} \\
\rhos \vsv_t &= \grads \cdot \sigmasv , \qquad &&\xvs \in \OmegaS,
\label{eq:solidMomentum} \\
\sigmasv_t &= \lambdas (\grads \cdot \vsv) \Iv 
+ \mus \left(\grads \vsv + \left(\grads \vsv \right)^T\right),\qquad &&\xvs \in \OmegaS,
\label{eq:solidStressTensorDeriv}
\end{alignat}
\ese
%
where $\vsv(\xsv,t)$ its velocity, and $\rhos$ its density (assumed constant).  
In this form, upwind solvers can be used to advance displacement, velocity and stress of the 
solid. We note that~\eqref{eq:solidStressTensor} is enforced at $t=0$.

The fluid and solid are coupled at an interface described by
$\xv\in\GammaIf(t)$ in physical space and $\xsv \in \GammaIs$
in the corresponding reference space. At the interface, the conversion between reference 
and physical coordinates is determined by the mapping in~\eqref{eq:solidPhysicalCoordinates}. 
The interface is assumed to be smooth so that a well-defined normal to the interface exists.  
Along the interface, the following matching conditions hold:
\bse
\begin{alignat}{2}
\vv &= \vsv, \qquad &&\xv \in \GammaIf(t),
\label{eq:velocityMatching} \\
\sigmav \nv &= 
\sigmasv \nv, \qquad &&\xv \in \GammaIf(t),
\label{eq:tractionMatching}
\end{alignat}
\ese
%\begin{alignat}{2}
%\vv &= \vsv, \qquad &&\xv \in \GammaIf(t), \qquad \xsv \in \GammaIs,
%\label{eq:velocityMatching} \\
%\sigmav \nv &= 
%\sigmasv \nv, \qquad &&\xv \in \GammaIf(t), \qquad \xsv \in \GammaIs, 
%\label{eq:tractionMatching}
%\end{alignat}
%
where $\nv(\xv,t)$ is the outward unit normal to the fluid domain, i.e.~$\nv$ points from the fluid domain to the solid domain.  Suitable boundary
conditions are applied on the boundaries of the fluid and solid domians not included in $\GammaIf(t)$, and initial
conditions on $\vv$, $\usv$ and $\vsv$ are set to close the problem.
%We note
%that the solid traction is defined using
%the solid reference normal, while the fluid traction is defined using the
%physical normal. Under the assumptions of linear elasticity, these choices
%are arbitrary. 

%%%%%%%%%%%
Since the equations governing the solid form a hyperbolic system, it 
is informative to consider the propagation of characteristics. The 
longitudinal and shear wave speeds are defined as
\begin{align}
\cp = \sqrt{\frac{\lambdas+2 \mus}{\rhos}}, \qquad
\cs = \sqrt{\frac{ \mus}{\rhos}},
\label{eq:solidWaveSpeeds}
\end{align}
%
respectively. At the interface, the Riemann variables corresponding to incoming and outgoing characteristics can be 
obtained from the first-order equations in~\eqref{eq:solidMomentum} and~\eqref{eq:solidStressTensorDeriv} projected onto the normal to the interface.  These variables for the longitudinal and shear waves are given by
\bse
\begin{alignat}{2}
\Ac(\sigmasv, \vsv) &= \nv^T \sigmasv \nv - \zp \nv^T \vsv ,
\quad \phantom{m = 1,2,}
\qquad &&\xv \in \GammaIf(t)
\quad \text{(incoming),}
\label{eq:ACharacteristic}
\\
\Ac_m(\sigmasv, \vsv) &= \tnv_m^T \sigmasv \nv - \zs \tnv_m^T \vsv, 
\quad m = 1,2,
\qquad &&\xv \in \GammaIf(t)
\quad \text{(incoming),}
\label{eq:AmCharacteristic}
\end{alignat}
corresponding to information propagating into the solid domain, and
\begin{alignat}{2}
\Bc(\sigmasv, \vsv) &= \nv^T \sigmasv \nv + \zp \nv^T \vsv ,
\quad \phantom{m = 1,2,}
\qquad &&\xv \in \GammaIf(t)
\quad \text{(outgoing),}
\label{eq:BCharacteristic}
\\
\Bc_m(\sigmasv, \vsv) &= \tnv_m^T \sigmasv \nv + \zs \tnv_m^T \vsv ,
\quad m = 1,2,
\qquad &&\xv \in \GammaIf(t)
\quad \text{(outgoing),}
\label{eq:BmCharacteristic}
\end{alignat}
\ese
corresponding to information propagating out of the solid domain.
%
Here, $\tnv_1(\xv,t)$ and $\tnv_2(\xv,t)$ are mutually orthogonal unit vectors tangent to $\GammaIf(t)$, and thus orthogonal to $\nv$, and
$\zp = \rhos \cp$ and $\zs = \rhos \cs$ are the solid impedances 
for longitudinal and shear waves, respectively. 



==> texFiles/inviscidAnalysis-11-03-18.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Inviscid analysis for second order scheme} \label{sec:inviscidAnalysis}

% todo
%
% replace \lambda_y with \ly etc.
%
%\noindent
%\textcolor{red}{(Current thoughts on editing this section: (1) Describe the model problem at a continuous level.  Simplify the notation by $v_2\rightarrow v$, $\sigma_{21}\rightarrow\sigma_1$, etc., basically dropping the 2 since everything is in the vertical direction anyway.  BTW: I wonder if it is too much to say that the solid velocity and stress tend to zero as $y\rightarrow-\infty$.  I think this would only be true if this property also holds for the initial data.  Requiring that the solution is bounded at infinity should be enough.  I wonder if this issue was discussed during the writing of FIB???  (2) Describe how the equations are approximated.  (3) Describe the AMP algorithm for the approximation of the model equations.  Here I think it is helpful to point back to the previously discussed algorithm so that the mapping between the general algorithm and the one in the model problem analysis is clear.  (4) Perform the analysis for the AMP scheme and give the results.  (5) State the corresponding results for the TP and ATP schemes, but leave any details to an appendix.)}

% \wdh{\bf This is from fib:
% In this section, we perform a stability analysis of the AMP algorithm applied to
% the two-dimensional FSI model problem MP-IA.  In this problem, the fluid is
% taken as inviscid and the solid is treated as an acoustic solid that only
% supports motion in the vertical direction. The governing equations for the model
% are given by~\eqref{eq:MP-IA}.
% % We are interested in the stability of different frequencies in the $x$ direction and thus consider a periodic problem in $x$. 
% We consider a semi-infinite solid domain ($\Hs=\infty$) and look for solutions in the solid that have finite $L_2$-norm (which implies the solutions decay to zero as $y\rightarrow\infty$).  The bottom boundary condition on the fluid at $y=-H$ is chosen as $\sigma=0$ (i.e. $p=0$).
% }

In this section, the stability of the AMP, TP and ATP algorithms are explored for a simplified two-dimensional FSI model problem.  A similar stability analysis was performed in~\cite{fib2014} for a first-order accurate scheme on a staggered grid.  The algorithms considered here are second-order accurate, as in the full AMP algorithm discussed in Section~\ref{sec:partitionedAlgorithms}, and thus the present analysis extends the previous results for less dissipative partitioned schemes.

\input texFiles/rectangularModelProblemCartoon

\subsection{FSI model problem}

The configuration of the model problem is shown in Figure~\ref{fig:rectangularModelProblem}.  The fluid is assumed to be inviscid and incompressible, and it occupies the region $\OmegaF$ given by $0<x<L$ and $0<y<H$.  The solid lies below the fluid in the semi-infinite region $\OmegaS$ given by $0<x<L$ and $-\infty<y<0$.  The solid is taken to be an ``acoustic'' solid that supports a motion in the vertical direction only.  The fluid-solid interface $\Gamma$ is linearized about the flat surface, $y=0$, and it is assumed that the vertical components of the velocity and stress between the fluid and solid match along $\Gamma$.  The fluid pressure is taken to be zero along the top boundary, $y=H$, and the solutions for the fluid and solid are assumed to be periodic in the $x$-direction with period equal to~$L$.  The governing equations for the FSI model problem are
%In this section, the stability of the second order accurate
%AMP, TP, and ATP algorithms are explored for a simplified two-dimensional 
%model problem. This extends the stability results of first order 
%accurate schemes in \cite{fib2014}.
%In this analysis, the TP scheme is considered 
%without under-relaxed sub-iterations. 
%To supplement this, an analysis of the TP scheme with sub-iterations is performed.
%In the model problem, we assume the fluid is inviscid and the solid 
%is acoustic with motion constrained to vertical direction. 
%We are interested in the stability of different frequencies 
%in the $x$ direction and thus consider a periodic problem in $x$. 
%The solid domain is semi-infinite ($\Hs \rightarrow \infty)$ and we require solutions
%to decay to zero as $y \rightarrow -\infty.$ The fluid pressure is given to be 
%$p=0$ at the top boundary. The interface conditions enforce matching of the 
%velocity and traction at $y=0.$
%The governing equations and boundary conditions are given by
\begin{align}
\text{Fluid: } &\begin{cases}
\rho \partial_t \vfy + \partial_y p = 0, & \xv\in\OmegaF \\
(\partial_x^2 + \partial_y^2) p =0, & \xv\in\OmegaF \\
p = 0, & x\in(0,L), \quad y=H
\end{cases} \label{eq:fluidModelInviscid} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsy = \partial_x \ssx + \partial_y \ssy, & \xv\in\OmegaS \\
\partial_t \ssx = \rhos\cp^2 \partial_x \vsy, & \xv\in\OmegaS \\
\partial_t \ssy = \rhos\cp^2 \partial_y \vsy, & \xv\in\OmegaS \\
|\vsy|^2+|\ssx|^2+|\ssy|^2 < \infty, & y\rightarrow - \infty
\end{cases} \label{eq:solidModelInviscid} \\
\text{Interface: } &\begin{cases}
\vfy = \vsy, & x\in(0,L), \quad y = 0 \\
p = -\ssy, & x\in(0,L), \quad y = 0.
\end{cases}
\end{align}
We note that the horizontal component of the fluid velocity is omitted from the equations for the fluid in~\eqref{eq:fluidModel} since it decouples in the simplified FSI problem and can be determined from the remaining fluid variables once the solution is known.  The model problem described here corresponds to the MP-IA model problem considered in~\cite{fib2014}.

% governing equations
% ------------------------------------------------------------------------------------------------
\subsection{Discretization}

The equations governing the fluid and solid are discretized in the $x$-direction on a uniform grid, $x_\ell = \ell \Delta x$ for $\ell = 0, 1,\ldots N_x$, with grid spacing $\dx = L/N_x$.  Since the problem is periodic, each variable can be represented as a discrete Fourier series
\begin{align}
q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2}  e^{2 \pi i k x_\ell/ L} \hat{q}_k (y,t), 
\qquad \ell=0,1,2,\ldots,N_x. \label{eq:discreteFourierInviscid}
\end{align}
%
where $q_\ell(y,t) \approx q(x_\ell,y,t)$ denotes an approximation of a fluid or solid variable and $\hat{q}_k(y,t)$ are the corresponding Fourier coefficients.  For convenience, $N_x$ is assumed to be an even integer.  Taking a discrete Fourier transform of the equations in~\eqref{eq:fluidModel} and~\eqref{eq:solidModel} gives
\begin{align}
\text{Fluid: } &\begin{cases}
\rho \partial_t \vfyh + \partial_y \ph = 0, & y\in(0,H) \\
\partial_y^2 \ph - k_x^2 \ph =0, & y\in(0,H) \\
\ph =0, & y=H
\end{cases} \label{eq:fluidModelDiscrete} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsyh = i k_x \ssxh + \partial_y \ssyh, & y\in(-\infty,0) \\
\partial_t \ssxh = i k_x \rhos\cp^2 \vsyh, & y\in(-\infty,0) \\
\partial_t \ssyh = \rhos\cp^2 \partial_y \vsyh, & y\in(-\infty,0) \\
|\vsy|^2+|\ssx|^2+|\ssy|^2 < \infty, & y\rightarrow - \infty
\end{cases} \label{eq:solidModelDiscrete}
\end{align}
%
%\begin{alignat}{2}
%\rho \partial_t \vfyh + \partial_y \ph &= 0, \quad && y\in(0,H), \\
%\partial_y^2 \ph - k_x^2 \ph &=0, \quad && y\in(0,H),
%\label{eq:phEqn} \\
%% \end{alignat}
%% %
%% The transformed equations for the solid are
%% \begin{alignat}{2}
%\rhos \partial_t \vsyh &= i k_x \ssxh + \partial_y \ssyh, \quad && y\in(-\infty,0) ,
%\label{eq:vsyhEqn} \\
%\partial_t \ssxh &= i k_x \rhos\cp^2 \vsyh, && y\in(-\infty,0), 
%\label{eq:ssxhEqn} \\
%\partial_t \ssyh &= \rhos\cp^2 \partial_y \vsyh, && y\in(-\infty,0)
%\label{eq:ssyhEqn}.
%\end{alignat}
%
where $k_x = 2 \pi k /L$ is a normalized wave number, and the hats and $k$ subscripts on the Fourier coefficients have been suppressed for notational convenience.  Since we are interested in wave propagation in the solid, it is useful to define the characteristics variables
\begin{align}
\bc = \ssyh + \zp\vsyh, \qquad
\ac = \ssyh - \zp\vsyh, \qquad
\dc = \ssxh,
\end{align}
and recast the solid equations in~\eqref{eq:solidModelDiscrete} in the characteristic form
\begin{alignat}{2}
\partial_t \bc - \cp \partial_y \bc &= i k_x \cp \dc, \qquad && y\in(-\infty,0),
\label{eq:advSrcB} \\
\partial_t \ac + \cp \partial_y \ac &= -i k_x \cp \dc, \qquad && y\in(-\infty,0), 
\label{eq:advSrcA} \\
\partial_t \dc &= \frac{i k_x \cp}{2} (\bc - \ac), \qquad && y\in(-\infty,0).
\label{eq:SrcD}
\end{alignat}
Equations~\eqref{eq:advSrcB} and~\eqref{eq:advSrcA} are advection equations for the incoming and outgoing characteristic variables $\bc$ and $\ac$, respectively, corresponding to the variables defined in~\eqref{eq:ACharacteristic} and \eqref{eq:BCharacteristic} for $\nv=[0,-1]^T$, while~\eqref{eq:SrcD} describes the evolution of the tangential component of the solid stress.

The solid characteristic variables are discretized in the $y$-direction using a uniform collocated grid, $y_j = j\dy$ for $j = 0, -1, -2 \ldots$, with grid spacing $\dy$.  Although a staggered grid is used for the analysis in~\cite{fib2014} (and for the stability analyses of other FSI algorithms in~\cite{BanksSjogreen2011,lrb2013}), it is cleaner to use a collocated grid for the second-order accurate scheme.  Define the grid functions $\ac^n_j \approx \ac(y_j, t^n)$, $\bc^n_j \approx \bc(y_j, t^n)$ and $\dc^n_j \approx \dc(y_j,t^n)$, where $t^n = n \Delta t$ for a (fixed) time step $\Delta t$.  The advection equations in~\eqref{eq:advSrcB} and~\eqref{eq:advSrcA} are approximated using a second-order accurate Lax-Wendroff-type scheme having the form
\begin{align}
\bc^{n+1}_{j} &= \bc^{n}_j + 
\frac{\lambda_y}{2} \delta_0 \bc^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \bc^{n}_j 
+ i \lambda_x \dc^n_j
+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j), \label{eq:bLax} \\
\ac^{n+1}_{j} &= \ac^{n}_j - 
\frac{\lambda_y}{2} \delta_0 \ac^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \ac^{n}_j 
- i \lambda_x \dc^n_j
+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
+ \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j),  \label{eq:aLax}
\end{align}
where $\lambda_x = k_x \cp \dt$ and $\lambda_y = \cp \dt / \dy$.  The centered approximations of the spatial derivatives in~\eqref{eq:bLax} and~\eqref{eq:aLax} are defined in terms of the undivided difference operators $\delta_+ u^{n}_j = u^{n}_{j+1} - u^{n}_j$, $\delta_- u^{n}_j = u^{n}_j - u^{n}_{j-1}$ and $\delta_0 u^{n}_j = u^{n}_{j+1} - u^{n}_{j-1}$ for an arbitrary grid function $u^{n}_j$.  The evolution equation in~\eqref{eq:SrcD} is approximated using a second-order accurate BDF scheme of the form
\begin{align}
\dc^{n+1}_j &= \frac{4}{3}\dc^{n}_j - \frac{1}{3} \dc^{n-1}+ \frac{i \lambda_x}{3}
\left(\bc^{n+1}_j - \ac^{n+1}_j \right). \label{eq:dTrap}
\end{align}
For reference, the Fourier coefficients of the solid velocity and normal stress are related to the incoming and outgoing characteristic variables by
\begin{align}
{\bar v}_{2,j}\sp n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \qquad
{\bar\sigma}_{22,j}\sp n = \frac{1}{2} (\bc^n_j+\ac^n_j),
\end{align}
%\begin{align}
%(\vsyh)_j^n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \qquad
%(\ssyh)_j^n = \frac{1}{2} (\bc^n_j+\ac^n_j), \qquad
%(\ssxh)_j^n = \dc^n_j,
%\end{align}
and the boundedness condition at infinity implies that
\begin{align}
\vert \ac^n_j \vert^2 +
\vert \bc^n_j \vert^2 +
\vert \dc^n_j \vert^2 < \infty, \qquad \text{as } j \rightarrow -\infty.
\label{eq:bcInf}
\end{align}

%Let $\Delta t$ be the time step and let $t^n = n \Delta t.$
%The solid equations are solved with a dissipative scheme to in order to exploit 
%some useful properties in the analysis.
%A second order centered scheme was chosen to minimize the stencil to 
%three grid points (a second order upwind scheme requires a five point stencil).
%The schemes for equations \eqref{eq:advSrcA}--\eqref{eq:advSrcB}
%are derived by taking a Taylor series in time and replacing time derivatives
%with spacial derivatives. 
%Define the grid functions
%$\ac^n_j \approx \ac(y_j, t^n), \bc^n_j \approx \bc(y_j, t^n),$ and
%$\dc^n_j \approx \dc(y_j,t^n),$
%then the Taylor series for $\ac$ is given by
%\begin{align}
%\ac(y_j,t^{n+1}) =\;& \ac(y_j,t^{n}) + 
%\dt \partial_t \ac(y_j,t^{n}) + 
%\frac{\dt^2}{2} \partial_t^2 \ac(y_j,t^{n}) + O(\dt^3)\\
%=\;& \ac(y_j,t^{n}) - 
%\cp \dt \partial_y \ac(y_j,t^{n}) + 
%\frac{\cp^2 \dt^2}{2} \partial_y^2 \ac(y_j,t^{n}) \nonumber \\
%&- i k_x \cp \dt \dc(y_j,t^n)
%+ \frac{i k_x \cp^2 \dt^2}{2} \partial_y \dc(y_j,t^n) \nonumber \\
%&+ \frac{k_x^2 \cp^2 \dt^2}{4} \left(\bc(y_j,t^{n}) - \ac(y_j,t^{n}) \right) + O(\dt^3).
%\end{align}
%% \begin{align}
%% \ac^{n+1}_j &= \ac^{n}_j + 
%% \dt \partial_t \ac^{n}_j + 
%% \frac{\dt^2}{2} \partial_t^2 \ac^{n}_j + O(\dt^3)\\
%% \ac^{n+1}_j &= \ac^{n}_j - 
%% \cp \dt \partial_y \ac^{n}_j + 
%% \frac{\cp^2 \dt^2}{2} \partial_y^2 \ac^{n}_j 
%% + i k_x \cp \dt \dc^n_j
%% - \frac{k_x^2 \cp^2 \dt^2}{4} (\bc^{n}_{j} - \ac^{n}_{j}) + O(\dt^3).
%% \end{align}
%%
%A similar series can be derived for $\bc.$
%The spacial derivatives are approximated by centered second order finite
%difference formulas. Define the undivided difference operators
%$\delta_+ u_j = u_{j+1} - u_j,$ 
%$\delta_- u_j = u_j - u_{j-1},$ and $\delta_0 u_j = u_{j+1} - u_{j-1}$ 
%for an arbitrary grid function $u_j.$ The scheme for $\ac$ and $\bc$
%can be written as 
%\begin{align}
%\ac^{n+1}_{j} &= \ac^{n}_j - 
%\frac{\lambda_y}{2} \delta_0 \ac^{n}_j + 
%\frac{\lambda_y^2}{2} \delta_+ \delta_- \ac^{n}_j 
%- i \lambda_x \dc^n_j
%+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
%+ \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j)  \label{eq:aLax} \\
%\bc^{n+1}_{j} &= \bc^{n}_j + 
%\frac{\lambda_y}{2} \delta_0 \bc^{n}_j + 
%\frac{\lambda_y^2}{2} \delta_+ \delta_- \bc^{n}_j 
%+ i \lambda_x \dc^n_j
%+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
%- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j) \label{eq:bLax}
%\end{align}
%%
%where $\lambda_x = k_x \cp \dt$ and $\lambda_y = \cp \dt / \dy.$
%This is a Lax-Wendroff scheme for an advection equation with a source.
%After advancing $\ac$ and $\bc$ to the next time level, $\dc$ can be
%advanced with a simple quadrature. Since a non-dissipative pseudo-spectral approximation
%is used in the $x$ direction, 
%% the trapezoidal rule 
%a BDF scheme
%is used to stabilize the approximation.
%% \begin{align}
%% \dc^{n+1}_j &= \dc^{n}_j + \frac{i \lambda_x}{4}
%% \left(\bc^{n+1}_j - \ac^{n+1}_j + \bc^n_j - \ac^n_j \right). \label{eq:dTrap}
%% \end{align}
%\begin{align}
%\dc^{n+1}_j &= \frac{4}{3}\dc^{n}_j - \frac{1}{3} \dc^{n-1}+ \frac{i \lambda_x}{3}
%\left(\bc^{n+1}_j - \ac^{n+1}_j \right). \label{eq:dTrap}
%\end{align}
%%
%The $\cp^+$ characteristic, $\ac,$ will be extrapolated to the interface ghost point.
%Additionally, the solution must be bounded as $y \rightarrow -\infty.$
%\begin{alignat}{2}
%\ac^n_{1} &= 2 \ac^n_{0} - \ac^n_{-1}, \quad && \\
%\vert \ac^n_j \vert^2 +
%\vert \bc^n_j \vert^2 +
%\vert \dc^n_j \vert^2 &< \infty, \quad &&\text{as } j \rightarrow -\infty
%\label{eq:bcInf}
%\end{alignat}
%%
%The interface condition will determine $b_{1}^n,$ and the initial conditions will 
%define $a_j^0, b_j^0,$ and $d_j^0$ for $j = 0,1,2,3,\ldots$.
%For reference, the Fourier 
%coefficients of the solid velocity and stress components are related to the characteristic 
%variables by
%\begin{align}
%(\vsyh)_j^n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \quad
%(\ssyh)_j^n = \frac{1}{2} (\bc^n_j+\ac^n_j), \quad
%(\ssxh)_j^n = \dc^n_j.
%\end{align}

The equations for the Fourier coefficients of the fluid variables in~\eqref{eq:fluidModelDiscrete} involve an evolution equation for the vertical component of the velocity and a reduced Laplace equation for the pressure.  Following the approach taken in~\cite{fib2014}, the Laplace equation for the pressure, with the boundary condition at $y=H$, is solved exactly at a time $t^n$ to give
\begin{align}
p(y,t^n) = p_I^n \frac{\sinh(k_x(H-y))}{\sinh(k_x H)},
\label{eq:pressureSubProblemSolution}
\end{align}
where $p_I^n$ is an interface pressure which is specified later by the chosen coupling at the interface.  For the purpose of the analysis, we only require the fluid velocity on the interface, which we define to be $v_I^{n}$.  The evolution of the interface velocity involves the gradient of pressure at $y=0$, which is given by
\begin{align}
\partial_y p(0,t^n) = - \frac{p_I^n}{\Heff},\qquad \Heff = \frac{\tanh(k_x H)}{k_x}.
\label{eq:interfacePressureGradient}
\end{align}
The effective fluid height, $\Heff$, in the formula for the pressure gradient depends on the normalized wave number, and it takes the limiting values of $\Heff=H$ as $k_x\rightarrow0$ and $\Heff=0$ as $k_x\rightarrow\infty$.

%The fluid variables are kept continuous in $y$ but discrete in time.
%The pressure sub-problem solves
%\begin{align}
%p_{yy}^{n}(y) - k_x^2 p^{n}(y) &= 0, \label{eq:pressureSubProblem}\\
%p^{n}(H) &= 0, \label{eq:pressureTopBoundary}
%\end{align}
%% 
%with an additional algorithm dependent interface condition at $y=0.$ The
%general solution to \eqref{eq:pressureSubProblem}--\eqref{eq:pressureTopBoundary}
%is
%\begin{align}
%p^n(y) = p_I^n \frac{\sinh(k_x(H-y))}{\sinh(k_x H)}, \label{eq:pressureSubProblemSolution}
%\end{align}
%%
%where $p_I^n$ is the interface pressure at time $t^n$, determined by the interface condition.
%The pressure gradient at the interface, needed to advance the fluid interface velocity,
%is given by
%\begin{align}
%\partial_y p^n(0) = - \frac{p_I^n}{\Heff},
%\end{align}
%%
%where
%\begin{align}
%\Heff = \frac{\tanh(k_x H)}{k_x}.
%\end{align}
%%
%For the 1D problem ($k_x = 0$), $\Heff = H.$ When $k_x \rightarrow \infty,$ 
%$\Heff \rightarrow 0.$
%For this simplified model problem analysis, only the fluid velocity at the interface
%is needed, which will be denoted as $v_f^n$ at time $t^n.$

\subsection{Interface coupling}

The evolution of the solid given by the equations in~\eqref{eq:advSrcB}, \eqref{eq:advSrcA} and~\eqref{eq:SrcD} requires a boundary condition on the interface, $y=0$, corresponding to the incoming characteristic variable.  Similarly, the evolution of the fluid given by the equations in~\eqref{eq:fluidModelDiscrete} requires a boundary condition at $y=0$, which can be interpreted as an interface pressure needed to complete the elliptic problem for the fluid pressure as in~\eqref{eq:pressureSubProblemSolution}.  These two boundary conditions come from the matching conditions at the interface involoving the vertical velocity and normal stress.  In terms of the discretization of the Fourier coefficents for the model problem, the coupling at the interface takes on different forms depending on the choice of the partitioned scheme.  Since the behavior of the fluid for the model problem is determined by the solution of an elliptic problem for the pressure and an evolution equation for the vertical velocity on the interface, the coupling of the fluid to the behavior of the solid can be reduced to a modified boundary condition for the solid depending on the partitioned scheme employed as we discuss below.

Let us first consider the AMP algorithm and its interface coupling scheme.  The general algorithm was described in Section~\ref{sec:partitionedAlgorithms}, and we follow this basic description but with suitable modifications for the choices of the discretizations made for the present model problem.  Let us assume that the discrete characteristic variables for the solid given by $\bc^{n}_j$, $\ac^{n}_j$ and $\dc^{n}_j$ are known at time levels $t\sp n$ and $t\sp{n-1}$ for all grid points, $y_j=j\dy$, $j=0,-1,\ldots$, including a ghost point at $j=1$.  We also assume that the interface velocity, $v_I\sp n$, is known at $t\sp n$ and $t\sp{n-1}$.  The evolution equations for the solid variables in~\eqref{eq:bLax}, \eqref{eq:aLax} and~\eqref{eq:dTrap} are used to advance the variables to $t\sp{n+1}$, and from these we compute the solid velocity and normal stress on the interface using
\begin{align}
{\bar v}_{2,0}\sp{n+1} = \frac{1}{2\zp} (\bc^{n+1}_0-\ac^{n+1}_0), \qquad
{\bar\sigma}_{22,0}\sp{n+1} = \frac{1}{2} (\bc^{n+1}_0+\ac^{n+1}_0).
\label{eq:interfaceSolidVelocityAndStress}
\end{align}
We next compute an extrapolated interface velocity, $v_I\sp{(e)}$, using a second-order accurate BDF-type integration of the evolution equation for the fluid velocity.  This gives the formula
\begin{align}
v_I^{(e)} = \frac{4}{3} v_I^n - \frac{1}{3} v_I^{n-1} - \frac{2\dt}{3 \rho}\partial_y p(0,t^{n+1}),
\label{eq:extrapInterfaceVelocity}
\end{align}
where the pressure gradient on the interface is given in~\eqref{eq:interfacePressureGradient}.  This extrapolated value for the fluid is averaged with the interface velocity for the solid from~\eqref{eq:interfaceSolidVelocityAndStress} to give
\begin{align}
v_I^{n+1} = \frac{\zf}{\zf + \zp}\,v_I^{(e)} + \frac{\zp}{\zf + \zp}\,{\bar v}_{2,0}\sp{n+1},
\label{eq:interfaceVelocityModel}
\end{align}
where we take $\zf = \rho H/\dt$.  For later convenience, define the weights
\begin{align}
\theta_f=\frac{\zf}{\zf + \zp},\qquad {\bar\theta}_p=\frac{\zp}{\zf + \zp},
\label{eq:weights}
\end{align}
and we note that $\theta_f+{\bar\theta}_p=1$.  The AMP condition for the fluid pressure given in~\eqref{eq:AMPpressureBC} requires an acceleration of the interface, and for this we use the backward difference formula
\begin{align}
\dot{v}_I^{n+1} = \frac{1}{2\Delta t} \left(3v_{I}^{n+1} - 4v_{I}^{n} + v_{I}^{n-1}  \right).
\label{eq:interfaceAcceleration}
\end{align}
Using~\eqref{eq:extrapInterfaceVelocity} in~\eqref{eq:interfaceVelocityModel} to eliminate $v_I\sp{(e)}$, and then using the computed result in~\eqref{eq:interfaceAcceleration} to eliminate $v_{I}^{n+1}$ gives an alternate expression for the acceleration having the form
\begin{align}
\dot{v}_I^{n+1} = \theta_f\left(\frac{p_I^{n+1}}{\rho \Heff}\right) + {\bar\theta}_p\left(\frac{3{\bar v}_{2,0}\sp{n+1} - 4v_{I}^{n} + v_{I}^{n-1}}{2\Delta t} \right),
\label{eq:interfaceAccelerationNew}
\end{align}
which shows that the acceleration of the interface is also a weighted average of the acceleration from the fluid and that computed from the solid.  Finally, the AMP condition for the fluid pressure in~\eqref{eq:AMPpressureBC} reduces to 
\begin{align}
-p_I^{n+1}-\frac{\zp \dt}{\rho\Heff}\, p_I^{n+1} = {\bar\sigma}_{22,0}^{n+1} - \zp \dt \,\dot{v}_I^{n+1}.
\label{eq:AMPpressureBCmodel}
\end{align}
Using~\eqref{eq:interfaceAccelerationNew} in~\eqref{eq:AMPpressureBCmodel} to eliminate $\dot{v}_I^{n+1}$, and then solving for the interface pressure gives
\begin{align}
-p_I^{n+1} = \frac{M}{M+{\bar\theta}_p}\left[{\bar\sigma}_{22,0}^{n+1} - \zp{\bar\theta}_p\left(\frac{3}{2}{\bar v}_{2,0}\sp{n+1} - 2v_{I}^{n} + \frac{1}{2}v_{I}^{n-1} \right)\right],
\label{eq:interfacePressureModel}
\end{align}
where $M$ is a mass ratio given by
\begin{align}
M = \frac{\rho\Heff}{\zp \dt} = \frac{\rho\Heff}{\rhos \cp \dt}.
\label{eq:AcousticMassRatio}
\end{align}
We may now complete the time step for the solid variables by specifying values for the incoming and outgoing characteristic variables in the ghost points using
\begin{align}
\bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 a_I\sp{n+1},\qquad \ac^{n+1}_1 = 2 \ac^{n+1}_0 - \ac^{n+1}_{-1},
\label{eq:interfaceBCsForSolid}
\end{align}
where $a_I\sp{n+1}$ is an interface value for the incoming characteristic variable determined by
\begin{align}
a_I\sp{n+1} = -p_I^{n+1} + \zp v_I^{n+1},
\label{eq:incomingCharacteristicInterfaceModel}
\end{align}
Thus, the boundary condition for incoming characteristic variable is specified by $a_I\sp{n+1}$ (using a second-order accurate average) and the outgoing characteristic variable at the ghost point is given by a simple extrapolation.

For the AMP algorithm, the interface velocity and pressure used in~\eqref{eq:incomingCharacteristicInterfaceModel} to define the interface value for the incoming characteristic variable are given by the formulas in~\eqref{eq:interfaceVelocityModel} and~\eqref{eq:interfacePressureModel}, respectively, while the corresponding interface values for the TP and ATP algorithms use difference formulas.  For the TP algorithm, the interface velocity is given by the solid, while the interface stress is determined by the fluid.  This specification leads to
\begin{align}
v_I\sp{n+1}={\bar v}_{2,0}\sp{n+1},\qquad p_I\sp{n+1}=\rho\Heff\, \dot{v}_I^{n+1},
\label{eq:interfaceValuesTPscheme}
\end{align}
where the solid velocity is given in~\eqref{eq:interfaceSolidVelocityAndStress} and the interface acceleration is given in~\eqref{eq:interfaceAcceleration}.  For the ATP algorithm, the interface velocity is given by the fluid, while the interface stress is determined by the solid, and this gives
\begin{align}
v_I\sp{n+1}=v_I\sp{(e)},\qquad p_I\sp{n+1}=-{\bar\sigma}_{22,0}^{n+1},
\label{eq:interfaceValuesATPscheme}
\end{align}
where the fluid velocity is given in~\eqref{eq:extrapInterfaceVelocity} and the solid stress is given in~\eqref{eq:interfaceSolidVelocityAndStress}.  It is worth noting that values specified for the TP and ATP algorithms in~\eqref{eq:interfaceValuesTPscheme} and~\eqref{eq:interfaceValuesATPscheme}, respectively, agree with values given by the AMP algorithm in the limiting cases of a heavy solid ($\zp\rightarrow\infty$) and a light solid ($\zp\rightarrow0$).

%Following section \ref{sec:partitionedAlgorithms}, the AMP algorithm is applied
%to the simplified model problem.
%In the limit of a heavy solid, the AMP conditions approach a 
%no-slip condition for the fluid and a traction condition for the solid.
%In the light solid limit, the conditions approach a traction condition for 
%the fluid and a no-slip condition for the solid.
%Only the fluid solution at the interface is necessary to advance the solid in time.
%The AMP algorithm is given by the following.
%
%\listAlgorithm{AMP Algorithm (added-mass partitioned)}{
%\item Advance the solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
%\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
%$j = 0,\, -1, \, -2, \, -3, \, \ldots$.
%
%\item Obtain the predicted velocity and traction from the solid.
%\begin{align}
%v_s^{n+1} &= \frac{1}{2 \zp} \left(\bc^{n+1}_0 - \ac^{n+1}_0 \right) \\
%\sigma_s^{n+1} &= \frac{1}{2} \left(\bc^{n+1}_0 + \ac^{n+1}_0 \right)
%\end{align}
%
%\item Advance the fluid interface velocity using a BDF scheme on
%the fluid momentum equation.
%\begin{align}
%v_f^{n+1} = \frac{4}{3} v_I^n - \frac{1}{3} v_I^{n-1} 
%+ \frac{2\dt}{3 \rho \Heff} 
% p_I^{n+1} 
%\end{align}
%%
%
%\item Set the interface velocity as the impedance weighted average
%of the fluid and solid velocities using $\zf = \rho H/\dt$. 
%\begin{align}
%v_I^{n+1} = \frac{\zf v_f + \zp v_s}{\zf + \zp} 
%\end{align}
%
%\item Calculate the interface acceleration using a second order accurate
%backward difference formula.
%\begin{align}
%\dot{v}_I^{n+1} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{n+1} 
%  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
%\end{align}
%
%\item Solve the Poisson equation for the fluid pressure with
%the following AMP Robin condition specified at $y=0.$
%\begin{alignat}{2}
%-\ph^{n+1}+\frac{\zp \dt}{\rho} \ph_y^{n+1} &= 
%\sigma_s^{n+1} - \zp \dt \dot{v}_I^{n+1}, \quad && y = 0, 
%\end{alignat}
%
%Given the general solution in equation \eqref{eq:pressureSubProblemSolution},
%the interface pressure is 
%\begin{align}
%p_I^{n+1} &= \frac{1}{M \eta+1} 
%\rho \dot{v}_I \Heff
% - \frac{M \eta}{M \eta+1} \sigma_s,
%\end{align}
%%
%where
%\begin{align}
%M &= \frac{\rho H}{\zp \dt} = \frac{\rho H}{\rhos \cp \dt}, \label{eq:AcousticMassRatio} \\
%\eta &= \frac{\Heff}{H} = \frac{\tanh(k_x H)}{k_x H} \label{eq:Eta}
%\end{align}
%
%\item 
%%Set the interface traction $\sigma_I^{n+1} = -p_I^{n+1}.$
%Set the incoming $\cp^-$ characteristic, $\bc,$ using the interface velocity and stress.
%%$\delta = \rho/\rhos.$
%\begin{align}
%\bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right).
%% \bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 
%% \left[\frac{1}{1+\delta} 
%% \left(2 \sigma_I^{n+1} - \frac{\ac^{n+1}_{1} + \ac^{n+1}_{-1}}{2} \right)
%% +\frac{\delta}{1+\delta} \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right) \right].
%\end{align}
%
%\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$
%\begin{align}
%\ac^{n+1}_1 = 2 \ac^{n+1}_0 - \ac^{n+1}_{-1}
%\end{align}
%
%} \\
%
%% The solid is advanced on the interior and the boundary in the first two steps.
%% Next the fluid velocity is obtained in step 3. 
%% The interface velocity is projected using an impedance weighted average of the
%% fluid and solid values. 
%% This is used to determine the interface acceleration, which is used in
%% the pressure solution for step 7.
%% Afterwards, the solid boundary conditions are applied to obtain the ghost points.
%
%The acoustic mass ratio, $M$, defined in \eqref{eq:AcousticMassRatio},
%is the ratio of the mass of the fluid in a column of height 
%$H$ over the mass of a solid with the same cross section
%of height $\cp \dt,$ or the distance a p-wave travels in a single time step.
%The mass ratio is a measure of the prevalence of the added mass effect.
%For a heavy solid, the mass ratio is small and therefore added mass effects are small. 
%The mass ratio is inversely proportional to $\rhos$ and $\dt,$ therefore
%added mass effects can arise both in light solids and solids with a fine mesh.
%$\eta$ is the ratio between the effective fluid column height and the true fluid column height.
%
%The key behavior of the AMP algorithm is observed by taking the heavy and
%light solid limits. When $\zp \rightarrow \infty,$ the interface velocity
%and pressure approach the following limits.
%\begin{align}
%v_I^{n+1} &= 
%\begin{cases}
%v_s, & \zp \rightarrow \infty \\
%v_f, & \zp \rightarrow 0 
%\end{cases} \\
%p_I^{n+1} &= 
%\begin{cases}
%-\sigma_s, & \zp \rightarrow \infty \\
%\rho \dot{v}_I \Heff, & \zp \rightarrow 0 
%\end{cases}
%\end{align}
%%
%Corresponding algorithms for the TP (traditional partitioned) and the
%ATP (anti-traditional partitioned) schemes can be applied to the simplified model 
%problem following section \ref{sec:partitionedAlgorithms}.


\subsection{Stability analysis of AMP, TP and ATP schemes}

%
\newcommand{\nn}{\alpha}

In order to assess the stability of the AMP, TP and ATP schemes, we consider normal mode solutions of the discrete equations for the solid with the appropriate interface conditions.  For this analysis, we let
\begin{align}
\bc^{n}_j = \amp^n \tbc_j, \qquad 
\ac^{n}_j = \amp^n \tac_j, \qquad 
\dc^{n}_j = \amp^n \tdc_j,
\end{align}
%
where $\amp$ is an amplification factor and $(\tbc_j,\tac_j,\tdc_j)$ are spatial grid functions. The scheme is said to be weakly stable if there are no non-trivial solutions with $|\amp| > 1$.  Our strategy for determining regions of stability will be to search for unstable modes with $|A| > 1$, and then identify regions of the parameter space where no non-trivial solution exist.  To do this, we begin by finding the general solution for the spatial grid functions satisfying the discrete equations and regularity condition as $j\rightarrow-\infty$, assuming $|A| > 1$.  We then apply the conditions at the interface to determine whether non-trivial solutions exist.
%First, the analysis is split into a spacial and temporal problem. The tilde variables 
%will be determined from the interior discretization and boundary condition as 
%$y \rightarrow -\infty.$ Solutions for the amplification factor will be found by
%finding non-trivial solutions when the normal mode anzatz is
%substituted into the interface conditions.

The discrete equations for the solid in~\eqref{eq:bLax}, \eqref{eq:aLax} and~\eqref{eq:dTrap}, with $\tacv_j = [\tbc_j,\tac_j,\tdc_j]^T$, can be written as a system of linear, second-order difference equations of the form
\begin{align}
[H_0 + H_1 \delta_0 + H_2 \delta_+ \delta_-] \tacv_j = 0,
\label{eq:DifferenceEquation}
\end{align}
%
where
% \begin{align}
% H_{0} &= 
% \left[\begin{array}{ccc}
% -\frac{\lx^2}{4}& \frac{\lx^2}{4}&-i \lx \\
% \frac{\lx^2}{4}&-\frac{\lx^2}{4}&i \lx \\
% - \frac{i \lx}{4} & \frac{i \lx}{4}&0 
% \end{array}\right], \\
% H_{1} &= 
% \left[\begin{array}{ccc}
% -\frac{\ly}{2} &0&\frac{i \lx \ly}{4} \\
% 0&\frac{\ly}{2}&\frac{i \lx \ly}{4} \\
% 0 & 0&0 
% \end{array}\right], \\
% H_{2} &= 
% \left[\begin{array}{ccc}
% \frac{\ly^2}{2} &0&0 \\
% 0&\frac{\ly^2}{2}&0 \\
% 0 & 0&0 
% \end{array}\right].
% \end{align}
%\begin{align}
%H_{0} &= 
%-A^2 
%\left[\begin{array}{ccc}
%1&0&0 \medskip\\
%0&1&0 \medskip\\
%-\frac{i \lx}{3}&\frac{i \lx}{3}&1
%\end{array}\right] 
%+A 
%\left[\begin{array}{ccc}
%1- \frac{\lx^2}{4}&\frac{\lx^2}{4}&i \lx \smallskip\\
%\frac{\lx^2}{4}&1-\frac{\lx^2}{4}&-i \lx \smallskip\\
%0&0&\frac{4}{3}
%\end{array}\right] 
%-
%\left[\begin{array}{ccc}
%0&0&0 \medskip\\
%0&0&0 \medskip\\
%0&0&\frac{1}{3}
%\end{array}\right] \\
%H_{1} &= 
%A \left[\begin{array}{ccc}
%\frac{\ly}{2} &0&\frac{i \lx \ly}{4} \\
%0&-\frac{\ly}{2}&\frac{i \lx \ly}{4} \\
%0 & 0&0 
%\end{array}\right], \\
%H_{2} &= 
%A \left[\begin{array}{ccc}
%\frac{\ly^2}{2} &0&0 \\
%0&\frac{\ly^2}{2}&0 \\
%0 & 0&0 
%\end{array}\right].
%\end{align}
\[
\begin{array}{c}
\displaystyle{
H_{0} = 
-A^2 
\left[\begin{array}{ccc}
1&0&0 \medskip\\
0&1&0 \medskip\\
-\frac{i \lx}{3}&\frac{i \lx}{3}&1
\end{array}\right] 
+A 
\left[\begin{array}{ccc}
1- \frac{\lx^2}{4}&\frac{\lx^2}{4}&i \lx \smallskip\\
\frac{\lx^2}{4}&1-\frac{\lx^2}{4}&-i \lx \smallskip\\
0&0&\frac{4}{3}
\end{array}\right] 
-
\left[\begin{array}{ccc}
0&0&0 \medskip\\
0&0&0 \medskip\\
0&0&\frac{1}{3}
\end{array}\right],
} \bigskip\\
\displaystyle{
H_{1} = 
A \left[\begin{array}{ccc}
\frac{\ly}{2} &0&\frac{i \lx \ly}{4} \\
0&-\frac{\ly}{2}&\frac{i \lx \ly}{4} \\
0 & 0&0 
\end{array}\right], \qquad
H_{2} = 
A \left[\begin{array}{ccc}
\frac{\ly^2}{2} &0&0 \\
0&\frac{\ly^2}{2}&0 \\
0 & 0&0 
\end{array}\right].
}
\end{array}
\]
%
Solutions of the difference equations in~\eqref{eq:DifferenceEquation} are sought in the form $\tacv_j = \tilde\rev \p^j$, where $\tilde\rev$ is a constant vector and $\p$ is a scalar.  This implies the homogeneous linear system
\begin{align}
\left[ H_0 + H_1 \left(\p - \p\sp{-1}\right) + H_2 \left(\p - 2 + \p\sp{-1} \right) \right] \tilde\rev = 0.
\label{eq:evProblem}
\end{align}
%
Non-trivial vectors $\tilde\rev$ exist for values of $\p$ satisfying
\begin{align}
\det\left[ H_0 + H_1 \left(\p - \p\sp{-1}\right) + H_2 \left(\p - 2 + \p\sp{-1} \right) \right] = 0.
\label{eq:quarticPhi}
\end{align}
%
It can be shown that the algebraic condition in~\eqref{eq:quarticPhi} is equivalent to a quartic polynomial in $\p$ for which there are four roots, $\p_\nn$, $\nn=1,2,3,4$.  Since we seek spatial grid functions that are bounded as $j\rightarrow-\infty$, we are only interested in the roots satisfying $\vert\p_\nn\vert\ge1$.
%There are four roots for $\p.$ Since we require the solid variables to 
%be bounded as
%$y \rightarrow -\infty,$ \eqref{eq:bcInf}, we are only interested in solutions 
%where $|\p|^j \le 1$ as $j \rightarrow -\infty.$ Therefore, only roots where
%$|\p| \ge 1$ are solutions to the boundary condition.

\medskip\noindent
\textbf{Lemma}: \textit{If $|A| > 1$ and if $\lx$ and $\ly$ are chosen to satisfy a CFL condition, then the roots of the quartic polynomial implied by~\eqref{eq:quarticPhi} satisfy}
\begin{align}
|\phi_1| > 1, \qquad |\phi_2| > 1, \qquad |\phi_3| < 1, \qquad |\phi_4| < 1.
\label{eq:SizeOfEigenvalues}
\end{align}

\medskip\noindent
This result follows from a similar argument to that given in~\cite{DifferenceApproximationsForTheInitialBoundary}.  We first consider the scheme applied to the pure initial-value problem (Cauchy problem).  Setting $\phi=e\sp{i\vartheta}$ in~\eqref{eq:quarticPhi}, we determine a region of the $\lx$-$\ly$ plane for which $\vert A\vert\le1$ for all $\vartheta\in[0,2\pi]$.  This region is found numerically as discussed in~\ref{sec:CFLRegionCauchy}, and it corresponds to a region where the Cauchy problem is (Fourier) stable.  It is also shown that this stability region includes a region of $(\lx,\ly)$ satisfying a reasonable CFL restriction, namely $\lx\sp2+\ly\sp2\le1$.
%For this region, which
%(Fourier stability). Let $\phi = e^{i \omega}$. 
%% Noting that 
%% $(I+H_{-1})^{-1} = I-H_{-1},$ the solution for the amplification factor reduces 
%% to the following eigenvalue problem for $A$.
%% \begin{align}
%% A \rv = (I - H_{-1})
%% \left( I + H_0 + H_1 \left(e^{i \omega} - e^{-i \omega}\right)
%% + H_2 \left(e^{i \omega} - 2 + e^{-i \omega} \right) \right) \rev.
%% \end{align}
%The solution for the amplification factor reduces to the following eigenvalue problem for $A$.
%\begin{align}
%\left( H_0 + H_1 \left(e^{i \omega} - e^{-i \omega}\right)
%+ H_2 \left(e^{i \omega} - 2 + e^{-i \omega} \right) 
% \right) \rev = 0 \label{eq:evProblem}
%\end{align}
%%
%\das{For a range of values in the
%$\lx-\ly$ plane, the maximum amplification factor over $\omega \in [0,2\pi]$ 
%was computed numerically to determine the region where $|A| \le 1.$ 
%See \ref{sec:CFLRegionCauchy} for the details of these calculations.}
%For a reasonable CFL restriction on $\lx$ and $\ly$, $|A| \le 1$
%for $0 \le \omega \le 2 \pi$ and therefore the Cauchy scheme is stable.
Next, since $|A| \le 1$ when $|\phi| = 1$, we have that $|\phi| \ne 1$ when $|A| > 1$.  Thus, if $|A| > 1$ and if $(\lx,\ly)$ remains within the CFL restriction, then $\phi$ cannot cross the unit circle, $|\phi|=1$, as $(\lx,\ly)$ vary.  It is therefore only necessary to prove that the conditions on the roots in~\eqref{eq:SizeOfEigenvalues} hold for one set of parameters.  For $\lx=0$, the difference scheme reduces to a pair of decoupled Lax-Wendroff schemes (and a BDF scheme applied to $\partial_td=0$), where it is well known (see~\cite{GKSII} for example) that the conditions in~\eqref{eq:SizeOfEigenvalues} hold provided $\vert\ly\vert\le1$.  Thus, the condition holds for all $(\lx,\ly)$ provided the CFL condition is satisfied.

In view of the above Lemma, we can now write the general solution for $\acv^n_j=[\bc^{n}_j,\ac^{n}_j,\dc^{n}_j]\sp T$, satisfying the regularity condition and assuming $\vert A\vert>1$, in the form
\begin{align}
\acv^n_j = \amp^n \left(k_1 \tilde\rev_1 \p_1^j + 
k_2 \tilde\rev_2 \p_2^j \right), \label{eq:EigenvectorExpansion}
\end{align}
where $k_1$ and $k_2$ are scalar constants.  Let $\tilde\rev_\nn = [\qn{\nn},\rn{\nn},\sn{\nn}]^T$ for $\nn = 1,2$.  We note that the third equation in the matrix system~\eqref{eq:evProblem} implies
%Using the third component of equation \eqref{eq:DifferenceEquation}, 
%$\sn{n}$ can be found in terms of $\qn{n}$ and $\rn{n}$.
\begin{align}
% \sn{n} = \frac{i \lx}{4} \frac{A+1}{A-1} (\rn{n} - \qn{n}) 
\sn{\nn} = \frac{A^2 i \lx}{3 A^2- 4 A + 1} (\qn{\nn} - \rn{\nn}),\qquad \nn = 1,2,
\end{align}
so that the third component of $\acv^n_j$ can be eliminated in terms of the first two components.  The final two constraints are given by the interface conditions in~\eqref{eq:interfaceBCsForSolid}, and this leads to a homogeneous system for $\kv=[k_1,k_2]\sp T$ of the form
\begin{align}
\dMat \kv= \left[\begin{array}{cc}
\dComp_{11} & \dComp_{12} \\
\dComp_{21} & \dComp_{22}
\end{array}\right] 
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right] = 0.
\label{eq:StabilitySystem}
\end{align}
%
The coefficients of the matrix $\dMat$ involve the amplitude factor $\amp$, and these are given in~\ref{sec:ComponentsOfDmat} for the AMP, TP and ATP schemes.  For non-trivial solutions, we seek solutions for $\amp$ such that
\begin{align}
\det(\dMat) = \dComp_{11} \dComp_{22} - \dComp_{12} \dComp_{21} = 0.
\label{eq:determinantCondition}
\end{align}
%
We first proceed with an analysis of the 1D case assuming $\lx = 0$.  After finding solutions for~$\amp$ when $\lx = 0$, we use a continuation procedure to determine solutions for $\amp$ numerically as $\lx$ increases from zero.

\subsubsection{1D schemes, $\lx=0$}

As noted earlier, the discrete evolution equations in~\eqref{eq:bLax} and~\eqref{eq:aLax} for the solid reduce to a pair of standard Lax-Wendroff schemes (without source terms) for the variables associated with incoming and outgoing characteristics when $\lx=0$.  Accordingly, the first two components of~\eqref{eq:DifferenceEquation} become
\begin{align}
A \tbc_j = \left( 1 + \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tbc_j,\qquad
A \tac_j = \left( 1 - \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tac_j.
\end{align}
%
Setting $\tbc_j=\tbc_0\p_{\bc}\sp j$ and $\tac_j=\tac_0\p_{\ac}\sp j$ yields the eigenvalues
\begin{align}
\p_{\bc,\pm} =\frac{\amp-(1-\ly\sp2) \pm \sqrt {\amp\sp2-(2\amp-1)(1-\ly\sp2)}}{\ly \left( \ly+1 \right) }, \qquad 
\p_{\ac,\pm} =  \frac{1}{\p_{\bc,\mp}}.
\label{eq:eigenvalueOneD}
\end{align}
%
If $\vert\amp\vert>1$ and if $\ly$ satisfies the CFL constraint $\vert\ly\vert\le1$, then one eigenvalue from each plus-minus pair in~\eqref{eq:eigenvalueOneD} has magnitude greater than one, while the other has magnitude less than one in agreement with~\eqref{eq:SizeOfEigenvalues}.  Let $\p_1$ to be the eigenvalue from $\p_{\bc,\pm}$ with magnitude greater than one and let $\p_2$ to be the corresponding eigenvalue $\p_{\ac,\pm}$.  Assuming the principal branch of the square-root function in~\eqref{eq:eigenvalueOneD}, we set
\begin{align}
(\p_1,\p_2)=
\begin{cases}
(\p_{\bc,+},\p_{\ac,+}), & \hbox{if $\Re(A) \ge 1 - \ly^2$}, \\
(\p_{\bc,-},\p_{\ac,-}), & \hbox{if $\Re(A) < 1 - \ly^2$}.
\end{cases}
\end{align}
%
%
%\das{In~\ref{sec:PiecewiseDefinition}, we show that 
%\begin{align}
%\p_1 &= 
%\begin{cases}
%\p_{\bc,+}, & \Re(A) > 1 - \ly^2 \\
%\p_{\bc,+}, & \Re(A) = 1 - \ly^2 \text{ and } \Im(A) > 0\\
%\p_{\bc,-}, & \Re(A) < 1 - \ly^2 \\
%\p_{\bc,-}, & \Re(A) = 1 - \ly^2 \text{ and } \Im(A) < 0
%\end{cases} \\
%\p_2 &= 
%\begin{cases}
%\p_{\ac,+}, & \Re(A) > 1 - \ly^2 \\
%\p_{\ac,+}, & \Re(A) = 1 - \ly^2 \text{ and } \Im(A) > 0\\
%\p_{\ac,-}, & \Re(A) < 1 - \ly^2 \\
%\p_{\ac,-}, & \Re(A) = 1 - \ly^2 \text{ and } \Im(A) < 0
%\end{cases} ,
%\end{align}
%%
%as long as $|A| > 1$ and $0 \le \ly \le 1.$}
%%
Since the evolution equations for $\bc_j\sp n$ and $\ac_j\sp n$ are decoupled, the corresponding eigenvectors in~\eqref{eq:EigenvectorExpansion} are unit vectors, $\tilde\rev_{1} = [1,0,0]^{T}$ and $\tilde\rev_{2} = [0,1,0]^{T}$, i.e.~$\qn{2} = \rn{1} = \sn{1} = \sn{2} = 0$, and the matrix $\dMat$ in~\eqref{eq:StabilitySystem} becomes diagonal. Thus, the determinant condition in~\eqref{eq:determinantCondition} reduces to
\begin{align}
\det(\dMat)= \dComp_{11} \dComp_{22} = 0.
\end{align}
\textcolor{red}{(Note changes here due to ordering of $a$ and $b$.)}
The component, $\dComp_{22}$, is associated with the extrapolation of the outgoing characteristic variable from~\eqref{eq:interfaceBCsForSolid}, and this factor is zero only if $\p_2=1$.  However, $\vert\p_2\vert>1$, so that $\dComp_{22}\ne0$ and thus $k_2=0$ in~\eqref{eq:EigenvectorExpansion}.  The remaining component, $\dComp_{11}$, is associated with the interface condition on the incoming characteristic variable, and this term takes different forms depending on the choice of the interface coupling (see~\ref{sec:ComponentsOfDmat}).  Manipulation of the constraint, $\dComp_{11}=0$, for the AMP, TP and ATP schemes leads to polynomials in $\amp$ of degrees~6, 6 and~4, respectively, whose coefficients depend on $\ly$ and $M_0=\rho H/(\zp \dt)$.
\textcolor{red}{(For now I am defining $M_0$ which is just $M$ with $\lx=0$.)}
  Due to the algebraic complexity, the software package Maple is used to generate the polynomials and compute the roots for given values of $(\ly,M_0)$.  We note that some roots of the polynomials may not be solutions of the determinant constraint and so these spurious roots are discarded.  If no valid roots are found satisfying $\vert\amp\vert>1$ for a given value of $(\ly,M_0)$, then we conclude that $k_1$ in~\eqref{eq:EigenvectorExpansion} must also be zero so that only the trivial solution exists and thus the scheme is (weakly) stable.

We find it convenient to explore the roots of the three polynomials in terms of the parameters $\ly$ and $\Mr$, where
\begin{align}
\Mr = M_0\ly= \frac{\rho H}{\rhos \dy}.
\label{eq:massRatio}
\end{align}
The latter parameter is the ratio of the mass contained in a fluid column of height $H$ to that of the solid with the same cross section and of height $\dy$.  Starting with the AMP scheme, we compute valid roots of its polynomial for an $800\times800$ array of parameter values on a logarithmic scale for the range $10^{-6} \le \lambda_y \le 1$ and $10^{-6} \le \Mr \le 10^{7}$.  For these values, no roots with $\vert\amp\vert>1$ are found, which provides a strong indication of stability of the 1D AMP scheme for $0<\ly\le1$ and $\Mr>0$.  Shaded contours of the maximum values of $\vert\amp\vert$ are displayed in the left plot of Figure~\ref{fig:acousticSolidStokesStabilityTP} for a range of values of $\Mr$ and $\ly$.  The roots of the polynomials associated with the 1D TP and ATP schemes are also computed for the same array of parameter values.  For these schemes, parameter values for which $\vert\amp\vert>1$ are found indicating that regions of instability exist for these scheme.  The right plot of Figure~\ref{fig:acousticSolidStokesStabilityTP} shows regions of stability of the TP and ATP schemes where no roots with $\vert\amp\vert>1$ are found.  We note that for a fixed value of $\ly=\cp \dt / \dy\in(0,1]$, decreasing the mesh spacings in both time and space corresponds to increasing the mass ratio $\Mr$ defined in~\eqref{eq:massRatio}.  The right plot in the figure indicates that the TP scheme becomes unstable as the mesh is refined, while the ATP scheme ultimately becomes stable.  In contrast, the AMP scheme is always stable, and these observations agree with the analysis of the first-order accurate difference schemes performed in~\cite{fib2014}.

% {
% % ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
% \newcommand{\figWidth}{8cm}
% \begin{figure}[h]
% \begin{center}
%   \includegraphics[width=\figWidth]{fig/AMPStability1D}
%   \includegraphics[width=\figWidth]{fig/FSIStabilityRegionBDF}
%   \caption{Left: Shaded contours of the maximum amplification factor $\vert\amp\vert$ 
%     for the AMP scheme for the parameters $\lambda_y = \cp \dt / \dy$ and $\Mr = \rho H / (\rhos \dy)$.
%     Right: Stability regions for the 1D TP and ATP schemes. 
%     Grid refinement corresponds to increasing $\Mr$, and thus the
%     TP scheme becomes unstable as the grid is refined while the ATP scheme becomes stable.
%   }  \label{fig:acousticSolidStokesStabilityTP}
% \end{center}
% \end{figure}
% }
{
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMPStability1D_log}
  \includegraphics[width=\figWidth]{fig/FSIStabilityRegionBDF_log}
  \caption{
    Left: Shaded contours of the maximum amplification factor $\vert\amp\vert$ 
    for the AMP scheme for the parameters $\lambda_y = \cp \dt / \dy$ and $\Mr = \rho H / (\rhos \dy)$.
    Right: Stability regions for the 1D TP and ATP schemes. 
    Grid refinement corresponds to increasing $\Mr$, and thus the
    TP scheme becomes unstable as the grid is refined while the ATP scheme becomes stable.
  }  \label{fig:acousticSolidStokesStabilityTP}
\end{center}
\end{figure}
}

%The roots of the AMP polynomial were found at an array of $800$ points in 
%$10^{-6} \le \lambda_y \le 1$ and $800$ points in $10^{-6} \le \Mr \le 10^{7}.$ 
%No unstable roots, $|A| > 1,$ were found. The same process was repeated for the 
%TP and ATP schemes for a range $10^{-6} \le \Mr \le 10.$ The stability region
%was plotted in figure \ref{fig:acousticSolidStokesStabilityTP}. 
%Since $\Mr \propto \dy^{-1},$ grid refinement will increase the mass ratio.
%The TP scheme will become unstable for sufficiently large $\Mr,$ therefore the 
%scheme is formally unconditionally unstable. On the other hand, the ATP scheme will 
%eventually become stable for a sufficiently large $\Mr.$ This scheme is weakly
%stable. Despite this, there is a significant
%region in parameter space where only the AMP scheme is stable.

The AMP, TP and ATP schemes can be implemented for the 1D FSI model problem, and then run numerically for different values of the parameters to check the results of the stability analysis.  
Initial conditions can be constructed so that the exact solution decays 
exponentially in time.
This corresponds to taking the initial condition, $b(y,0) = b_0(y) = 0$
(see~\ref{sec:SolutionToOneDimensional}). 
Since the interface velocity is expected to decay in time, we can assess the stability of the scheme by checking the 
magnitude of the interface velocity.  If this velocity grows in time, becoming larger than the initial interface velocity, then we consider the scheme to be unstable for the choice of parameter values.
For the AMP scheme, no parameter values are found for which the numerical results are unstable.  For the TP and ATP schemes, the colored marks in Figure~\ref{fig:acousticSolidStokesStabilityTPNumerical} indicate stability or instability of the numerical scheme for selected parameter values.  The black curves in the figure correspond to the stability boundaries obtained from the stability analysis.  We note that there is good agreement between the numerical results of the schemes and that given by the analysis.


%A 1D FSI numerical solver was used to verify the stability regions for the TP and ATP
%schemes. In figure \ref{fig:acousticSolidStokesStabilityTPNumerical}, points in
%$\Mr$-$\ly$ space were sampled to test for numerical instability. 
%It was found that the numerical results confirm that the stability region holds.


{
% ---- from codes/analysis/numerical/b4_runTP1DStability ---- $
% ---- from codes/analysis/numerical/b5_runATP1DStability ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/FSIStabilityTP1DNumerical}
  \includegraphics[width=\figWidth]{fig/FSIStabilityATP1DNumerical}
  \caption{Verification of the stability regions for the TP scheme (left)
    and the ATP scheme (right) using numerical solutions of the 1D FSI model problem. Green marks 
    correspond to a stable numerical solution, while red markers correspond to numerical instability.  The black curves give the stability boundaries obtained from the stability analysis.
  }  \label{fig:acousticSolidStokesStabilityTPNumerical}
\end{center}
\end{figure}
}


% talk about numerical results

% Numerical Results:
%  - convergence for each scheme
%  - confirm stability region for each scheme
%
%   TP:
%     - heavy solid convergence study
%     - show stability region
%   ATP: 
%     - light solid convergence study
%     - show stability region
%   AMP:
%     - heavy/light solid convergence study
%     - really heavy/really light

\subsubsection{2D schemes, $\vert\lx\vert>0$}

\newcommand{\zz}{{z}}  % root index
\newcommand{\NN}{{\mathcal{Z}}}  % number of roots

% derive eigenvectors with the idea that lx is small
% Now we approach the 2D model problem by considering $\lx$ to be a small 
% perturbation to the 1D problem. The main motivation for this is
% that the stability limit for the Cauchy problem requires $\lx < .3,$ (\todo{show this})
% and only $\lx^2$ appears in the discretization. 
%Additionally, the 2D added mass ratio
%$\Mr = (\rho \tanh(k_x H))/(k_x \rhos \dy)$ will only decrease as $k_x$ increases
The strategy for finding solutions of the determinant condition in~\eqref{eq:determinantCondition} for $\vert\lx\vert \ne 0$ is to use the solutions for $\amp$ of the 1D determinant condition as a starting point for a numerical root solver that performs a continuation as $\lx$ varies.  In addition to the principal continuation parameter $\lx$, the roots also depend on the parameters $\ly$ and $M=\rho\Heff/(\zp\dt)$, where $\Heff$ was defined previously in~\eqref{eq:interfacePressureGradient}.  As before, we find it convenient to examine the roots in terms of the mass ratio $\Mr$ introduced in~\eqref{eq:massRatio} and the height ratio, $\eta=\Heff/H$, which varies on $(0,1]$, and we note that $M=\Mr\eta$.  Using our continuation procedure, we are able to compute the roots of the determinant condition as a function of the parameters $\lx$, $\ly$ and $M=\Mr\eta$.  Though there are multiple roots, $\amp_\zz$, $\zz=1,2,\ldots,\NN$, for a given set of parameters, we are only interested in the amplification factor with the maximum modulus.  Define
\begin{align}
A_{\max}(\lx,\,\ly,\,\Mr \eta)=\max_{1\le\zz\le\NN}\vert\amp_\zz(\lx,\,\ly,\,\Mr \eta)\vert,
\end{align}
to be the maximum amplification factor in magnitude for a given set of parameters.  The pseudo-spectral approximation of the model problem given in~\eqref{eq:fluidModelDiscrete} and~\eqref{eq:solidModelDiscrete} depends on the normalized wave number $k_x$.  The corresponding discrete evolution equations for each Fourier mode of the approximation must all be stable for the chosen partitioned scheme to be stable (either the AMP, TP or ATP schemes).  Since $\lx$ and $\eta$ both depend on $k_x$, we are interested in the values of $A_{\max}$ for all possible values for $\lx$ and $\eta$.  Define
\begin{align}
\mathcal{A}_{\max}(\Mr,\ly) = 
\max_{\lx \in \mathcal{D}(\ly),\, \eta \in (0,1]} A_{\max}(\lx,\,\ly,\,\Mr \eta),
\label{eq:AmaxDefinition2D}
\end{align}
%
where $\mathcal{D}(\ly)$ gives the interval of $\lx$ satisfying the Cauchy stability bound for a given value of $\ly$ (see~\ref{sec:CFLRegionCauchy}).  We take $\mathcal{D}(\ly) = [0, (1 - \ly^2)^{1/2}]$.
Since the maximum amplification factor for the 1D case (with $\lx=0$) must be less than or equal to $\mathcal{A}_{\max}$, we are effectively examining whether the maximum amplification can increase when $\vert\lx\vert>0$. Figure~\ref{fig:lysmAMP2D} shows shaded contours of $\mathcal{A}_{\max}(\Mr,\ly)$ on the left, and the stability regions of the TP and ATP schemes on the right.  These plots are similar to the ones for the 1D analysis in Figure~\ref{fig:acousticSolidStokesStabilityTP}, indicating that the stability results provided by the 1D analysis are essentially unchanged when variations in the transfer direction are considered.  In fact, Figure~\ref{fig:lysmAMP2Doverlay} shows the stability regions for the TP and ATP schemes given by the 1D and 2D analyses overlayed.  Here, we observe that the stability regions given by the 2D analysis are only slightly smaller than those given by the 1D analysis.
% a surface plot of $\mathcal{A}_{\Mr}$
%and the stability region, $|A| \le 1$ in the $\Mr$-$\ly$ plane.
%There is a finite range of $\ly$ for which the AMP scheme is stable for all 
%$\lx,\,\Mr,$ and $\eta$.

\textcolor{red}{Will come back to this later.  I think the main point here is that we just showed above that the AMP scheme is stable for a large range of $\ly$ and mass ratios $\Mr$.  Given this, we can turn the question around and consider the region of stability of the AMP scheme in the $\lx$-$\ly$ plane for all values of $M=\Mr\eta$.  The objective of this analysis is to arrive at a CFL condition involving $\lx$ and $\ly$ such the AMP scheme is stable for any choice of the mass ratio.  Of course, the analysis is performed for a chosen model problem, but the results of the analysis can be used as a guide for the AMP scheme applied to the full FSI problem over a wide range of mass ratios.}  We can also search for a maximum amplification factor over all mass ratios,
$\mathcal{A}_{\text{CFL}},$ to see the CFL region for the AMP scheme in $\lx$-$\ly$ plane. 
Define
\begin{align}
\mathcal{A}_{\text{CFL}}(\lx,\ly) = 
\max_{0 < \Mr \eta < \infty} A_{\max}(\lx,\,\ly,\,\Mr \eta) .
\end{align}
%
This definition allows us to find a time step restriction regardless of the
mass ratio of the problem.
Figure \ref{fig:lylxAMP2D} shows a surface plot of $\mathcal{A}_{\text{CFL}}$
and the stability region, $|A| \le 1$ in the $\lx$-$\ly$ plane.

\textbf{Theorem}: \textit{By numerical evaluation of $\ACFL(\lx,\ly)$,
we have found that the AMP algorithm is weakly stable ($|\ACFL| \le 1$)
provided that $\lx^2 + \ly^2 \le 1$, i.e.}
\begin{align}
\dt \le \frac{1}{\cp} \left[\frac{1}{\dy^2} + k_x^2 \right]^{-1/2}.
\end{align}
%
\textit{This is a sufficient but not a necessary condition.}

%
% {
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
% \newcommand{\figWidth}{8cm}
% \begin{figure}[H]
% \begin{center}
%   \includegraphics[width=\figWidth]{fig/FSIStabilityRegion2D}
%   \caption{Stability region for the 1D and 2D TP and ATP schemes. 
%     $\bar{\Mr}$ is defined from 
%     equations \eqref{eq:MrbarTP}--\eqref{eq:MrbarATP} and is the worst
%     case mass ratio for all Fourier modes.
%     $\lambda_y = \bar{c} \dt / \dy$ is the CFL number.
%     The stability region for the AMP scheme spans 
%     $0 < \ly < 1,$ $0 < \bar{\Mr} < \infty.$ 
%     An increase in $\bar{\Mr}$ corresponds to grid refinement,
%     therefore TP scheme will become unstable and the ATP scheme will become stable.
%   }  \label{fig:acousticSolidStokesStabilityTP2D}
% \end{center}
% \end{figure}
% }
% {
% \newcommand{\figWidth}{8cm}
% \begin{figure}[h]
% \begin{center}
%   \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_sm_surf}
%   \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_sm_cont}
%   \caption{Left: surface plot of maximum $|A|$ over $\lx \in [0,1]$
%     and $\eta \in (0,1]$ for the AMP scheme.
%     Right: the green fill indicates the stability region $|A| \le 1.$
%     For reference, 
%     $\ly = \cp \dt / \dy,\, \Mr = \rho H / (\rhos \dy),\, \lx = \cp k_x \dt,\, 
%     \eta = \tanh(k_x H)/ (k_x H).$
%   } \label{fig:lysmAMP2D}
% \end{center}
% \end{figure}
% }
{
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_03_03_N50_LargeRange_Nep200_new_ly_sm_surf}
  \includegraphics[width=\figWidth]{fig/TP_continuation_03_03_N50_LargeRange_Nep200_newerStabilityRegions2D}
  \caption{Left: Shaded contours of the maximum amplification factor 
    $\mathcal{A}_{\max}(\Mr,\ly)$ 
    (as defined in equation \eqref{eq:AmaxDefinition2D})
    for the AMP scheme for the parameters $\ly=\cp \dt/\dy$ and $\Mr=\rho H/ (\rhos \dy).$
    Right: Stability regions (ie. where $\mathcal{A}_{\max}(\Mr,\ly) \le 1$)
    for the 2D TP and ATP schemes. 
    Grid refinement corresponds 
    to increasing $\Mr$, and thus the
    TP scheme becomes unstable as the grid is refined while the ATP scheme becomes stable.
  } \label{fig:lysmAMP2D}
\end{center}
\end{figure}
}
{
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/TP_continuation_03_03_N50_LargeRange_Nep200_newerStabilityRegions_1D_and_2D}
  \caption{Stability regions for the TP and ATP schemes in 1D and 2D for the 
    parameters $\ly=\cp \dt/\dy$ and $\Mr=\rho H/ (\rhos \dy).$
    The lighter shaded colors represent the 1D regions and the darker shaded colors represent
    the 2D regions.
    Grid refinement corresponds to increasing $\Mr$, and thus the
    TP scheme becomes unstable as the grid is refined while the ATP scheme becomes stable.
  } \label{fig:lysmAMP2Doverlay}
\end{center}
\end{figure}
}
{
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_lx_surf}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_lx_cont}
  \caption{
    Left: surface plot of maximum $|A|$ over $\Mr \eta \in [10^{-6},10^{6}]$
    for the AMP scheme.
    Right: the green fill indicates the stability region $|A| \le 1.$
    The dotted line is a plot of
    $\lx^2 + \ly^2 = 1$. 
    For reference, 
    $\ly = \cp \dt / \dy,\, \Mr = \rho H / (\rhos \dy),\, \lx = \cp k_x \dt,\, 
    \eta = \tanh(k_x H)/ (k_x H).$
  } \label{fig:lylxAMP2D}
\end{center}
\end{figure}
}

%\subsection{Stability analysis of TP scheme with iterations}
%
%\das{Should this be in this paper?}
%\textcolor{red}{DWS: not sure, but will skip this for now...}
%\das{Put iterations scheme here. Also want to note that there are better iterative
%schemes such as Aitken acceleration.}
%The TP scheme is more commonly used with iterations to avoid the added mass instability
%when refining grids. We perform an analysis of the TP iteration to understand
%how to choose the under-relaxation factor and how many iterations to take.
%Define the error between iterations to be the difference in interface velocities
%\begin{align}
%e^{(k)} = v_I^{(k+1)} - v_I^{(k)}.
%\end{align}
%%
%By taking the difference between the current and previous iteration variable for
%each step of the TP iteration, one can derive that
%\begin{align}
%e^{(k)} &= \left(1 - \omega \left(\frac{3}{2} \Mra + 1 \right)\right) e^{(k-1)}.
%\end{align}
%%
%Define the amplification factor, $\ampI = 1 - \omega \left(\frac{3}{2} \Mra + 1 \right)$
%where $e^{(k)} = A^{k} e^{(0)}.$
%$\Mra$ is dependent on the wave number, $k_x.$ In order to optimize the convergence rate,
%$\ampI$ needs to be optimized for all wave numbers.
%\begin{align}
%\Mra = \frac{\rho \tanh(k_x H)}{\zp \dt k_x} 
%= \frac{\rho H}{\zp \dt} \frac{\tanh(k_x H)}{k_x H} 
%= \Mra_0 \eta
%\end{align}
%%
%where $\Mra_0 = (\rho H) / (\zp \dt)$ is the 1D acoustic mass ratio and 
%$\eta = \tanh(k_x H) / (k_x H)$ is the 2D scale factor. To accommodate all
%potential wave numbers in the $x$ direction, we consider $\eta \in [0,1].$
%Let $\Mra = \Mra(\eta) = \Mra_0 \eta.$ The amplification factor for a given
%$\omega$ and $\eta$ is
%\begin{align}
%\ampI(\eta,\omega) = a - \omega \left(\frac{3}{2} M_0 \eta + 1 \right).
%\end{align}
%%
%We pose the following optimization problem to find the optimal 
%under-relaxation parameter, $\omega^*$.
%\begin{align}
%\omega^* = \argmin_{\omega} \max_{0 \le \eta \le 1} |A(\eta,\omega)|
%\end{align}
%%
%Since $\ampI$ is linear in $\eta$ and $\omega$ and $|\ampI| > 0,$ the maximum 
%amplification factor for a 
%given $\omega$ will occur on the boundary, $\eta = 0$ or $\eta = 1.$ 
%\begin{align}
%\ampI(\eta=0,\omega) = |1-\omega|, \quad 
%\ampI(\eta=1,\omega) = \left| 1 - \omega \left(\frac{3}{2} M_0 + 1 \right) \right|
%\end{align}
%%
%The choice of $\omega$ that minimizes both expressions corresponds to solving
%$\ampI(\eta=0,\omega^*) = \ampI(\eta=1,\omega^*).$ It can be shown that
%\begin{align}
%\omega^* = \frac{4}{3 \Mra_0 + 4}, \quad \ampI^* = \frac{3 M_0}{3 M_0 + 4}.
%\end{align}
%%
%This is a sensible result. The TP scheme suffers from added mass instability
%for fine grids and light solids, which correspond to large acoustic mass ratios.
%The under-relaxation parameter scales with $\Mra_0^{-1}$ to stabilize the added mass
%effects. As a penalty, the amplification factor approaches $1$ for large $\Mra_0.$
%To get a sense of computational cost for using TP iterations, we look at the number
%of iterations needed for the relative error, $|e^{(k)}/e^{(0)}|,$ to converge to 
%a desired tolerance, $\tau.$  It is easy to show that if $|A^*|^k < \tau,$ $k$ must 
%satisfy
%\begin{align}
%k &> \frac{\log (\tau) }
%{\log \left(\frac{3 M_0}{3 M_0 + 4} \right)} .
%\end{align}
%% 
%We are interested in the asymptotic behavior for $\Mra_0 \gg 1.$ The denominator
%of the above expression is asymptotically equivalent to
%\begin{align}
%\log \left(\frac{3 \Mra_0}{3 \Mra_0 + 4} \right) =
% \log \left(\frac{1}{1 + \frac{4}{3 \Mra_0} } \right)
%\sim  \log \left(1 - \frac{4}{3 \Mra_0} + ... \right) 
%\sim -\frac{4}{3 \Mra_0} + ...
%\end{align}
%%
%Therefore 
%\begin{align}
%k > -\frac{3}{4} M_0 \log(\tau) = 
%-\frac{3 }{4} \frac{\rho H }{ \bar{\rho} \bar{c} \Delta t} \log(\tau).
%\end{align}
%% 
%The required number of iterations is proportional to $\dt^{-1}.$ 
%For a viscous fluid simulation, the viscous terms can be treated as
%implicitly or explicitly.
%When an implicit solver is chosen, the time step will be proportional to
%the grid spacing and the number of iterations will double when the grid is refined 
%by a factor of $2$. 
%When an explicit solver is chosen, the time step will be proportional to the 
%square of the grid spacing and the number of iterations will quadruple when the grid
%is refined by a factor of $2.$
%

% numerical results 



%%%%%%%%%%%%% old paper
% \subsection{Discretization}

% talk about fluid and solid discretization in x. 
% discrete fourier series on grid 
% % \wdh{We discretize the fluid and solid variables in the $x$~direction using a uniform
% % grid with spacing $\dx=L/(N_x+1)$. The grid points are given by $x_\ell=\ell\dx$,
% % $\ell=0,1,\ldots,N_x$.  The choice of discrete approximations to the
% % $x$~derivatives in the equations plays little role in the analysis.  Therefore, it is
% % convenient to use a pseudo-spectral approximation by expanding
% % each component $q$ of the solution $(\qv,\qsv)$ in a discrete Fourier series of
% % the form
% % % which gives a formally {\em exact} approximation,  $i\kx$, to an $x$-derivative.
% % % After discretizing in the $x$~direction we will expand the solution in a discrete Fourier series of the form
% % \begin{align}
% %    q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_\ell/L} \qHat_{k}(y,t), \qquad \ell=0,1,2,\ldots,N_x, \label{eq:discreteFourier}
% % \end{align}
% % where $q_\ell(y,t)\approx q(x_\ell,y,t)$ and $\qHat_{k}(y,t)$ are Fourier coefficients, 
% % and where $N_x$ is assumed to be even for convenience.
% % Transforming the governing equations to Fourier space leads to the following equations for the Fourier coefficients of the solution variables:
% % \begin{alignat}{3}
% % &   \rhos \partial_t \vs = i\kx \sigmas_{21} + \partial_y \sigmas_{22} , \quad&& y\in(0,\infty), \label{eq:vEqn} \\
% % &   \partial_t \sigmas_{22} = \rhos \cp^2 \partial_y\vs , \quad&&y\in(0,\infty), \label{eq:s22Eqn} \\
% % &   \partial_t \sigmas_{21} = i\kx \rhos \cp^2 \vs , \quad&&y\in(0,\infty) , \label{eq:s21Eqn} \\
% % & \rho \partial_t v_1 = i\kx      \sigma, \quad &&y\in(-H,0), \label{eq:v1HatEqn} \\
% % & \rho \partial_t v_2 = \partial_y\sigma, \quad && y\in(-H,0), \label{eq:v2HatEqn} \\
% % &  i\kx v_1 + \partial_y v_2 =0 ,                  \quad&&y\in(-H,0) , \label{eq:divHatEqn}
% % \end{alignat}
% % where $\kx = 2\pi k/L$ is a normalized wave number in the $x$~direction and the
% % equations hold for each $k=-N_x/2,-N_x/2+1,\ldots,N_x/2$. The hats on the
% % Fourier coefficients, along with the $k$ subscripts, have been dropped for
% % notational convenience.  Note that the horizontal component of the fluid
% % velocity, $v_1$, is decoupled from the other equations and boundary conditions, 
% % and can be determined once $v_2$ is known. Equations~\eqref{eq:v1HatEqn}--\eqref{eq:divHatEqn} are used to obtain
% % \[
% % \partial_y^2 \sigma - \kx^2 \sigma =0,      \qquad y\in(-H,0) ,
% % \]
% % which is a Laplace equation for pressure (in Fourier space).  The equations for the Fourier coefficients of the solid variables will be discretized using an upwind scheme.  In preparation for this, it is convenient to define the characteristic variables
% % \[
% % a=\sigmas_{22}-\rhos\cp\vs,\qquad b=\sigmas_{22}+\rhos\cp\vs,\qquad d=\sigmas_{21},
% % \]
% % which, from~\eqref{eq:vEqn}--\eqref{eq:s21Eqn}, satisfy
% % \begin{alignat}{3}
% % &   \partial_t a + \cp \partial_y a =  i\kx\cp\, d , \qquad&& y\in(0,\infty),  \label{eq:aHatEqnII}\\
% % &   \partial_t b - \cp \partial_y b = -i\kx\cp\, d , \qquad&& y\in(0,\infty),  \\
% % &   \partial_t d = \frac{i\kx\cp}{2}(b-a) , \qquad&& y\in(0,\infty).  \label{eq:dHatEqnII} 
% % \end{alignat}}
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% The solid variables are discretized in the $y$~direction using a uniform grid with
% spacing $\dy$.  The grid points for the solid domain are defined as $y_j=
% (j-\half)\dy$, $j=0,1,2,\ldots$. 
% Following the analysis in~\cite{BanksSjogreen2011,lrb2013}, the grid is staggered with respect to the
% interface at $y=0$ and has a ghost point at $j=0$; use of a non-staggered grid leads to similar results.
% %  This staggering simplifies the analysis but is not critical {\bf (I'm not convinced of this ?!?!)}.  
% Let  $\dt$ be the time step and let $t^n=n\dt$.  The
% equations~\eqref{eq:aHatEqnII}--\eqref{eq:dHatEqnII} are discretized using the
% first-order upwind scheme,
% \begin{alignat}{3}
% &   \frac{ a_j^{n+1}- a_j^n}{\dt} + \cp\frac{( a_j^n - a_{j-1}^n)}{\dy} =   i\kx\cp\, d_j^{n}, \label{eq:aEqnIII} \\
% &   \frac{ b_j^{n+1}- b_j^n}{\dt} - \cp\frac{( b_{j+1}^n - b_j^n)}{\dy} = - i\kx\cp\, d_j^{n}, \label{eq:bEqnIII} \\
% &   \frac{ d_j^{n+1}- d_j^n}{\dt} = \frac{i\kx\cp}{2}(b_j^{n+1} - a_j^{n+1}), \label{eq:dEqnIII}
% \end{alignat}
% where $a_j^{n}\approx a(y_j,t^n)$, $b_j^{n}\approx b(y_j,t^n)$ and
% $d_j^{n}\approx d(y_j,t^n)$. 
% Since we have used a non-dissipative pseudo-spectral approximation, rather than a two-dimensional upwind scheme, 
% the right-hand side terms in~\eqref{eq:dEqnIII} are taken at time $t^{n+1}$ in order to stabilize the approximation.
% A von Neumann stability analysis of equations~\eqref{eq:aEqnIII} and~\eqref{eq:bEqnIII} (for a
% periodic problem in $y$) shows that this time-stepping scheme is stable under
% reasonable conditions on the constants $\ly=\cp\dt/\dy$ and $\lx=\cp\kx\dt$.
% The fluid variables are kept continuous in $y$ in order to simplify the
% presentation; a discrete version can be introduced but this makes only
% insignificant changes to the fundamental results.  We are thus led to the
% following semi-discrete approximation for the solid and fluid equations,
% \begin{alignat}{3}
% &   a_j^{n+1} = a_j^n -\ly( a_j^n - a_{j-1}^n) - i \lx d_j^{n} , \quad&& j=1,2,3,\ldots\;, \label{eq:aEqn} \\
% &   b_j^{n+1} = b_j^n +\ly( b_{j+1}^n - b_j^n) + i \lx d_j^{n},  \quad&& j=0,1,2,\ldots\;, \label{eq:bEqn}  \\
% &   d_j^{n+1} = d_j^n +  \frac{i\lx}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=0,1,2,\ldots\;,  \\
% % 
% &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0), \\
% &  0=\partial_y^2 \sigma^{n+1}- \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), \label{eq:sigmaEqn}
% \end{alignat}
% where $v^n(y)=v(y,t^n)$ and $\sigma^n(y)=\sigma(y,t^n)$.  For reference, the discrete values for the (Fourier coefficients of the) velocity and components of stress in the solid are related to the characteristic variables by
% \[
% \vs_j^n=\frac{1}{2\zp}(b_j^n-a_j^n),\qquad\sigmas_{22,j}^n=\frac{1}{2}(b_j^n+a_j^n),\qquad \sigmas_{21,j}^n=d_j^n.
% \]
% The conditions at the top and bottom boundaries are 
% \begin{align}
% &   \vert a_j^{n}\vert^2 + \vert b_j^{n}\vert^2 + \vert d_j^{n}\vert^2 \rightarrow 0, 
%          \quad\text{as $j\rightarrow \infty$} ,  \label{eq:BCtop}\\
% &   \sigma^n(-H)=0. \label{eq:BCbottom}
% \end{align}
% Initial conditions are required to define $a_j^{0}$, $b_j^{0}$ and $d_j^{0}$ for $j=0,1,2,3,\ldots$, as well as $v^0(y)$ for  $y\in(-H,0)$, but these conditions are of no significance in the subsequent stability analysis.

% Approximations to the interface conditions are needed to complete the discrete
% formulation of the FSI model problem, and various choices are possible depending
% on the algorithm used.  
% For the AMP algorithm, the pressure Robin
% condition~\eqref{eq:AddedMassPressureBC} is imposed on the fluid; this is derived from the
% outgoing characteristic variables~\eqref{eq:AMPoutgoing}. In addition, the 
% incoming characteristic variable~\eqref{eq:AMPincoming} is used to specify a condition
% on the solid.  The latter condition uses an interface velocity defined
% in~\eqref{eq:ImpedenceWeightedVn} based on an impedance-weighted average.  
% First-order accurate approximations of these conditions are
% \begin{alignat}{3}
% &  \sigma^{n+1}(0) + \frac{\zp\dt}{\rho} \sigma_y^{n+1}(0) = \sigmas_{22,1}^{n+1} + \zp(\vs_1^{n+1} - v^{I,n})
%                                            = b_1^{n+1} -\zp v^{I,n}, && \label{eq:1dSigmaBC}\\
% &  a_0^{n+1} = \sigma^{I,n+1} - \zp v^{I,n+1}, &&\label{eq:1dSolidBC}
% \end{alignat}
% where $\sigma^{I,n}\equiv\sigma^n(0)$ and $v^{I,n}$ are the interface traction and velocity, respectively.  The latter is given by the impedance-weighted average
% \begin{alignat}{3}
% &   v^{I,n+1} = \frac{\zf}{\zf+\zp} v^{n+1}(0) + \frac{\zp}{\zf+\zp}\vs_1^{n+1} + \frac{1}{\zf+\zp}(\sigma_{22,1}^{n+1} - \sigma^{I,n+1} ) && \nonumber\\
% & \hphantom{v^{I,n+1}} = \gamma v^{n+1}(0) + \frac{1-\gamma}{\zp}( b_1^{n+1} - \sigma^{I,n+1} ), && \label{eq:1dVelocityBC}\end{alignat}
% where
% \[
% \gamma=\frac{\zf}{\zf+\zp},
% \]
% and where $\zf$ is a measure of the fluid impedance as introduced in Section~\ref{sec:partitionedAlgorithms}.

% The traditional partitioned (TP) algorithm uses the velocity from the solid as a boundary condition for the fluid and the traction from the fluid as a boundary condition for the solid.  First-order accurate approximations of these conditions are
% \begin{alignat}{3}
%  &   v^{n+1}(0)=\vs_1^{n+1}  
%         , &&   \label{eq:1dTradv} \\
%  &   \sigmas^{n+1}_{22,0} = \sigma^{n+1}(0). &&\label{eq:1dTradsigma}
% \end{alignat}
% It is also instructive to consider an anti-traditional algorithm in which
% the roles of the fluid and solid are reversed in the application of the
% partitioned interface conditions.  Approximations of these conditions are
% \begin{alignat}{3}
% &   \sigma^{n+1}(0) = \sigmas^{n+1}_{22,1}\,,  &&  \label{eq:1dAntiTradsigma} \\
% &   a_0^{n+1} = \sigma^{n+1}(0) - \zp v^{n+1}(0) .&& \label{eq:1dAntiTradv} 
% \end{alignat}
% The condition in~\eqref{eq:1dAntiTradv} is equivalent to setting the velocity of solid at the interface equal to the velocity in the fluid since the stresses have already been equilibrated in~\eqref{eq:1dAntiTradsigma}. 

% % 
% % 
% % % On the interface we assign the out-going characteristic variable by imposing~\eqref{eq:bEqn} at $j=0$.
% % The boundary conditions for the fluid are $\sigma^n(-H)=0$, while the solid solution should decay to zero 
% % as $j\rightarrow\infty$. 
% % The solution for $\sigma^n$ satisfying the boundary condition $\sigma^n(-H)=0$ can be written as
% % \begin{alignat}{3}
% % &  \sigma^{n}= \sigma^{I,n} \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \quad&& y\in(-H,0), 
% % \end{alignat}
% % where $\sigma^{I,n}=\sigma^n(0)$. 



% %- \vskip3\baselineskip
% %- 
% %- 
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- Let $\dt$ be the time step and let $t^n=n\dt$. 
% %- Introduce fully discrete approximations for the solid variables of the form $\qs_j^n \approx \qsHat(y_j,t^n)$ and
% %- semi-discrete approximations for the fluid variables of the form $q^n(y) \approx \qHat(y,t^n)$. 
% %- 
% %- This leads to the approximation
% %- \begin{alignat}{3}
% %- &   a_j^{n+1} = a_j^n -\lambda( a_j^n - a_{j-1}^n) - i \lambdax d_j^{n} , \quad&& j=1,2,3,\ldots \\
% %- &   b_j^{n+1} = b_j^n +\lambda( b_{j+1}^n - b_j^n) + i \lambdax d_j^{n},  \quad&& j=1,2,\ldots  \\
% %- &   d_j^{n+1} = d_j^n + i \frac{\lambdax}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=1,2,\ldots  \\
% %- % 
% %- &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0) \\
% %- &  \partial_y^2 \sigma^{n+1}= \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), 
% %- \end{alignat}
% %- where $\lambday=\frac{\cb\dt}{\dy}$ and $\lambdax=\cb\dt\kx$ and where $a_j^{n}$, $b_j^{n}$ and $d_j^n$
% %- are the characteristic variables in the solid given by 
% %- \begin{alignat}{3}
% %-    a_j^{n} = \sigmas_j^n -\zb \vs_j^n, \quad&& \vs_j^n &=\frac{1}{2\zb}(b_j^n-a_j^n), \\
% %-    b_j^{n} = \sigmas_j^n +\zb \vs_j^n, \quad&& \sigmas_j^n &=\frac{1}{2}(b_j^n+a_j^n), \\
% %-    d_j^n = \sigma^n_{21,j}
% %- \end{alignat}
% %- The boundary conditions for the fluid are $\sigma^n(-H)=0$, while for the solid the solution should remain bounded
% %- as $j\rightarrow\infty$. Initial conditions are needed for $a_j^{0}$, $b_j^{0}$, $d_j^{0}$, $j=0,1,2,3,\ldots$, 
% %- and $v^0(y)$, $y\in(-H,0)$.
% %- Approximations to the interface conditions are needed; various choices for these will be specified later. 
% %- 
% %- 
% %- 
% %- \vskip3\baselineskip
% %- 
% %- Introduce the fully discrete approximations $\vs_{ij}^n \approx \vs(x_i, y_j, t^n)$, 
% %- $\sigmas_{22,ij}^n \approx \sigmas^{22}(x_i, y_j, t^n)$, 
% %- $\sigmas_{21,ij}^n \approx \sigmas^{21}(x_i, y_j, t^n)$, 
% %- in the solid, 
% %- and the semi-discrete approximations $\vv_i^n(y)\approx \vv(x_i,y,t^n)$, $\sigma_i^n(y)\approx \sigma(x_i,y,t^n)$ in the fluid.
% %- We 
% %- expand the solution in a Fourier series in $x$,
% %- \begin{align}
% %-    \vs_{ij}^n = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat_{k,j}^n, \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}


% %- 
% %- 
% %- 
% %- We 
% %- expand the solution in a Fourier series in $x$. 
% %- We introduce the approximations $\vs_j(y,t) \approx \vs(x_j,y,t)$, $\sigma_{22,j}(y,t) \approx \sigmas_{22}(x_j,y,t)$, 
% %- $\sigma_{21,j}(y,t) \approx \sigmas_{21}(x_j,y,t)$, for the solid and 
% %- $\vv_j(y,t) \approx \vv(x_j,y,t)$, and $\sigma_{j}(y,t) \approx \sigma(x_j,y,t)$ for the fluid. 
% %- where 
% %- \begin{align}
% %-    \vs_j(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat(k,y,t), \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}
% %- We let $\kx = 2\pi k/L$ be the normalized wave number.
% %- 
% %- 
% %- 
% %- We discretize the solid in the $y$~direction with a grid spacing $\dy$.
% %- The grid for the solid is defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$. This grid is staggered
% %- with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- simplies the analysis but is not critical.
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- 
% %- % with grid spacing $\dy$ and use 
% %- % a first-order upwind scheme (in the $y$~direction) for the resulting solid equations. 
% %- % The grid for the solid, defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$, is staggered
% %- % with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- % simplies the analysis but is not critical.
% %- 
% %- In the solid we introduce grid functions $\vs_j^n\approx \vsHat(\kx,y_j,t^n)$, etc. 
% %- For the fluid we form approximations that are continuous in $y$ but discerete in time denoted by  
% %- $\sigma^n(y) \approx \sigmaHat(\kx,y,t^n)$,  and 
% %- $v^n(y) \approx \vHat_2(\kx,y,t^n)$. The horizontal component of the fluid velocity, $\vHat_1^n$, plays no role 
% %- in the analysis and can be determined from $v^n(y)$ using  $i\kx \vHat_1^n + \partial_y v^n(y)=0$, if needed.
% %- 
% %- 
% %- 


% % ------------------------------------------------------------------------------------------------
% \subsection{Stability analysis}

% \renewcommand{\aHat}{{\tilde a}}
% \renewcommand{\bHat}{{\tilde b}}
% \renewcommand{\dHat}{{\tilde d}}
% \renewcommand{\vHat}{{\tilde v}}
% \renewcommand{\sigmaHat}{{\tilde\sigma}}
% % \renewcommand{\aTilde}{{\bar a}}
% % \renewcommand{\bTilde}{{\bar b}}
% \renewcommand{\aTilde}{\alpha}
% \renewcommand{\bTilde}{\beta}

% To analyze the stability of the approximation
% in~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn}, we look for solutions of the form \[
% a_j^n=\amp^n\aHat_j, \qquad b_j^n=\amp^n\bHat_j, \qquad d_j^n=\amp^n\dHat_j,
% \qquad v^n(y)=\amp^n\vHat(y), \qquad \sigma^n(y)=\amp^n\sigmaHat(y),
% \] 
% where $\amp\in\Complex$ is the amplification factor,
% $(\aHat_j,\bHat_j,\dHat_j)$ are grid functions, and $(\vHat(y),\sigmaHat(y))$
% are functions for $y\in[-H,0]$. 
%  Substituting these forms
% into~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} results in the following system of
% equations
% \begin{alignat}{3}
% &  \amp \aHat_j = \aHat_j -\ly( \aHat_j - \aHat_{j-1}) - i \lx \dHat_j , \qquad&& j=1,2,3,\ldots\,, \label{eq:aHatEqn} \\
% &  \amp  \bHat_j = \bHat_j +\ly( \bHat_{j+1} - \bHat_j) + i \lx \dHat_j,  \qquad&& j=0,1,2,\ldots\,, \label{eq:bHatEqn}  \\
% &  \amp  \dHat_j = \dHat_j + \frac{i\lx}{2}\amp  ( \bHat_j - \aHat_j),    \qquad&& j=0,1,2,\ldots\,,  \label{eq:dHatEqn} \\
% % 
% &  \amp  \vHat(y) = \vHat(y) + \amp\dt\,\sigmaHat^I\,\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},  \qquad&& y\in[-H,0], \label{eq:vHatEqn} \\
% &  \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \qquad&& y\in[-H,0].\label{eq:sigmaHatEqn}
% \end{alignat}
% To obtain~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn},  the
% ODE in~\eqref{eq:sigmaEqn} was integrated using the boundary conditions $\sigmaHat(-H)=0$
% and $\sigmaHat(0)=\sigmaHat^I$, where the fluid stress at the interface, $\sigmaHat^I$, is as
% yet unspecified.  Note that the solution in the one-dimensional case,
% $\kk=0$, is a special case that can be found by taking the limit $\kk\rightarrow
% 0$ in~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn}. 
% Together with the interface
% conditions, equations~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} define
% a homogeneous set of difference equations. These equations have
% non-trivial solutions (i.e. eigenfunctions) only for particular values of $\amp$ (i.e. eigenvalues).
% The scheme is said to be weakly stable, or stable in the sense of
% Godunov-Ryabenkii, for given values of the parameters $\dt$, $\dy$, $\kx$, $H$, etc., 
% if there are no solutions (i.e.~eigenfunctions) to this
% eigenvalue problem with $\vert \amp\vert>1$. 
% The {\em region of stability} of the scheme is the region in parameter space where there are no roots with $\vert \amp\vert>1$. 
% In order to delineate the stability region 
% it is generally easier to look for regions where the scheme is {\em not} stable. Therefore, we 
% assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % we look for regions in the space of parameters where $\vert \amp\vert>1$  and the scheme is unstable.
% % We thus 
% % assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % If no such solutions exist for some given values of the parameters, then the scheme is (weakly) stable there. 
% % The stability domain is defined to be the region in parameter space where there are no roots with $\amp>1$.


% Equations~\eqref{eq:aHatEqn}--\eqref{eq:dHatEqn} are a system of
% constant-coefficient difference equations for the solid characteristic
% variables.  After solving for $\dHat_j$ from~\eqref{eq:dHatEqn} and substituting
% into~\eqref{eq:aHatEqn} and~\eqref{eq:bHatEqn}, $\aHat_j$ and
% $\bHat_j$ are found to satisfy the recursion
% \begin{equation}
%  \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = K \begin{bmatrix} \aHat_{j-1} \\ \bHat_{j-1} \end{bmatrix}, \qquad K =\begin{bmatrix}  ( 1 - \theta^2)/R & -\theta \\ \theta & R \end{bmatrix} ,
% \label{eq:recursion}
% \end{equation}
% where
% \begin{equation}
% R = r-\theta, \qquad r = \frac{\amp-1+\ly}{\ly}, \qquad \theta = -\frac{\amp\lx^2}{2\ly(\amp-1)} . 
% \label{eq:RandTheta}
% \end{equation}
% The eigenvalues, $\phi_-$ and $\phi_+$, of
% the $2\times2$ matrix $K$ in~\eqref{eq:recursion}
% %  \old{are the roots of a quadratic polynomial, and are given by} 
% are given by
% % \old{
% % We are interested in solutions for $\aHat_j$ and $\bHat_j$ that decay as
% % $j\rightarrow\infty$ so that the boundary condition in~\eqref{eq:BCtop} is
% % satisfied.  This leads us to consider the eigenvalues, $\phi_-$ and $\phi_+$, of
% % the $2\times2$ matrix $K$ in~\eqref{eq:recursion}, which are found by finding
% % the roots of a quadratic polynomial.  The result is
% % }
% \begin{equation}
% \phim = B - \sqrt{ B^2 - 1}, \qquad \phip=1/\phim, \qquad B = \frac{1}{2}\left(R + \frac{1 - \thetaj^2}{R}\right).
% \label{eq:phipm}
% \end{equation}
% Note that the product of the eigenvalues is one.  
% If both eigenvalues 
% % \old{were to have magnitude one} 
% had magnitude equal to one, then there would be no solution of the recursion
% in~\eqref{eq:recursion} satisfying the boundary condition~\eqref{eq:BCtop}.
% Therefore, for a valid solution, there is one eigenvalue (either $\phi_-$ or $\phi_+$),
% denoted by $\phis$ (for {\em small} $\phi$), that has magnitude strictly less
% than one, i.e.~$\vert\phis\vert<1$.  Let $\phib=1/\phis$ (for {\em big} $\phi$)
% be the other eigenvalue with $\vert\phib\vert>1$.  Note that when $\theta=0$,
% $0<\ly\le 1$, and $\vert\amp\vert>1$, then $\phis=\phim=1/r$ (but in general
% $\phis$ is not always equal to $\phim$).  Given that the eigenvalues are
% distinct, $K$ can be diagonalized as 
% \[
% K = S^{-1} \Phi S , \qquad
% \Phi =\begin{bmatrix}  \phis &  0 \\
%                            0 & \phib \end{bmatrix}, \qquad
% S =\begin{bmatrix}  R-\phis & \thetaj \\
%                     R-\phib & \theta \end{bmatrix}.
% \]
% By setting 
% \begin{align}
% &   \begin{bmatrix} \aTilde_j \\ \bTilde_j \end{bmatrix}
%    =  S \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = 
%    \begin{bmatrix} (R-\phis)\aHat_j + \theta \bHat_j \\
%                    (R-\phib)\aHat_j + \theta \bHat_j
%    \end{bmatrix}, \label{eq:abTildeEqn}
% \end{align}
% the general solution of the recursion in~\eqref{eq:recursion} is given by 
% \begin{equation}
% \begin{array}{l}
%    \aTilde_j = \phis^j \aTilde_0, \smallskip\\
%    \bTilde_j = \phib^j \bTilde_0.
% \end{array}
% \label{eq:abBarEqn}
% \end{equation}
% Since the solution must decay to zero as $j\rightarrow \infty$ and since $\vert\phib\vert>1$, it follows that $\bTilde_0=0$ and thus $\bTilde_j=0$ for all $j=0,1,2,\ldots$.  Since $\bTilde_j=0$, it follows from~\eqref{eq:abTildeEqn} that
% \begin{equation}
% \bHat_j = Q \aHat_j,\qquad \aTilde_j=(\phib-\phis)\aHat_j,\qquad Q = \frac{\phib-R}{\theta},
% \label{eq:Qdef}
% \end{equation}
% and thus from~\eqref{eq:abBarEqn}, 
% \[
% \aHat_j=\phi_s^j\aHat_0\,.
% \]
% Whence,
% % ------------------------------------------- PROP -------------------------------------------------
% \begin{proposition}
% Solutions to the system in~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} with $\vert\amp\vert>1$ satisfying the boundary conditions in~\eqref{eq:BCtop} and~\eqref{eq:BCbottom} are given by
% \[
% \begin{array}{c}
% \displaystyle{
% \aHat_j=\phi_s^j\aHat_0,\qquad \bHat_j=Q\aHat_j,\qquad \dHat_j=\frac{i\lx(Q-1)\amp}{2(\amp-1)}\aHat_j,\qquad j=0,1,2,\ldots\,,
% } \bigskip\\
% \displaystyle{
% \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},\qquad \vHat(y)=\sigmaHat^I\,\frac{\amp\dt}{\amp-1}\;\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},\qquad y\in[-H,0],
% }
% \end{array}
% \]
% % \old{where the two free constants, $\aHat_0$ and $\sigmaHat^I$, will be determined by two interface conditions.} 
% where $\aHat_0$ and $\sigmaHat^I$ are free constants.
% \end{proposition}

% The remaining constraints needed to complete the eigenvalue problem, which then determines the amplification factor $\amp$, are provided by two interface conditions.  Choices for these interface conditions are discussed in the subsections below.

% % \bigskip\noindent
% % \textcolor{green}{Note: I have chosen the wording above since the two interface conditions don't actually determine the two free constants, but rather they determine $\amp$ and a relationship between the constants.  I believe the constants would still be arbitrary to within a multiplicative constant.}

% % --------------------------------------------------------------------------------------------------------
% \subsection{AMP interface conditions} 
% Imposing the AMP interface conditions in~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC} with the formula for the interface velocity in~\eqref{eq:1dVelocityBC} gives
% % The AMP Robin boundary condition for $\sigma$ is~\eqref{eq:1dSigmaBC} which gives
% % follows from~\eqref{eq:AddedMassPressureBC}.
% % A first-order approximation is 
% % \begin{align}
% %   \sigma^{n+1} + \frac{\zb\dt}{\rho} \sigma_y^{n+1} &= \sigmas_{22,1}^{n+1} + \zb\vs_1^{n+1} - \zb v^{I,n}
% %                                            = b_1^{n+1} -\zb v^{I,n}, \qquad\text{for $y=0$}, \label{eq:1dSigmaBC}
% % \end{align}
% % where we have introduced the interface velocity $v^{I,n}$.
% % This gives,
% % \begin{align}
% % &  \sigma^{I,n+1} = \eta\Big( b_1^{n+1} - \zb v^{I,n}\Big), \\
% % & v^{I,n+1}  = \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \\
% % &  a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}, 
% % \end{align}
% \begin{align}
% &  \amp\sigmaHat^{I} = \eta\left( \amp\bHat_1 - \zp \vHat^{I}\right), \label{eq:AmpSigmaHat} \\
% &  \aHat_0 = \sigmaHat^{I} - \zp \vHat^{I} , \label{eq:AmpaHat} \\
% &  \vHat^{I}  = \gamma \vHat(0) + \frac{1-\gamma}{\zp}( \bHat_1 - \sigmaHat^{I} ), \label{eq:AmpvHatI}
% \end{align}
% where
% \begin{align*}
%  & \eta \equiv \frac{1}{1 + \frac{\zp\kk\dt}{\rho}\coth(\kk H)}  = \frac{1}{1 + \frac{\rhos\lx}{\rho}\coth(\kk H)}. 
% \end{align*}
% From~\eqref{eq:vHatEqn} and~\eqref{eq:AmpSigmaHat} we also have
% \begin{align}
%   (\amp-1) \vHat(0) = \frac{1-\eta}{\zb}(\amp \bHat_1 - \zb\vHat^I). \label{eq:AmpvHat} 
% \end{align}
% Using $\bHat_1=Q\phis \aHat_0$ to eliminate $\bHat_1$ in terms of $\aHat_0$ and using~\eqref{eq:AmpSigmaHat} to
% eliminate $\sigmaHat^{I}$, equations~\eqref{eq:AmpaHat}, \eqref{eq:AmpvHat} and~\eqref{eq:AmpvHatI} can be written
% in the form 
% %- The interface velocity follows from~\eqref{eq:1dVelocityBC}, giving 
% %- \begin{align}
% %- %    v^{I,n+1} &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( \zb\vs_1^{n+1} + \sigma_{22,1}^{n+1} - \sigma^{I,n+1} ), \\
% %- v^{I,n+1}   &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \label{eq:1dVelocityBCb}
% %- \end{align}
% %- where $\gamma=\zf/(\zf+\zb)$.
% %- For the final interface condition we set the incoming characteristic variable in the solid using the interface
% %- stress and velocity, 
% %- \begin{align}
% %-   a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}. \label{eq:1dSolidBCb}
% %- \end{align}
% % addedMass.mample : 
% % M := Matrix( [ [ A*(1-eta*Q*phim) , 0   , eta+A] , 
% %                [ (1-eta)*A*Q*phim , 1-A , -(1-eta) ], 
% %                [ -(1-g)*(1-eta)*Q*phim    , -g   , 1-(1-g)*eta/A ] ] );
% %
% %-The equations defining the AMP approximation can thus be written in the form
% \begin{align}
% \begin{bmatrix}
%    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
%    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
%   -(1-\gamma)(1-\eta)Q\phis  & -\gamma &  1-(1-\gamma)\eta \amp^{-1} 
% \end{bmatrix} 
% \begin{bmatrix} \aHat_0 \\ \zb \vHat(0) \\ \zb\vHat^I \end{bmatrix} =0 .  \label{eq:AMPmatrix}
% \end{align}
% The determinant of the matrix in~\eqref{eq:AMPmatrix} must be zero for non-trivial solutions to exist, and this leads to the following equation for $\amp$:
% \begin{align*}
% %    \tilde{f(\amp) :=& 
%    \big(\amp-(1-\gamma)\big) \left(\amp-\eta - \big( (2\eta-1)\amp -\eta \big)Q \phis\right) =0.
% \end{align*}
% % For $0\le \gamma\le 2$ the root $A=1-\gamma$ has magnitude less than or equal to one.
% Since $\amp-(1-\gamma)\ne0$ when $\vert\amp\vert>1$ and $0\le \gamma\le 2$, we have the following result.
% % --------------------------------------------------------------------------------------------------
% \begin{theorem} \label{th:amp1d}
% The AMP interface approximation to the
% scheme~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary
% conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, interface
% conditions~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC}, and interface
% velocity~\eqref{eq:1dVelocityBC} is weakly stable if and only if $0\le \gamma\le 2$ and there are no roots $\amp$ with $\vert \amp\vert>1$ to the equation
% \begin{align}
%    f(\amp) \equiv& \amp -\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis =0. \label{eq:fAMP}
% \end{align}
% \end{theorem}
% \noindent Note that $f(\amp)$ does not depend on $\gamma$, i.e.~the weighting in the definition of the interface velocity, and thus the stability of the scheme is independent of $\gamma$ provided $0\le \gamma\le 2$.  From a numerical conditioning point of view, however, we recommend the choice $\gamma=\zf/(\zf+\zp)$ as used in~\eqref{eq:1dVelocityBC}.


% %
% %- 
% %- \begin{align}
% %- &  A \sigma^{I} = \eta\Big( A \bHat_1 - \zb v^{I}\Big), \label{eq:AddedMassSigmaI} \\
% %- % &  \aHat_0 = \sigmasHat_0 - \zb \vsHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- &  \aHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- & (A-1)\vHat(0)= \frac{1-\eta}{\eta\zb} A \sigma^{I}, \\
% %- & v^{I} = \gamma \vHat(0) + (1-\gamma)\frac{1}{\zb}( \bHat_1 - \sigma^{I} )
% %- % &  b^{I,n+1}= b_1^{n+1},  ~~\text{(first order approximations)}, 
% %- \end{align}
% %- Using the expressions for $b_1^n$, etc. 
% %- lead to the conditions
% %- \begin{align}
% %- &  A(1-\eta Q\phis)\aHat_0 + (\eta+A) (\zb\vHat^I) =0 ,   \\
% %- & (A-1)(\zb\vHat(0)) -(1-\eta) A Q \phis \aHat_0 + (1-\eta) (\zb \vHat^I) = 0, \\
% %- & (1 - (1-\gamma)\eta A^{-1}) (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(1-\eta) Q \phis\aHat_0 = 0. 
% %- % & (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(Q-1)\half\phis \aHat_0=0. 
% %- \end{align}
% %- This is an eigenvalue problem for $\amp$. 
% %- Taking the determinant of the associated matrix leads to 
% %- \begin{align}
% %- & f(\amp) \equiv
% %- \det
% %- \begin{bmatrix}
% %-    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
% %-    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
% %-    \half(1-\gamma)(Q-1) \phis  & \gamma & -1 
% %- \end{bmatrix} =0,\\
% %- & f(\amp)=  \amp(1-\eta Q\phis) \Big( 1-\amp +\gamma(1-\eta)\Big) + 
% %-          (\amp+\eta)\phis\Big(  \gamma(1-\eta)\amp Q - \half(1-\amp)(1-\gamma)(Q-1)   \Big) .
% %- \end{align}
% %-The scheme is unstable if there are solutions to $f(\amp)=0$ with $\vert\amp\vert>1$. 
% %-The scheme is said to be (weakly stable) at particular values of $\lambdax,\lambday,\gamma$
% %-if there are no roots with $\vert\amp\vert>1$. Given a choice for $\gamma$ we can plot the
% %-region of stability in the $(\lambdax,\lambday)$ plane. 


% \paragraph{Reduction to a polynomial equation for $\amp$} To examine the stability of the AMP algorithm we must consider all solutions of $f(\amp)=0$.  The function $f(\amp)$ in~\eqref{eq:fAMP} involves square roots of $\amp$ through the eigenvalues, $\phis$ and $\phib$, of the matrix $K$ in~\eqref{eq:recursion} and the definition of $Q$ in~\eqref{eq:Qdef}.  
% To ensure that all possible solutions are found, 
% a polynomial $P(\amp)$ can be derived whose roots include
% all the roots of $f(\amp)$.  To this end, 
% note that from the definition for $Q$ and $\phis\phib=1$ it follows that 
% \begin{align*}
%   Q\phis = \frac{1-R\phis}{\theta}.
% \end{align*}
% Thus $f$ is a linear function of $\phis$ since $f$ only depends on the product $Q\phis$. 
% Note 
% also that $Q\phis$ is a rational function of $\amp$ according the definitions of $R$ and $\theta$ in~\eqref{eq:RandTheta}.  
% Thus, $f(\amp)=0$ can be written in the form
% \begin{align*}
%     \phis = F(\amp) ,
% \end{align*}
% where $F$ is a rational function of $\amp$. 
% Since $\phis$ is equal to one of the two eigenvalues, $\phi_\pm$, defined in~\eqref{eq:phipm}, it follows that 
% \begin{equation}
%   \pm \sqrt{ B^2 - 1} = F(\amp)-B,
% \label{eq:Fratio}
% \end{equation}
% where the sign in front of the square root is chosen to be consistent with $\vert\phis\vert<1$.
% % \old{where the sign in front of the square root is chosen based on the assignment of $\phis$ so that $\vert\phis\vert<1$.}
% Upon squaring both sides of~\eqref{eq:Fratio}, which introduces new roots, one obtains
% %  
% %  Since $\phis$ also satisfies a quadradic equation
% %  with coefficients that are polynomials of $A$, 
% %  \begin{align}
% %   (\amp-1)^2 R \phis^2 - (\amp-1)^2 R B \phis + (\amp-1)^2 R=0,
% %  \end{align}
% % we can eliminate $\phis$ to derive a higher degree polynomial satisfied by $A$,
% \begin{equation}
%    P(\amp)=0,
% \label{eq:PAMP}
% \end{equation}
% where $P(\amp)$ is a polynomial (as described below).  We have thus shown the following:
% \begin{proposition}
%   Any solution of $f(\amp)=0$ is also a root of the polynomial $P(\amp)$. 
% \end{proposition}
% All of the roots of $P(\amp)$ can be found numerically using well-developed
% algorithms (e.g.~solving the eigenvalue problem for the companion matrix).  
% In
% deriving $P(\amp)$, however, new roots have been introduced. Therefore, each
% root $\amp^*$ of $P(\amp)$ must be checked to ensure that it is also solution of
% $f(\amp)=0$.
% % To do this we set $\phis=\phi_-(\amp_0)$ if $\vert\phi_-(\amp_0)\vert<1 $ otherwise we set $\phis=\phi_+(\amp_0)$,
% % and then check that $f(\amp_0)=0$. 
% \begin{proposition}
%   A root, $\amp^*$, of $P(\amp)$ is also a root of $f(\amp)$, if $\phis$ in the definition of $f$ satisfies
% \begin{equation*}
%     \phis = \begin{cases}
%                 \phi_-(\amp^*) & \text{if $\vert\phi_-(\amp^*)\vert<1 $}, \\
%                 \phi_+(\amp^*) & \text{otherwise} ,
%             \end{cases}
% \end{equation*}
% and if $f(\amp^*)=0$.
% \end{proposition}
% % \begin{align}
% %    P(\amp)=0, \quad f(\amp)=0, \quad \vert\phis(\amp)\vert<1. 
% % \end{align}
% % {\bf Scheme 1:} Taking $\gamma=1$ (interface velocity from the fluid), gives (removing a factor of $2\amp$)
% % ff := phim Q A - eta - 2 eta Q phim A + eta Q phim + A
% % 
% \newcommand{\Pamp}{P_{\rm AMP}}
% The polynomial in~\eqref{eq:PAMP} is (after removing uninteresting factors of $\amp-1$) a polynomial of degree 5 given by 
% \[
% \Pamp(\amp)=\alpha_5\amp^5+\alpha_4\amp^4+\alpha_3\amp^3+\alpha_2\amp^2+\alpha_1\amp+\alpha_0,
% \]
% where the coefficients in the polynomial are
% \[
% \begin{array}{l}
% \alpha_0=-\eta^2+2 \eta^2 \ly, \smallskip\\
% \alpha_1=-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2, \smallskip\\
% \alpha_2=10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly, \smallskip\\
% \alpha_3=-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2, \smallskip\\
% \alpha_4=3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2, \smallskip\\
% \alpha_5=-1+2 \eta.
% \end{array}
% \]
% %\begin{align*}
% %%  f_1(\amp) :=&  A-\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis, \\
% % \Pamp(\amp) =&  (-1+2 \eta) A^5+(3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2) A^4+\\
% %&    (-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2) A^3+\\
% %&    (10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly) A^2+(-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2) A\\
% %&    -\eta^2+2 \eta^2 \ly .
% %\end{align*}
% It turns out that $\Pamp(\amp)$ is the same polynomial generated by the Maple symbolic algebra program when asked to solve $f(\amp)=0$.

% To determine if there are any roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$, we
% evaluate the roots numerically for an array of parameter values in the region
% $0<\lx<1.2$, $0<\ly<1.2$ and $0\le \eta \le 1$ with $N_\amp$ equally spaced
% points in each parameter direction.  The stability region of the scheme is the
% region in the space of $(\lx,\ly,\eta)$ where the magnitude of the largest
% valid root satisfies $\vert\amp\vert\le 1$.  This region is computed on a grid with
% $N_\amp=800$ points for each parameter.  In
% Figure~\ref{fig:acousticSolidStokestability}, we plot the curve in the
% $(\lx,\ly)$ plane for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  (The
% curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is also plotted for
% reference.)  Observe that the region of stability contains the region
% $0\le\eta\le1$ and $\lx^2 + \ly^2 \le \kappa^2$
% (for $\lx\ge0$ and $\ly\ge 0$) where the maximum value for $\kappa$ appears to be $\kappa=1$. 
% Further evidence for $\kappa=1$ being the upper bound is provided by the restriction of the analysis to one dimension given below.
% % \old{, where $\kappa$ is a positive constant strictly less than 1.  }
% The curve $\lx^2 + \ly^2 = (.99)^2$
% is shown in the figure as an example.  Since $\lx=\cp\kx\dt$ and $\ly=\cp\dt/\dy$,
% the condition $\lx^2+\ly^2\le 1$ implies the following result.

% % To determine if there are any roots of $\Pamp(\amp)=0$ with $\vert\amp\vert>1$ we evaluate the roots numerically for 
% % values of $\lambda$, $\lambdax$ and $\eta$ in the ranges $0<\lambda<1$, $0<\lambdax<1$, and $0\le \eta \le 1$.
% % We choose $M$ equally spaced values of each of $\lambda$, $\lambdax$ and $\eta$ over their ranges, resulting
% % in finding the roots for $M^3$ points. Using Maple we computed roots with $M=50$ and $M=100$ and using $20$ digits of precision.
% \begin{theorem}
% By numerical evaluation of the stability polynomial, $\Pamp(\amp)$,
% we have found that the AMP algorithm is weakly stable (i.e.~there are no valid roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$) 
% provided $\lx^2+\ly^2\le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{1}{\cp}\left[ \frac{1}{\dy^2} + \kx^2 \right]^{-1/2}. 
%  \end{align*}
% % where $0\le\kappa<1$. 
% This is a sufficient but not a necessary condition. 
% \end{theorem}
% Note that the time step $\dt$ satisfies a typical CFL constraint arising from the fastest wave speed in the solid.
% In the incompressible limit when $\cp \rightarrow \infty$, the maximum stable $\dt$ would go to zero,
% as it would for the solid in isolation. For incompressible solids, alternative formulations should be considered.
% Developing AMP algorithms for incompressible solids is a subject for future work. 

% % \noindent{\bf Note 1:} There are generally four valid roots to $\Pamp(\amp)=0$.
% % Figure~\ref{fig:acousticSolidStokestability} shows a plot of the computed stability region.

% {
% % ---- from codes/cauchy.m  (and cauchy.maple) ----
% \newcommand{\figWidth}{8cm}
% \begin{figure}
% \begin{center}
% %   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP_num50}
%   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP}
%   \caption{Stability region for the two-dimensional model problem using the AMP algorithm.  The curve marked 1 is the curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  The curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is shown for reference.  The dashed curve shows the curve $\lx^2+\ly^2=(.99)^2$.}
%   \label{fig:acousticSolidStokestability}
% \end{center}
% \end{figure}
% }


% % \noindent{\bf Note 2:} The scheme is found to be unstable for $\lambda>1$. Note, however, that the stability bound
% % derived in Section~\ref{} for a periodic strip in $y$ is somewhat more restrictive than the bound found here
% % for the seimi-infinite strip. For example, the periodic strip is unstable for $(\lambda,\lambdax)=(.9,9.)$.

% % {\bf TO-DO: Check the $\eta=0$ limit -- decoupled solid -- we should get von-Neumann stability bound.}

% % --------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% The stability of the one-dimensional version of the AMP algorithm 
% % \old{(described previously in Section~{\bf ?????})}
% may be examined by considering the special case of the two-dimensional algorithm with $\lx=0$ and $Q=0$.  In this case there are two solutions of $f(\amp)=0$ given by
% \begin{align*}
%    \amp = 1-2\ly \qquad\text{or}\qquad \amp =\eta. % \label{eq:fAMP1D}
% \end{align*}
% We are interested in whether there are solutions with $\vert\amp\vert>1$.  Since $0\le \eta\le 1$ we have the result.
% \begin{theorem}
% The one-dimensional AMP algorithm is weakly stable provided  $0\le\gamma\le 2$ and $0 \le \ly \le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{\dy}{\cp}. 
%  \end{align*}
% \end{theorem}

% % \noindent{\bf Note 2:} Even though there are no roots $\vert\amp\vert>1$ to $\Pamp$ for even larger values of $\lambda$ and $\lambdax$,
% %   the orginial scheme should respect the time step restriction from the solid scheme 
% % {\bf But why? Does some assumption go bad? e.g. $\vert\phis\vert<1$?}


% For comparison, we now discuss briefly the corresponding stability results for the scheme given by~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, and with interface conditions given by either the 
% traditional (TP) algorithm or the anti-traditional algorithm.



% % ==========================================================================================================
% \subsection{TP interface conditions} \label{sec:TPanalysis}
% % \newcommand{\Mr}{\Mc}% mass ratio

% The interface conditions for the TP algorithm are given by~\eqref{eq:1dTradv} and~\eqref{eq:1dTradsigma}.  
% Following the previous analysis, $\amp$ is found to satisfy 
% \begin{align}
% &   f_{{\rm TP}}(\amp) \equiv \amp(Q+1) - \frac{\eta-1}{\eta} (\amp-1)(Q-1)\phis =0 . \label{eq:traditionalSchemeF}
% % &   \mr \equiv \frac{\zb\dt\kx}{\rho\tanh(\kx H)} = \frac{\eta-1}{\eta} ...
% \end{align}

% % {\bf TO-DO} The stability region for this scheme is computed numerically and shown in Fig.~\ref{??}.
% % We could plot the stability regions for fixed values of $\eta$ and show that as $\eta\rightarrow 1$ the
% % stability region shrinks to nothing. This shows that as $\dt\rightarrow 0$ ($\eta\rightarrow 1$) the
% % scheme is unstable. 


% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 

% In one dimension, the condition in~\eqref{eq:traditionalSchemeF} reduces to the polynomial equation
% \begin{align*}
% P_{{\rm TP}}(\amp) = \amp^2 + (\Mr + \ly-1) \amp - \Mr = 0, \quad\text{where}~~
%   \Mr = \frac{\rho H}{\rhos \dy}.
% \end{align*}
% (Here, all of the roots of this quadratic are valid since no spurious roots were introduced in deriving the equation.)  The product of the roots is $-\Mr$ and thus a necessary condition for stability is that $\vert \Mr\vert\le 1$.
% Thus the mass of the solid in a thin strip one grid cell wide, $\rhos\dy L$, 
% must be larger than the mass of the entire fluid domain $\rho H L$. 
% Using the theory of von Neumann polynomials~\cite{Miller1971,Strikwerda89} one can show the following necessary and
% sufficient condition.  
% % {\bf (It is a little unclear to me how $\Delta y$ appears.) WDH: Multiply the expression below with $\cp/\dy$ and $\lambda$ and $\Mr$ appear. }
% % ---------------------------------- THEOREM -------------------------------------------------
% \begin{theorem} \label{lemma:traditional}
% The one-dimensional TP algorithm is weakly stable if and only if 
% \begin{align*}
% %      \Mr = \frac{\rho H}{\rhos \dy} <1, \\
%      \dt \le \frac{2}{\cp}\Big( \dy - \frac{\rho H}{\rhos} \Big). 
% %      \lambda < 2(1-\Mr). 
% \end{align*}
% \end{theorem}
% This is a curious result.  For a given {\em large} value of $\dy$ the one-dimensional scheme may be stable, but it will eventually become unstable as the mesh is refined and $\dy$ becomes less than $(\rho H)/\rhos$.  The one-dimensional TP algorithm is thus formally {\em unconditionally unstable}.  
% The numerical results in Section~\ref{sec:travelingWaveResults} show that this behaviour also holds for 
% the second-order accurate discretization of the two-dimensional model problem MP-VE.
% % This behaviour of the traditional scheme is also found to hold in the two-dimensional
% %  since as the mesh is refined eventually $\dy$ will be less than $\frac{\rho H}{\rhos}$. 


% % --------------------------------------------------------------------------------------------------------
% \subsection{Anti-traditional interface conditions} \label{sec:ATPanalysis}

% The interface conditions for the anti-traditional algorithm are given by~\eqref{eq:1dAntiTradsigma} and~\eqref{eq:1dAntiTradv}.  The analysis for this choice leads to the constraint
% %These can be written as 
% %\begin{align*}
% %&  \sigmaHat^I = \sigmasHat_{22,1}= \half(Q+1)\phis\aHat_0, \\
% %&  \aHat_0 = \sigmaHat^I -\zb\Big( \frac{\kk\dt}{\rho}\coth(\kk H)\frac{\amp}{\amp-1} \Big)\sigmaHat^I, 
% %\end{align*}
% % The anti-traditional scheme takes the interface velocity from the fluid and the interface
% % stress from the solid,
% % \begin{align}
% % &   \vHat^I = \vHat(0) = \frac{1-\eta}{\eta}\frac{1}{\zb} \frac{\amp}{\amp-1} \sigmaHat^I, \\
% % &   \sigmaHat^I = \sigmasHat_1 = \half(Q+1) \aHat_0, \\
% % &   \aHat_0 = \sigmaHat^I - \zb \vHat^I = (1- \frac{1-\eta}{\eta}\frac{\amp}{\amp-1}) \half(Q+1) \aHat_0.
% % \end{align}
% % ese interface conditions lead to the eigenvalue equation for $\amp$ of 
% %which leads to the eigenvalue equation for $\amp$ of 
% \begin{align}
% &   f_{{\rm AT}}(\amp) = 1- \amp + \half\left( \frac{2\eta-1}{\eta} \amp -1 \right) (Q+1)\phis=0 .  \label{eq:antiTraditional2d}
% \end{align}

% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% In one dimension, \eqref{eq:antiTraditional2d} reduces to the polynomial constraint
% \begin{align*}
% %      \amp^2 + ( \frac{\lambda}{2\eta} -2)\amp + 1-\frac{\lambda}{2} = 0.  \\
%      P_{{\rm AT}}(\amp) = \amp^2 + \left( \frac{\ly}{2}\left(1+\frac{\ly}{\Mr}\right) -2\right)\amp + 1-\frac{\ly}{2} = 0.  
% %     \amp^2 + (  \frac{\lambda}{2} + \frac{\lambda^2}{2\Mr} -2)\amp + 1-\frac{\lambda}{2} = 0. 
% \end{align*}
% % The anti-traditional scheme is weakly stable in one-dimension if and only if the following conditions
% %  are satisfied (**CHECK ME**)
% %  \begin{align}
% %  &    \lambda < 4, \\
% %  &    \frac{\lambda^2}{2\Mr} < 4-\lambda. 
% %  \end{align}
% %  where $\Mr = \frac{\rho H}{\rhos \dy}$. {\bf TO-DO:} $\Mr$ depends on $\dy$ so we really need to find the condition on $\dt$ in terms of $\dy$.
% An analysis of the roots of $P_{{\rm AT}}(\amp)$ leads us to the following result:
% \begin{theorem}
%   The one-dimensional anti-traditional algorithm is weakly stable if and only if $\ly\le 4$ and 
% % \begin{align}
% % %    \lambda \le \sqrt{ 8\Mr + \Mr^2  } -       \Mr     =       \Mr     \Big( \sqrt{ 1+\frac{8 }{\Mr}} -1 \Big). \\
% %     \half G \dt^2 + \dt < \frac{4\dy}{\cb}, \qquad G=\frac{\rhos\cb}{\rho H}
% % \end{align}
% % or 
% \begin{align}
% %    \dt  < \frac{ \sqrt{1+\frac{8\rhos}{\rho H} \dy} -1 }{G}, \qquad G=\frac{\rhos\cb}{\rho H} . \\
%    \dt  \le \frac{\dy}{\cp}\left( \sqrt{\Mr^2+8\Mr}-\Mr \right).   \label{eq:ATStability}
% \end{align}
% \end{theorem}

% We observe that the one-dimensional anti-traditional scheme is (weakly) stable for any value of the added-mass ratio $\Mr=(\rho H)/(\rhos \dy)$ provided that $\dt$ is taken sufficiently small. 
% The anti-traditional scheme is thus a stable alternative to the AMP scheme. However, in the {\em heavy solid} regime 
% when $\Mr$ is small, the anti-traditional requires a smaller $\dt$ than the AMP scheme, scaling
% like $\sqrt{8\Mr}$ for $\Mr\ll 1$,  as can be seen from~\eqref{eq:ATStability}.



==> texFiles/inviscidAnalysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Stability analysis of an inviscid  model problem} \label{sec:inviscidAnalysis}

% todo
%
% replace \lambda_y with \ly etc.
%
%\noindent
%\textcolor{red}{(Current thoughts on editing this section: (1) Describe the model problem at a continuous level.  Simplify the notation by $v_2\rightarrow v$, $\sigma_{21}\rightarrow\sigma_1$, etc., basically dropping the 2 since everything is in the vertical direction anyway.  BTW: I wonder if it is too much to say that the solid velocity and stress tend to zero as $y\rightarrow-\infty$.  I think this would only be true if this property also holds for the initial data.  Requiring that the solution is bounded at infinity should be enough.  I wonder if this issue was discussed during the writing of FIB???  (2) Describe how the equations are approximated.  (3) Describe the AMP algorithm for the approximation of the model equations.  Here I think it is helpful to point back to the previously discussed algorithm so that the mapping between the general algorithm and the one in the model problem analysis is clear.  (4) Perform the analysis for the AMP scheme and give the results.  (5) State the corresponding results for the TP and ATP schemes, but leave any details to an appendix.)}

% \wdh{\bf This is from fib:
% In this section, we perform a stability analysis of the AMP algorithm applied to
% the two-dimensional FSI model problem MP-IA.  In this problem, the fluid is
% taken as inviscid and the solid is treated as an acoustic solid that only
% supports motion in the vertical direction. The governing equations for the model
% are given by~\eqref{eq:MP-IA}.
% % We are interested in the stability of different frequencies in the $x$ direction and thus consider a periodic problem in $x$. 
% We consider a semi-infinite solid domain ($\Hs=\infty$) and look for solutions in the solid that have finite $L_2$-norm (which implies the solutions decay to zero as $y\rightarrow\infty$).  The bottom boundary condition on the fluid at $y=-H$ is chosen as $\sigma=0$ (i.e. $p=0$).
% }

In this section, the stability of the AMP, TP and ATP algorithms are explored for a simplified two-dimensional FSI model problem.  A similar stability analysis was performed in~\cite{fib2014} for a first-order accurate scheme on a staggered grid.  The algorithms considered here are second-order accurate, as in the full AMP algorithm discussed in Section~\ref{sec:algorithm}, and thus the present analysis extends the previous results for less dissipative partitioned schemes.

\input texFiles/rectangularModelProblemCartoon

\subsection{FSI model problem}


% \das{Consider model problem MP-VA described in Section~\ref{sec:FSIModelProblems}
% and the geometry  is shown in Figure~\ref{fig:rectangularModelProblemCartoon}
% The fluid is assumed to be inviscid and incompressible. 
% A zero pressure boundary condition is applied at the fluid boundary $y=H.$ 
% The governing equations and interface conditions
% for the fluid solid are given by \eqref{eq:mpiaEquations}--\eqref{eq:mpiaInterface}.}

The fluid is assumed to be inviscid and incompressible, and it occupies the region $\OmegaF$ given by $0<x<L$ and $0<y<H$.  The solid lies below the fluid in the semi-infinite region $\OmegaS$ given by $0<x<L$ and $-\infty<y<0$.  The solid is taken to be an ``acoustic'' solid that supports a motion in the vertical direction only.  The fluid-solid interface $\Gamma$ is linearized about the flat surface, $y=0$, and it is assumed that the vertical components of the velocity and stress between the fluid and solid match along $\Gamma$.  The fluid pressure is taken to be zero along the top boundary, $y=H$, and the solutions for the fluid and solid are assumed to be periodic in the $x$-direction with period equal to~$L$.  The governing equations for the FSI model problem are
%In this section, the stability of the second order accurate
%AMP, TP, and ATP algorithms are explored for a simplified two-dimensional 
%model problem. This extends the stability results of first order 
%accurate schemes in \cite{fib2014}.
%In this analysis, the TP scheme is considered 
%without under-relaxed sub-iterations. 
%To supplement this, an analysis of the TP scheme with sub-iterations is performed.
%In the model problem, we assume the fluid is inviscid and the solid 
%is acoustic with motion constrained to vertical direction. 
%We are interested in the stability of different frequencies 
%in the $x$ direction and thus consider a periodic problem in $x$. 
%The solid domain is semi-infinite ($\Hs \rightarrow \infty)$ and we require solutions
%to decay to zero as $y \rightarrow -\infty.$ The fluid pressure is given to be 
%$p=0$ at the top boundary. The interface conditions enforce matching of the 
%velocity and traction at $y=0.$
%The governing equations and boundary conditions are given by
\bse
\begin{align}
\text{Fluid: } &\begin{cases}
\rho \partial_t \vfy + \partial_y p = 0, & \xv\in\OmegaF \\
(\partial_x^2 + \partial_y^2) p =0, & \xv\in\OmegaF \\
p = 0, & x\in(0,L), \quad y=H
\end{cases} \label{eq:fluidModelInviscid} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsy = \partial_x \ssx + \partial_y \ssy, & \xv\in\OmegaS \\
\partial_t \ssx = \rhos\cp^2 \partial_x \vsy, & \xv\in\OmegaS \\
\partial_t \ssy = \rhos\cp^2 \partial_y \vsy, & \xv\in\OmegaS \\
|\vsy|^2+|\ssx|^2+|\ssy|^2 < \infty, & y\rightarrow - \infty
\end{cases} \label{eq:solidModelInviscid} \\
\text{Interface: } &\begin{cases}
\vfy = \vsy, & x\in(0,L), \quad y = 0 \\
p = -\ssy, & x\in(0,L), \quad y = 0.
\end{cases}
\end{align}
\ese
We note that the horizontal component of the fluid velocity is omitted from the equations for the fluid in~\eqref{eq:fluidModelInviscid} since it decouples in the simplified FSI problem and can be determined from the remaining fluid variables once the solution is known.  The model problem described here corresponds to the MP-IA model problem considered in~\cite{fib2014}.

% governing equations
% ------------------------------------------------------------------------------------------------
\subsection{Discretization}

\das{As in Section~\ref{sec:viscousAnalysis}, 
the solution is represented as a discrete Fourier series
in the transverse direction using equation~\eqref{eq:discreteFourier}.
Taking a discrete Fourier transform of the equations in~\eqref{eq:fluidModelInviscid}--\eqref{eq:solidModelInviscid} gives}
% The equations governing the fluid and solid are discretized in the $x$-direction on a uniform grid, $x_\ell = \ell \Delta x$ for $\ell = 0, 1,\ldots N_x$, with grid spacing $\dx = L/N_x$.  Since the problem is periodic, each variable can be represented as a discrete Fourier series
% \begin{align}
% q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2}  e^{2 \pi i k x_\ell/ L} \hat{q}_k (y,t), 
% \qquad \ell=0,1,2,\ldots,N_x. \label{eq:discreteFourierInviscid}
% \end{align}
% %
% where $q_\ell(y,t) \approx q(x_\ell,y,t)$ denotes an approximation of a fluid or solid variable and $\hat{q}_k(y,t)$ are the corresponding Fourier coefficients.  For convenience, $N_x$ is assumed to be an even integer.  Taking a discrete Fourier transform of the equations in~\eqref{eq:fluidModel} and~\eqref{eq:solidModel} gives
\begin{align}
\text{Fluid: } &\begin{cases}
\rho \partial_t \vfyh + \partial_y \ph = 0, &  y\in(0,H) \\
\partial_y^2 \ph - k_x^2 \ph =0, &  y\in(0,H) \\
\ph =0, & x \in (0,L), \quad y=H
\end{cases}
 \label{eq:fluidModelDiscrete} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsyh = i k_x \ssxh + \partial_y \ssyh, & y\in(-\infty,0) \\
\partial_t \ssxh = i k_x \rhos\cp^2 \vsyh, & y\in(-\infty,0) \\
\partial_t \ssyh = \rhos\cp^2 \partial_y \vsyh, & y\in(-\infty,0) \\
|\vsy|^2+|\ssx|^2+|\ssy|^2 < \infty, & y\rightarrow - \infty
\end{cases} \label{eq:solidModelDiscreteA}
\end{align}
%
%\begin{alignat}{2}
%\rho \partial_t \vfyh + \partial_y \ph &= 0, \quad && y\in(0,H), \\
%\partial_y^2 \ph - k_x^2 \ph &=0, \quad && y\in(0,H),
%\label{eq:phEqn} \\
%% \end{alignat}
%% %
%% The transformed equations for the solid are
%% \begin{alignat}{2}
%\rhos \partial_t \vsyh &= i k_x \ssxh + \partial_y \ssyh, \quad && y\in(-\infty,0) ,
%\label{eq:vsyhEqn} \\
%\partial_t \ssxh &= i k_x \rhos\cp^2 \vsyh, && y\in(-\infty,0), 
%\label{eq:ssxhEqn} \\
%\partial_t \ssyh &= \rhos\cp^2 \partial_y \vsyh, && y\in(-\infty,0)
%\label{eq:ssyhEqn}.
%\end{alignat}
%
\das{where $k_x = 2 \pi k /L$ is a normalized wave number. 
As before, the hats and $k$ subscripts on the Fourier coefficients have been 
suppressed for notational convenience.  
As in Section~\ref{sec:viscousAnalysis}, the characteristic form of the solid 
equations are considered.}
% The equations for the solid characteristics defined by the 
% transformation~\eqref{eq:mpiaTransformation}
% and are given by~\eqref{eq:mpiaAdvSrcB}--\eqref{eq:mpiaSrcD}.}
Since we are interested in wave propagation in the solid, it is useful to define the characteristics variables
\begin{align}
\bc = \ssyh + \zp\vsyh, \qquad
\ac = \ssyh - \zp\vsyh, \qquad
\dc = \ssxh,
\end{align}
and recast the solid equations in~\eqref{eq:solidModelDiscreteA} in the characteristic form
% \das{The discrete Fourier transform of these equations gives}
\bse
\begin{alignat}{2}
\partial_t \bc - \cp \partial_y \bc &= i k_x \cp \dc, \qquad && y\in(-\infty,0),
\label{eq:advSrcB} \\
\partial_t \ac + \cp \partial_y \ac &= -i k_x \cp \dc, \qquad && y\in(-\infty,0), 
\label{eq:advSrcA} \\
\partial_t \dc &= \frac{i k_x \cp}{2} (\bc - \ac), \qquad && y\in(-\infty,0).
\label{eq:SrcD}
\end{alignat}
\ese
%
% the comments are already mentioned in the model problem section
Equations~\eqref{eq:advSrcB} and~\eqref{eq:advSrcA} are advection equations for the incoming and outgoing characteristic variables $\bc$ and $\ac$, respectively,
%, corresponding to the variables defined in~\eqref{eq:ACharacteristic} and \eqref{eq:BCharacteristic} for $\nv=[0,-1]^T$, 
while~\eqref{eq:SrcD} describes the evolution of the tangential component of the solid stress.

The solid characteristic variables are discretized in the $y$-direction using a uniform collocated grid, $y_j = j\dy$ for $j = 0, -1, -2 \ldots$, with grid spacing $\dy$.  Although a staggered grid is used for the analysis in~\cite{fib2014} (and for the stability analyses of other FSI algorithms in~\cite{BanksSjogreen2011,lrb2013}), it is cleaner to use a collocated grid for the second-order accurate scheme.  Define the grid functions $\ac^n_j \approx \ac(y_j, t^n)$, $\bc^n_j \approx \bc(y_j, t^n)$ and $\dc^n_j \approx \dc(y_j,t^n)$, where $t^n = n \Delta t$ for a (fixed) time step $\Delta t$.  The advection equations in~\eqref{eq:advSrcB} and~\eqref{eq:advSrcA} are approximated using a second-order accurate Lax-Wendroff-type scheme having the form
\bse
\begin{align}
\bc^{n+1}_{j} &= \bc^{n}_j + 
\frac{\lambda_y}{2} \delta_0 \bc^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \bc^{n}_j 
+ i \lambda_x \dc^n_j
+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j), \label{eq:bLax} \\
\ac^{n+1}_{j} &= \ac^{n}_j - 
\frac{\lambda_y}{2} \delta_0 \ac^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \ac^{n}_j 
- i \lambda_x \dc^n_j
+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
+ \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j),  \label{eq:aLax}
\end{align}
\ese
where $\lambda_x = k_x \cp \dt$ and $\lambda_y = \cp \dt / \dy$ \das{take the same definition
as in Section~\ref{sec:viscousAnalysis}}.  The centered approximations of the spatial derivatives in~\eqref{eq:bLax} and~\eqref{eq:aLax} are defined in terms of the undivided difference operators $\delta_+ u^{n}_j = u^{n}_{j+1} - u^{n}_j$, $\delta_- u^{n}_j = u^{n}_j - u^{n}_{j-1}$ and $\delta_0 u^{n}_j = u^{n}_{j+1} - u^{n}_{j-1}$ for an arbitrary grid function $u^{n}_j$.  The evolution equation in~\eqref{eq:SrcD} is approximated using a second-order accurate BDF scheme of the form
\begin{align}
\dc^{n+1}_j &= \frac{4}{3}\dc^{n}_j - \frac{1}{3} \dc^{n-1}+ \frac{i \lambda_x}{3}
\left(\bc^{n+1}_j - \ac^{n+1}_j \right). \label{eq:dTrap}
\end{align}
For reference, the Fourier coefficients of the solid velocity and normal stress are related to the incoming and outgoing characteristic variables by
\begin{align}
{\bar v}_{2,j}\sp n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \qquad
{\bar\sigma}_{22,j}\sp n = \frac{1}{2} (\bc^n_j+\ac^n_j),
\end{align}
%\begin{align}
%(\vsyh)_j^n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \qquad
%(\ssyh)_j^n = \frac{1}{2} (\bc^n_j+\ac^n_j), \qquad
%(\ssxh)_j^n = \dc^n_j,
%\end{align}
and the boundedness condition at infinity implies that
\begin{align}
\vert \ac^n_j \vert^2 +
\vert \bc^n_j \vert^2 +
\vert \dc^n_j \vert^2 < \infty, \qquad \text{as } j \rightarrow -\infty.
\label{eq:bcInf}
\end{align}

%Let $\Delta t$ be the time step and let $t^n = n \Delta t.$
%The solid equations are solved with a dissipative scheme to in order to exploit 
%some useful properties in the analysis.
%A second order centered scheme was chosen to minimize the stencil to 
%three grid points (a second order upwind scheme requires a five point stencil).
%The schemes for equations \eqref{eq:advSrcA}--\eqref{eq:advSrcB}
%are derived by taking a Taylor series in time and replacing time derivatives
%with spacial derivatives. 
%Define the grid functions
%$\ac^n_j \approx \ac(y_j, t^n), \bc^n_j \approx \bc(y_j, t^n),$ and
%$\dc^n_j \approx \dc(y_j,t^n),$
%then the Taylor series for $\ac$ is given by
%\begin{align}
%\ac(y_j,t^{n+1}) =\;& \ac(y_j,t^{n}) + 
%\dt \partial_t \ac(y_j,t^{n}) + 
%\frac{\dt^2}{2} \partial_t^2 \ac(y_j,t^{n}) + O(\dt^3)\\
%=\;& \ac(y_j,t^{n}) - 
%\cp \dt \partial_y \ac(y_j,t^{n}) + 
%\frac{\cp^2 \dt^2}{2} \partial_y^2 \ac(y_j,t^{n}) \nonumber \\
%&- i k_x \cp \dt \dc(y_j,t^n)
%+ \frac{i k_x \cp^2 \dt^2}{2} \partial_y \dc(y_j,t^n) \nonumber \\
%&+ \frac{k_x^2 \cp^2 \dt^2}{4} \left(\bc(y_j,t^{n}) - \ac(y_j,t^{n}) \right) + O(\dt^3).
%\end{align}
%% \begin{align}
%% \ac^{n+1}_j &= \ac^{n}_j + 
%% \dt \partial_t \ac^{n}_j + 
%% \frac{\dt^2}{2} \partial_t^2 \ac^{n}_j + O(\dt^3)\\
%% \ac^{n+1}_j &= \ac^{n}_j - 
%% \cp \dt \partial_y \ac^{n}_j + 
%% \frac{\cp^2 \dt^2}{2} \partial_y^2 \ac^{n}_j 
%% + i k_x \cp \dt \dc^n_j
%% - \frac{k_x^2 \cp^2 \dt^2}{4} (\bc^{n}_{j} - \ac^{n}_{j}) + O(\dt^3).
%% \end{align}
%%
%A similar series can be derived for $\bc.$
%The spacial derivatives are approximated by centered second order finite
%difference formulas. Define the undivided difference operators
%$\delta_+ u_j = u_{j+1} - u_j,$ 
%$\delta_- u_j = u_j - u_{j-1},$ and $\delta_0 u_j = u_{j+1} - u_{j-1}$ 
%for an arbitrary grid function $u_j.$ The scheme for $\ac$ and $\bc$
%can be written as 
%\begin{align}
%\ac^{n+1}_{j} &= \ac^{n}_j - 
%\frac{\lambda_y}{2} \delta_0 \ac^{n}_j + 
%\frac{\lambda_y^2}{2} \delta_+ \delta_- \ac^{n}_j 
%- i \lambda_x \dc^n_j
%+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
%+ \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j)  \label{eq:aLax} \\
%\bc^{n+1}_{j} &= \bc^{n}_j + 
%\frac{\lambda_y}{2} \delta_0 \bc^{n}_j + 
%\frac{\lambda_y^2}{2} \delta_+ \delta_- \bc^{n}_j 
%+ i \lambda_x \dc^n_j
%+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
%- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j) \label{eq:bLax}
%\end{align}
%%
%where $\lambda_x = k_x \cp \dt$ and $\lambda_y = \cp \dt / \dy.$
%This is a Lax-Wendroff scheme for an advection equation with a source.
%After advancing $\ac$ and $\bc$ to the next time level, $\dc$ can be
%advanced with a simple quadrature. Since a non-dissipative pseudo-spectral approximation
%is used in the $x$ direction, 
%% the trapezoidal rule 
%a BDF scheme
%is used to stabilize the approximation.
%% \begin{align}
%% \dc^{n+1}_j &= \dc^{n}_j + \frac{i \lambda_x}{4}
%% \left(\bc^{n+1}_j - \ac^{n+1}_j + \bc^n_j - \ac^n_j \right). \label{eq:dTrap}
%% \end{align}
%\begin{align}
%\dc^{n+1}_j &= \frac{4}{3}\dc^{n}_j - \frac{1}{3} \dc^{n-1}+ \frac{i \lambda_x}{3}
%\left(\bc^{n+1}_j - \ac^{n+1}_j \right). \label{eq:dTrap}
%\end{align}
%%
%The $\cp^+$ characteristic, $\ac,$ will be extrapolated to the interface ghost point.
%Additionally, the solution must be bounded as $y \rightarrow -\infty.$
%\begin{alignat}{2}
%\ac^n_{1} &= 2 \ac^n_{0} - \ac^n_{-1}, \quad && \\
%\vert \ac^n_j \vert^2 +
%\vert \bc^n_j \vert^2 +
%\vert \dc^n_j \vert^2 &< \infty, \quad &&\text{as } j \rightarrow -\infty
%\label{eq:bcInf}
%\end{alignat}
%%
%The interface condition will determine $b_{1}^n,$ and the initial conditions will 
%define $a_j^0, b_j^0,$ and $d_j^0$ for $j = 0,1,2,3,\ldots$.
%For reference, the Fourier 
%coefficients of the solid velocity and stress components are related to the characteristic 
%variables by
%\begin{align}
%(\vsyh)_j^n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \quad
%(\ssyh)_j^n = \frac{1}{2} (\bc^n_j+\ac^n_j), \quad
%(\ssxh)_j^n = \dc^n_j.
%\end{align}

The equations for the Fourier coefficients of the fluid variables in~\eqref{eq:solidModelDiscrete} involve an evolution equation for the vertical component of the velocity and a reduced Laplace equation for the pressure.  Following the approach taken in~\cite{fib2014}, the Laplace equation for the pressure, with the boundary condition at $y=H$, is solved exactly at a time $t^n$ to give
\begin{align}
p(y,t^n) = p_I^n \frac{\sinh(k_x(H-y))}{\sinh(k_x H)},
\label{eq:pressureSubProblemSolution}
\end{align}
where $p_I^n$ is an interface pressure which is specified later by the chosen coupling at the interface.  For the purpose of the analysis, we only require the fluid velocity on the interface, which we define to be $v_I^{n}$.  The evolution of the interface velocity involves the gradient of pressure at $y=0$, which is given by
\begin{align}
\partial_y p(0,t^n) = - \frac{p_I^n}{\Heff},\qquad \Heff = \frac{\tanh(k_x H)}{k_x}.
\label{eq:interfacePressureGradient}
\end{align}
The effective fluid height, $\Heff$, in the formula for the pressure gradient depends on the normalized wave number, and it takes the limiting values of $\Heff=H$ as $k_x\rightarrow0$ and $\Heff=0$ as $k_x\rightarrow\infty$.

%The fluid variables are kept continuous in $y$ but discrete in time.
%The pressure sub-problem solves
%\begin{align}
%p_{yy}^{n}(y) - k_x^2 p^{n}(y) &= 0, \label{eq:pressureSubProblem}\\
%p^{n}(H) &= 0, \label{eq:pressureTopBoundary}
%\end{align}
%% 
%with an additional algorithm dependent interface condition at $y=0.$ The
%general solution to \eqref{eq:pressureSubProblem}--\eqref{eq:pressureTopBoundary}
%is
%\begin{align}
%p^n(y) = p_I^n \frac{\sinh(k_x(H-y))}{\sinh(k_x H)}, \label{eq:pressureSubProblemSolution}
%\end{align}
%%
%where $p_I^n$ is the interface pressure at time $t^n$, determined by the interface condition.
%The pressure gradient at the interface, needed to advance the fluid interface velocity,
%is given by
%\begin{align}
%\partial_y p^n(0) = - \frac{p_I^n}{\Heff},
%\end{align}
%%
%where
%\begin{align}
%\Heff = \frac{\tanh(k_x H)}{k_x}.
%\end{align}
%%
%For the 1D problem ($k_x = 0$), $\Heff = H.$ When $k_x \rightarrow \infty,$ 
%$\Heff \rightarrow 0.$
%For this simplified model problem analysis, only the fluid velocity at the interface
%is needed, which will be denoted as $v_f^n$ at time $t^n.$

\subsection{Interface coupling}

The evolution of the solid given by the equations in~\eqref{eq:advSrcB}, \eqref{eq:advSrcA} and~\eqref{eq:SrcD} requires a boundary condition on the interface, $y=0$, corresponding to the incoming characteristic variable.  Similarly, the evolution of the fluid given by the equations in~\eqref{eq:solidModelDiscrete} requires a boundary condition at $y=0$, which can be interpreted as an interface pressure needed to complete the elliptic problem for the fluid pressure as in~\eqref{eq:pressureSubProblemSolution}.  These two boundary conditions come from the matching conditions at the interface involoving the vertical velocity and normal stress.  In terms of the discretization of the Fourier coefficents for the model problem, the coupling at the interface takes on different forms depending on the choice of the partitioned scheme.  Since the behavior of the fluid for the model problem is determined by the solution of an elliptic problem for the pressure and an evolution equation for the vertical velocity on the interface, the coupling of the fluid to the behavior of the solid can be reduced to a modified boundary condition for the solid depending on the partitioned scheme employed as we discuss below.

Let us first consider the AMP algorithm and its interface coupling scheme.  
\das{The general algorithm is briefly described in Section~\ref{sec:algorithm} 
  and in more detail in~\cite{fibr2019}} 
and we follow this basic description but with suitable modifications for the choices of the discretizations made for the present model problem.  Let us assume that the discrete characteristic variables for the solid given by $\bc^{n}_j$, $\ac^{n}_j$ and $\dc^{n}_j$ are known at time levels $t\sp n$ and $t\sp{n-1}$ for all grid points, $y_j=j\dy$, $j=0,-1,\ldots$, including a ghost point at $j=1$.  We also assume that the interface velocity, $v_I\sp n$, is known at $t\sp n$ and $t\sp{n-1}$.  The evolution equations for the solid variables in~\eqref{eq:bLax}, \eqref{eq:aLax} and~\eqref{eq:dTrap} are used to advance the variables to $t\sp{n+1}$, and from these we compute the solid velocity and normal stress on the interface using
\begin{align}
{\bar v}_{2,0}\sp{n+1} = \frac{1}{2\zp} (\bc^{n+1}_0-\ac^{n+1}_0), \qquad
{\bar\sigma}_{22,0}\sp{n+1} = \frac{1}{2} (\bc^{n+1}_0+\ac^{n+1}_0).
\label{eq:interfaceSolidVelocityAndStress}
\end{align}
We next compute an extrapolated interface velocity, $v_I\sp{(e)}$, using a second-order accurate BDF-type integration of the evolution equation for the fluid velocity.  This gives the formula
\begin{align}
v_I^{(e)} = \frac{4}{3} v_I^n - \frac{1}{3} v_I^{n-1} - \frac{2\dt}{3 \rho}\partial_y p(0,t^{n+1}),
\label{eq:extrapInterfaceVelocity}
\end{align}
where the pressure gradient on the interface is given in~\eqref{eq:interfacePressureGradient}.  This extrapolated value for the fluid is averaged with the interface velocity for the solid from~\eqref{eq:interfaceSolidVelocityAndStress} to give
\begin{align}
v_I^{n+1} = \frac{\zf}{\zf + \zp}\,v_I^{(e)} + \frac{\zp}{\zf + \zp}\,{\bar v}_{2,0}\sp{n+1},
\label{eq:interfaceVelocityModel}
\end{align}
where we take $\zf = \rho H/\dt$.  For later convenience, define the weights
\begin{align}
\theta_f=\frac{\zf}{\zf + \zp},\qquad {\bar\theta}_p=\frac{\zp}{\zf + \zp},
\label{eq:weights}
\end{align}
and we note that $\theta_f+{\bar\theta}_p=1$.  \das{The AMP condition for the fluid pressure 
given in~\eqref{eq:AMPpressureBC} 
% given in~\eqref{eq:pressureConditionFractional}
requires an acceleration of the interface, and for this we use the backward difference formula}
\begin{align}
\dot{v}_I^{n+1} = \frac{1}{2\Delta t} \left(3v_{I}^{n+1} - 4v_{I}^{n} + v_{I}^{n-1}  \right).
\label{eq:interfaceAcceleration}
\end{align}
Using~\eqref{eq:extrapInterfaceVelocity} in~\eqref{eq:interfaceVelocityModel} to eliminate $v_I\sp{(e)}$, and then using the computed result in~\eqref{eq:interfaceAcceleration} to eliminate $v_{I}^{n+1}$ gives an alternate expression for the acceleration having the form
\begin{align}
\dot{v}_I^{n+1} = \theta_f\left(\frac{p_I^{n+1}}{\rho \Heff}\right) + {\bar\theta}_p\left(\frac{3{\bar v}_{2,0}\sp{n+1} - 4v_{I}^{n} + v_{I}^{n-1}}{2\Delta t} \right),
\label{eq:interfaceAccelerationNew}
\end{align}
which shows that the acceleration of the interface is also a weighted average of the acceleration from the fluid and that computed from the solid.  
\das{Finally, the AMP condition 
for the fluid pressure 
in~\eqref{eq:AMPpressureBC} 
% in~\eqref{eq:pressureConditionFractional}
reduces to }
\begin{align}
-p_I^{n+1}-\frac{\zp \dt}{\rho\Heff}\, p_I^{n+1} = {\bar\sigma}_{22,0}^{n+1} - \zp \dt \,\dot{v}_I^{n+1}.
\label{eq:AMPpressureBCmodel}
\end{align}
Using~\eqref{eq:interfaceAccelerationNew} in~\eqref{eq:AMPpressureBCmodel} to eliminate $\dot{v}_I^{n+1}$, and then solving for the interface pressure gives
\begin{align}
-p_I^{n+1} = \frac{M}{M+{\bar\theta}_p}\left[{\bar\sigma}_{22,0}^{n+1} - \zp{\bar\theta}_p\left(\frac{3}{2}{\bar v}_{2,0}\sp{n+1} - 2v_{I}^{n} + \frac{1}{2}v_{I}^{n-1} \right)\right],
\label{eq:interfacePressureModel}
\end{align}
where $M$ is a mass ratio given by
\begin{align}
M = \frac{\rho\Heff}{\zp \dt} = \frac{\rho\Heff}{\rhos \cp \dt}.
\label{eq:AcousticMassRatio}
\end{align}
We may now complete the time step for the solid variables by specifying values for the incoming and outgoing characteristic variables in the ghost points using
\begin{align}
\bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 a_I\sp{n+1},\qquad \ac^{n+1}_1 = 2 \ac^{n+1}_0 - \ac^{n+1}_{-1},
\label{eq:interfaceBCsForSolid}
\end{align}
where $a_I\sp{n+1}$ is an interface value for the incoming characteristic variable determined by
\begin{align}
a_I\sp{n+1} = -p_I^{n+1} + \zp v_I^{n+1},
\label{eq:incomingCharacteristicInterfaceModel}
\end{align}
Thus, the boundary condition for incoming characteristic variable is specified by $a_I\sp{n+1}$ (using a second-order accurate average) and the outgoing characteristic variable at the ghost point is given by a simple extrapolation.

For the AMP algorithm, the interface velocity and pressure used in~\eqref{eq:incomingCharacteristicInterfaceModel} to define the interface value for the incoming characteristic variable are given by the formulas in~\eqref{eq:interfaceVelocityModel} and~\eqref{eq:interfacePressureModel}, respectively, while the corresponding interface values for the TP and ATP algorithms use difference formulas.  For the TP algorithm, the interface velocity is given by the solid, while the interface stress is determined by the fluid.  This specification leads to
\begin{align}
v_I\sp{n+1}={\bar v}_{2,0}\sp{n+1},\qquad p_I\sp{n+1}=\rho\Heff\, \dot{v}_I^{n+1},
\label{eq:interfaceValuesTPscheme}
\end{align}
where the solid velocity is given in~\eqref{eq:interfaceSolidVelocityAndStress} and the interface acceleration is given in~\eqref{eq:interfaceAcceleration}.  For the ATP algorithm, the interface velocity is given by the fluid, while the interface stress is determined by the solid, and this gives
\begin{align}
v_I\sp{n+1}=v_I\sp{(e)},\qquad p_I\sp{n+1}=-{\bar\sigma}_{22,0}^{n+1},
\label{eq:interfaceValuesATPscheme}
\end{align}
where the fluid velocity is given in~\eqref{eq:extrapInterfaceVelocity} and the solid stress is given in~\eqref{eq:interfaceSolidVelocityAndStress}.  It is worth noting that values specified for the TP and ATP algorithms in~\eqref{eq:interfaceValuesTPscheme} and~\eqref{eq:interfaceValuesATPscheme}, respectively, agree with values given by the AMP algorithm in the limiting cases of a heavy solid ($\zp\rightarrow\infty$) and a light solid ($\zp\rightarrow0$).

%Following section \ref{sec:partitionedAlgorithms}, the AMP algorithm is applied
%to the simplified model problem.
%In the limit of a heavy solid, the AMP conditions approach a 
%no-slip condition for the fluid and a traction condition for the solid.
%In the light solid limit, the conditions approach a traction condition for 
%the fluid and a no-slip condition for the solid.
%Only the fluid solution at the interface is necessary to advance the solid in time.
%The AMP algorithm is given by the following.
%
%\listAlgorithm{AMP Algorithm (added-mass partitioned)}{
%\item Advance the solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
%\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
%$j = 0,\, -1, \, -2, \, -3, \, \ldots$.
%
%\item Obtain the predicted velocity and traction from the solid.
%\begin{align}
%v_s^{n+1} &= \frac{1}{2 \zp} \left(\bc^{n+1}_0 - \ac^{n+1}_0 \right) \\
%\sigma_s^{n+1} &= \frac{1}{2} \left(\bc^{n+1}_0 + \ac^{n+1}_0 \right)
%\end{align}
%
%\item Advance the fluid interface velocity using a BDF scheme on
%the fluid momentum equation.
%\begin{align}
%v_f^{n+1} = \frac{4}{3} v_I^n - \frac{1}{3} v_I^{n-1} 
%+ \frac{2\dt}{3 \rho \Heff} 
% p_I^{n+1} 
%\end{align}
%%
%
%\item Set the interface velocity as the impedance weighted average
%of the fluid and solid velocities using $\zf = \rho H/\dt$. 
%\begin{align}
%v_I^{n+1} = \frac{\zf v_f + \zp v_s}{\zf + \zp} 
%\end{align}
%
%\item Calculate the interface acceleration using a second order accurate
%backward difference formula.
%\begin{align}
%\dot{v}_I^{n+1} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{n+1} 
%  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
%\end{align}
%
%\item Solve the Poisson equation for the fluid pressure with
%the following AMP Robin condition specified at $y=0.$
%\begin{alignat}{2}
%-\ph^{n+1}+\frac{\zp \dt}{\rho} \ph_y^{n+1} &= 
%\sigma_s^{n+1} - \zp \dt \dot{v}_I^{n+1}, \quad && y = 0, 
%\end{alignat}
%
%Given the general solution in equation \eqref{eq:pressureSubProblemSolution},
%the interface pressure is 
%\begin{align}
%p_I^{n+1} &= \frac{1}{M \eta+1} 
%\rho \dot{v}_I \Heff
% - \frac{M \eta}{M \eta+1} \sigma_s,
%\end{align}
%%
%where
%\begin{align}
%M &= \frac{\rho H}{\zp \dt} = \frac{\rho H}{\rhos \cp \dt}, \label{eq:AcousticMassRatio} \\
%\eta &= \frac{\Heff}{H} = \frac{\tanh(k_x H)}{k_x H} \label{eq:Eta}
%\end{align}
%
%\item 
%%Set the interface traction $\sigma_I^{n+1} = -p_I^{n+1}.$
%Set the incoming $\cp^-$ characteristic, $\bc,$ using the interface velocity and stress.
%%$\delta = \rho/\rhos.$
%\begin{align}
%\bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right).
%% \bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 
%% \left[\frac{1}{1+\delta} 
%% \left(2 \sigma_I^{n+1} - \frac{\ac^{n+1}_{1} + \ac^{n+1}_{-1}}{2} \right)
%% +\frac{\delta}{1+\delta} \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right) \right].
%\end{align}
%
%\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$
%\begin{align}
%\ac^{n+1}_1 = 2 \ac^{n+1}_0 - \ac^{n+1}_{-1}
%\end{align}
%
%} \\
%
%% The solid is advanced on the interior and the boundary in the first two steps.
%% Next the fluid velocity is obtained in step 3. 
%% The interface velocity is projected using an impedance weighted average of the
%% fluid and solid values. 
%% This is used to determine the interface acceleration, which is used in
%% the pressure solution for step 7.
%% Afterwards, the solid boundary conditions are applied to obtain the ghost points.
%
%The acoustic mass ratio, $M$, defined in \eqref{eq:AcousticMassRatio},
%is the ratio of the mass of the fluid in a column of height 
%$H$ over the mass of a solid with the same cross section
%of height $\cp \dt,$ or the distance a p-wave travels in a single time step.
%The mass ratio is a measure of the prevalence of the added mass effect.
%For a heavy solid, the mass ratio is small and therefore added mass effects are small. 
%The mass ratio is inversely proportional to $\rhos$ and $\dt,$ therefore
%added mass effects can arise both in light solids and solids with a fine mesh.
%$\eta$ is the ratio between the effective fluid column height and the true fluid column height.
%
%The key behavior of the AMP algorithm is observed by taking the heavy and
%light solid limits. When $\zp \rightarrow \infty,$ the interface velocity
%and pressure approach the following limits.
%\begin{align}
%v_I^{n+1} &= 
%\begin{cases}
%v_s, & \zp \rightarrow \infty \\
%v_f, & \zp \rightarrow 0 
%\end{cases} \\
%p_I^{n+1} &= 
%\begin{cases}
%-\sigma_s, & \zp \rightarrow \infty \\
%\rho \dot{v}_I \Heff, & \zp \rightarrow 0 
%\end{cases}
%\end{align}
%%
%Corresponding algorithms for the TP (traditional partitioned) and the
%ATP (anti-traditional partitioned) schemes can be applied to the simplified model 
%problem following section \ref{sec:partitionedAlgorithms}.


\subsection{Stability analysis of AMP, TP and ATP schemes}

%
\newcommand{\nn}{\alpha}

In order to assess the stability of the AMP, TP and ATP schemes, we consider normal mode solutions of the discrete equations for the solid with the appropriate interface conditions.  For this analysis, we let
\begin{align}
\bc^{n}_j = \amp^n \tbc_j, \qquad 
\ac^{n}_j = \amp^n \tac_j, \qquad 
\dc^{n}_j = \amp^n \tdc_j,
\end{align}
%
where $\amp$ is an amplification factor and $(\tbc_j,\tac_j,\tdc_j)$ are spatial grid functions. 
\das{As in Section~\ref{sec:viscousAnalysis}, showing the scheme is weakly stable 
  is equivalent to showing there are no non-trivial solutions where $|\amp| > 1$
  for a given set of parameters.
  We first make the assumption $|A| > 1$ and solve the spacial problem by finding 
  general solutions of the discretization and boundedness condition as $j\rightarrow-\infty.$
  The interface conditions are then used to find if the amplification factor satisfies the
  assumption $|A|>1.$}  
% This is used in the viscous analysis section. I rephrased this.
%Our strategy for determining regions of stability will be to search for unstable modes with $|A| > 1$, and then identify regions of the parameter space where no non-trivial solution exist.  To do this, we begin by finding the general solution for the spatial grid functions satisfying the discrete equations and regularity condition as $j\rightarrow-\infty$, assuming $|A| > 1$.  We then apply the conditions at the interface to determine whether non-trivial solutions exist.


The discrete equations for the solid in~\eqref{eq:bLax}, \eqref{eq:aLax} and~\eqref{eq:dTrap}, with $\tacv_j = [\tbc_j,\tac_j,\tdc_j]^T$, can be written as a system of linear, second-order difference equations of the form
\begin{align}
[H_0 + H_1 \delta_0 + H_2 \delta_+ \delta_-] \tacv_j = 0,
\label{eq:DifferenceEquation}
\end{align}
%
where
% \begin{align}
% H_{0} &= 
% \left[\begin{array}{ccc}
% -\frac{\lx^2}{4}& \frac{\lx^2}{4}&-i \lx \\
% \frac{\lx^2}{4}&-\frac{\lx^2}{4}&i \lx \\
% - \frac{i \lx}{4} & \frac{i \lx}{4}&0 
% \end{array}\right], \\
% H_{1} &= 
% \left[\begin{array}{ccc}
% -\frac{\ly}{2} &0&\frac{i \lx \ly}{4} \\
% 0&\frac{\ly}{2}&\frac{i \lx \ly}{4} \\
% 0 & 0&0 
% \end{array}\right], \\
% H_{2} &= 
% \left[\begin{array}{ccc}
% \frac{\ly^2}{2} &0&0 \\
% 0&\frac{\ly^2}{2}&0 \\
% 0 & 0&0 
% \end{array}\right].
% \end{align}
%\begin{align}
%H_{0} &= 
%-A^2 
%\left[\begin{array}{ccc}
%1&0&0 \medskip\\
%0&1&0 \medskip\\
%-\frac{i \lx}{3}&\frac{i \lx}{3}&1
%\end{array}\right] 
%+A 
%\left[\begin{array}{ccc}
%1- \frac{\lx^2}{4}&\frac{\lx^2}{4}&i \lx \smallskip\\
%\frac{\lx^2}{4}&1-\frac{\lx^2}{4}&-i \lx \smallskip\\
%0&0&\frac{4}{3}
%\end{array}\right] 
%-
%\left[\begin{array}{ccc}
%0&0&0 \medskip\\
%0&0&0 \medskip\\
%0&0&\frac{1}{3}
%\end{array}\right] \\
%H_{1} &= 
%A \left[\begin{array}{ccc}
%\frac{\ly}{2} &0&\frac{i \lx \ly}{4} \\
%0&-\frac{\ly}{2}&\frac{i \lx \ly}{4} \\
%0 & 0&0 
%\end{array}\right], \\
%H_{2} &= 
%A \left[\begin{array}{ccc}
%\frac{\ly^2}{2} &0&0 \\
%0&\frac{\ly^2}{2}&0 \\
%0 & 0&0 
%\end{array}\right].
%\end{align}
\[
\begin{array}{c}
\displaystyle{
H_{0} = 
-A^2 
\left[\begin{array}{ccc}
1&0&0 \medskip\\
0&1&0 \medskip\\
-\frac{i \lx}{3}&\frac{i \lx}{3}&1
\end{array}\right] 
+A 
\left[\begin{array}{ccc}
1- \frac{\lx^2}{4}&\frac{\lx^2}{4}&i \lx \smallskip\\
\frac{\lx^2}{4}&1-\frac{\lx^2}{4}&-i \lx \smallskip\\
0&0&\frac{4}{3}
\end{array}\right] 
-
\left[\begin{array}{ccc}
0&0&0 \medskip\\
0&0&0 \medskip\\
0&0&\frac{1}{3}
\end{array}\right],
} \bigskip\\
\displaystyle{
H_{1} = 
A \left[\begin{array}{ccc}
\frac{\ly}{2} &0&\frac{i \lx \ly}{4} \\
0&-\frac{\ly}{2}&\frac{i \lx \ly}{4} \\
0 & 0&0 
\end{array}\right], \qquad
H_{2} = 
A \left[\begin{array}{ccc}
\frac{\ly^2}{2} &0&0 \\
0&\frac{\ly^2}{2}&0 \\
0 & 0&0 
\end{array}\right].
}
\end{array}
\]
%
Solutions of the difference equations in~\eqref{eq:DifferenceEquation} are sought in the form $\tacv_j = \tilde\rev \p^j$, where $\tilde\rev$ is a constant vector and $\p$ is a scalar.  This implies the homogeneous linear system
\begin{align}
\left[ H_0 + H_1 \left(\p - \p\sp{-1}\right) + H_2 \left(\p - 2 + \p\sp{-1} \right) \right] \tilde\rev = 0.
\label{eq:evProblem}
\end{align}
%
Non-trivial vectors $\tilde\rev$ exist for values of $\p$ satisfying
\begin{align}
\det\left[ H_0 + H_1 \left(\p - \p\sp{-1}\right) + H_2 \left(\p - 2 + \p\sp{-1} \right) \right] = 0.
\label{eq:quarticPhi}
\end{align}
%
It can be shown that the algebraic condition in~\eqref{eq:quarticPhi} is equivalent to a quartic polynomial in $\p$ for which there are four roots, $\p_\nn$, $\nn=1,2,3,4$.  Since we seek spatial grid functions that are bounded as $j\rightarrow-\infty$, we are only interested in the roots satisfying $\vert\p_\nn\vert\ge1$.
%There are four roots for $\p.$ Since we require the solid variables to 
%be bounded as
%$y \rightarrow -\infty,$ \eqref{eq:bcInf}, we are only interested in solutions 
%where $|\p|^j \le 1$ as $j \rightarrow -\infty.$ Therefore, only roots where
%$|\p| \ge 1$ are solutions to the boundary condition.

\medskip\noindent
\textbf{Lemma}: \textit{If $|A| > 1$ and if $\lx$ and $\ly$ are chosen to satisfy a CFL condition, then the roots of the quartic polynomial implied by~\eqref{eq:quarticPhi} satisfy}
\begin{align}
|\phi_1| > 1, \qquad |\phi_2| > 1, \qquad |\phi_3| < 1, \qquad |\phi_4| < 1.
\label{eq:SizeOfEigenvalues}
\end{align}

\medskip\noindent
\das{The analogous lemma for the viscous stability analysis 
  was proven in Section~\ref{sec:viscousAnalysis}.
  The following proof is structured similarly. 
  First, the stability for the
  scheme applied to the pure initial-value problem (Cauchy problem) is considered.
  This corresponds to setting $\phi=e^{i\vartheta}$ in~\eqref{eq:quarticPhi} and 
  finding the region of stability $|A|\le 1$ in the $\lx$-$\ly$ plane for all 
  $\vartheta \in [0,2\pi].$
  This region is found in~\ref{sec:CFLRegionCauchy} and shown in Figure~\ref{fig:inviscidCFL}.
  This region contains the quarter circle defined by $\lx^2+\ly^2\le 1$ and $\lx,\ly\ge 0.$
}
%This result follows from a similar argument to that given in~\cite{DifferenceApproximationsForTheInitialBoundary}.  We first consider the scheme applied to the pure initial-value problem (Cauchy problem).  Setting $\phi=e\sp{i\vartheta}$ in~\eqref{eq:quarticPhi}, we determine a region of the $\lx$-$\ly$ plane for which $\vert A\vert\le1$ for all $\vartheta\in[0,2\pi]$.  This region is found numerically as discussed in~\ref{sec:CFLRegionCauchy}, and it corresponds to a region where the Cauchy problem is (Fourier) stable.  It is also shown that this stability region includes a region of $(\lx,\ly)$ satisfying a reasonable CFL restriction, namely $\lx\sp2+\ly\sp2\le1$.
%
\das{When $|\phi|=1,$ we must have $|A| \le 1.$ Therefore $|A|>1$ implies $|\phi| \ne 1.$
  Due to the continuity of $\phi,$ if $|A| > 1$ and if $(\lx,\ly)$ remains within 
  the CFL restriction, $\phi$ cannot cross the unit circle, $|\phi|=1$, as $(\lx,\ly)$ vary. 
}
%Next, since $|A| \le 1$ when $|\phi| = 1$, we have that $|\phi| \ne 1$ when $|A| > 1$.  Thus, if $|A| > 1$ and if $(\lx,\ly)$ remains within the CFL restriction, then $\phi$ cannot cross the unit circle, $|\phi|=1$, as $(\lx,\ly)$ vary.  
\das{Therefore, it is only necessary to prove that the conditions on the roots 
in~\eqref{eq:SizeOfEigenvalues} hold for one set of parameters.  }
For $\lx=0$, the difference scheme reduces to a pair of decoupled Lax-Wendroff schemes (and a BDF scheme applied to $\partial_td=0$), where it is well known (see~\cite{GKSII} for example) that the conditions in~\eqref{eq:SizeOfEigenvalues} hold provided $\vert\ly\vert\le1$.  Thus, the condition holds for all $(\lx,\ly)$ provided the CFL condition is satisfied.

In view of the above Lemma, we can now write the general solution for $\acv^n_j=[\bc^{n}_j,\ac^{n}_j,\dc^{n}_j]\sp T$, satisfying the regularity condition and assuming $\vert A\vert>1$, in the form
\begin{align}
\acv^n_j = \amp^n \left(k_1 \tilde\rev_1 \p_1^j + 
k_2 \tilde\rev_2 \p_2^j \right), \label{eq:EigenvectorExpansion}
\end{align}
where $k_1$ and $k_2$ are scalar constants.  Let $\tilde\rev_\nn = [\qn{\nn},\rn{\nn},\sn{\nn}]^T$ for $\nn = 1,2$.  We note that the third equation in the matrix system~\eqref{eq:evProblem} implies
%Using the third component of equation \eqref{eq:DifferenceEquation}, 
%$\sn{n}$ can be found in terms of $\qn{n}$ and $\rn{n}$.
\begin{align}
% \sn{n} = \frac{i \lx}{4} \frac{A+1}{A-1} (\rn{n} - \qn{n}) 
\sn{\nn} = \frac{A^2 i \lx}{3 A^2- 4 A + 1} (\qn{\nn} - \rn{\nn}),\qquad \nn = 1,2,
\end{align}
so that the third component of $\acv^n_j$ can be eliminated in terms of the first two components.  The final two constraints are given by the interface conditions in~\eqref{eq:interfaceBCsForSolid}, and this leads to a homogeneous system for $\kv=[k_1,k_2]\sp T$ of the form
\begin{align}
\dMat \kv= \left[\begin{array}{cc}
\dComp_{11} & \dComp_{12} \\
\dComp_{21} & \dComp_{22}
\end{array}\right] 
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right] = 0.
\label{eq:StabilitySystem}
\end{align}
%
The coefficients of the matrix $\dMat$ involve the amplitude factor $\amp$, and these are given in~\ref{sec:ComponentsOfDmat} for the AMP, TP and ATP schemes.  For non-trivial solutions, we seek solutions for $\amp$ such that
\begin{align}
\det(\dMat) = \dComp_{11} \dComp_{22} - \dComp_{12} \dComp_{21} = 0.
\label{eq:determinantCondition}
\end{align}
%
We first proceed with an analysis of the 1D case assuming $\lx = 0$.  After finding solutions for~$\amp$ when $\lx = 0$, we use a continuation procedure to determine solutions for $\amp$ numerically as $\lx$ increases from zero.

\subsubsection{1D schemes, $\lx=0$}

As noted earlier, the discrete evolution equations in~\eqref{eq:bLax} and~\eqref{eq:aLax} for the solid reduce to a pair of standard Lax-Wendroff schemes (without source terms) for the variables associated with incoming and outgoing characteristics when $\lx=0$.  Accordingly, the first two components of~\eqref{eq:DifferenceEquation} become
\begin{align}
A \tbc_j = \left( 1 + \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tbc_j,\qquad
A \tac_j = \left( 1 - \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tac_j.
\end{align}
%
Setting $\tbc_j=\tbc_0\p_{\bc}\sp j$ and $\tac_j=\tac_0\p_{\ac}\sp j$ yields the eigenvalues
\begin{align}
\p_{\bc,\pm} =\frac{\amp-(1-\ly\sp2) \pm \sqrt {\amp\sp2-(2\amp-1)(1-\ly\sp2)}}{\ly \left( \ly+1 \right) }, \qquad 
\p_{\ac,\pm} =  \frac{1}{\p_{\bc,\mp}}.
\label{eq:eigenvalueOneD}
\end{align}
%
If $\vert\amp\vert>1$ and if $\ly$ satisfies the CFL constraint $\vert\ly\vert\le1$, then one eigenvalue from each plus-minus pair in~\eqref{eq:eigenvalueOneD} has magnitude greater than one, while the other has magnitude less than one in agreement with~\eqref{eq:SizeOfEigenvalues}.  Let $\p_1$ to be the eigenvalue from $\p_{\bc,\pm}$ with magnitude greater than one and let $\p_2$ to be the corresponding eigenvalue $\p_{\ac,\pm}$.  Assuming the principal branch of the square-root function in~\eqref{eq:eigenvalueOneD}, we set
\begin{align}
(\p_1,\p_2)=
\begin{cases}
(\p_{\bc,+},\p_{\ac,+}), & \hbox{if $\Re(A) \ge 1 - \ly^2$}, \\
(\p_{\bc,-},\p_{\ac,-}), & \hbox{if $\Re(A) < 1 - \ly^2$}.
\end{cases}
\end{align}
%
%
%\das{In~\ref{sec:PiecewiseDefinition}, we show that 
%\begin{align}
%\p_1 &= 
%\begin{cases}
%\p_{\bc,+}, & \Re(A) > 1 - \ly^2 \\
%\p_{\bc,+}, & \Re(A) = 1 - \ly^2 \text{ and } \Im(A) > 0\\
%\p_{\bc,-}, & \Re(A) < 1 - \ly^2 \\
%\p_{\bc,-}, & \Re(A) = 1 - \ly^2 \text{ and } \Im(A) < 0
%\end{cases} \\
%\p_2 &= 
%\begin{cases}
%\p_{\ac,+}, & \Re(A) > 1 - \ly^2 \\
%\p_{\ac,+}, & \Re(A) = 1 - \ly^2 \text{ and } \Im(A) > 0\\
%\p_{\ac,-}, & \Re(A) < 1 - \ly^2 \\
%\p_{\ac,-}, & \Re(A) = 1 - \ly^2 \text{ and } \Im(A) < 0
%\end{cases} ,
%\end{align}
%%
%as long as $|A| > 1$ and $0 \le \ly \le 1.$}
%%
Since the evolution equations for $\bc_j\sp n$ and $\ac_j\sp n$ are decoupled, the corresponding eigenvectors in~\eqref{eq:EigenvectorExpansion} are unit vectors, $\tilde\rev_{1} = [1,0,0]^{T}$ and $\tilde\rev_{2} = [0,1,0]^{T}$, i.e.~$\qn{2} = \rn{1} = \sn{1} = \sn{2} = 0$, and the matrix $\dMat$ in~\eqref{eq:StabilitySystem} becomes diagonal. Thus, the determinant condition in~\eqref{eq:determinantCondition} reduces to
\begin{align}
\det(\dMat)= \dComp_{11} \dComp_{22} = 0.
\end{align}
% \textcolor{red}{(Note changes here due to ordering of $a$ and $b$.)}
The component, $\dComp_{22}$, is associated with the extrapolation of the outgoing characteristic variable from~\eqref{eq:interfaceBCsForSolid}, and this factor is zero only if $\p_2=1$.  However, $\vert\p_2\vert>1$, so that $\dComp_{22}\ne0$ and thus $k_2=0$ in~\eqref{eq:EigenvectorExpansion}.  The remaining component, $\dComp_{11}$, is associated with the interface condition on the incoming characteristic variable, and this term takes different forms depending on the choice of the interface coupling (see~\ref{sec:ComponentsOfDmat}).  Manipulation of the constraint, $\dComp_{11}=0$, for the AMP, TP and ATP schemes leads to polynomials in $\amp$ of degrees~6, 6 and~4, respectively, whose coefficients depend on $\ly$ and $M_0=\rho H/(\zp \dt)$.
\textcolor{red}{(For now I am defining $M_0$ which is just $M$ with $\lx=0$.)}
  Due to the algebraic complexity, the software package Maple is used to generate the polynomials and compute the roots for given values of $(\ly,M_0)$.  We note that some roots of the polynomials may not be solutions of the determinant constraint and so these spurious roots are discarded.  If no valid roots are found satisfying $\vert\amp\vert>1$ for a given value of $(\ly,M_0)$, then we conclude that $k_1$ in~\eqref{eq:EigenvectorExpansion} must also be zero so that only the trivial solution exists and thus the scheme is (weakly) stable.

We find it convenient to explore the roots of the three polynomials in terms of the parameters $\ly$ and $\Mr$, where
\begin{align}
\Mr = M_0\ly= \frac{\rho H}{\rhos \dy}.
\label{eq:massRatio}
\end{align}
The latter parameter is the ratio of the mass contained in a fluid column of height $H$ to that of the solid with the same cross section and of height $\dy$.  Starting with the AMP scheme, we compute valid roots of its polynomial for an $800\times800$ array of parameter values on a logarithmic scale for the range $10^{-6} \le \lambda_y \le 1$ and $10^{-6} \le \Mr \le 10^{7}$.  For these values, no roots with $\vert\amp\vert>1$ are found, which provides a strong indication of stability of the 1D AMP scheme for $0<\ly\le1$ and $\Mr>0$.  Shaded contours of the maximum values of $\vert\amp\vert$ are displayed in the left plot of Figure~\ref{fig:acousticSolidStokesStabilityTP} for a range of values of $\Mr$ and $\ly$.  The roots of the polynomials associated with the 1D TP and ATP schemes are also computed for the same array of parameter values.  For these schemes, parameter values for which $\vert\amp\vert>1$ are found indicating that regions of instability exist for these scheme.  The right plot of Figure~\ref{fig:acousticSolidStokesStabilityTP} shows regions of stability of the TP and ATP schemes where no roots with $\vert\amp\vert>1$ are found.  We note that for a fixed value of $\ly=\cp \dt / \dy\in(0,1]$, decreasing the mesh spacings in both time and space corresponds to increasing the mass ratio $\Mr$ defined in~\eqref{eq:massRatio}.  The right plot in the figure indicates that the TP scheme becomes unstable as the mesh is refined, while the ATP scheme ultimately becomes stable.  In contrast, the AMP scheme is always stable, and these observations agree with the analysis of the first-order accurate difference schemes performed in~\cite{fib2014}.

% {
% % ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
% \newcommand{\figWidth}{8cm}
% \begin{figure}[h]
% \begin{center}
%   \includegraphics[width=\figWidth]{fig/AMPStability1D}
%   \includegraphics[width=\figWidth]{fig/FSIStabilityRegionBDF}
%   \caption{Left: Shaded contours of the maximum amplification factor $\vert\amp\vert$ 
%     for the AMP scheme for the parameters $\lambda_y = \cp \dt / \dy$ and $\Mr = \rho H / (\rhos \dy)$.
%     Right: Stability regions for the 1D TP and ATP schemes. 
%     Grid refinement corresponds to increasing $\Mr$, and thus the
%     TP scheme becomes unstable as the grid is refined while the ATP scheme becomes stable.
%   }  \label{fig:acousticSolidStokesStabilityTP}
% \end{center}
% \end{figure}
% }
{
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
\newcommand{\figWidth}{6cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMPStability1D_log}
  \includegraphics[width=\figWidth]{fig/FSIStabilityRegionBDF_log}
  \caption{
    Left: Shaded contours of the maximum amplification factor $\vert\amp\vert$ 
    for the AMP scheme for the parameters $\lambda_y = \cp \dt / \dy$ and $\Mr = \rho H / (\rhos \dy)$.
    Right: Stability regions for the 1D TP and ATP schemes. 
    Grid refinement corresponds to increasing $\Mr$, and thus the
    TP scheme becomes unstable as the grid is refined while the ATP scheme becomes stable.
  }  \label{fig:acousticSolidStokesStabilityTP}
\end{center}
\end{figure}
}

%The roots of the AMP polynomial were found at an array of $800$ points in 
%$10^{-6} \le \lambda_y \le 1$ and $800$ points in $10^{-6} \le \Mr \le 10^{7}.$ 
%No unstable roots, $|A| > 1,$ were found. The same process was repeated for the 
%TP and ATP schemes for a range $10^{-6} \le \Mr \le 10.$ The stability region
%was plotted in figure \ref{fig:acousticSolidStokesStabilityTP}. 
%Since $\Mr \propto \dy^{-1},$ grid refinement will increase the mass ratio.
%The TP scheme will become unstable for sufficiently large $\Mr,$ therefore the 
%scheme is formally unconditionally unstable. On the other hand, the ATP scheme will 
%eventually become stable for a sufficiently large $\Mr.$ This scheme is weakly
%stable. Despite this, there is a significant
%region in parameter space where only the AMP scheme is stable.

The AMP, TP and ATP schemes can be implemented for the 1D FSI model problem, and then run numerically for different values of the parameters to check the results of the stability analysis.  
Initial conditions can be constructed so that the exact solution decays 
exponentially in time.
This corresponds to taking the initial condition, $b(y,0) = b_0(y) = 0$
(see~\ref{sec:SolutionToOneDimensional}). 
Since the interface velocity is expected to decay in time, we can assess the stability of the scheme by checking the 
magnitude of the interface velocity.  If this velocity grows in time, becoming larger than the initial interface velocity, then we consider the scheme to be unstable for the choice of parameter values.
For the AMP scheme, no parameter values are found for which the numerical results are unstable.  For the TP and ATP schemes, the colored marks in Figure~\ref{fig:acousticSolidStokesStabilityTPNumerical} indicate stability or instability of the numerical scheme for selected parameter values.  The black curves in the figure correspond to the stability boundaries obtained from the stability analysis.  We note that there is good agreement between the numerical results of the schemes and that given by the analysis.


%A 1D FSI numerical solver was used to verify the stability regions for the TP and ATP
%schemes. In figure \ref{fig:acousticSolidStokesStabilityTPNumerical}, points in
%$\Mr$-$\ly$ space were sampled to test for numerical instability. 
%It was found that the numerical results confirm that the stability region holds.


{
% ---- from codes/analysis/numerical/b4_runTP1DStability ---- $
% ---- from codes/analysis/numerical/b5_runATP1DStability ---- $
\newcommand{\figWidth}{6cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/FSIStabilityTP1DNumerical}
  \includegraphics[width=\figWidth]{fig/FSIStabilityATP1DNumerical}
  \caption{Verification of the stability regions for the TP scheme (left)
    and the ATP scheme (right) using numerical solutions of the 1D FSI model problem. Green marks 
    correspond to a stable numerical solution, while red markers correspond to numerical instability.  The black curves give the stability boundaries obtained from the stability analysis.
  }  \label{fig:acousticSolidStokesStabilityTPNumerical}
\end{center}
\end{figure}
}


% talk about numerical results

% Numerical Results:
%  - convergence for each scheme
%  - confirm stability region for each scheme
%
%   TP:
%     - heavy solid convergence study
%     - show stability region
%   ATP: 
%     - light solid convergence study
%     - show stability region
%   AMP:
%     - heavy/light solid convergence study
%     - really heavy/really light

\subsubsection{2D schemes, $\vert\lx\vert>0$}

\newcommand{\zz}{{z}}  % root index
\newcommand{\NN}{{\mathcal{Z}}}  % number of roots

% derive eigenvectors with the idea that lx is small
% Now we approach the 2D model problem by considering $\lx$ to be a small 
% perturbation to the 1D problem. The main motivation for this is
% that the stability limit for the Cauchy problem requires $\lx < .3,$ (\todo{show this})
% and only $\lx^2$ appears in the discretization. 
%Additionally, the 2D added mass ratio
%$\Mr = (\rho \tanh(k_x H))/(k_x \rhos \dy)$ will only decrease as $k_x$ increases
The strategy for finding solutions of the determinant condition in~\eqref{eq:determinantCondition} for $\vert\lx\vert \ne 0$ is to use the solutions for $\amp$ of the 1D determinant condition as a starting point for a numerical root solver that performs a continuation as $\lx$ varies.  In addition to the principal continuation parameter $\lx$, the roots also depend on the parameters $\ly$ and $M=\rho\Heff/(\zp\dt)$, where $\Heff$ was defined previously in~\eqref{eq:interfacePressureGradient}.  As before, we find it convenient to examine the roots in terms of the mass ratio $\Mr$ introduced in~\eqref{eq:massRatio} and the height ratio, $\eta=\Heff/H$, which varies on $(0,1]$, and we note that $M=\Mr\eta$.  Using our continuation procedure, we are able to compute the roots of the determinant condition as a function of the parameters $\lx$, $\ly$ and $M=\Mr\eta$.  Though there are multiple roots, $\amp_\zz$, $\zz=1,2,\ldots,\NN$, for a given set of parameters, we are only interested in the amplification factor with the maximum modulus.  Define
\begin{align}
A_{\max}(\lx,\,\ly,\,\Mr \eta)=\max_{1\le\zz\le\NN}\vert\amp_\zz(\lx,\,\ly,\,\Mr \eta)\vert,
\end{align}
to be the maximum amplification factor in magnitude for a given set of parameters.  The pseudo-spectral approximation of the model problem given in~\eqref{eq:solidModelDiscrete} depends on the normalized wave number $k_x$.  The corresponding discrete evolution equations for each Fourier mode of the approximation must all be stable for the chosen partitioned scheme to be stable (either the AMP, TP or ATP schemes).  Since $\lx$ and $\eta$ both depend on $k_x$, we are interested in the values of $A_{\max}$ for all possible values for $\lx$ and $\eta$.  Define
\begin{align}
\mathcal{A}_{\max}(\Mr,\ly) = 
\max_{\lx \in \mathcal{D}(\ly),\, \eta \in (0,1]} A_{\max}(\lx,\,\ly,\,\Mr \eta),
\label{eq:AmaxDefinition2D}
\end{align}
%
where $\mathcal{D}(\ly)$ gives the interval of $\lx$ satisfying the Cauchy stability bound for a given value of $\ly$ (see~\ref{sec:CFLRegionCauchy}).  We take $\mathcal{D}(\ly) = [0, (1 - \ly^2)^{1/2}]$.
Since the maximum amplification factor for the 1D case (with $\lx=0$) must be less than or equal to $\mathcal{A}_{\max}$, we are effectively examining whether the maximum amplification can increase when $\vert\lx\vert>0$. Figure~\ref{fig:lysmAMP2D} shows shaded contours of $\mathcal{A}_{\max}(\Mr,\ly)$ on the left, and the stability regions of the TP and ATP schemes on the right.  These plots are similar to the ones for the 1D analysis in Figure~\ref{fig:acousticSolidStokesStabilityTP}, indicating that the stability results provided by the 1D analysis are essentially unchanged when variations in the transfer direction are considered.  In fact, Figure~\ref{fig:lysmAMP2Doverlay} shows the stability regions for the TP and ATP schemes given by the 1D and 2D analyses overlayed.  Here, we observe that the stability regions given by the 2D analysis are only slightly smaller than those given by the 1D analysis.
% a surface plot of $\mathcal{A}_{\Mr}$
%and the stability region, $|A| \le 1$ in the $\Mr$-$\ly$ plane.
%There is a finite range of $\ly$ for which the AMP scheme is stable for all 
%$\lx,\,\Mr,$ and $\eta$.

\textcolor{red}{Will come back to this later.  I think the main point here is that we just showed above that the AMP scheme is stable for a large range of $\ly$ and mass ratios $\Mr$.  Given this, we can turn the question around and consider the region of stability of the AMP scheme in the $\lx$-$\ly$ plane for all values of $M=\Mr\eta$.  The objective of this analysis is to arrive at a CFL condition involving $\lx$ and $\ly$ such the AMP scheme is stable for any choice of the mass ratio.  Of course, the analysis is performed for a chosen model problem, but the results of the analysis can be used as a guide for the AMP scheme applied to the full FSI problem over a wide range of mass ratios.}  We can also search for a maximum amplification factor over all mass ratios,
$\mathcal{A}_{\text{CFL}},$ to see the CFL region for the AMP scheme in $\lx$-$\ly$ plane. 
Define
\begin{align}
\mathcal{A}_{\text{CFL}}(\lx,\ly) = 
\max_{0 < \Mr \eta < \infty} A_{\max}(\lx,\,\ly,\,\Mr \eta) .
\end{align}
%
This definition allows us to find a time step restriction regardless of the
mass ratio of the problem.
Figure \ref{fig:lylxAMP2D} shows a surface plot of $\mathcal{A}_{\text{CFL}}$
and the stability region, $|A| \le 1$ in the $\lx$-$\ly$ plane.

\medskip\noindent
\textbf{Theorem}: \textit{By numerical evaluation of $\ACFL(\lx,\ly)$,
we have found that the AMP algorithm is weakly stable ($|\ACFL| \le 1$)
provided that $\lx^2 + \ly^2 \le 1$, i.e.}
\begin{align}
\dt \le \frac{1}{\cp} \left[\frac{1}{\dy^2} + k_x^2 \right]^{-1/2}.
\end{align}
%
\textit{This is a sufficient but not a necessary condition.}

%
% {
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
% \newcommand{\figWidth}{8cm}
% \begin{figure}[H]
% \begin{center}
%   \includegraphics[width=\figWidth]{fig/FSIStabilityRegion2D}
%   \caption{Stability region for the 1D and 2D TP and ATP schemes. 
%     $\bar{\Mr}$ is defined from 
%     equations \eqref{eq:MrbarTP}--\eqref{eq:MrbarATP} and is the worst
%     case mass ratio for all Fourier modes.
%     $\lambda_y = \bar{c} \dt / \dy$ is the CFL number.
%     The stability region for the AMP scheme spans 
%     $0 < \ly < 1,$ $0 < \bar{\Mr} < \infty.$ 
%     An increase in $\bar{\Mr}$ corresponds to grid refinement,
%     therefore TP scheme will become unstable and the ATP scheme will become stable.
%   }  \label{fig:acousticSolidStokesStabilityTP2D}
% \end{center}
% \end{figure}
% }
% {
% \newcommand{\figWidth}{8cm}
% \begin{figure}[h]
% \begin{center}
%   \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_sm_surf}
%   \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_sm_cont}
%   \caption{Left: surface plot of maximum $|A|$ over $\lx \in [0,1]$
%     and $\eta \in (0,1]$ for the AMP scheme.
%     Right: the green fill indicates the stability region $|A| \le 1.$
%     For reference, 
%     $\ly = \cp \dt / \dy,\, \Mr = \rho H / (\rhos \dy),\, \lx = \cp k_x \dt,\, 
%     \eta = \tanh(k_x H)/ (k_x H).$
%   } \label{fig:lysmAMP2D}
% \end{center}
% \end{figure}
% }
{
\newcommand{\figWidth}{6cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_03_03_N50_LargeRange_Nep200_new_ly_sm_surf}
  \includegraphics[width=\figWidth]{fig/TP_continuation_03_03_N50_LargeRange_Nep200_newerStabilityRegions2D}
  \caption{Left: Shaded contours of the maximum amplification factor 
    $\mathcal{A}_{\max}(\Mr,\ly)$ 
    (as defined in equation \eqref{eq:AmaxDefinition2D})
    for the AMP scheme for the parameters $\ly=\cp \dt/\dy$ and $\Mr=\rho H/ (\rhos \dy).$
    Right: Stability regions (ie. where $\mathcal{A}_{\max}(\Mr,\ly) \le 1$)
    for the 2D TP and ATP schemes. 
    Grid refinement corresponds 
    to increasing $\Mr$, and thus the
    TP scheme becomes unstable as the grid is refined while the ATP scheme becomes stable.
  } \label{fig:lysmAMP2D}
\end{center}
\end{figure}
}
{
\newcommand{\figWidth}{6cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/TP_continuation_03_03_N50_LargeRange_Nep200_newerStabilityRegions_1D_and_2D}
  \caption{Stability regions for the TP and ATP schemes in 1D and 2D for the 
    parameters $\ly=\cp \dt/\dy$ and $\Mr=\rho H/ (\rhos \dy).$
    The lighter shaded colors represent the 1D regions and the darker shaded colors represent
    the 2D regions.
    Grid refinement corresponds to increasing $\Mr$, and thus the
    TP scheme becomes unstable as the grid is refined while the ATP scheme becomes stable.
  } \label{fig:lysmAMP2Doverlay}
\end{center}
\end{figure}
}
{
\newcommand{\figWidth}{6cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_lx_surf}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_lx_cont}
  \caption{
    Left: surface plot of maximum $|A|$ over $\Mr \eta \in [10^{-6},10^{6}]$
    for the AMP scheme.
    Right: the green fill indicates the stability region $|A| \le 1.$
    The dotted line is a plot of
    $\lx^2 + \ly^2 = 1$. 
    For reference, 
    $\ly = \cp \dt / \dy,\, \Mr = \rho H / (\rhos \dy),\, \lx = \cp k_x \dt,\, 
    \eta = \tanh(k_x H)/ (k_x H).$
  } \label{fig:lylxAMP2D}
\end{center}
\end{figure}
}

%\subsection{Stability analysis of TP scheme with iterations}
%
%\das{Should this be in this paper?}
%\textcolor{red}{DWS: not sure, but will skip this for now...}
%\das{Put iterations scheme here. Also want to note that there are better iterative
%schemes such as Aitken acceleration.}
%The TP scheme is more commonly used with iterations to avoid the added mass instability
%when refining grids. We perform an analysis of the TP iteration to understand
%how to choose the under-relaxation factor and how many iterations to take.
%Define the error between iterations to be the difference in interface velocities
%\begin{align}
%e^{(k)} = v_I^{(k+1)} - v_I^{(k)}.
%\end{align}
%%
%By taking the difference between the current and previous iteration variable for
%each step of the TP iteration, one can derive that
%\begin{align}
%e^{(k)} &= \left(1 - \omega \left(\frac{3}{2} \Mra + 1 \right)\right) e^{(k-1)}.
%\end{align}
%%
%Define the amplification factor, $\ampI = 1 - \omega \left(\frac{3}{2} \Mra + 1 \right)$
%where $e^{(k)} = A^{k} e^{(0)}.$
%$\Mra$ is dependent on the wave number, $k_x.$ In order to optimize the convergence rate,
%$\ampI$ needs to be optimized for all wave numbers.
%\begin{align}
%\Mra = \frac{\rho \tanh(k_x H)}{\zp \dt k_x} 
%= \frac{\rho H}{\zp \dt} \frac{\tanh(k_x H)}{k_x H} 
%= \Mra_0 \eta
%\end{align}
%%
%where $\Mra_0 = (\rho H) / (\zp \dt)$ is the 1D acoustic mass ratio and 
%$\eta = \tanh(k_x H) / (k_x H)$ is the 2D scale factor. To accommodate all
%potential wave numbers in the $x$ direction, we consider $\eta \in [0,1].$
%Let $\Mra = \Mra(\eta) = \Mra_0 \eta.$ The amplification factor for a given
%$\omega$ and $\eta$ is
%\begin{align}
%\ampI(\eta,\omega) = a - \omega \left(\frac{3}{2} M_0 \eta + 1 \right).
%\end{align}
%%
%We pose the following optimization problem to find the optimal 
%under-relaxation parameter, $\omega^*$.
%\begin{align}
%\omega^* = \argmin_{\omega} \max_{0 \le \eta \le 1} |A(\eta,\omega)|
%\end{align}
%%
%Since $\ampI$ is linear in $\eta$ and $\omega$ and $|\ampI| > 0,$ the maximum 
%amplification factor for a 
%given $\omega$ will occur on the boundary, $\eta = 0$ or $\eta = 1.$ 
%\begin{align}
%\ampI(\eta=0,\omega) = |1-\omega|, \quad 
%\ampI(\eta=1,\omega) = \left| 1 - \omega \left(\frac{3}{2} M_0 + 1 \right) \right|
%\end{align}
%%
%The choice of $\omega$ that minimizes both expressions corresponds to solving
%$\ampI(\eta=0,\omega^*) = \ampI(\eta=1,\omega^*).$ It can be shown that
%\begin{align}
%\omega^* = \frac{4}{3 \Mra_0 + 4}, \quad \ampI^* = \frac{3 M_0}{3 M_0 + 4}.
%\end{align}
%%
%This is a sensible result. The TP scheme suffers from added mass instability
%for fine grids and light solids, which correspond to large acoustic mass ratios.
%The under-relaxation parameter scales with $\Mra_0^{-1}$ to stabilize the added mass
%effects. As a penalty, the amplification factor approaches $1$ for large $\Mra_0.$
%To get a sense of computational cost for using TP iterations, we look at the number
%of iterations needed for the relative error, $|e^{(k)}/e^{(0)}|,$ to converge to 
%a desired tolerance, $\tau.$  It is easy to show that if $|A^*|^k < \tau,$ $k$ must 
%satisfy
%\begin{align}
%k &> \frac{\log (\tau) }
%{\log \left(\frac{3 M_0}{3 M_0 + 4} \right)} .
%\end{align}
%% 
%We are interested in the asymptotic behavior for $\Mra_0 \gg 1.$ The denominator
%of the above expression is asymptotically equivalent to
%\begin{align}
%\log \left(\frac{3 \Mra_0}{3 \Mra_0 + 4} \right) =
% \log \left(\frac{1}{1 + \frac{4}{3 \Mra_0} } \right)
%\sim  \log \left(1 - \frac{4}{3 \Mra_0} + ... \right) 
%\sim -\frac{4}{3 \Mra_0} + ...
%\end{align}
%%
%Therefore 
%\begin{align}
%k > -\frac{3}{4} M_0 \log(\tau) = 
%-\frac{3 }{4} \frac{\rho H }{ \bar{\rho} \bar{c} \Delta t} \log(\tau).
%\end{align}
%% 
%The required number of iterations is proportional to $\dt^{-1}.$ 
%For a viscous fluid simulation, the viscous terms can be treated as
%implicitly or explicitly.
%When an implicit solver is chosen, the time step will be proportional to
%the grid spacing and the number of iterations will double when the grid is refined 
%by a factor of $2$. 
%When an explicit solver is chosen, the time step will be proportional to the 
%square of the grid spacing and the number of iterations will quadruple when the grid
%is refined by a factor of $2.$
%

% numerical results 



%%%%%%%%%%%%% old paper
% \subsection{Discretization}

% talk about fluid and solid discretization in x. 
% discrete fourier series on grid 
% % \wdh{We discretize the fluid and solid variables in the $x$~direction using a uniform
% % grid with spacing $\dx=L/(N_x+1)$. The grid points are given by $x_\ell=\ell\dx$,
% % $\ell=0,1,\ldots,N_x$.  The choice of discrete approximations to the
% % $x$~derivatives in the equations plays little role in the analysis.  Therefore, it is
% % convenient to use a pseudo-spectral approximation by expanding
% % each component $q$ of the solution $(\qv,\qsv)$ in a discrete Fourier series of
% % the form
% % % which gives a formally {\em exact} approximation,  $i\kx$, to an $x$-derivative.
% % % After discretizing in the $x$~direction we will expand the solution in a discrete Fourier series of the form
% % \begin{align}
% %    q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_\ell/L} \qHat_{k}(y,t), \qquad \ell=0,1,2,\ldots,N_x, \label{eq:discreteFourier}
% % \end{align}
% % where $q_\ell(y,t)\approx q(x_\ell,y,t)$ and $\qHat_{k}(y,t)$ are Fourier coefficients, 
% % and where $N_x$ is assumed to be even for convenience.
% % Transforming the governing equations to Fourier space leads to the following equations for the Fourier coefficients of the solution variables:
% % \begin{alignat}{3}
% % &   \rhos \partial_t \vs = i\kx \sigmas_{21} + \partial_y \sigmas_{22} , \quad&& y\in(0,\infty), \label{eq:vEqn} \\
% % &   \partial_t \sigmas_{22} = \rhos \cp^2 \partial_y\vs , \quad&&y\in(0,\infty), \label{eq:s22Eqn} \\
% % &   \partial_t \sigmas_{21} = i\kx \rhos \cp^2 \vs , \quad&&y\in(0,\infty) , \label{eq:s21Eqn} \\
% % & \rho \partial_t v_1 = i\kx      \sigma, \quad &&y\in(-H,0), \label{eq:v1HatEqn} \\
% % & \rho \partial_t v_2 = \partial_y\sigma, \quad && y\in(-H,0), \label{eq:v2HatEqn} \\
% % &  i\kx v_1 + \partial_y v_2 =0 ,                  \quad&&y\in(-H,0) , \label{eq:divHatEqn}
% % \end{alignat}
% % where $\kx = 2\pi k/L$ is a normalized wave number in the $x$~direction and the
% % equations hold for each $k=-N_x/2,-N_x/2+1,\ldots,N_x/2$. The hats on the
% % Fourier coefficients, along with the $k$ subscripts, have been dropped for
% % notational convenience.  Note that the horizontal component of the fluid
% % velocity, $v_1$, is decoupled from the other equations and boundary conditions, 
% % and can be determined once $v_2$ is known. Equations~\eqref{eq:v1HatEqn}--\eqref{eq:divHatEqn} are used to obtain
% % \[
% % \partial_y^2 \sigma - \kx^2 \sigma =0,      \qquad y\in(-H,0) ,
% % \]
% % which is a Laplace equation for pressure (in Fourier space).  The equations for the Fourier coefficients of the solid variables will be discretized using an upwind scheme.  In preparation for this, it is convenient to define the characteristic variables
% % \[
% % a=\sigmas_{22}-\rhos\cp\vs,\qquad b=\sigmas_{22}+\rhos\cp\vs,\qquad d=\sigmas_{21},
% % \]
% % which, from~\eqref{eq:vEqn}--\eqref{eq:s21Eqn}, satisfy
% % \begin{alignat}{3}
% % &   \partial_t a + \cp \partial_y a =  i\kx\cp\, d , \qquad&& y\in(0,\infty),  \label{eq:aHatEqnII}\\
% % &   \partial_t b - \cp \partial_y b = -i\kx\cp\, d , \qquad&& y\in(0,\infty),  \\
% % &   \partial_t d = \frac{i\kx\cp}{2}(b-a) , \qquad&& y\in(0,\infty).  \label{eq:dHatEqnII} 
% % \end{alignat}}
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% The solid variables are discretized in the $y$~direction using a uniform grid with
% spacing $\dy$.  The grid points for the solid domain are defined as $y_j=
% (j-\half)\dy$, $j=0,1,2,\ldots$. 
% Following the analysis in~\cite{BanksSjogreen2011,lrb2013}, the grid is staggered with respect to the
% interface at $y=0$ and has a ghost point at $j=0$; use of a non-staggered grid leads to similar results.
% %  This staggering simplifies the analysis but is not critical {\bf (I'm not convinced of this ?!?!)}.  
% Let  $\dt$ be the time step and let $t^n=n\dt$.  The
% equations~\eqref{eq:aHatEqnII}--\eqref{eq:dHatEqnII} are discretized using the
% first-order upwind scheme,
% \begin{alignat}{3}
% &   \frac{ a_j^{n+1}- a_j^n}{\dt} + \cp\frac{( a_j^n - a_{j-1}^n)}{\dy} =   i\kx\cp\, d_j^{n}, \label{eq:aEqnIII} \\
% &   \frac{ b_j^{n+1}- b_j^n}{\dt} - \cp\frac{( b_{j+1}^n - b_j^n)}{\dy} = - i\kx\cp\, d_j^{n}, \label{eq:bEqnIII} \\
% &   \frac{ d_j^{n+1}- d_j^n}{\dt} = \frac{i\kx\cp}{2}(b_j^{n+1} - a_j^{n+1}), \label{eq:dEqnIII}
% \end{alignat}
% where $a_j^{n}\approx a(y_j,t^n)$, $b_j^{n}\approx b(y_j,t^n)$ and
% $d_j^{n}\approx d(y_j,t^n)$. 
% Since we have used a non-dissipative pseudo-spectral approximation, rather than a two-dimensional upwind scheme, 
% the right-hand side terms in~\eqref{eq:dEqnIII} are taken at time $t^{n+1}$ in order to stabilize the approximation.
% A von Neumann stability analysis of equations~\eqref{eq:aEqnIII} and~\eqref{eq:bEqnIII} (for a
% periodic problem in $y$) shows that this time-stepping scheme is stable under
% reasonable conditions on the constants $\ly=\cp\dt/\dy$ and $\lx=\cp\kx\dt$.
% The fluid variables are kept continuous in $y$ in order to simplify the
% presentation; a discrete version can be introduced but this makes only
% insignificant changes to the fundamental results.  We are thus led to the
% following semi-discrete approximation for the solid and fluid equations,
% \begin{alignat}{3}
% &   a_j^{n+1} = a_j^n -\ly( a_j^n - a_{j-1}^n) - i \lx d_j^{n} , \quad&& j=1,2,3,\ldots\;, \label{eq:aEqn} \\
% &   b_j^{n+1} = b_j^n +\ly( b_{j+1}^n - b_j^n) + i \lx d_j^{n},  \quad&& j=0,1,2,\ldots\;, \label{eq:bEqn}  \\
% &   d_j^{n+1} = d_j^n +  \frac{i\lx}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=0,1,2,\ldots\;,  \\
% % 
% &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0), \\
% &  0=\partial_y^2 \sigma^{n+1}- \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), \label{eq:sigmaEqn}
% \end{alignat}
% where $v^n(y)=v(y,t^n)$ and $\sigma^n(y)=\sigma(y,t^n)$.  For reference, the discrete values for the (Fourier coefficients of the) velocity and components of stress in the solid are related to the characteristic variables by
% \[
% \vs_j^n=\frac{1}{2\zp}(b_j^n-a_j^n),\qquad\sigmas_{22,j}^n=\frac{1}{2}(b_j^n+a_j^n),\qquad \sigmas_{21,j}^n=d_j^n.
% \]
% The conditions at the top and bottom boundaries are 
% \begin{align}
% &   \vert a_j^{n}\vert^2 + \vert b_j^{n}\vert^2 + \vert d_j^{n}\vert^2 \rightarrow 0, 
%          \quad\text{as $j\rightarrow \infty$} ,  \label{eq:BCtop}\\
% &   \sigma^n(-H)=0. \label{eq:BCbottom}
% \end{align}
% Initial conditions are required to define $a_j^{0}$, $b_j^{0}$ and $d_j^{0}$ for $j=0,1,2,3,\ldots$, as well as $v^0(y)$ for  $y\in(-H,0)$, but these conditions are of no significance in the subsequent stability analysis.

% Approximations to the interface conditions are needed to complete the discrete
% formulation of the FSI model problem, and various choices are possible depending
% on the algorithm used.  
% For the AMP algorithm, the pressure Robin
% condition~\eqref{eq:AddedMassPressureBC} is imposed on the fluid; this is derived from the
% outgoing characteristic variables~\eqref{eq:AMPoutgoing}. In addition, the 
% incoming characteristic variable~\eqref{eq:AMPincoming} is used to specify a condition
% on the solid.  The latter condition uses an interface velocity defined
% in~\eqref{eq:ImpedenceWeightedVn} based on an impedance-weighted average.  
% First-order accurate approximations of these conditions are
% \begin{alignat}{3}
% &  \sigma^{n+1}(0) + \frac{\zp\dt}{\rho} \sigma_y^{n+1}(0) = \sigmas_{22,1}^{n+1} + \zp(\vs_1^{n+1} - v^{I,n})
%                                            = b_1^{n+1} -\zp v^{I,n}, && \label{eq:1dSigmaBC}\\
% &  a_0^{n+1} = \sigma^{I,n+1} - \zp v^{I,n+1}, &&\label{eq:1dSolidBC}
% \end{alignat}
% where $\sigma^{I,n}\equiv\sigma^n(0)$ and $v^{I,n}$ are the interface traction and velocity, respectively.  The latter is given by the impedance-weighted average
% \begin{alignat}{3}
% &   v^{I,n+1} = \frac{\zf}{\zf+\zp} v^{n+1}(0) + \frac{\zp}{\zf+\zp}\vs_1^{n+1} + \frac{1}{\zf+\zp}(\sigma_{22,1}^{n+1} - \sigma^{I,n+1} ) && \nonumber\\
% & \hphantom{v^{I,n+1}} = \gamma v^{n+1}(0) + \frac{1-\gamma}{\zp}( b_1^{n+1} - \sigma^{I,n+1} ), && \label{eq:1dVelocityBC}\end{alignat}
% where
% \[
% \gamma=\frac{\zf}{\zf+\zp},
% \]
% and where $\zf$ is a measure of the fluid impedance as introduced in Section~\ref{sec:partitionedAlgorithms}.

% The traditional partitioned (TP) algorithm uses the velocity from the solid as a boundary condition for the fluid and the traction from the fluid as a boundary condition for the solid.  First-order accurate approximations of these conditions are
% \begin{alignat}{3}
%  &   v^{n+1}(0)=\vs_1^{n+1}  
%         , &&   \label{eq:1dTradv} \\
%  &   \sigmas^{n+1}_{22,0} = \sigma^{n+1}(0). &&\label{eq:1dTradsigma}
% \end{alignat}
% It is also instructive to consider an anti-traditional algorithm in which
% the roles of the fluid and solid are reversed in the application of the
% partitioned interface conditions.  Approximations of these conditions are
% \begin{alignat}{3}
% &   \sigma^{n+1}(0) = \sigmas^{n+1}_{22,1}\,,  &&  \label{eq:1dAntiTradsigma} \\
% &   a_0^{n+1} = \sigma^{n+1}(0) - \zp v^{n+1}(0) .&& \label{eq:1dAntiTradv} 
% \end{alignat}
% The condition in~\eqref{eq:1dAntiTradv} is equivalent to setting the velocity of solid at the interface equal to the velocity in the fluid since the stresses have already been equilibrated in~\eqref{eq:1dAntiTradsigma}. 

% % 
% % 
% % % On the interface we assign the out-going characteristic variable by imposing~\eqref{eq:bEqn} at $j=0$.
% % The boundary conditions for the fluid are $\sigma^n(-H)=0$, while the solid solution should decay to zero 
% % as $j\rightarrow\infty$. 
% % The solution for $\sigma^n$ satisfying the boundary condition $\sigma^n(-H)=0$ can be written as
% % \begin{alignat}{3}
% % &  \sigma^{n}= \sigma^{I,n} \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \quad&& y\in(-H,0), 
% % \end{alignat}
% % where $\sigma^{I,n}=\sigma^n(0)$. 



% %- \vskip3\baselineskip
% %- 
% %- 
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- Let $\dt$ be the time step and let $t^n=n\dt$. 
% %- Introduce fully discrete approximations for the solid variables of the form $\qs_j^n \approx \qsHat(y_j,t^n)$ and
% %- semi-discrete approximations for the fluid variables of the form $q^n(y) \approx \qHat(y,t^n)$. 
% %- 
% %- This leads to the approximation
% %- \begin{alignat}{3}
% %- &   a_j^{n+1} = a_j^n -\lambda( a_j^n - a_{j-1}^n) - i \lambdax d_j^{n} , \quad&& j=1,2,3,\ldots \\
% %- &   b_j^{n+1} = b_j^n +\lambda( b_{j+1}^n - b_j^n) + i \lambdax d_j^{n},  \quad&& j=1,2,\ldots  \\
% %- &   d_j^{n+1} = d_j^n + i \frac{\lambdax}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=1,2,\ldots  \\
% %- % 
% %- &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0) \\
% %- &  \partial_y^2 \sigma^{n+1}= \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), 
% %- \end{alignat}
% %- where $\lambday=\frac{\cb\dt}{\dy}$ and $\lambdax=\cb\dt\kx$ and where $a_j^{n}$, $b_j^{n}$ and $d_j^n$
% %- are the characteristic variables in the solid given by 
% %- \begin{alignat}{3}
% %-    a_j^{n} = \sigmas_j^n -\zb \vs_j^n, \quad&& \vs_j^n &=\frac{1}{2\zb}(b_j^n-a_j^n), \\
% %-    b_j^{n} = \sigmas_j^n +\zb \vs_j^n, \quad&& \sigmas_j^n &=\frac{1}{2}(b_j^n+a_j^n), \\
% %-    d_j^n = \sigma^n_{21,j}
% %- \end{alignat}
% %- The boundary conditions for the fluid are $\sigma^n(-H)=0$, while for the solid the solution should remain bounded
% %- as $j\rightarrow\infty$. Initial conditions are needed for $a_j^{0}$, $b_j^{0}$, $d_j^{0}$, $j=0,1,2,3,\ldots$, 
% %- and $v^0(y)$, $y\in(-H,0)$.
% %- Approximations to the interface conditions are needed; various choices for these will be specified later. 
% %- 
% %- 
% %- 
% %- \vskip3\baselineskip
% %- 
% %- Introduce the fully discrete approximations $\vs_{ij}^n \approx \vs(x_i, y_j, t^n)$, 
% %- $\sigmas_{22,ij}^n \approx \sigmas^{22}(x_i, y_j, t^n)$, 
% %- $\sigmas_{21,ij}^n \approx \sigmas^{21}(x_i, y_j, t^n)$, 
% %- in the solid, 
% %- and the semi-discrete approximations $\vv_i^n(y)\approx \vv(x_i,y,t^n)$, $\sigma_i^n(y)\approx \sigma(x_i,y,t^n)$ in the fluid.
% %- We 
% %- expand the solution in a Fourier series in $x$,
% %- \begin{align}
% %-    \vs_{ij}^n = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat_{k,j}^n, \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}


% %- 
% %- 
% %- 
% %- We 
% %- expand the solution in a Fourier series in $x$. 
% %- We introduce the approximations $\vs_j(y,t) \approx \vs(x_j,y,t)$, $\sigma_{22,j}(y,t) \approx \sigmas_{22}(x_j,y,t)$, 
% %- $\sigma_{21,j}(y,t) \approx \sigmas_{21}(x_j,y,t)$, for the solid and 
% %- $\vv_j(y,t) \approx \vv(x_j,y,t)$, and $\sigma_{j}(y,t) \approx \sigma(x_j,y,t)$ for the fluid. 
% %- where 
% %- \begin{align}
% %-    \vs_j(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat(k,y,t), \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}
% %- We let $\kx = 2\pi k/L$ be the normalized wave number.
% %- 
% %- 
% %- 
% %- We discretize the solid in the $y$~direction with a grid spacing $\dy$.
% %- The grid for the solid is defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$. This grid is staggered
% %- with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- simplies the analysis but is not critical.
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- 
% %- % with grid spacing $\dy$ and use 
% %- % a first-order upwind scheme (in the $y$~direction) for the resulting solid equations. 
% %- % The grid for the solid, defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$, is staggered
% %- % with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- % simplies the analysis but is not critical.
% %- 
% %- In the solid we introduce grid functions $\vs_j^n\approx \vsHat(\kx,y_j,t^n)$, etc. 
% %- For the fluid we form approximations that are continuous in $y$ but discerete in time denoted by  
% %- $\sigma^n(y) \approx \sigmaHat(\kx,y,t^n)$,  and 
% %- $v^n(y) \approx \vHat_2(\kx,y,t^n)$. The horizontal component of the fluid velocity, $\vHat_1^n$, plays no role 
% %- in the analysis and can be determined from $v^n(y)$ using  $i\kx \vHat_1^n + \partial_y v^n(y)=0$, if needed.
% %- 
% %- 
% %- 


% % ------------------------------------------------------------------------------------------------
% \subsection{Stability analysis}

% \renewcommand{\aHat}{{\tilde a}}
% \renewcommand{\bHat}{{\tilde b}}
% \renewcommand{\dHat}{{\tilde d}}
% \renewcommand{\vHat}{{\tilde v}}
% \renewcommand{\sigmaHat}{{\tilde\sigma}}
% % \renewcommand{\aTilde}{{\bar a}}
% % \renewcommand{\bTilde}{{\bar b}}
% \renewcommand{\aTilde}{\alpha}
% \renewcommand{\bTilde}{\beta}

% To analyze the stability of the approximation
% in~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn}, we look for solutions of the form \[
% a_j^n=\amp^n\aHat_j, \qquad b_j^n=\amp^n\bHat_j, \qquad d_j^n=\amp^n\dHat_j,
% \qquad v^n(y)=\amp^n\vHat(y), \qquad \sigma^n(y)=\amp^n\sigmaHat(y),
% \] 
% where $\amp\in\Complex$ is the amplification factor,
% $(\aHat_j,\bHat_j,\dHat_j)$ are grid functions, and $(\vHat(y),\sigmaHat(y))$
% are functions for $y\in[-H,0]$. 
%  Substituting these forms
% into~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} results in the following system of
% equations
% \begin{alignat}{3}
% &  \amp \aHat_j = \aHat_j -\ly( \aHat_j - \aHat_{j-1}) - i \lx \dHat_j , \qquad&& j=1,2,3,\ldots\,, \label{eq:aHatEqn} \\
% &  \amp  \bHat_j = \bHat_j +\ly( \bHat_{j+1} - \bHat_j) + i \lx \dHat_j,  \qquad&& j=0,1,2,\ldots\,, \label{eq:bHatEqn}  \\
% &  \amp  \dHat_j = \dHat_j + \frac{i\lx}{2}\amp  ( \bHat_j - \aHat_j),    \qquad&& j=0,1,2,\ldots\,,  \label{eq:dHatEqn} \\
% % 
% &  \amp  \vHat(y) = \vHat(y) + \amp\dt\,\sigmaHat^I\,\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},  \qquad&& y\in[-H,0], \label{eq:vHatEqn} \\
% &  \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \qquad&& y\in[-H,0].\label{eq:sigmaHatEqn}
% \end{alignat}
% To obtain~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn},  the
% ODE in~\eqref{eq:sigmaEqn} was integrated using the boundary conditions $\sigmaHat(-H)=0$
% and $\sigmaHat(0)=\sigmaHat^I$, where the fluid stress at the interface, $\sigmaHat^I$, is as
% yet unspecified.  Note that the solution in the one-dimensional case,
% $\kk=0$, is a special case that can be found by taking the limit $\kk\rightarrow
% 0$ in~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn}. 
% Together with the interface
% conditions, equations~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} define
% a homogeneous set of difference equations. These equations have
% non-trivial solutions (i.e. eigenfunctions) only for particular values of $\amp$ (i.e. eigenvalues).
% The scheme is said to be weakly stable, or stable in the sense of
% Godunov-Ryabenkii, for given values of the parameters $\dt$, $\dy$, $\kx$, $H$, etc., 
% if there are no solutions (i.e.~eigenfunctions) to this
% eigenvalue problem with $\vert \amp\vert>1$. 
% The {\em region of stability} of the scheme is the region in parameter space where there are no roots with $\vert \amp\vert>1$. 
% In order to delineate the stability region 
% it is generally easier to look for regions where the scheme is {\em not} stable. Therefore, we 
% assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % we look for regions in the space of parameters where $\vert \amp\vert>1$  and the scheme is unstable.
% % We thus 
% % assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % If no such solutions exist for some given values of the parameters, then the scheme is (weakly) stable there. 
% % The stability domain is defined to be the region in parameter space where there are no roots with $\amp>1$.


% Equations~\eqref{eq:aHatEqn}--\eqref{eq:dHatEqn} are a system of
% constant-coefficient difference equations for the solid characteristic
% variables.  After solving for $\dHat_j$ from~\eqref{eq:dHatEqn} and substituting
% into~\eqref{eq:aHatEqn} and~\eqref{eq:bHatEqn}, $\aHat_j$ and
% $\bHat_j$ are found to satisfy the recursion
% \begin{equation}
%  \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = K \begin{bmatrix} \aHat_{j-1} \\ \bHat_{j-1} \end{bmatrix}, \qquad K =\begin{bmatrix}  ( 1 - \theta^2)/R & -\theta \\ \theta & R \end{bmatrix} ,
% \label{eq:recursion}
% \end{equation}
% where
% \begin{equation}
% R = r-\theta, \qquad r = \frac{\amp-1+\ly}{\ly}, \qquad \theta = -\frac{\amp\lx^2}{2\ly(\amp-1)} . 
% \label{eq:RandTheta}
% \end{equation}
% The eigenvalues, $\phi_-$ and $\phi_+$, of
% the $2\times2$ matrix $K$ in~\eqref{eq:recursion}
% %  \old{are the roots of a quadratic polynomial, and are given by} 
% are given by
% % \old{
% % We are interested in solutions for $\aHat_j$ and $\bHat_j$ that decay as
% % $j\rightarrow\infty$ so that the boundary condition in~\eqref{eq:BCtop} is
% % satisfied.  This leads us to consider the eigenvalues, $\phi_-$ and $\phi_+$, of
% % the $2\times2$ matrix $K$ in~\eqref{eq:recursion}, which are found by finding
% % the roots of a quadratic polynomial.  The result is
% % }
% \begin{equation}
% \phim = B - \sqrt{ B^2 - 1}, \qquad \phip=1/\phim, \qquad B = \frac{1}{2}\left(R + \frac{1 - \thetaj^2}{R}\right).
% \label{eq:phipm}
% \end{equation}
% Note that the product of the eigenvalues is one.  
% If both eigenvalues 
% % \old{were to have magnitude one} 
% had magnitude equal to one, then there would be no solution of the recursion
% in~\eqref{eq:recursion} satisfying the boundary condition~\eqref{eq:BCtop}.
% Therefore, for a valid solution, there is one eigenvalue (either $\phi_-$ or $\phi_+$),
% denoted by $\phis$ (for {\em small} $\phi$), that has magnitude strictly less
% than one, i.e.~$\vert\phis\vert<1$.  Let $\phib=1/\phis$ (for {\em big} $\phi$)
% be the other eigenvalue with $\vert\phib\vert>1$.  Note that when $\theta=0$,
% $0<\ly\le 1$, and $\vert\amp\vert>1$, then $\phis=\phim=1/r$ (but in general
% $\phis$ is not always equal to $\phim$).  Given that the eigenvalues are
% distinct, $K$ can be diagonalized as 
% \[
% K = S^{-1} \Phi S , \qquad
% \Phi =\begin{bmatrix}  \phis &  0 \\
%                            0 & \phib \end{bmatrix}, \qquad
% S =\begin{bmatrix}  R-\phis & \thetaj \\
%                     R-\phib & \theta \end{bmatrix}.
% \]
% By setting 
% \begin{align}
% &   \begin{bmatrix} \aTilde_j \\ \bTilde_j \end{bmatrix}
%    =  S \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = 
%    \begin{bmatrix} (R-\phis)\aHat_j + \theta \bHat_j \\
%                    (R-\phib)\aHat_j + \theta \bHat_j
%    \end{bmatrix}, \label{eq:abTildeEqn}
% \end{align}
% the general solution of the recursion in~\eqref{eq:recursion} is given by 
% \begin{equation}
% \begin{array}{l}
%    \aTilde_j = \phis^j \aTilde_0, \smallskip\\
%    \bTilde_j = \phib^j \bTilde_0.
% \end{array}
% \label{eq:abBarEqn}
% \end{equation}
% Since the solution must decay to zero as $j\rightarrow \infty$ and since $\vert\phib\vert>1$, it follows that $\bTilde_0=0$ and thus $\bTilde_j=0$ for all $j=0,1,2,\ldots$.  Since $\bTilde_j=0$, it follows from~\eqref{eq:abTildeEqn} that
% \begin{equation}
% \bHat_j = Q \aHat_j,\qquad \aTilde_j=(\phib-\phis)\aHat_j,\qquad Q = \frac{\phib-R}{\theta},
% \label{eq:Qdef}
% \end{equation}
% and thus from~\eqref{eq:abBarEqn}, 
% \[
% \aHat_j=\phi_s^j\aHat_0\,.
% \]
% Whence,
% % ------------------------------------------- PROP -------------------------------------------------
% \begin{proposition}
% Solutions to the system in~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} with $\vert\amp\vert>1$ satisfying the boundary conditions in~\eqref{eq:BCtop} and~\eqref{eq:BCbottom} are given by
% \[
% \begin{array}{c}
% \displaystyle{
% \aHat_j=\phi_s^j\aHat_0,\qquad \bHat_j=Q\aHat_j,\qquad \dHat_j=\frac{i\lx(Q-1)\amp}{2(\amp-1)}\aHat_j,\qquad j=0,1,2,\ldots\,,
% } \bigskip\\
% \displaystyle{
% \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},\qquad \vHat(y)=\sigmaHat^I\,\frac{\amp\dt}{\amp-1}\;\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},\qquad y\in[-H,0],
% }
% \end{array}
% \]
% % \old{where the two free constants, $\aHat_0$ and $\sigmaHat^I$, will be determined by two interface conditions.} 
% where $\aHat_0$ and $\sigmaHat^I$ are free constants.
% \end{proposition}

% The remaining constraints needed to complete the eigenvalue problem, which then determines the amplification factor $\amp$, are provided by two interface conditions.  Choices for these interface conditions are discussed in the subsections below.

% % \bigskip\noindent
% % \textcolor{green}{Note: I have chosen the wording above since the two interface conditions don't actually determine the two free constants, but rather they determine $\amp$ and a relationship between the constants.  I believe the constants would still be arbitrary to within a multiplicative constant.}

% % --------------------------------------------------------------------------------------------------------
% \subsection{AMP interface conditions} 
% Imposing the AMP interface conditions in~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC} with the formula for the interface velocity in~\eqref{eq:1dVelocityBC} gives
% % The AMP Robin boundary condition for $\sigma$ is~\eqref{eq:1dSigmaBC} which gives
% % follows from~\eqref{eq:AddedMassPressureBC}.
% % A first-order approximation is 
% % \begin{align}
% %   \sigma^{n+1} + \frac{\zb\dt}{\rho} \sigma_y^{n+1} &= \sigmas_{22,1}^{n+1} + \zb\vs_1^{n+1} - \zb v^{I,n}
% %                                            = b_1^{n+1} -\zb v^{I,n}, \qquad\text{for $y=0$}, \label{eq:1dSigmaBC}
% % \end{align}
% % where we have introduced the interface velocity $v^{I,n}$.
% % This gives,
% % \begin{align}
% % &  \sigma^{I,n+1} = \eta\Big( b_1^{n+1} - \zb v^{I,n}\Big), \\
% % & v^{I,n+1}  = \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \\
% % &  a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}, 
% % \end{align}
% \begin{align}
% &  \amp\sigmaHat^{I} = \eta\left( \amp\bHat_1 - \zp \vHat^{I}\right), \label{eq:AmpSigmaHat} \\
% &  \aHat_0 = \sigmaHat^{I} - \zp \vHat^{I} , \label{eq:AmpaHat} \\
% &  \vHat^{I}  = \gamma \vHat(0) + \frac{1-\gamma}{\zp}( \bHat_1 - \sigmaHat^{I} ), \label{eq:AmpvHatI}
% \end{align}
% where
% \begin{align*}
%  & \eta \equiv \frac{1}{1 + \frac{\zp\kk\dt}{\rho}\coth(\kk H)}  = \frac{1}{1 + \frac{\rhos\lx}{\rho}\coth(\kk H)}. 
% \end{align*}
% From~\eqref{eq:vHatEqn} and~\eqref{eq:AmpSigmaHat} we also have
% \begin{align}
%   (\amp-1) \vHat(0) = \frac{1-\eta}{\zb}(\amp \bHat_1 - \zb\vHat^I). \label{eq:AmpvHat} 
% \end{align}
% Using $\bHat_1=Q\phis \aHat_0$ to eliminate $\bHat_1$ in terms of $\aHat_0$ and using~\eqref{eq:AmpSigmaHat} to
% eliminate $\sigmaHat^{I}$, equations~\eqref{eq:AmpaHat}, \eqref{eq:AmpvHat} and~\eqref{eq:AmpvHatI} can be written
% in the form 
% %- The interface velocity follows from~\eqref{eq:1dVelocityBC}, giving 
% %- \begin{align}
% %- %    v^{I,n+1} &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( \zb\vs_1^{n+1} + \sigma_{22,1}^{n+1} - \sigma^{I,n+1} ), \\
% %- v^{I,n+1}   &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \label{eq:1dVelocityBCb}
% %- \end{align}
% %- where $\gamma=\zf/(\zf+\zb)$.
% %- For the final interface condition we set the incoming characteristic variable in the solid using the interface
% %- stress and velocity, 
% %- \begin{align}
% %-   a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}. \label{eq:1dSolidBCb}
% %- \end{align}
% % addedMass.mample : 
% % M := Matrix( [ [ A*(1-eta*Q*phim) , 0   , eta+A] , 
% %                [ (1-eta)*A*Q*phim , 1-A , -(1-eta) ], 
% %                [ -(1-g)*(1-eta)*Q*phim    , -g   , 1-(1-g)*eta/A ] ] );
% %
% %-The equations defining the AMP approximation can thus be written in the form
% \begin{align}
% \begin{bmatrix}
%    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
%    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
%   -(1-\gamma)(1-\eta)Q\phis  & -\gamma &  1-(1-\gamma)\eta \amp^{-1} 
% \end{bmatrix} 
% \begin{bmatrix} \aHat_0 \\ \zb \vHat(0) \\ \zb\vHat^I \end{bmatrix} =0 .  \label{eq:AMPmatrix}
% \end{align}
% The determinant of the matrix in~\eqref{eq:AMPmatrix} must be zero for non-trivial solutions to exist, and this leads to the following equation for $\amp$:
% \begin{align*}
% %    \tilde{f(\amp) :=& 
%    \big(\amp-(1-\gamma)\big) \left(\amp-\eta - \big( (2\eta-1)\amp -\eta \big)Q \phis\right) =0.
% \end{align*}
% % For $0\le \gamma\le 2$ the root $A=1-\gamma$ has magnitude less than or equal to one.
% Since $\amp-(1-\gamma)\ne0$ when $\vert\amp\vert>1$ and $0\le \gamma\le 2$, we have the following result.
% % --------------------------------------------------------------------------------------------------
% \begin{theorem} \label{th:amp1d}
% The AMP interface approximation to the
% scheme~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary
% conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, interface
% conditions~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC}, and interface
% velocity~\eqref{eq:1dVelocityBC} is weakly stable if and only if $0\le \gamma\le 2$ and there are no roots $\amp$ with $\vert \amp\vert>1$ to the equation
% \begin{align}
%    f(\amp) \equiv& \amp -\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis =0. \label{eq:fAMP}
% \end{align}
% \end{theorem}
% \noindent Note that $f(\amp)$ does not depend on $\gamma$, i.e.~the weighting in the definition of the interface velocity, and thus the stability of the scheme is independent of $\gamma$ provided $0\le \gamma\le 2$.  From a numerical conditioning point of view, however, we recommend the choice $\gamma=\zf/(\zf+\zp)$ as used in~\eqref{eq:1dVelocityBC}.


% %
% %- 
% %- \begin{align}
% %- &  A \sigma^{I} = \eta\Big( A \bHat_1 - \zb v^{I}\Big), \label{eq:AddedMassSigmaI} \\
% %- % &  \aHat_0 = \sigmasHat_0 - \zb \vsHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- &  \aHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- & (A-1)\vHat(0)= \frac{1-\eta}{\eta\zb} A \sigma^{I}, \\
% %- & v^{I} = \gamma \vHat(0) + (1-\gamma)\frac{1}{\zb}( \bHat_1 - \sigma^{I} )
% %- % &  b^{I,n+1}= b_1^{n+1},  ~~\text{(first order approximations)}, 
% %- \end{align}
% %- Using the expressions for $b_1^n$, etc. 
% %- lead to the conditions
% %- \begin{align}
% %- &  A(1-\eta Q\phis)\aHat_0 + (\eta+A) (\zb\vHat^I) =0 ,   \\
% %- & (A-1)(\zb\vHat(0)) -(1-\eta) A Q \phis \aHat_0 + (1-\eta) (\zb \vHat^I) = 0, \\
% %- & (1 - (1-\gamma)\eta A^{-1}) (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(1-\eta) Q \phis\aHat_0 = 0. 
% %- % & (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(Q-1)\half\phis \aHat_0=0. 
% %- \end{align}
% %- This is an eigenvalue problem for $\amp$. 
% %- Taking the determinant of the associated matrix leads to 
% %- \begin{align}
% %- & f(\amp) \equiv
% %- \det
% %- \begin{bmatrix}
% %-    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
% %-    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
% %-    \half(1-\gamma)(Q-1) \phis  & \gamma & -1 
% %- \end{bmatrix} =0,\\
% %- & f(\amp)=  \amp(1-\eta Q\phis) \Big( 1-\amp +\gamma(1-\eta)\Big) + 
% %-          (\amp+\eta)\phis\Big(  \gamma(1-\eta)\amp Q - \half(1-\amp)(1-\gamma)(Q-1)   \Big) .
% %- \end{align}
% %-The scheme is unstable if there are solutions to $f(\amp)=0$ with $\vert\amp\vert>1$. 
% %-The scheme is said to be (weakly stable) at particular values of $\lambdax,\lambday,\gamma$
% %-if there are no roots with $\vert\amp\vert>1$. Given a choice for $\gamma$ we can plot the
% %-region of stability in the $(\lambdax,\lambday)$ plane. 


% \paragraph{Reduction to a polynomial equation for $\amp$} To examine the stability of the AMP algorithm we must consider all solutions of $f(\amp)=0$.  The function $f(\amp)$ in~\eqref{eq:fAMP} involves square roots of $\amp$ through the eigenvalues, $\phis$ and $\phib$, of the matrix $K$ in~\eqref{eq:recursion} and the definition of $Q$ in~\eqref{eq:Qdef}.  
% To ensure that all possible solutions are found, 
% a polynomial $P(\amp)$ can be derived whose roots include
% all the roots of $f(\amp)$.  To this end, 
% note that from the definition for $Q$ and $\phis\phib=1$ it follows that 
% \begin{align*}
%   Q\phis = \frac{1-R\phis}{\theta}.
% \end{align*}
% Thus $f$ is a linear function of $\phis$ since $f$ only depends on the product $Q\phis$. 
% Note 
% also that $Q\phis$ is a rational function of $\amp$ according the definitions of $R$ and $\theta$ in~\eqref{eq:RandTheta}.  
% Thus, $f(\amp)=0$ can be written in the form
% \begin{align*}
%     \phis = F(\amp) ,
% \end{align*}
% where $F$ is a rational function of $\amp$. 
% Since $\phis$ is equal to one of the two eigenvalues, $\phi_\pm$, defined in~\eqref{eq:phipm}, it follows that 
% \begin{equation}
%   \pm \sqrt{ B^2 - 1} = F(\amp)-B,
% \label{eq:Fratio}
% \end{equation}
% where the sign in front of the square root is chosen to be consistent with $\vert\phis\vert<1$.
% % \old{where the sign in front of the square root is chosen based on the assignment of $\phis$ so that $\vert\phis\vert<1$.}
% Upon squaring both sides of~\eqref{eq:Fratio}, which introduces new roots, one obtains
% %  
% %  Since $\phis$ also satisfies a quadradic equation
% %  with coefficients that are polynomials of $A$, 
% %  \begin{align}
% %   (\amp-1)^2 R \phis^2 - (\amp-1)^2 R B \phis + (\amp-1)^2 R=0,
% %  \end{align}
% % we can eliminate $\phis$ to derive a higher degree polynomial satisfied by $A$,
% \begin{equation}
%    P(\amp)=0,
% \label{eq:PAMP}
% \end{equation}
% where $P(\amp)$ is a polynomial (as described below).  We have thus shown the following:
% \begin{proposition}
%   Any solution of $f(\amp)=0$ is also a root of the polynomial $P(\amp)$. 
% \end{proposition}
% All of the roots of $P(\amp)$ can be found numerically using well-developed
% algorithms (e.g.~solving the eigenvalue problem for the companion matrix).  
% In
% deriving $P(\amp)$, however, new roots have been introduced. Therefore, each
% root $\amp^*$ of $P(\amp)$ must be checked to ensure that it is also solution of
% $f(\amp)=0$.
% % To do this we set $\phis=\phi_-(\amp_0)$ if $\vert\phi_-(\amp_0)\vert<1 $ otherwise we set $\phis=\phi_+(\amp_0)$,
% % and then check that $f(\amp_0)=0$. 
% \begin{proposition}
%   A root, $\amp^*$, of $P(\amp)$ is also a root of $f(\amp)$, if $\phis$ in the definition of $f$ satisfies
% \begin{equation*}
%     \phis = \begin{cases}
%                 \phi_-(\amp^*) & \text{if $\vert\phi_-(\amp^*)\vert<1 $}, \\
%                 \phi_+(\amp^*) & \text{otherwise} ,
%             \end{cases}
% \end{equation*}
% and if $f(\amp^*)=0$.
% \end{proposition}
% % \begin{align}
% %    P(\amp)=0, \quad f(\amp)=0, \quad \vert\phis(\amp)\vert<1. 
% % \end{align}
% % {\bf Scheme 1:} Taking $\gamma=1$ (interface velocity from the fluid), gives (removing a factor of $2\amp$)
% % ff := phim Q A - eta - 2 eta Q phim A + eta Q phim + A
% % 
% \newcommand{\Pamp}{P_{\rm AMP}}
% The polynomial in~\eqref{eq:PAMP} is (after removing uninteresting factors of $\amp-1$) a polynomial of degree 5 given by 
% \[
% \Pamp(\amp)=\alpha_5\amp^5+\alpha_4\amp^4+\alpha_3\amp^3+\alpha_2\amp^2+\alpha_1\amp+\alpha_0,
% \]
% where the coefficients in the polynomial are
% \[
% \begin{array}{l}
% \alpha_0=-\eta^2+2 \eta^2 \ly, \smallskip\\
% \alpha_1=-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2, \smallskip\\
% \alpha_2=10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly, \smallskip\\
% \alpha_3=-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2, \smallskip\\
% \alpha_4=3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2, \smallskip\\
% \alpha_5=-1+2 \eta.
% \end{array}
% \]
% %\begin{align*}
% %%  f_1(\amp) :=&  A-\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis, \\
% % \Pamp(\amp) =&  (-1+2 \eta) A^5+(3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2) A^4+\\
% %&    (-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2) A^3+\\
% %&    (10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly) A^2+(-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2) A\\
% %&    -\eta^2+2 \eta^2 \ly .
% %\end{align*}
% It turns out that $\Pamp(\amp)$ is the same polynomial generated by the Maple symbolic algebra program when asked to solve $f(\amp)=0$.

% To determine if there are any roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$, we
% evaluate the roots numerically for an array of parameter values in the region
% $0<\lx<1.2$, $0<\ly<1.2$ and $0\le \eta \le 1$ with $N_\amp$ equally spaced
% points in each parameter direction.  The stability region of the scheme is the
% region in the space of $(\lx,\ly,\eta)$ where the magnitude of the largest
% valid root satisfies $\vert\amp\vert\le 1$.  This region is computed on a grid with
% $N_\amp=800$ points for each parameter.  In
% Figure~\ref{fig:acousticSolidStokestability}, we plot the curve in the
% $(\lx,\ly)$ plane for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  (The
% curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is also plotted for
% reference.)  Observe that the region of stability contains the region
% $0\le\eta\le1$ and $\lx^2 + \ly^2 \le \kappa^2$
% (for $\lx\ge0$ and $\ly\ge 0$) where the maximum value for $\kappa$ appears to be $\kappa=1$. 
% Further evidence for $\kappa=1$ being the upper bound is provided by the restriction of the analysis to one dimension given below.
% % \old{, where $\kappa$ is a positive constant strictly less than 1.  }
% The curve $\lx^2 + \ly^2 = (.99)^2$
% is shown in the figure as an example.  Since $\lx=\cp\kx\dt$ and $\ly=\cp\dt/\dy$,
% the condition $\lx^2+\ly^2\le 1$ implies the following result.

% % To determine if there are any roots of $\Pamp(\amp)=0$ with $\vert\amp\vert>1$ we evaluate the roots numerically for 
% % values of $\lambda$, $\lambdax$ and $\eta$ in the ranges $0<\lambda<1$, $0<\lambdax<1$, and $0\le \eta \le 1$.
% % We choose $M$ equally spaced values of each of $\lambda$, $\lambdax$ and $\eta$ over their ranges, resulting
% % in finding the roots for $M^3$ points. Using Maple we computed roots with $M=50$ and $M=100$ and using $20$ digits of precision.
% \begin{theorem}
% By numerical evaluation of the stability polynomial, $\Pamp(\amp)$,
% we have found that the AMP algorithm is weakly stable (i.e.~there are no valid roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$) 
% provided $\lx^2+\ly^2\le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{1}{\cp}\left[ \frac{1}{\dy^2} + \kx^2 \right]^{-1/2}. 
%  \end{align*}
% % where $0\le\kappa<1$. 
% This is a sufficient but not a necessary condition. 
% \end{theorem}
% Note that the time step $\dt$ satisfies a typical CFL constraint arising from the fastest wave speed in the solid.
% In the incompressible limit when $\cp \rightarrow \infty$, the maximum stable $\dt$ would go to zero,
% as it would for the solid in isolation. For incompressible solids, alternative formulations should be considered.
% Developing AMP algorithms for incompressible solids is a subject for future work. 

% % \noindent{\bf Note 1:} There are generally four valid roots to $\Pamp(\amp)=0$.
% % Figure~\ref{fig:acousticSolidStokestability} shows a plot of the computed stability region.

% {
% % ---- from codes/cauchy.m  (and cauchy.maple) ----
% \newcommand{\figWidth}{8cm}
% \begin{figure}
% \begin{center}
% %   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP_num50}
%   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP}
%   \caption{Stability region for the two-dimensional model problem using the AMP algorithm.  The curve marked 1 is the curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  The curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is shown for reference.  The dashed curve shows the curve $\lx^2+\ly^2=(.99)^2$.}
%   \label{fig:acousticSolidStokestability}
% \end{center}
% \end{figure}
% }


% % \noindent{\bf Note 2:} The scheme is found to be unstable for $\lambda>1$. Note, however, that the stability bound
% % derived in Section~\ref{} for a periodic strip in $y$ is somewhat more restrictive than the bound found here
% % for the seimi-infinite strip. For example, the periodic strip is unstable for $(\lambda,\lambdax)=(.9,9.)$.

% % {\bf TO-DO: Check the $\eta=0$ limit -- decoupled solid -- we should get von-Neumann stability bound.}

% % --------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% The stability of the one-dimensional version of the AMP algorithm 
% % \old{(described previously in Section~{\bf ?????})}
% may be examined by considering the special case of the two-dimensional algorithm with $\lx=0$ and $Q=0$.  In this case there are two solutions of $f(\amp)=0$ given by
% \begin{align*}
%    \amp = 1-2\ly \qquad\text{or}\qquad \amp =\eta. % \label{eq:fAMP1D}
% \end{align*}
% We are interested in whether there are solutions with $\vert\amp\vert>1$.  Since $0\le \eta\le 1$ we have the result.
% \begin{theorem}
% The one-dimensional AMP algorithm is weakly stable provided  $0\le\gamma\le 2$ and $0 \le \ly \le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{\dy}{\cp}. 
%  \end{align*}
% \end{theorem}

% % \noindent{\bf Note 2:} Even though there are no roots $\vert\amp\vert>1$ to $\Pamp$ for even larger values of $\lambda$ and $\lambdax$,
% %   the orginial scheme should respect the time step restriction from the solid scheme 
% % {\bf But why? Does some assumption go bad? e.g. $\vert\phis\vert<1$?}


% For comparison, we now discuss briefly the corresponding stability results for the scheme given by~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, and with interface conditions given by either the 
% traditional (TP) algorithm or the anti-traditional algorithm.



% % ==========================================================================================================
% \subsection{TP interface conditions} \label{sec:TPanalysis}
% % \newcommand{\Mr}{\Mc}% mass ratio

% The interface conditions for the TP algorithm are given by~\eqref{eq:1dTradv} and~\eqref{eq:1dTradsigma}.  
% Following the previous analysis, $\amp$ is found to satisfy 
% \begin{align}
% &   f_{{\rm TP}}(\amp) \equiv \amp(Q+1) - \frac{\eta-1}{\eta} (\amp-1)(Q-1)\phis =0 . \label{eq:traditionalSchemeF}
% % &   \mr \equiv \frac{\zb\dt\kx}{\rho\tanh(\kx H)} = \frac{\eta-1}{\eta} ...
% \end{align}

% % {\bf TO-DO} The stability region for this scheme is computed numerically and shown in Fig.~\ref{??}.
% % We could plot the stability regions for fixed values of $\eta$ and show that as $\eta\rightarrow 1$ the
% % stability region shrinks to nothing. This shows that as $\dt\rightarrow 0$ ($\eta\rightarrow 1$) the
% % scheme is unstable. 


% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 

% In one dimension, the condition in~\eqref{eq:traditionalSchemeF} reduces to the polynomial equation
% \begin{align*}
% P_{{\rm TP}}(\amp) = \amp^2 + (\Mr + \ly-1) \amp - \Mr = 0, \quad\text{where}~~
%   \Mr = \frac{\rho H}{\rhos \dy}.
% \end{align*}
% (Here, all of the roots of this quadratic are valid since no spurious roots were introduced in deriving the equation.)  The product of the roots is $-\Mr$ and thus a necessary condition for stability is that $\vert \Mr\vert\le 1$.
% Thus the mass of the solid in a thin strip one grid cell wide, $\rhos\dy L$, 
% must be larger than the mass of the entire fluid domain $\rho H L$. 
% Using the theory of von Neumann polynomials~\cite{Miller1971,Strikwerda89} one can show the following necessary and
% sufficient condition.  
% % {\bf (It is a little unclear to me how $\Delta y$ appears.) WDH: Multiply the expression below with $\cp/\dy$ and $\lambda$ and $\Mr$ appear. }
% % ---------------------------------- THEOREM -------------------------------------------------
% \begin{theorem} \label{lemma:traditional}
% The one-dimensional TP algorithm is weakly stable if and only if 
% \begin{align*}
% %      \Mr = \frac{\rho H}{\rhos \dy} <1, \\
%      \dt \le \frac{2}{\cp}\Big( \dy - \frac{\rho H}{\rhos} \Big). 
% %      \lambda < 2(1-\Mr). 
% \end{align*}
% \end{theorem}
% This is a curious result.  For a given {\em large} value of $\dy$ the one-dimensional scheme may be stable, but it will eventually become unstable as the mesh is refined and $\dy$ becomes less than $(\rho H)/\rhos$.  The one-dimensional TP algorithm is thus formally {\em unconditionally unstable}.  
% The numerical results in Section~\ref{sec:travelingWaveResults} show that this behaviour also holds for 
% the second-order accurate discretization of the two-dimensional model problem MP-VE.
% % This behaviour of the traditional scheme is also found to hold in the two-dimensional
% %  since as the mesh is refined eventually $\dy$ will be less than $\frac{\rho H}{\rhos}$. 


% % --------------------------------------------------------------------------------------------------------
% \subsection{Anti-traditional interface conditions} \label{sec:ATPanalysis}

% The interface conditions for the anti-traditional algorithm are given by~\eqref{eq:1dAntiTradsigma} and~\eqref{eq:1dAntiTradv}.  The analysis for this choice leads to the constraint
% %These can be written as 
% %\begin{align*}
% %&  \sigmaHat^I = \sigmasHat_{22,1}= \half(Q+1)\phis\aHat_0, \\
% %&  \aHat_0 = \sigmaHat^I -\zb\Big( \frac{\kk\dt}{\rho}\coth(\kk H)\frac{\amp}{\amp-1} \Big)\sigmaHat^I, 
% %\end{align*}
% % The anti-traditional scheme takes the interface velocity from the fluid and the interface
% % stress from the solid,
% % \begin{align}
% % &   \vHat^I = \vHat(0) = \frac{1-\eta}{\eta}\frac{1}{\zb} \frac{\amp}{\amp-1} \sigmaHat^I, \\
% % &   \sigmaHat^I = \sigmasHat_1 = \half(Q+1) \aHat_0, \\
% % &   \aHat_0 = \sigmaHat^I - \zb \vHat^I = (1- \frac{1-\eta}{\eta}\frac{\amp}{\amp-1}) \half(Q+1) \aHat_0.
% % \end{align}
% % ese interface conditions lead to the eigenvalue equation for $\amp$ of 
% %which leads to the eigenvalue equation for $\amp$ of 
% \begin{align}
% &   f_{{\rm AT}}(\amp) = 1- \amp + \half\left( \frac{2\eta-1}{\eta} \amp -1 \right) (Q+1)\phis=0 .  \label{eq:antiTraditional2d}
% \end{align}

% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% In one dimension, \eqref{eq:antiTraditional2d} reduces to the polynomial constraint
% \begin{align*}
% %      \amp^2 + ( \frac{\lambda}{2\eta} -2)\amp + 1-\frac{\lambda}{2} = 0.  \\
%      P_{{\rm AT}}(\amp) = \amp^2 + \left( \frac{\ly}{2}\left(1+\frac{\ly}{\Mr}\right) -2\right)\amp + 1-\frac{\ly}{2} = 0.  
% %     \amp^2 + (  \frac{\lambda}{2} + \frac{\lambda^2}{2\Mr} -2)\amp + 1-\frac{\lambda}{2} = 0. 
% \end{align*}
% % The anti-traditional scheme is weakly stable in one-dimension if and only if the following conditions
% %  are satisfied (**CHECK ME**)
% %  \begin{align}
% %  &    \lambda < 4, \\
% %  &    \frac{\lambda^2}{2\Mr} < 4-\lambda. 
% %  \end{align}
% %  where $\Mr = \frac{\rho H}{\rhos \dy}$. {\bf TO-DO:} $\Mr$ depends on $\dy$ so we really need to find the condition on $\dt$ in terms of $\dy$.
% An analysis of the roots of $P_{{\rm AT}}(\amp)$ leads us to the following result:
% \begin{theorem}
%   The one-dimensional anti-traditional algorithm is weakly stable if and only if $\ly\le 4$ and 
% % \begin{align}
% % %    \lambda \le \sqrt{ 8\Mr + \Mr^2  } -       \Mr     =       \Mr     \Big( \sqrt{ 1+\frac{8 }{\Mr}} -1 \Big). \\
% %     \half G \dt^2 + \dt < \frac{4\dy}{\cb}, \qquad G=\frac{\rhos\cb}{\rho H}
% % \end{align}
% % or 
% \begin{align}
% %    \dt  < \frac{ \sqrt{1+\frac{8\rhos}{\rho H} \dy} -1 }{G}, \qquad G=\frac{\rhos\cb}{\rho H} . \\
%    \dt  \le \frac{\dy}{\cp}\left( \sqrt{\Mr^2+8\Mr}-\Mr \right).   \label{eq:ATStability}
% \end{align}
% \end{theorem}

% We observe that the one-dimensional anti-traditional scheme is (weakly) stable for any value of the added-mass ratio $\Mr=(\rho H)/(\rhos \dy)$ provided that $\dt$ is taken sufficiently small. 
% The anti-traditional scheme is thus a stable alternative to the AMP scheme. However, in the {\em heavy solid} regime 
% when $\Mr$ is small, the anti-traditional requires a smaller $\dt$ than the AMP scheme, scaling
% like $\sqrt{8\Mr}$ for $\Mr\ll 1$,  as can be seen from~\eqref{eq:ATStability}.



==> texFiles/modelProblems.tex <==
\section{FSI model problems} \label{sec:FSIModelProblems}

We now describe two simplified model problems that are analyzed in 
Sections~\ref{sec:monolithic}, \ref{sec:viscousAnalysis} and~\ref{sec:inviscidAnalysis}.
The first model problem consists of a viscous incompressible fluid and an ``acoustic'' solid
(defined below)
and is the basis for the monolithic scheme analysis in Section~\ref{sec:monolithic}
and viscous analysis in Section~\ref{sec:viscousAnalysis}. 
The second model problem consists of an inviscid, incompressible fluid with an acoustic
solid that is constrained to deform vertically and is used in the 
inviscid analysis described in Section~\ref{sec:inviscidAnalysis}.

\dws{[Aside: My sense is that this paper is really a necessary middle step between FIB and FIBR.
It provides new analysis, thus extending FIB, that is needed for FIBR.  I wonder if this is
useful to state in the Introduction or elsewhere.]}

The geometry of the model problem is shown in Figure
\ref{fig:rectangularModelProblemCartoon}. The fluid 
occupies the region $\Omega$ given by $0 < x < L$
and $0 < y < H$ and the solid occupies the semi-infinite region $\OmegaS$ given by 
$0 < x < L$ and $-\infty < y < 0.$ 
The fluid-solid interface $\Gamma$ is linearized about the flat surface, $y=0$,
and it is assumed that the vertical components of the velocity and stress between the
fluid and solid match along $\Gamma$. 
The solutions for the fluid and solid are assumed to be periodic in the $x$-direction 
with period equal to $L$. 

\input texFiles/rectangularModelProblemCartoon

\medskip
\noindent \textbf{Model Problem MP-VA}. \textit{Model problem MP-VA defines a 
  viscous incompressible fluid and an acoustic solid, where the pressure and shear waves
  propagate at the same speed. It is also assumed that $H\rightarrow \infty.$}
\bse
\begin{align}
&\text{Fluid: } \begin{cases}
\rho \partial_t\vv + \grad p = \mu \Delta \vv, & \xv\in\OmegaF \\
\Delta p = 0, & \xv \in \OmegaF \\
|\vv| \rightarrow 0, & y \rightarrow \infty \\
\grad \cdot \vv = 0, & \xv \in \Gamma
\end{cases},
\qquad
\text{Solid: } \begin{cases}
\rhos \partial_t \vsv = \grad \cdot \sigmasv, & \xv\in\OmegaS \\
\partial_t \sigmasv = -\mus (\grad \cdot \vv) \Iv \\
\phantom{\partial_t \sigmasv =}
+ \mus (\grad \vv + (\grad \vv)^T), & \xv\in\OmegaS \\
\bar{z} |\vsv|^2+|\sigmasv|^2 < \infty, & y\rightarrow - \infty
\end{cases}  \label{eq:mpvaEquations}\\
&\text{Interface: } \begin{cases}
\vv = \vsv, & \xv \in \Gamma\\
\sigmav \nv = \sigmasv \nv, & \xv \in \Gamma
\label{eq:mpvaInterface}
\end{cases}
\end{align}
\ese

We note here that the acoustic solid corresponds to the case of linear elasticity 
when $\lambdas = - \mus$. For this choice, it can be shown that both components of
the displacement satisfy the canonical wave equation with speed $\cb=\sqrt{\mus/\rho}.$
It is useful to write the equations in terms of characteristic variables given by
\begin{align}
\aone = \sigmas_{12} + \bar{z} \vs_1 , \quad
\bone = \sigmas_{12} - \bar{z} \vs_1, \quad
\atwo = \sigmas_{22} + \bar{z} \vs_2, \quad
\btwo = \sigmas_{22} - \bar{z} \vs_2, \quad
d = \sigmas_{11} + \sigmas_{22},
\label{eq:CharDef}
\end{align}
%
where
\begin{align}
\bar{z} = \rhos \bar{c}, \qquad \bar{c} = \sqrt{\mus \over \rhos}. 
\label{eq:solidImpedance}
\end{align}
%
The solid equations reduce to
\bse
\label{eq:advFull}
\begin{alignat}{2}
\partial_t \aone - \bar{c} \partial_y \aone &= \bar{c} (\partial_x d - \partial_x \btwo),
\quad & \xv \in \OmegaS \label{eq:advA1}\\
\partial_t \bone + \bar{c} \partial_y \bone &= \bar{c} (\partial_x \atwo - \partial_x d),
\quad & \xv \in \OmegaS \label{eq:advB1}\\
\partial_t \atwo - \bar{c} \partial_y \atwo &= \bar{c} \partial_x \bone, 
\quad & \xv \in \OmegaS \label{eq:advA2}\\
\partial_t \btwo + \bar{c} \partial_y \btwo &= - \bar{c} \partial_x \aone,
\quad & \xv \in \OmegaS \label{eq:advB2}\\
\partial_t d &= 0,
\quad & \xv \in \OmegaS \label{eq:advD}
\end{alignat}
\ese
%
Equations~\eqref{eq:advA1}--\eqref{eq:advB2} are advection equations for the incoming 
characteristic variables, $\aone$ and $\atwo$,
and the outgoing characteristic variables $\bone$ and $\btwo$, corresponding to the variables defined in equations~\eqref{eq:ACharacteristic}--\eqref{eq:BmCharacteristic} for $\nv=[0,-1]^T$. 
Equation~\eqref{eq:advD} states that that the characteristic $d$ will remain constant 
in time.

\medskip

\noindent \textbf{Model Problem MP-IA}. \textit{Model problem MP-IA defines an 
  inviscid incompressible fluid and an acoustic solid
  that is constrained to deform vertically.
  The fluid pressure
  is taken to be zero along the top boundary, y = H.}
\bse
\begin{align}
&\text{Fluid: } \begin{cases}
\rho \partial_t \vfy + \partial_y p = 0, & \xv\in\OmegaF \\
(\partial_x^2 + \partial_y^2) p =0, & \xv\in\OmegaF \\
p = 0, & y=H
\end{cases} 
\qquad
\text{Solid: } \begin{cases}
\rhos \partial_t \vsy = \partial_x \ssx + \partial_y \ssy, & \xv\in\OmegaS \\
\partial_t \ssx = \rhos\cp^2 \partial_x \vsy, & \xv\in\OmegaS \\
\partial_t \ssy = \rhos\cp^2 \partial_y \vsy, & \xv\in\OmegaS \\
|\vsy|^2+|\ssx|^2+|\ssy|^2 < \infty, & y\rightarrow - \infty
\end{cases}  \label{eq:mpiaEquations}\\
&\text{Interface: } \begin{cases}
\vfy = \vsy, & \xv \in \Gamma \\
p = -\ssy, & \xv\in\Gamma
\label{eq:mpiaInterface}
\end{cases}
\end{align}
\ese

Model problem MP-IA can be derived from MP-VA by taking the fluid viscosity and the
horizontal solid displacement to be zero ($\mu=0$ and $\us_1 = 0$).
We note that the horizontal component of the fluid velocity is omitted from the equations 
for the fluid in~\eqref{eq:mpiaEquations} since it decouples in the simplified FSI problem and 
can be determined from the remaining fluid variables once the solution is known.  
The model problem described here corresponds to the MP-IA model problem considered 
in~\cite{fib2014}.
As in the MP-VA model problem, 
it is useful to define the characteristics variables
\begin{align}
\bc = \ssyh + \zp\vsyh, \qquad
\ac = \ssyh - \zp\vsyh, \qquad
\dc = \ssxh, \label{eq:mpiaTransformation}
\end{align}
and recast the solid equations in~\eqref{eq:mpiaEquations} in the characteristic form
\bse
\begin{alignat}{2}
\partial_t \bc - \cp \partial_y \bc &= \partial_x \cp \dc, \qquad && \xv\in\OmegaS
\label{eq:mpiaAdvSrcB} \\
\partial_t \ac + \cp \partial_y \ac &= -\partial_x \cp \dc, \qquad && \xv\in\OmegaS
\label{eq:mpiaAdvSrcA} \\
\partial_t \dc &= \frac{ \cp}{2} \partial_x (\bc - \ac), \qquad && \xv\in\OmegaS.
\label{eq:mpiaSrcD}
\end{alignat}
\ese
%
As for the case of MP-VA, 
equations~\eqref{eq:mpiaAdvSrcB} and~\eqref{eq:mpiaAdvSrcA} are advection equations for the incoming and outgoing characteristic variables $\bc$ and $\ac$, respectively, corresponding to the variables defined in~\eqref{eq:ACharacteristic} and \eqref{eq:BCharacteristic} for $\nv=[0,-1]^T$. 
Equation~\eqref{eq:mpiaSrcD} describes the evolution of the tangential component of the solid stress.



==> texFiles/monolithic-new.tex <==
\section{Derivation of the fluid impedance} \label{sec:monolithic}

The focus of this section is an analysis of a FSI problem leading to an expression for the fluid
impedance that guides the choice for $\zf$ introduced in~\eqref{eq:fluidImpedanceAlg}.  A value for
the fluid impedance is required in the formulas for the interface projections
in~\eqref{eq:AMPinterfaceVelocity} and~\eqref{eq:AMPinterfaceTraction}, and also for the
implementation of the IMEX fractional-step scheme for the fluid velocity.  The interface projections
were also used in our earlier paper~\cite{fib2014}, as these provide formulas for the interface
velocity and traction that ensure the fluid and solid velocities and tractions match at the
  interface and that smoothly accommodate the limiting cases of light and heavy solids.  In the
earlier paper~\cite{fib2014},
we used a fluid impedance given by $\zf=\rho H/\dt$, where $H$ was a measure of the depth of the fluid layer,
% \old{the height of the fluid layer},
and found that this choice led to a stable AMP algorithm when using an explicit
fractional-step scheme for the fluid. It was also noted that the scheme was quite insensitive to the choice of $H$.
 For the present AMP scheme, we use an IMEX fractional-step
scheme.  Since the viscous terms in the fluid equations are now treated implicitly, the viscous CFL
number, $\Lambda=\nu \dt / h^2$, can be large in which case the choice for $\zf$ used
in~\cite{fib2014} is no longer sufficient for stability.  We have found that the difficulty can be
resolved by considering an analysis of a more general FSI problem for which the viscous terms in the
fluid equations contribute.

\newcommand{\bsp}{b_p}
\newcommand{\bss}{b_s}

Consider the equations for the fluid in the vicinity of a point on the interface,
$\xv=\fluidPoint(t)$.  In two dimensions, we linearize the equations about a flat interface, and let
$x$ measure distance along the interface and $y>0$ be distance normal to the interface.  The point
$\fluidPoint(t)$ corresponds to the origin $x=y=0$ in the local coordinate system.  The advective
terms in the equations vanish at $\fluidPoint(t)$ in the local (moving) system, and are thus neglected in
the analysis.  
Assuming solutions of the form
\wdh{
  wdh: We could maybe start by discussing a fully discrete scheme and then arguing that
  we can simplify by considering the spatially continuous problem. 
  Should we return to defining a horizontal length scale $L$ and a maximum wave number so that
  we have the notion of a grid spacing $h$?
}  
\[
\vv(x,y,t)=\hat{\vv}(y,t)e\sp{ikx},\qquad p(x,y,t)=\hat{p}(y,t)e\sp{ikx},
\]
where $k>0$ is a wave number, the Fourier coefficient functions satisfy
\bse
\label{eq:fourierFull}
\begin{alignat}{2}
\rho \partial_t v_1 + i k p &= \mu (\partial_y^2 - k^2) v_1, \qquad && y>0,\quad t>0,\label{eq:fourierV1}\\
\rho \partial_t v_2 + \partial_y p &= \mu (\partial_y^2 - k^2) v_2, \qquad && y>0,\quad t>0, \label{eq:fourierV2}\\
(\partial_y^2 - k^2) p &= 0, \qquad && y>0,\quad t>0. \label{eq:fourierP}
\end{alignat}
\ese
The hats on the coefficient functions have been dropped for notational convenience.  The equations for the Fourier coefficient functions are now discretized in time.  Define the grid functions $\vv^n(y) \approx \vv(y, t^n)$ and $p^n \approx p(y,t^n)$, where $t^n = n \Delta t$ for a (fixed) time step $\Delta t$. An implicit scheme to advance the solution from $t^n$ to $t^{n+1}$, based on backward-Euler time-stepping, is given by
\bse
\label{eq:backwardEuler}
\begin{alignat}{2}
 \rho \f{v_1^{n+1} - v_1^n}{\dt} + i k p^{n+1} &= \mu (\partial_y^2 - k^2) v_1^{n+1} , \qquad && y>0, \\
 \rho \f{v_2^{n+1} - v_2^n}{\dt} + \partial_y p^{n+1} &= \mu (\partial_y^2 - k^2) v_2^{n+1} , \qquad && y>0, \\
(\partial_y^2 - k^2)  p^{n+1} &= 0, \qquad && y>0.
\end{alignat}
\ese
This system is closed by assuming a bounded solution as $y\rightarrow \infty$ and by specifying boundary conditions at the fluid-solid interface $y=0$.  The boundary conditions at $y=0$, obtained from~\eqref{eq:fluidInterfaceConditions}, take the form
\bse
\label{eq:interfaceNT}
\begin{alignat}{2}
-p^{n+1} + \tau_{22}^{n+1} - \zp v_2^{n+1} &= \bsp^{n+1}, \qquad && y=0,\label{eq:interfaceNormal} \\
\tau_{12}^{n+1} - \zs v_1^{n+1} &= \bss^{n+1}, \qquad && y=0, \label{eq:interfaceTangent}
\end{alignat}
\ese
where $\bsp^{n+1}$ and $\bss^{n+1}$ are, respectively, the normal and tangential components of the outgoing characteristic variables of the solid at $t\sp{n+1}$.
These outgoing solid characteristic variables (defined in the general case by the right-hand-sides of
equations~\eqref{eq:fluidInterfaceConditions}) are assumed given from the solution to the solid equations, using, for example,
an upwind scheme.
The components of the fluid shear stress in~\eqref{eq:interfaceNT} are given by
\begin{align}
\tau_{12}^{n+1} = \mu \left(i k v_2^{n+1} + \partial_y v_1^{n+1} \right),
\qquad
\tau_{22}^{n+1} = 2 \mu \partial_y v_2^{n+1}. 
\end{align}
The implicit scheme in~\eqref{eq:backwardEuler} with boundary conditions in~\eqref{eq:interfaceNT} at $y=0$ and boundedness as $y\rightarrow \infty$ determine the grid functions for the fluid at $t\sp{n+1}$ in terms the fluid velocity at $t\sp n$ and the outgoing solid data $(\bsp^{n+1},\bss^{n+1})$.

\newcommand{\Bsp}{B_p}
\newcommand{\Bss}{B_s}

Consider perturbations in the grid functions of the fluid at $t\sp{n+1}$ for $y>0$ subject to perturbations in the interface data $\bsp^{n+1}$ and $\bss^{n+1}$ at $y=0$.  Define
\begin{align*}
&V_1^{n+1} = v_1^{n+1} + \delta V_1,\qquad
V_2^{n+1} = v_2^{n+1} + \delta V_2,\qquad
P^{n+1} = p^{n+1} + \delta P,\qquad y>0,
\end{align*}
and
\begin{align*}
&\Bsp^{n+1} = \bsp^{n+1} + \delta \Bsp,\qquad
\Bss^{n+1} = \bss^{n+1} + \delta \Bss,
\end{align*}
where $(\delta V_1,\delta V_2,\delta P)$ and $(\delta \Bsp,\delta \Bss)$ are small perturbations.  Assuming the fluid velocity at $t\sp n$ is fixed, the variational equations corresponding to~\eqref{eq:backwardEuler} are 
\bse
\begin{alignat}{2}
 \frac{\rho}{\dt} \delta V_1 + i k \delta P &= \mu (\partial_y^2 - k^2) \delta V_1 , \qquad && y>0, \\
 \frac{\rho}{\dt} \delta V_2 + \partial_y \delta P &= \mu (\partial_y^2 - k^2) \delta V_2 , \qquad && y>0, \\
(\partial_y^2 - k^2)  \delta P &= 0 , \qquad && y>0.
\end{alignat}
\ese
Solution to these equations that remain bounded as $y\rightarrow \infty$ are
\bse
\begin{align}
\delta V_1(y) &= -\frac{1}{i k} \partial_y\delta V_2(y), \\
\delta V_2(y) &= \delta V_0 e^{-\beta y} + \frac{k \dt \delta P_0}{\rho}\left(e^{-k y}-e\sp{-\beta y}\right), \\
\delta P(y) &= \delta P_0 e^{-k y}, 
\end{align}
\ese
where
\[
\delta V_0=\delta V_2(0),\qquad \delta P_0=\delta P(0),\qquad \beta = \left[k\sp2+{\rho\over\mu \dt}\right]\sp{1/2}.
\]
Substituting the solution for the perturbations of the fluid variables into the variational equations~\eqref{eq:interfaceNT}
for the interface conditions leads to the linear system
\begin{align}
\left[\begin{array}{cc}
a_{11} & a_{12} \\
a_{21} & a_{22}
\end{array}\right]
\left[\begin{array}{c}
\delta V_0 \\
\delta P_0
\end{array}\right]
=
\left[\begin{array}{c}
\delta \Bsp \\
\delta \Bss
\end{array}\right],
\label{eq:monolithicBC}
\end{align}
where
\[
\begin{array}{ll}
\displaystyle{
a_{11} = -\mu k\left(2\gamma+\theta_p\right),
}
& \quad
\displaystyle{
a_{12} = -1+2\Lambda\left(\gamma-1\right),
} \medskip\\
\displaystyle{
a_{21} = i\mu k\left(\gamma\sp2+1+\theta_s\gamma\right),
}
& \quad
\displaystyle{
a_{22} = -i\Lambda(\gamma-1)\left(\gamma+1+\theta_s\right).
}
\end{array}
\]
The coefficients $a_{ij}$ in the linear system are defined in terms of the dimensionless parameters
\[
\Lambda=\nu k\sp2 \dt,\qquad \gamma={\beta\over k}=\sqrt{1+{1\over\Lambda}},\qquad \theta_\alpha={\bar z_\alpha\over \mu k},\quad\hbox{$\alpha=p$ or $s$}.
\]
The solution of the linear system
\begin{align}
\delta V_0={a_{22}\delta \Bsp-a_{12}\delta \Bss\over a_{11}a_{22}-a_{12}a_{21}},\qquad \delta P_0={a_{11}\delta \Bss-a_{21}\delta \Bsp\over a_{11}a_{22}-a_{12}a_{21}},
\label{eq:variationalSolution}
\end{align}
determines the variation in the interface values of the fluid velocity and pressure in terms of the variations in the outgoing characteristic variables of the solid.

The AMP algorithm uses impedance-weighted averages to set values for the velocity and pressure at the interface.  For example, the normal component of velocity at the interface is given by~\eqref{eq:AMPinterfaceNormalVelocity}.  In terms of the variational problem, \eqref{eq:AMPinterfaceNormalVelocity} reduces to
\begin{align}
\delta V_0 = -\frac{1}{\zf+\zp} \delta \Bsp,
\end{align}
assuming that the fluid velocity and stress on the right-hand side are held fixed.  In view of the solution in~\eqref{eq:variationalSolution}, we have
\begin{align}
\frac{1}{\zf+\zp} = -{a_{22}\over a_{11}a_{22}-a_{12}a_{21}},
\end{align}
which, after some manipulation, gives
\begin{equation}
z_f=\mu k R,\qquad R=2\gamma+{(\gamma\sp2+\gamma\theta_s+1)(1-2\Lambda(\gamma-1))\over\Lambda(\gamma-1)(\gamma+\theta_s+1)}.
\label{eq:fluidImpedanceFull}
\end{equation}
Of particular interest are the limiting cases when the viscous CFL number, $\Lambda$, is small and large.  A straightforward analysis of the dimensionless parameter $R$ in~\eqref{eq:fluidImpedanceFull} gives
\begin{align}
R \sim
\begin{cases}
\frac{1}{\Lambda}, & \Lambda \rightarrow 0, \\
2, & \Lambda \rightarrow \infty,
\end{cases}
\label{eq:limits}
\end{align}
to leading order.  In view of~\eqref{eq:limits}, we define the relatively simple approximation
\[
\tilde R\eqdef {1\over\Lambda}+2.
\]
The plots in Figure~\ref{fig:Rplot} show that $R/\tilde R\approx1$ over a wide range of values for $\theta_s$, so that the fluid impedance given by
\begin{equation}
\zf=\mu k\tilde R=\mu k\left({1\over\Lambda}+2\right)={\rho\over k\dt}+2\mu k,
\label{eq:fluidImpedance}
\end{equation}
is a good approximation of the more complicated form given in~\eqref{eq:fluidImpedanceFull}.

%The first term in the sum on the right-hand side of~\eqref{eq:fluidImpedance} corresponds the a fluid impedance for an inertial-dominated flow, while the second term is suitable for a viscous-dominated flow.

%We note that the analysis of an inviscid model problem in

\begin{figure}[h]
\begin{center}
\begin{tikzpicture}
  \useasboundingbox (0,.4) rectangle (8.25,5.);  % set the bounding box (so we have less surrounding white space)
    \draw(0,0)  node[anchor=south west] {\includegraphics[width=.5\textwidth]{fig/Rplot.eps}}; 
 % \draw[step=1cm,gray] (0,0) grid (8,5.);
\end{tikzpicture}
\end{center}
\caption{Behavior of the ratio, $R/\tilde R$, versus the viscous CFL number
        $\Lambda$, for $\theta_s=10\sp{-3}$, $5$ and $10\sp3$ showing that
  $\tilde{R}$ is a reasonable approximation to $R$ over a wide range of $\Lambda$ and $\theta_s$.}
\label{fig:Rplot}
\end{figure}

\wdh{\red Notes: $k$ is the wave number in the tangential direction to the boundary so $h$ should be the grid-spacing
  in the tangential direction -- Is this what we do? \dws{Bill: $k$ also provides a scale for the length in the $y$ direction in the exact solution.  So, $h$ could refer to the grid spacing in either $x$ or $y$ I believe.}}

In terms of the AMP algorithm described in Section~\ref{sec:interface}, the analysis here suggests
the fluid impedance given in~\eqref{eq:fluidImpedanceAlg} with $\Cam=1$ and $\Cad=2$, assuming
$k\approx 1/h$ {\red why is this true?} corresponds to the most sensitive Fourier mode.

\wdh{In a discrete approximation of the equations~\eqref{eq:fourierFull}, $k$ would be replaced
  by factors proportional to $1/h$, where $h$ is the grid spacing in the tangential direction. For example, using a
  second-order accurate approximation to the second-derivative in $x$ would lead to $-k^2$ being replaced
  by the factor $-4\sin^2(\xi/2)/h^2$ where $|\xi|\le \pi$. In this case $|k|$ would be effectively bounded
  by $2/h$. Experience shows that instabilities
  are generally caused by high-frequency modes on the mesh (e.g. $\pi/2 \le |\xi|\le \pi$)
  and thus we are led to make the choice $k \approx 1/h$.}

As noted earlier, the analysis
in~\cite{fib2014} suggested the choice $\zf=\rho H/\dt$ based on an analysis of an inviscid model
problem.  This choice corresponds to the form in~\eqref{eq:fluidImpedance} with the second term
omitted, and it works well in practice when $\Lambda$ is small.  However, when $\Lambda$ is large,
which typically occurs for IMEX-type schemes, the choice for $z_f$ based on the first term alone
leads to instability in the AMP scheme since this fluid impedance becomes vanishingly small for
$\Lambda\gg1$.  The stability analyses performed in Sections~\ref{sec:viscousAnalysis}
and~\ref{sec:inviscidAnalysis}, and the numerical results in Section~\ref{sec:numericalResults},
verify that the AMP scheme with the fluid impedance determined from~\eqref{eq:fluidImpedance} gives
stable and accurate solutions for a range of FSI problems involving light and heavy solids.

%The first term in the sum on the right-hand side of~\eqref{eq:fluidImpedance} corresponds the a fluid impedance for an inertial-dominated flow, and this term (for $k\approx 1/H$) agrees with the one obtained in~\cite{fib2014} based on an analysis of an inviscid model problem.
%
%Guided by the local analysis leading to $\zf\approx \mu k\tilde R$ and assuming $k\approx 1/h$ corresponds to the most sensitive Fourier mode, we make the following choice:
%, we choose to adopt a simpler form of the fluid impedance given by
%\begin{equation}
%z_f=\mu k\left({1\over\Lambda}+2\right)={\rho\over k\dt}+2\mu k.
%\end{equation}
%The first term in the sum on the right-hand side of~\eqref{eq:fluidImpedance} corresponds the a fluid impedance for an inertial-dominated flow, and this term (for $k\approx 1/H$) agrees with the one obtained in~\cite{fib2014} based on an analysis of an inviscid model problem.  This choice works well in practice when $\Lambda \ll 1$.  However, when $\Lambda \gg 1$, which typically occurs for IMEX-type schemes, the choice for $z_f$ based on the first term alone leads to instability in the AMP scheme since this fluid impedance becomes vanishingly small in this limit.  The formula in~\eqref{eq:fluidImpedance}, which includes both limiting cases, suggests the constants $\Cam=1$ and $\Cad=2$ in~\eqref{eq:fluidImpedanceAlg} assuming $k\approx 1/h$.  It is found that this is an effective choice for $\zf$ in the AMP scheme.
%

%\newcommand{\zm}{z_\mu}
%
%\begin{figure}[h]
%% \includegraphics[width=.49\textwidth]{fig/eta}
%% \includegraphics[width=.49\textwidth]{fig/etahat}
%\includegraphics[width=.49\textwidth]{fig/etaline}
%\includegraphics[width=.49\textwidth]{fig/etaclose}
%\caption{Left: Line plots as a function of $\Lambda$ 
%  comparing $\eta$ and $\tilde{\eta}$ for multiple values of $Z.$
%  Right: close-up view of the line plots on the left.
%\label{fig:monolithic}}
%\end{figure}


==> texFiles/monolithic.tex <==
\section{\dws{Fluid impedance} \old{Monolithic scheme description and derivation of the fluid impedance, $\zf$}} \label{sec:monolithic}

In this section, the fluid impedance $\zf$ is derived from a model problem analysis of 
the monolithic scheme. Defining the fluid impedance correctly is a critical to the stability
of the AMP algorithm. 
In~\cite{fib2014}, a definition of the fluid impedance was first proposed. 
This definition was discovered to be problematic when the viscous CFL number,
$\Lambda=\nu \dt / h^2$, is too large. 
This parameter typically grows large when the time step is chosen to be proportional to 
the grid spacing ($\dt \propto h$).
In the scheme described in this paper and~\cite{fibr2019}, the viscous terms are treated
implicitly which allows us to choose the time step in this way.
In this section, we derive a fluid impedance which takes into account viscous effects.
The stability of the AMP algorithm for the new definition of $\zf$ is analyzed below in 
Sections \ref{sec:viscousAnalysis} and \ref{sec:inviscidAnalysis}.

Consider the governing equations and geometry of 
model problem MP-VA described in Section~\ref{sec:FSIModelProblems}.
The fluid is taken to be semi-infinite ($H \rightarrow \infty$).
The equations governing the fluid and solid are discretized in the $x$-direction on a 
uniform grid, $x_\ell = \ell \Delta x$ for $\ell = 0, 1,\ldots N_x$, with grid spacing 
$\dx = L/N_x$.  Since the problem is periodic, each variable can be represented as a 
discrete Fourier series
\begin{align}
q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2}  e^{2 \pi i k x_\ell/ L} \hat{q}_k (y,t), 
\qquad \ell=0,1,2,\ldots,N_x. \label{eq:discreteFourier}
\end{align}
%
where $q_\ell(y,t) \approx q(x_\ell,y,t)$ denotes an approximation of a fluid or solid variable and $\hat{q}_k(y,t)$ are the corresponding Fourier coefficients.  For convenience, $N_x$ is assumed to be an even integer.  Taking a discrete Fourier transform of the fluid equations in model problem
MP-VA gives
\bse
\label{eq:fourierFull}
\begin{alignat}{2}
\rho \partial_t v_1 + i k_x p &= \mu (\partial_y^2 - k_x^2) v_1, \qquad && y>0,\quad t>0,\label{eq:fourierV1}\\
\rho \partial_t v_2 + \partial_y p &= \mu (\partial_y^2 - k_x^2) v_2, \qquad && y>0,\quad t>0, \label{eq:fourierV2}\\
(\partial_y^2 - k_x^2) p &= 0, \qquad && y>0,\quad t>0, \label{eq:fourierP}
\end{alignat}
\ese
%
where $k_x = 2 \pi k /L$ is a normalized wave number, and the hats and $k$ subscripts on the Fourier coefficients have been suppressed for notational convenience.
The equations for the fluid Fourier coefficients are now discretized in time.
Define the grid functions $v_1^n(y) \approx v_1(y, t^n)$, $v_2^n \approx v_2(y, t^n)$ 
and $p^n \approx p(y,t^n)$, where $t^n = n \Delta t$ for a (fixed) time step $\Delta t$.
A backward-Euler scheme is used to advance the fluid velocity in time and has the form
\bse
\begin{alignat}{2}
 \rho \f{v_1^{n+1} - v_1^n}{\dt} + i k_x p^{n+1} &= \mu (\partial_y^2 - k_x^2) v_1^{n+1} , \qquad && y>0, \\
 \rho \f{v_2^{n+1} - v_2^n}{\dt} + \partial_y p^{n+1} &= \mu (\partial_y^2 - k_x^2) v_2^{n+1} , \qquad && y>0, \\
(\partial_y^2 - k_x^2)  p^{n+1} &= 0, \qquad && y>0.
\end{alignat}
\ese
%
%This is a system of differential-difference equations. 
This system is closed by enforcing boundedness of the fluid velocity as 
$y\rightarrow \infty$ and boundary conditions at the fluid-solid interface.
Let the Fourier coefficients for the two outgoing solid characteristics 
at time $t^{n+1}$ be $\bone^{n+1}$ and $\btwo^{n+1}$ 
as defined in~\eqref{eq:CharDef}.
At the interface, the matching conditions are
\bse
\begin{alignat}{2}
\tau_{12}^{n+1} - \zb v_1^{n+1} &= \bone^{n+1}, \qquad && y=0, \label{eq:interface1}\\
-p^{n+1} + \tau_{22}^{n+1} - \zb v_2^{n+1} &= \btwo^{n+1}, \qquad && y=0,\label{eq:interface2}
\end{alignat}
\ese
%
where
\begin{align}
\tau_{12}^{n+1} = \mu \left(i k_x v_2^{n+1} + \partial_y v_1^{n+1} \right),
\qquad
\tau_{22}^{n+1} = 2 \mu \partial_y v_2^{n+1}. 
\end{align}
%
The above equations define the solution at the new time in terms of the boundary conditions.

\dws{
Consider perturbations in the fluid variables at $t\sp{n+1}$ for $y>0$ subject to perturbations in the interface data $\bone^{n+1}$ and $\btwo^{n+1}$ at $y=0$, i.e.
\begin{align*}
&V_1^{n+1} = v_1^{n+1} + \delta V_1,\qquad
V_2^{n+1} = v_2^{n+1} + \delta V_2,\qquad
P^{n+1} = p^{n+1} + \delta P,\qquad y>0,
\end{align*}
where
\begin{align*}
&B_1^{n+1} = \bone^{n+1} + \delta B_1,\quad
B_2^{n+1} = \btwo^{n+1} + \delta B_2,\qquad y=0.
\end{align*}
The variational equations for the fluid variables are 
\bse
\begin{alignat}{2}
 \frac{\rho}{\dt} \delta V_1 + i k_x \delta P &= \mu (\partial_y^2 - k_x^2) \delta V_1 , \qquad && y>0, \\
 \frac{\rho}{\dt} \delta V_2 + \partial_y \delta P &= \mu (\partial_y^2 - k_x^2) \delta V_2 , \qquad && y>0, \\
(\partial_y^2 - k_x^2)  \delta P &= 0 , \qquad && y>0.
\end{alignat}
\ese
Bounded solutions as $y\rightarrow \infty$ of the equations are
\bse
\begin{align}
\delta V_1(y) &= -\frac{1}{i k_x} \partial_y\delta V_2(y), \\
\delta V_2(y) &= \delta v^I e^{-\beta y} + \frac{k_x \dt \delta p^I}{\rho}\left(e^{-k_x y}-e\sp{-\beta y}\right), \\
\delta P(y) &= \delta p^I e^{-k_x y}, 
\end{align}
\ese
where
\[
\beta = \left[k_x^2+{\rho\over\mu \dt}\right]\sp{1/2}.
\]
Here, $\delta v^I$ and $\delta p^I$ are perturbations in the vertical component of the velocity and the pressure of the fluid at the interface, respectively.  Substituting the solution for the perturbations of the fluid variables into the variational equations for the interface conditions leads to the linear system
\begin{align}
\left[\begin{array}{cc}
a_{11} & a_{12} \\
a_{21} & a_{22}
\end{array}\right]
\left[\begin{array}{c}
\delta v^I \\
\delta p^I
\end{array}\right]
=
\left[\begin{array}{c}
\delta B_1 \\
\delta B_2
\end{array}\right],
\label{eq:monolithicBC}
\end{align}
where
\begin{equation}
\begin{array}{ll}
\displaystyle{
 a_{11} = i\mu k_x\left(\gamma\sp2+1+\theta\gamma\right),
}
& \quad
\displaystyle{
a_{12} = -i\Lambda(\gamma-1)\left(\gamma+1+\theta\right),
} \medskip\\
\displaystyle{
 a_{21} = -\mu k_x\left(2\gamma+\theta\right),
}
& \quad
\displaystyle{
a_{22} = -1+2\Lambda\left(\gamma-1\right).
}
\end{array}
\label{eq:coeffs}
\end{equation}
The coefficients $a_{ij}$ in the linear system are defined in terms of the dimensionless parameters
\[
\Lambda=\nu k_x\sp2 \dt,\qquad \gamma={\beta\over k_x}=\sqrt{{1\over\Lambda}+1},\qquad \theta={\bar z\over \mu k_x}.
\]
The solution of the linear system
\begin{align}
\delta v^I={a_{22}\delta B_1-a_{12}\delta B_2\over a_{11}a_{22}-a_{12}a_{21}},\qquad \delta p^I={a_{11}\delta B_2-a_{21}\delta B_1\over a_{11}a_{22}-a_{12}a_{21}},
\label{eq:variationalSolution}
\end{align}
determines the variation in the interface values of the fluid velocity and pressure in terms of the variations in the outgoing characteristic variables of the solid.

The AMP algorithm uses impedance-weighted averages to set values for the velocity and pressure at the interface.  For example, the vertical component of velocity is taken to be
\begin{align}
v^I &= \frac{\zf}{\zf + \zb} v_2 + \frac{\zb}{\zf+\zb} \vs_2 
- \frac{1}{\zf + \zb} (\sigmas_{22} - \sigma_{22}),
\label{eq:impavg}
\end{align}
with a similar expression for pressure (stress).  In terms of the variational problem, \eqref{eq:impavg} reduces to
\begin{align}
\delta v^I = -\frac{1}{\zf+\zb} \delta B_2,
\end{align}
assuming that the fluid velocity and stress on the right-hand side are fixed (as they would be given by predicted values in the AMP algorithm).  In view of the solution in~\eqref{eq:variationalSolution}, we have
\begin{align}
\frac{1}{\zf+\zb} = {a_{12}\over a_{11}a_{22}-a_{12}a_{21}}.
\end{align}
Using the coefficients in~\eqref{eq:coeffs}, we find
\begin{equation}
z_f=\mu k_x R,\qquad R=2\gamma+{(\gamma\sp2+\gamma\theta+1)(1-2\Lambda(\gamma-1))\over\Lambda(\gamma-1)(\gamma+\theta+1)}
\label{eq:fluidImpedanceFull}
\end{equation}
Of particular interest are the limiting cases when the viscous CFL number, $\Lambda$, is small and large.  A straightforward analysis of the dimensionless parameter $R$ in~\eqref{eq:fluidImpedanceFull} gives
\begin{align}
R \sim
\begin{cases}
\frac{1}{\Lambda}, & \Lambda \rightarrow 0, \\
2, & \Lambda \rightarrow \infty,
\end{cases}
\label{eq:limits}
\end{align}
to leading order.  Guided by the limiting behavior found in~\eqref{eq:limits}, we choose to adopt a simpler form of the fluid impedance given by
\begin{equation}
z_f=\mu k_x\left({1\over\Lambda}+2\right)={\rho\over k_x\dt}+2\mu k_x.
\label{eq:fluidImpedance}
\end{equation}
The first term in the sum on the right-hand side of~\eqref{eq:fluidImpedance} corresponds the a fluid impedance for an inertial-dominated flow, and this term agrees with the one obtained in~\cite{fib2014} based on an analysis of an inviscid model problem.  This choice works well in practice when $\Lambda \ll 1$.  However, when $\Lambda \gg 1$, which typically occurs for IMEX-type schemes, the choice for $z_f$ based on the first term alone leads to instability in the AMP scheme since this fluid impedance becomes vanishingly small in this limit.  The choice given in~\eqref{eq:fluidImpedance}, which includes both limiting cases, is found to be an effective choice in the AMP scheme.

}


\old{Consider a perturbation of the solution at time $t^{n+1}.$
\begin{align*}
&V_1^{n+1} = v_1^{n+1} + \delta V_1,\quad
V_2^{n+1} = v_2^{n+1} + \delta V_2,\quad
P^{n+1} = p^{n+1} + \delta P,\\
&B_1^{n+1} = (\bone)_I^{n+1} + \delta B_1,\quad
B_2^{n+1} = (\btwo)_I^{n+1} + \delta B_2,
\end{align*}
%
The variational equations for the perturbations are 
\bse
\begin{align}
 \frac{\rho}{\dt} V_1^{n+1} + i k_x P^{n+1} &= \mu (\partial_y^2 - k_x^2) V_1^{n+1} , \\
 \frac{\rho}{\dt} V_2^{n+1} + \partial_y P^{n+1} &= \mu (\partial_y^2 - k_x^2) V_2^{n+1} , \\
(\partial_y^2 - k_x^2)  P^{n+1} &= 0 ,
\end{align}
\ese
%
where $\delta$ is dropped for notational convenience. Similarly the 
interface conditions for the perturbations can be derived from 
equations \eqref{eq:interface1}--\eqref{eq:interface2}.
The solution to the equations for the perturbations and the boundedness condition
as $y\rightarrow \infty$ is given by
\begin{align}
V_1(y) &= -\frac{1}{i k_x} V_2'(y), \qquad
V_2(y) = \left(v_f - \frac{k_x \dt p_f}{\rho} \right) e^{-\beta y} + \frac{k_x \dt p_f}{\rho} e^{-k_x y}, \qquad
P(y) = p_f e^{-k_x y}, 
\end{align}
%
where $\beta^2 = k_x^2+\rho/ (\mu \dt).$
Here, $v_f$ is the vertical component of the velocity at the interface and $p_f$ is the pressure
at the interface. 
Substituting the fluid solution into the boundary conditions 
reveals a linear system of equations for $v_f$ and $p_f$, given by
\begin{align}
\left[\begin{array}{cc}
a_{11}
&
a_{12}
\\
a_{21}
&
a_{22}
\end{array}\right]
\left[\begin{array}{c} v_f \\ p_f \end{array}\right]
=
\left[\begin{array}{c} B_1 \\ B_2 \end{array}\right],
\label{eq:monolithicBC}
\end{align}
% \begin{align}
% \left[\begin{array}{cc}
% -2\gamma\zm - \zb
% &
% -1 + 2 \Lambda (\gamma-1)
% \\
% i\left(\gamma^2 \zm + \gamma \zb + \zm\right)
% &
% -i\Lambda (\gamma-1) ((\gamma+1) \zm + \zb) / \zm
% \end{array}\right]
% \left[\begin{array}{c} v_f \\ p_f \end{array}\right]
% =
% \left[\begin{array}{c} B_1 \\ B_2 \end{array}\right],
% \label{eq:monolithicBC}
% \end{align}
%
where
\newcommand{\zm}{z_\mu}
\newcommand{\zr}{z_\rho}
\begin{alignat*}{2}
&a_{11} = -2\gamma\zm - \zb,
\qquad&&a_{12} = -1 + 2 \Lambda (\gamma-1), \\
&a_{21} =  i\left(\gamma^2 \zm + \gamma \zb + \zm\right),
\qquad&&a_{22} =  -i\Lambda (\gamma-1) ((\gamma+1) \zm + \zb) / \zm.
\end{alignat*}
%
and
\begin{align}
\zm = \mu k_x, 
\qquad
\Lambda = \nu k_x^2 \dt
\qquad
\gamma = \sqrt{\frac{1}{\Lambda}+1},
\end{align}
%
Here, $\zm$ represents an impedance based on the viscous speed of propagation,
$\nu k_x$. The viscous CFL number in the fluid is given by $\Lambda$. The parameter 
$\gamma$ is the ratio of $\beta$ over $k_x.$ 
We are interested in expressing the interface velocity, $v_f$, as an impedance weighted
average in terms of the the predicted fluid velocity $v^{(p)}_2$, 
predicted fluid stress $\sigma_{22}^{(p)}$, solid velocity $\vs_2$, and 
solid stress $\sigmas_{22}.$
\begin{align}
v_f &= \frac{\zf}{\zf + \zb} v^{(p)}_2 + \frac{\zb}{\zf+\zb} \vs_2 
- \frac{1}{\zf + \zb} (\sigmas_{22} - \sigma_{22}^{(p)}) 
\end{align}
%
Let $B_2 =  \sigmas_{22} - \zb \vs_2,$ then
the expression for $v_f$ can be expressed in terms of the solid characteristic.
\begin{align}
v_f &= - \frac{1}{\zf + \zb} \left( \sigma_{22}^{(p)} - \zf v_2^{(p)}\right)
  - \frac{1}{\zf + \zb}\left( \sigmas_{22} - \zb \vs_2 \right)
=- \frac{1}{\zf + \zb} \left( \sigma_{22}^{(p)} - \zf v_2^{(p)}\right)
  - \frac{1}{\zf + \zb} B_2
\end{align}
%
Therefore, we solve for $v_f$ using \eqref{eq:monolithicBC}
and use the coefficient of $B_2$ to derive an estimate for $z_f.$
Using Cramer's rule, the coefficient of $B_2$ is given by
\begin{align}
-\frac{1}{\zf + \zb} = \frac{a_{22}}{a_{11} a_{22} - a_{12} a_{21}}.
\end{align}
%
Therefore, the fluid impedance is given by
\begin{align}
\zf &= -\zb - a_{11} + \frac{a_{12} a_{21}}{a_{22}} 
% &= 2 \gamma \zm + 
% \zm \frac{(\gamma^2 \zm + \gamma \zb + \zm) (1 - 2 \Lambda (\gamma - 1)  )}
% {\Lambda (\gamma - 1) ((\gamma + 1) \zm + \zb) }
\end{align}
%
Let $Z = \zm / \zb$ be the ratio of the viscous impedance and solid impedance.
This leads to the fluid impedance $\zf$ being of the form
\begin{align}
  \zf = \zm\; \eta, \qquad
\eta =  2 \gamma 
+ \frac{\gamma^2 + \gamma Z^{-1} + 1}
        {\Lambda (\gamma-1) ((\gamma+1) + Z^{-1})} 
\left(1 - 2 \Lambda (\gamma-1) \right).
\end{align}
%
That is, the fluid impedance is twice the viscous impedance times a scale factor
$\eta$ which depends solely on $\Lambda$ and $Z$. A simpler expression for 
$\eta$ can be developed by looking at the asymptotic behavior of $\eta$
as $\Lambda\rightarrow (0,\infty).$ 
Observe that for large $\Lambda,$ $\gamma\sim 1$ and for small $\Lambda,$
$\gamma\sim \Lambda^{-1/2}.$ 
To leading order, the asymptotic behavior of $\eta$ is given by
\begin{align}
\eta \sim
\begin{cases}
2, & \Lambda \rightarrow \infty \\
\frac{1}{\Lambda}, & \Lambda \rightarrow 0
\end{cases}.
\end{align}
%
We introduce $\tilde{z}_f = \zm\; \tilde{\eta}$ which is an approximation that is
asymptotically equivalent to $\zf$, given by
\begin{align}
\tilde{z}_f = \zm \left( 2 + \frac{1}{\Lambda} \right)
= 2 \mu k_x + \frac{\rho}{k_x \dt}.
\end{align}
%
The fluid impedance therefore is the sum of a viscous impedance and an inviscid impedance.
The inviscid impedance, $\rho / (k_x \dt),$ was used in the AMP scheme described in~\cite{fib2014}.
This choice works well in practice when $\Lambda \ll 1.$ However, when $\Lambda \gg 1,$
which typically occurs for IMEX-type schemes, the inviscid impedance vanishes while 
the true fluid impedance approaches $2 \zm.$
In Figure \ref{fig:monolithic}, line plots of $\tilde{\eta}$ and $\eta$ as a function of 
$\Lambda$ are shown. There is good agreement between $\tilde{\eta}$ and $\eta.$ 
Additionally, the correct asymptotic behavior is observed.
}  % end OLD

\newcommand{\zm}{z_\mu}

\begin{figure}[h]
% \includegraphics[width=.49\textwidth]{fig/eta}
% \includegraphics[width=.49\textwidth]{fig/etahat}
\includegraphics[width=.49\textwidth]{fig/etaline}
\includegraphics[width=.49\textwidth]{fig/etaclose}
\caption{Left: Line plots as a function of $\Lambda$ 
  comparing $\eta$ and $\tilde{\eta}$ for multiple values of $Z.$
  Right: close-up view of the line plots on the left.
\label{fig:monolithic}}
\end{figure}


==> texFiles/numericalResults-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO:
% - convert figures to latex tables
% - steady state runs
% - plots for cases


\section{Numerical results} \label{sec:numericalResults}


\das{Using Matlab results.}
We now present numerical results for various simulations to 
verify the order of accuracy and demonstrate the robustness of the AMP scheme.
Exact solutions for several FSI benchmark problems are presented, and these solutions are used to verify the stability and accuracy of the AMP algorithm for a range of the problem parameters.

\input texFiles/rectangularGeometryNumericalResults

\subsection{Longitudinal motion of a one-dimensional elastic piston}\label{sec:elasticPistonSolution}

The geometry of the one-dimensional elastic piston problem is shown in Figure~\ref{fig:rectangularModelProblemNumericalResults}.  The plot on the left shows the configuration at $t=0$.  The fluid occupies the physical domain between $y=0$ and $y=H$ initially, while the solid lies in its reference domain between $\ys=-\Hs$ and $\ys=0$.  It is assumed that there is no dependence in the $x$-direction so that the fluid-solid interface remains flat at a position $y=y_I(t)$ as shown in the plot on the right.  In the fluid domain, $\Omega(t)$, it is assumed that the horizontal component of velocity $v_1$ is zero, and thus the vertical component $v_2$ is a function of $t$ alone according to the continuity equation.  The fluid pressure is a linear function $y$, and is given by
\begin{equation}
p(y,t)={(H-y)p_I(t)+(y-y_I(t))p_H(t)\over H-y_I(t)},
\label{eq:oneDimFluidPressure}
\end{equation}
where $p_I(t)$ is the pressure on the interface and $p_H(t)$ is a specified fluid pressure at $y=H$.  The momentum equation for the fluid in the vertical direction reduces to
\begin{equation}
\rho \dot{v}_2=-p_y={p_I(t)-p_H(t)\over H-y_I(t)},
\label{eq:oneDimFluidMom}
\end{equation}
where $\rho$ is the (constant) fluid density.

With the displacement of the solid in the horizontal direction assumed to be zero, the equation for the vertical component of the displacement in the reference domain, $\bar\Omega(0)$, becomes
\begin{equation}
\us_{2,tt} = \cp^2 \us_{2,\ys\ys},\qquad -\Hs<\ys<0,
\label{eq:oneDimWaveEquation}
\end{equation}
where $\cp$ is the longitudinal wave speed.  The general solution of~\eqref{eq:oneDimWaveEquation}, assuming a zero-displacement condition at $\ys=-\Hs$, is
\begin{equation}
\us_2(\ys,t) = \bar F(t - (\ys+\Hs)/\cp ) -  \bar F(t + (\ys+\Hs)/\cp),
\label{eq:oneDimSolidDisplacement}
\end{equation}
where $\bar F(\bar\tau)$ is any smooth function.  The vertical position of the fluid-solid interface is determined by the solid displacement evaluated at $\ys=0$.  Thus,
\begin{equation}
y_I(t)=\us_2(0,t),
\label{eq:oneDimInterface}
\end{equation}
and the matching conditions on velocity and stress imply
\begin{equation}
v_2(t) = \us_{2,t}(0,t),\qquad -p_I(t)=(\lambdas + 2 \mus) \us_{2,\bar{y}}(0,t).
\label{eq:oneDimMatching}
\end{equation}
The interface conditions in~\eqref{eq:oneDimInterface} and~\eqref{eq:oneDimMatching} can be used in~\eqref{eq:oneDimFluidMom} to eliminate the fluid variables, which leads to a boundary condition involving the solid displacement and its derivatives.  This boundary condition can be written in the form
\begin{equation}
\rho\bigl(H-\us_2(0,t)\bigr)\us_{2,tt}(0,t)+(\lambdas + 2 \mus) \us_{2,\bar{y}}(0,t)=-p_H(t).
\label{eq:oneDimSolidBC}
\end{equation}

In principle, a function $\bar F(\bar\tau)$ in~\eqref{eq:oneDimSolidDisplacement} could be found so that $\us_2(\ys,t)$ satisfies some given initial conditions on $\us_2$ and $\us_{2,t}$, and the nonlinear boundary condition in~\eqref{eq:oneDimSolidBC} for a specified fluid pressure $p_H(t)$, but this would be difficult in general.  Alternatively, an exact solution can be constructed by making a choice for $\bar F(\bar\tau)$, and then backing out the corresponding initial conditions on $\us_2(\ys,t)$ and the fluid pressure $p_H(t)$.  This is done in our verification tests using the choice
\[
\bar F(\bar\tau)=\alpha\cos(\omega\bar\tau),
\]
where $\alpha$ and $\omega$ are parameters.  With $\us_2(\ys,t)$ and $p_H(t)$ known from~\eqref{eq:oneDimSolidDisplacement} and~\eqref{eq:oneDimSolidBC}, respectively, the remaining fluid variables can be obtained from~\eqref{eq:oneDimFluidPressure}, \eqref{eq:oneDimInterface} and~\eqref{eq:oneDimMatching}.  In particular, we note that for this choice, the position of the fluid-solid interface oscillates with frequency $\omega$ and an amplitude $a$ given by
\[
y_I(t)=a\sin(\omega t),\qquad a=2\alpha\sin(\omega\Hs/\cp).
\]

Numerical results are obtained for the case $H=1, \rho=1,$ and $\mu=0.01$ for the fluid, 
$\Hs=0.5$ and $\mus=\lambdas=\rhos=\delta$ for the solid, 
and $a=0.1$ and $\omega=2\pi$ for the interface position. 
The density ratio, $\rhos/\rho = \delta$, is taken to be $10\sp{-3}$, 1 and $10\sp3$, 
representing FSI problems with light, moderate and heavy solids, respectively.  
Numerical solutions are computed using the AMP algorithm on a two-dimensional rectangular 
configuration (as shown in Figure~\ref{fig:rectangularModelProblemNumericalResults}) with 
periodic boundary conditions taken at $x=0$ and $x=L$ consistent with a one-dimensional solution.  
The composite grid for the calculations 
consists of ... (describe only, no figure needed in my view).  
Table~\ref{fig:ElasticPistonConvergence} gives the maximum-norm errors for solutions computed 
using the AMP algorithm to $t_{{\rm final}}=0.3$ with grid resolutions $h = (2)^{-j}/10,$ for
$j=1,2,3,4.$  
The coarsest grid configuration is shown in Figure \ref{fig:elasticPistonGrid}.
The errors in Table \ref{fig:ElasticPistonConvergence} indicate that the solution is 
converging at second order accuracy.
The solution is plotted in Figure \ref{fig:elasticPistonPlot}.

\input tables/ElasticPistonConvergence.tex

{
\begin{figure}[h]
\centering
\includegraphics[width=.5\textwidth]{fig/ElasticPistonGrid}
\caption{Grid for the elastic piston and elastic shear solution.
  \label{fig:elasticPistonGrid}}
\end{figure}
}
{
\begin{figure}
\includegraphics[width=.49\textwidth]{fig/ElasticPiston_delta1_tf0p3_s22}
\includegraphics[width=.49\textwidth]{fig/ElasticPiston_delta1_tf0p3_v2}
\caption{Shaded contours of the numerical solution for
  $(\sigma_{22},\sigmas_{22})$ on the left and $(v_2,\vs_2)$ on the right at 
  $t=0.3.$ for $\delta = 1.$ \label{fig:elasticPistonPlot}}
\end{figure}
}


%{% ------ GRIDS ------  
%%
%\newcommand{\Gcep}{\Gv_{\rm ep}}
%\newcommand{\figWidth}{6cm}% height 
%\newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.225}{.225}{.09}{.09}}
%\begin{figure}[htb]
%\begin{center}
%\begin{tikzpicture}[scale=1]
%  \useasboundingbox (0,0.5) rectangle (16,6);  % set the bounding box (so we have less surrounding white space)
%
%   \draw( 0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/elasticPistonGrid}{\figWidth}};
%% 
%   \draw( 5.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/pistonG4stress0p7}{\figWidth}};
%   \draw(10.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/pistonG4stress0p8}{\figWidth}};
%   % grid:
%% \draw[step=1cm,gray] (0,0) grid (16,6);
%\end{tikzpicture}
%\end{center}
%  \caption{Composite grid $\Gcep^{(2)}$ for an elastic piston adjacent to a fluid channel. 
%    The green fluid grid adjacent to the piston moves over time. The blue fluid background grid remains fixed.
%    The red grid for the solid reference domain also remains fixed over time.
%   Middle and right: pressure and $\sigma_{22}$. 
%}
%\label{fig:elasticPistonGrid}
%\end{figure}
%}

% is this figure necessary?
\input texFiles/rectangularGeometryShearSolution


\subsection{Transverse motion of a one-dimensional elastic piston}\label{sec:elasticPistonShearSolution}

Exact solutions can also be constructed for an FSI problem involving transverse motion of a one-dimensional elastic piston.  For this case, the vertical components of the fluid velocity and solid displacement are taken to be zero, while the corresponding horizontal components are assumed to be functions of $y$ and $t$ alone.  As a result, the interface remains in its initial position, $y_I(t) = y_I(0) = 0$, and so the solid reference coordinate $\ys$ is equivalent to the physical coordinate $y$.  The equations governing the horizontal components of the fluid velocity and solid displacement reduce to
\begin{equation}
v_{1,t} = \nu v_{1,yy}, \qquad 0<y<H, 
\label{eq:oneDimTransFluid}
\end{equation}
and
\begin{equation}
\us_{1,tt} = \cs^2 \us_{1,yy}, \qquad -\Hs<y<0, 
\label{eq:oneDimTransSolid}
\end{equation}
respectively, where $\nu=\mu/\rho$ is the kinematic viscosity of the fluid and $\cs$ is shear wave speed of the solid.  Solutions of~\eqref{eq:oneDimTransFluid} and~\eqref{eq:oneDimTransSolid} are sought in the form
\begin{equation}
v_1(y,t) = \hat{v}_1(y) e^{i \omega t}, \qquad \us_1(y,t) = \hat{\us}_1(y) e^{i \omega t},
\label{eq:oneDimTransSolutions}
\end{equation}
where $\omega$ is a parameter (ultimately an eigenvalue).  The coefficient functions, $\hat{v}_1(y)$ and $\hat{\us}_1(y)$, in~\eqref{eq:oneDimTransSolutions} satisfy
\begin{equation}
\hat{v}_1'' + \lambda^2 \hat{v}_1 = 0,\qquad \hat{\us}_1'' + k_s^2 \hat{\us}_1 = 0,
\label{eq:oneDimTransHelmholtz}
\end{equation}
where
\begin{equation}
\lambda^2 = - \frac{i \omega}{\nu}, \qquad k_s^2 = \frac{\omega^2}{\cs^2}.
\label{eq:oneDimTransParams}
\end{equation}
Solutions of the second-order ODEs in~\eqref{eq:oneDimTransHelmholtz} satisfying a no-slip condition in the fluid at $y=H$ and a zero-displacement condition in the solid at $y=-\Hs$ are
\begin{equation}
\hat{v}_1(y) =  b \sin(\lambda (H-y)),\qquad \hat{\us}_1(y) = \bar{b}\sin(k_s (\Hs+y)),
\label{eq:oneDimTransHelmholtzSolutions}
\end{equation}
where $(b,\bar{b})$ are constants.  The interface matching conditions on velocity and shear stress imply
\begin{equation}
\hat{v}_1(0) = i\omega\hat{\us}_1(0),  \qquad \mu \hat{v}_1'(0) = \mus \hat{\us}_1'(0).
\label{eq:oneDimTransMatching}
\end{equation}
Using~\eqref{eq:oneDimTransHelmholtzSolutions} in~\eqref{eq:oneDimTransMatching} leads to the system
\begin{equation}
\left[\begin{array}{cc}
\sin(\lambda H) & -i \omega \sin(k_s \Hs) \smallskip\\
\mu \lambda  \cos(\lambda H) & \mus k_s \cos(k_s \Hs)
\end{array}\right]
\left[\begin{array}{c}
b \smallskip\\ \bar{b}
\end{array}\right]
= 0 .
\label{eq:oneDimTransSystem}
\end{equation}
Nontrivial solutions for $(b,\bar{b})$ exist if the determinant of the coefficient matrix in~\eqref{eq:oneDimTransSystem} is zero, which implies
\begin{equation}
\mathcal{D}(\omega)=\frac{\mus}{\mu \omega} \tan(\lambda H) +  \frac{i \lambda}{k_s} \tan(k_s \Hs) = 0.
\label{eq:oneDimTransConstraint}
\end{equation}

What about the fluid pressure?  I am thinking that it would be constant.  Yes?  And we should mention that we use the real part of~\eqref{eq:oneDimTransSolutions} as solutions.

Values of $\omega$ with $\Re(\omega) > 0$ satisfying $\mathcal{D}(\omega)=0$ correspond to solutions of the transverse elastic piston problem that decay in time.  Selected values of $\omega$ for $H=??$, $\Hs=??$, $\nu=??$, $\cs=??$ and $\Re(\us_1(0,0)) = \us_0=???$ are listed in Table~?? for different values of $\delta=\rhos/\rho$.  (In the table, list $\delta$, real and imaginary parts of $\omega$, $b$ and $\bar{b}$.)  


This solution is tested with the AMP code. 
{
\begin{table}[h]
\caption{\label{fig:ElasticShearFrequencies}
Selected solutions to the dispersion relation in equation 
\eqref{eq:ShearSolutionDispersionRelation} used to test the numerical solution.
The parameters were chosen to be $\Hs = \frac{1}{2}, H = 1, \cs = 1, \rho = 1$.}
\begin{center}
\begin{tabular}{ccc}
\hline
$\mus$ & $\mu$ & $\omega$ \\
\hline
$10^{-3}$ & $10^{-4}$ & $0.296+0.169i$ \\
$10^{-2}$ & $10^{-3}$ & $0.637+0.347i$ \\
$10^{-1}$ & $10^{-2}$ & $1.344+0.597i$ \\
$10^{0}$ & $10^{0}$ & $1.646+0.993i$ \\
$10^{1}$ & $10^{1}$ & $2.370+2.742i$ \\
$10^{2}$ & $10^{2}$ & $2.626+4.702i$ \\
$10^{3}$ & $10^{3}$ & $2.752+6.716i$ \\
\hline
\end{tabular}
\end{center}
\end{table}
}

\input tables/ShearSolutionConvergence.tex

% {% ------ GRIDS ------  
% %
% \newcommand{\Gcep}{\Gv_{\rm ep}}
% \newcommand{\figWidth}{6cm}% height 
% \newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.225}{.225}{.09}{.09}}
% \begin{figure}[htb]
% \begin{center}
% \begin{tikzpicture}[scale=1]
%   \useasboundingbox (0,0.5) rectangle (16,6);  % set the bounding box (so we have less surrounding white space)

%    \draw( 0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/elasticPistonGrid}{\figWidth}};
% % 
%    \draw( 5.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/pistonG4stress0p7}{\figWidth}};
%    \draw(10.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/pistonG4stress0p8}{\figWidth}};
%    % grid:
% % \draw[step=1cm,gray] (0,0) grid (16,6);
% \end{tikzpicture}
% \end{center}
% \caption{\das{Placeholder for shear solution figures}
% }
% \label{fig:elasticPistonGrid}
% \end{figure}
% }



==> texFiles/viscousAnalysis.tex <==
\section{Stability analysis of a viscous model problem} \label{sec:viscousAnalysis}

The stability analysis of the AMP algorithm in~\cite{fib2014} is extended in two directions
in this paper. A first-order accurate discretization of a 
viscous model problem is explored in this section
and a second-order accurate discretization of an inviscid model problem 
is explored in Section~\ref{sec:inviscidAnalysis}.
Analyzing stability when viscosity is involved is challenging since instabilities 
arise from both added mass and added damping effects.
Due to this, both horizontal and vertical motions in the solid must be considered.
This relaxes the assumption in~\cite{fib2014} where the model problem was constrained 
to vertical motions only.
Another difficulty is the introduction of the fluid viscous CFL number as a 
new dimensionless parameter. 
In Section~\ref{sec:monolithic}, a fluid impedance was derived which is a function of 
the viscous CFL number. This impedance is used in the interface projection step of the 
AMP algorithm and is critical to achieving stability.

We will compare the stability of the AMP scheme to that of the traditional partitioned (TP)
scheme and the anti-traditional partitioned (ATP) scheme. 
In the TP scheme, the solid provides a Dirichlet (no-slip)
boundary condition for the fluid, and then the fluid supplies a Neumann (traction) 
boundary condition for the solid. 
The ATP scheme reverses the role of the solid and fluid. 
In this scheme, the solid provides a Neumann (traction) boundary condition for the fluid
and the fluid supplies a Dirichlet (no-slip) boundary condition for the solid.

% In this section, the stability of the AMP, TP, and ATP algorithms 
% are explored for a viscous model problem.
% This extends the analysis of the inviscid model problem in~\cite{fib2014} to 
% a viscous model problem. 
% When viscosity is involved, stability is more challenging since instabilities 
% arise from both added mass and added damping effects.
% Due to this, both horizontal and vertical motions in the solid must be considered.
% This relaxes the assumption in~\cite{fib2014} where the model problem was constrained 
% to vertical motions only.
% Another difficulty is the introduction of the viscous CFL number in the fluid as a 
% new dimensionless parameter. 
% In Section~\ref{sec:monolithic}, a fluid impedance was derived which is a function of 
% the viscous CFL number. This impedance is used in the interface projection step of the 
% AMP algorithm and is critical to achieving stability.

\subsection{Viscous model problem}

% \dws{Consider model problem MP-VA described in Section~\ref{sec:FSIModelProblems} and illustrated in Figure~\ref{fig:rectangularModelProblemCartoon} with $H \rightarrow \infty$.}
% \old{Consider model problem MP-VA described in Section~\ref{sec:FSIModelProblems}. }


The geometry of the model problem is shown in Figure~\ref{fig:rectangularModelProblemCartoonInfinite}. 
Consider a viscous incompressible Stokes fluid in the semi-infinite rectangular region
$\Omega$ defined by $0<x<L$ and $0<y<\infty$ 
and an acoustic solid in the semi-infinite rectangular region $\OmegaS$ given by 
$0<x<L$ and $-\infty <y<0.$
The fluid-solid interface $\Gamma$ is linearized about the flat surface, $y=0$,
and it is assumed that the velocity and traction between the fluid and solid match 
along $\Gamma$. The solutions for the fluid and solid are assumed to be periodic in 
the $x$-direction with period equal to $L$. 
The governing equations for the FSI model problem are
\bse
\begin{align}
&\text{Fluid: } \begin{cases}
\rho \partial_t\vv + \grad p = \mu \Delta \vv, & \xv\in\OmegaF \\
\Delta p = 0, & \xv \in \OmegaF \\
|\vv| \rightarrow 0, & y \rightarrow \infty \\
\grad \cdot \vv = 0, & \xv \in \Gamma
\end{cases},
\qquad
\text{Solid: } \begin{cases}
\rhos \partial_t \vsv = \grad \cdot \sigmasv, & \xv\in\OmegaS \\
\partial_t \sigmasv = -\mus (\grad \cdot \vv) \Iv \\
\phantom{\partial_t \sigmasv =}
+ \mus (\grad \vv + (\grad \vv)^T), & \xv\in\OmegaS \\
|\vsv|,|\sigmasv| < \infty, & y\rightarrow - \infty
\end{cases}  \label{eq:mpvaEquations}\\
&\text{Interface: } \begin{cases}
\vv = \vsv, & \xv \in \Gamma\\
\sigmav \nv = \sigmasv \nv, & \xv \in \Gamma
\label{eq:mpvaInterface}
\end{cases}
\end{align}
\ese

\input texFiles/rectangularModelProblemCartoonInfinite

We note here that the acoustic solid corresponds to the case of linear elasticity 
when $\lambdas = - \mus$. For this choice, it can be shown that both components of
the displacement satisfy the canonical wave equation with speed $\cb=\sqrt{\mus/\rhos}.$
It is useful to write the equations in terms of characteristic variables given by
\begin{align}
\aone = \sigmas_{12} + \bar{z} \vs_1 , \quad
\bone = \sigmas_{12} - \bar{z} \vs_1, \quad
\atwo = \sigmas_{22} + \bar{z} \vs_2, \quad
\btwo = \sigmas_{22} - \bar{z} \vs_2, \quad
d = \sigmas_{11} + \sigmas_{22},
\label{eq:CharDef}
\end{align}
%
where $\bar{z}= \rhos \bar{c}$ is the solid impedance.
The solid equations reduce to
\bse
\label{eq:advFull}
\begin{alignat}{2}
\partial_t \aone - \bar{c} \partial_y \aone &= \bar{c} (\partial_x d - \partial_x \btwo),
\quad & \xv \in \OmegaS \label{eq:advA1}\\
\partial_t \bone + \bar{c} \partial_y \bone &= \bar{c} (\partial_x \atwo - \partial_x d),
\quad & \xv \in \OmegaS \label{eq:advB1}\\
\partial_t \atwo - \bar{c} \partial_y \atwo &= \bar{c} \partial_x \bone, 
\quad & \xv \in \OmegaS \label{eq:advA2}\\
\partial_t \btwo + \bar{c} \partial_y \btwo &= - \bar{c} \partial_x \aone,
\quad & \xv \in \OmegaS \label{eq:advB2}\\
\partial_t d &= 0,
\quad & \xv \in \OmegaS \label{eq:advD}
\end{alignat}
\ese
%
Equations~\eqref{eq:advA1}--\eqref{eq:advB2} are advection equations for the incoming 
characteristic variables, $\aone$ and $\atwo$,
and the outgoing characteristic variables $\bone$ and $\btwo$.
 % corresponding to the variables defined in equations~\eqref{eq:ACharacteristic}--\eqref{eq:BmCharacteristic} for $\nv=[0,-1]^T$. 
Equation~\eqref{eq:advD} states that that the characteristic $d$ will remain constant 
in time.

\subsection{Discretization}

The equations governing the fluid and solid are discretized in the $x$-direction on a 
uniform grid, $x_\ell = \ell \Delta x$ for $\ell = 0, 1,\ldots N_x$, with grid spacing 
$\dx = L/N_x$.  Since the problem is periodic, each variable can be represented as a 
discrete Fourier series
\begin{align}
q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2}  e^{2 \pi i k x_\ell/ L} \hat{q}_k (y,t), 
\qquad \ell=0,1,2,\ldots,N_x. \label{eq:discreteFourierII}
\end{align}

where $q_\ell(y,t) \approx q(x_\ell,y,t)$ denotes an approximation of a fluid or solid variable and $\hat{q}_k(y,t)$ are the corresponding Fourier coefficients.  For convenience, $N_x$ is assumed to be an even integer.  Taking a discrete Fourier transform of the fluid equations in 
equation~\eqref{eq:mpvaEquations} results in
\bse
\label{eq:fourierFullEquations}
\begin{alignat}{2}
\rho \partial_t v_1 + i k_x p &= \mu (\partial_y^2 - k_x^2) v_1, \qquad && y>0,\quad t>0,\label{eq:fourierV1Viscous}\\
\rho \partial_t v_2 + \partial_y p &= \mu (\partial_y^2 - k_x^2) v_2, \qquad && y>0,\quad t>0, \label{eq:fourierV2Viscous}\\
(\partial_y^2 - k_x^2) p &= 0, \qquad && y>0,\quad t>0, \label{eq:fourierPViscous}
\end{alignat}
\ese

where $k_x = 2 \pi k /L$ is a normalized wave number, and the hats and $k$ subscripts on the Fourier coefficients have been suppressed for notational convenience.
Similarly, the Fourier transform of the equations for the solid variables are
\bse
\begin{alignat}{2}
\partial_t \aone - \bar{c} \partial_y \aone &= \bar{c} i k_x ( d - \btwo),
\label{eq:advA1Fouriero}\\
\partial_t \bone + \bar{c} \partial_y \bone &= \bar{c} i k_x ( \atwo -  d),
\\
\partial_t \atwo - \bar{c} \partial_y \atwo &= \bar{c} i k_x \bone, 
\\
\partial_t \btwo + \bar{c} \partial_y \btwo &= - \bar{c} i k_x \aone,
\\
\partial_t d &= 0.
\label{eq:advDFouriero}
\end{alignat}
\ese


The equations for the fluid Fourier coefficients are now discretized in time.
Define the grid functions $(v_1)^n(y) \approx v_1(y, t^n)$, $(v_2)^n \approx v_2(y, t^n)$ 
and $p^n \approx p(y,t^n)$, where $t^n = n \Delta t$ for a (fixed) time step $\Delta t$.
The fluid velocity is advanced using (implicit) backward Euler for the viscous terms and
(explicit) forward Euler for the pressure gradient terms. 
This choice corresponds to an IMEX discretization.
The Poisson equation for the pressure is solved at each time step.
The scheme is given by
\bse
\begin{align}
(v_1)^{n+1} &= (v_1)^n 
- \frac{i k_x \dt}{\rho} p^{n}
+ \nu \dt \left( - k_x^2 + \partial_y^2  \right) (v_1)^{n+1}, \label{eq:viscousV1}\\
(v_2)^{n+1} &= (v_2)^n 
- \frac{\dt}{\rho} \partial_y p^{n}
+ \nu \dt \left( - k_x^2 + \partial_y^2\right) (v_2)^{n+1}, \label{eq:viscousV2}\\
\left(-k_x^2 + \partial_y^2\right) p^{n+1} &= 0 .\label{eq:viscousP}
\end{align}
\ese

%In this discretization, the viscous terms in~\eqref{eq:viscousV1} and~\eqref{eq:viscousV2} are treated implicitly, while the pressure gradient terms can be treated explicitly. This choice corresponds to an IMEX discretization.  As before, we enforce that the Fourier coefficents of the fluid are bounded as $y\rightarrow\infty$.
We enforce that the Fourier coefficents of the fluid are bounded as $y\rightarrow\infty$.

The equations for the Fourier coefficients of the solid variables corresponding to the characteristic form in~\eqref{eq:advFull} are discretized in both time and space using an upwind-type scheme given by
\bse
\begin{align}
(\aone)_j^{n+1} &= (\aone)_j^n + \ly ((\aone)_{j+1}^n-(\aone)_{j}^n) + i \lx ((d)_{j}^{n+1} - (\btwo)_{j}^{n+1}) \label{eq:schemeA1}\\
(\bone)_j^{n+1} &= (\bone)_j^n - \ly ((\bone)_{j}^n-(\bone)_{j-1}^n) + i \lx ((\atwo)_{j}^{n+1} - (d)_{j}^{n+1}) \label{eq:schemeB1}\\
(\atwo)_j^{n+1} &= (\atwo)_j^n + \ly ((\atwo)_{j+1}^n-(\atwo)_{j}^n) + i \lx (\bone)_{j}^{n+1} \label{eq:schemeA2}\\
(\btwo)_j^{n+1} &= (\btwo)_j^n - \ly ((\btwo)_{j}^n-(\btwo)_{j-1}^n) - i \lx (\aone)_{j}^{n+1} \label{eq:schemeB2}\\
(d)_j^{n+1} &= (d)_j^n, \label{eq:schemeD}
\end{align}
\ese
%
where, for example, $(\aone)_j^{n+1}\approx \aone(y_j,t_n)$ with $y_j = j \dy$, and where $\lx = \bar{c}\kx \dt$ and $\ly = \bar{c} \dt / \dy$.  
The grid in the $y$-direction is collocated about the interface at $y=0$.  
The terms involving transverse derivatives are treated implicitly to stabilize the pseudo-spectral approximation. For reference, the solid velocity and stress are related to the characteristic variables by
\bse
\begin{align}
(\vs_1)_j^n = \frac{1}{2 \bar{z}} \left( (\aone)_j^n - (\bone)_j^n \right), \qquad
(\vs_2)_j^n = \frac{1}{2 \bar{z}} \left( (\atwo)_j^n - (\btwo)_j^n \right), \label{eq:solidGridVelocity}\\
(\sigmas_{12})_j^n = \frac{1}{2 } \left( (\aone)_j^n + (\bone)_j^n \right), \qquad 
(\sigmas_{22})_j^n = \frac{1}{2 } \left( (\atwo)_j^n + (\btwo)_j^n \right). \label{eq:solidGridStress}
\end{align}
\ese
%
We enforce that the solid solution remains bounded as $y\rightarrow -\infty$, which implies
\begin{align}
|(\aone)_j^n|^2 +  |(\bone)_j^n|^2 + |(\atwo)_j^n|^2 + |(\btwo)_j^n|^2 < \infty,
\quad \text{ as } j \rightarrow -\infty.
\end{align}


\subsection{Interface coupling}

We explore different choices of interface coupling for the AMP, TP, and ATP schemes.
The evolution of the fluid equations in~\eqref{eq:viscousV1}--\eqref{eq:viscousP} requires 
three boundary conditions on the interface, $y=0$, to determine the interface velocity and
pressure.
Similarly the evolution of the solid 
equations in~\eqref{eq:schemeA1}--\eqref{eq:schemeD} require two incoming boundary conditions
at $y=0,$ corresponding to the two incoming characteristics.

We first describe the AMP interface conditions. This discussion follows 
Section~\ref{sec:interface}, where the key details of the AMP algorithm are
summarized. We assume the fluid and solid solutions are known at time $t^n.$ 
The solid solution is first advanced to time $t^{n+1}$ on grid points $j=0,-1,-2,\hdots$
using the evolution equations in~\eqref{eq:schemeA1}--\eqref{eq:schemeD}.
The solid interface velocity and stress are computed using 
\begin{align}
(\vs_m)^{n+1}_0 = \frac{1}{2 \zb} \left((a_m)_0^{n+1} - (b_m)_0^{n+1}  \right),
\qquad
(\sigmas_{m2})^{n+1}_0 = \frac{1}{2} \left((a_m)_0^{n+1} + (b_m)_0^{n+1}  \right),
\qquad m=1,2.
\end{align}
%
The fluid velocity is advanced using~\eqref{eq:viscousV1}--\eqref{eq:viscousV2}.
Two boundary conditions are required at $y=0$ to obtain the fluid velocity at time
$t^{n+1}.$
The condition on the outgoing solid tangential characteristic 
in~\eqref{eq:AMPTangentialCharacteristic} becomes
\begin{align}
\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right) - \zb (v_1)^{n+1} 
= (\sigmas_{12})^{n+1}_0 - \zb (\vs_1)^{n+1}_0,
\qquad y=0. \label{eq:fracTangential} 
\end{align}
%
The normal component of the velocity is projected to obtain the proper limiting behaviors
for heavy and light solids.
This condition in equation~\eqref{eq:normalVelociityFix} reduces to
\begin{align}
&(v_2)^{n+1} = \frac{\zf}{\zf+\zb}  V^p(v_2^{n+1}) + \frac{\zb}{\zf+\zb} (\vs_2)^{n+1}_0, \qquad y=0.
\label{eq:fracProject}
\end{align}
%
The fluid impedance is taken to be 
\begin{align}
\zf = \frac{\rho}{k_x \dt} + 2 \mu k_x,
\end{align}
%
in agreement with Section~\ref{sec:monolithic}.
$V^p(v_2^{n+1})$ is a predicted velocity given by
\begin{align}
V^p(v_2^{n+1}) = (v_2)^{n} 
- \frac{\dt }{\rho} \partial_y p^{n}
- \nu \dt \left(k_x^2 (v_2)^{n+1} + i k_x \partial_y (v_1)^{n+1}\right) .
\label{eq:predictedVelocity}
\end{align}
%
This definition is analogous to equation~\eqref{eq:veDef}, 
but with the substitution $\partial_y (v_2)^{n+1} = -i k_x (v_1)^{n+1}.$
The pressure is updated using equation~\eqref{eq:viscousP}
along with the AMP pressure condition described in~\eqref{eq:AMPpressureBC}.
This condition reduces to 
\begin{align}
-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} 
=\;& (\sigmas_{22})^{n+1}_0 + 2 i k_x \mu  (v_1)^{n+1} 
- \zb \dt (\dot{\vs}_2)^{n+1}_0 \nonumber \\
&
-\nu \zb \dt \left( k_x^2 (v_2)^{n+1} + i k_x \partial_y (v_1)^{n+1} \right),
\qquad y=0.
\label{eq:fracPressure} 
\end{align}
%
Again the substitution, $\partial_y (v_2)^{n+1} = -i k_x (v_1)^{n+1},$ was made.
$(\dot{\vs}_2)$ represents the solid interface acceleration and is taken to be
\begin{align}
(\dot{\vs}_2)^{n+1}_0 = \frac{(\vs_2)_0^{n+1}-(\vs_2)_0^{n}}{\dt}.
\end{align}
%
After solving for the fluid velocity and pressure, fluid interface quantities 
are obtained using
\bse
\begin{align}
(v_1)_f^{n+1} &= (v_1)^{n+1}(0), \\
(v_2)_f^{n+1} &= (v_2)^{n+1}(0), \\
p_f^{n+1} &= p^{n+1}(0), \\
(\sigma_{12})_f^{n+1} &= \mu \left(\partial_y (v_1)^{n+1}(0) + i k_x (v_2)^{n+1}(0) \right), \\
(\sigma_{22})_f^{n+1} &= -p^{n+1}(0) + 2 \mu \partial_y (v_2)^{n+1}(0) .
\end{align}
\ese
%
The interface velocity and traction are projected from fluid and solid values 
using equations~\eqref{eq:AMPinterfaceVelocity} and~\eqref{eq:AMPinterfaceTraction}.
These equations reduce to
\bse
\begin{align}
(v_1)_I^{n+1} &= \frac{\zf}{\zf+\zb} (v_{1})_f^{n+1} 
+ \frac{\zb}{\zf+\zb} (\vs_1)_0^{n+1}
+ \frac{1}{\zf+\zb} ( (\sigmas_{12})_0^{n+1} - (\sigma_{12})_f^{n+1}  ), \label{eq:project1}\\
(v_2)_I^{n+1} &= \frac{\zf}{\zf+\zb} (v_{2})_f^{n+1}
+ \frac{\zb}{\zf+\zb} (\vs_2)_0^{n+1}
+ \frac{1}{\zf+\zb} ( (\sigmas_{22})_0^{n+1} - (\sigma_{22})_f^{n+1}  ), \label{eq:project2}\\
(\sigma_{12})_I^{n+1} &= \frac{\zf^{-1}}{\zf^{-1}+\zb^{-1}} (\sigma_{12})_f^{n+1}
+ \frac{\zb^{-1}}{\zf^{-1}+\zb^{-1}} (\sigmas_{12})_0^{n+1}
+ \frac{1}{\zf^{-1}+\zb^{-1}} ( (\vs_1)_0^{n+1} - (v_1)_f^{n+1} ), \label{eq:project3}\\
(\sigma_{22})_I^{n+1} &= \frac{\zf^{-1}}{\zf^{-1}+\zb^{-1}} (\sigma_{22})_f^{n+1}
+ \frac{\zb^{-1}}{\zf^{-1}+\zb^{-1}} (\sigmas_{22})_0^{n+1}
+ \frac{1}{\zf^{-1}+\zb^{-1}} ( (\vs_2)_0^{n+1} - (v_2)_f^{n+1} ).\label{eq:project4}
\end{align}
\ese
%
Given the interface velocity and traction, the ghost points for the 
incoming solid characteristics are set using
\bse
\begin{align}
(\aone)_1^{n+1} &= (\sigma_{12})_I^{n+1}+ \zb (v_1)_I^{n+1}, \label{eq:a1CharBoundary}\\
(\atwo)_1^{n+1} &= (\sigma_{22})_I^{n+1}+ \zb (v_2)_I^{n+1}. \label{eq:a2CharBoundary}
\end{align}
\ese
This condition is a first-order accurate approximation.

For the AMP algorithm, the fluid velocity and pressure conditions are given in
equations~\eqref{eq:fracTangential},~\eqref{eq:fracProject}, and~\eqref{eq:fracPressure}
and the final interface values are defined by equations~\eqref{eq:project1}--\eqref{eq:project4}.
However, these conditions are modified for the TP and ATP algorithms.
The TP algorithm is obtained by taking the heavy-solid limit of the AMP 
conditions ($\zb\rightarrow\infty$). In this limit,
equations~\eqref{eq:fracTangential} and~\eqref{eq:fracProject} 
reduce to Dirichlet conditions on the fluid velocity given by
\bse
\begin{align}
(v_1)^{n+1} 
&=  (\vs_1)^{n+1}_0, \qquad y=0\label{eq:TPTangential} \\
(v_2)^{n+1} &= (\vs_2)^{n+1}_0, \qquad y=0.
\label{eq:TPNormal} 
\end{align}
\ese
%
The pressure condition in equation~\eqref{eq:fracPressure} becomes a 
Neumann condition given by
\begin{align}
\partial_y p^{n+1} 
&= 
- (\dot{\vs}_2)^{n+1}_0 
-\nu \left( k_x^2 (v_2)^{n+1} + i k_x \partial_y (v_1)^{n+1} \right), \qquad y=0.
\label{eq:TPPressure} 
\end{align}
%
For the TP scheme, the interface velocity is taken to be the solid velocity
($(v_1)_I^{n+1} = (\vs_1)_0^{n+1},$ $(v_2)_I^{n+1} = (\vs_2)_0^{n+1}$) and
the interface traction is taken to be the fluid traction
($(\sigma_{12})_I^{n+1} = (\sigma_{12})_f^{n+1},$ $(\sigma_{22})_I^{n+1} = (\sigma_{22})_f^{n+1}$).
Similarly, we can obtain the ATP scheme by taking the light-solid limit of the AMP 
conditions ($\zb\rightarrow 0$).
In this limit, equation~\eqref{eq:fracTangential} reduces to a Neumann condition for the
velocity.
\begin{align}
\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right)
&= (\sigmas_{12})^{n+1}_0, \qquad y=0.\label{eq:ATPV1} 
\end{align}
%
Equation~\eqref{eq:fracTangential} reduces to
\begin{align}
(v_2)^{n+1} = V^p(v_2^{n+1}), \qquad y=0,
\label{eq:ATPV2}
\end{align}
%
where $V^p(v_2^{n+1})$ is given by~\eqref{eq:predictedVelocity}.
Using equation~\eqref{eq:viscousV2}, it can be shown that equation~\eqref{eq:ATPV2}
can be replaced by
\begin{align}
\partial_y \left( i k_x (v_1)^{n+1} + \partial_y (v_2)^{n+1} \right)
&= 0, \qquad y=0, \label{eq:ATPDiv}
\end{align}
%
which is equivalent to setting the velocity to be divergence-free on the interface.
For the ATP scheme, the pressure condition in~\eqref{eq:fracPressure} reduces to 
\begin{align}
-p^{n+1} + 2 \mu \partial_y (v_2)^{n+1} 
&= (\sigmas_{22})^{n+1}_0, \qquad y=0. \label{eq:ATPP}
\end{align}
%
For the TP scheme, the interface velocity is taken to be the fluid velocity
($(v_1)_I^{n+1} = (v_1)_f^{n+1},$ $(v_2)_I^{n+1} = (v_2)_f^{n+1}$) and
the interface traction is taken to be the solid traction
($(\sigma_{12})_I^{n+1} = (\sigmas_{12})_0^{n+1},$ $(\sigma_{22})_I^{n+1} = (\sigmas_{22})_0^{n+1}$).




%
% \begin{align}
% (v_1)_I^{n+1} &= \alpha_1 (v_{1})_f^{n+1} 
% + (1-\alpha_1) (\vs_1)_0^{n+1}
% + \gamma_1 \bar{z}^{-1} ( (\sigmas_{12})_0^{n+1} - (\sigma_{12})_f^{n+1}  ), \label{eq:project1}\\
% (v_2)_I^{n+1} &= \alpha_2 (v_{2})_f^{n+1}
% + (1-\alpha_2) (\vs_2)_0^{n+1}
% + \gamma_2 \bar{z}^{-1} ( (\sigmas_{22})_0^{n+1} - (\sigma_{22})_f^{n+1}  ), \label{eq:project2}\\
% (\sigma_{12})_I^{n+1} &= \beta_1 (\sigma_{12})_f^{n+1}
% + (1-\beta_1) (\sigmas_{12})_0^{n+1}
% + \delta_1 \bar{z} ( (\vs_1)_0^{n+1} - (v_1)_f^{n+1} ), \label{eq:project3}\\
% (\sigma_{22})_I^{n+1} &= \beta_2 (\sigma_{22})_f^{n+1}
% + (1-\beta_2) (\sigmas_{22})_0^{n+1}
% + \delta_2 \bar{z} ( (\vs_2)_0^{n+1} - (v_2)_f^{n+1} ).\label{eq:project4}
% \end{align}
%


\subsection{Stability analysis}

In order to assess the stability of the AMP, TP and ATP schemes, 
we search for normal mode solutions to the discretization. In the fluid,
solutions are of the form
\begin{align}
(v_1)^n(y) = A^n \tilde{v}_1(y), \quad 
(v_2)^n(y) = A^n \tilde{v}_2(y), \quad
p^n(y) = A^n \tilde{p}(y),
\end{align}
%
where $A$ is the amplification factor and $(\tilde{v}_1(y), \tilde{v}_2(y),\tilde{p})$
are functions of space given by
\bse
\begin{align}
\tilde{v}_1(y) 
  &= (v_1)_f^0 e^{-\gamma k_x y} 
    - \frac{i p_f^0}{\rho k_x A (\gamma^2 - 1)} \left( e^{-k_x y} - e^{-\gamma k_x y} \right), \\
\tilde{v}_2(y) 
  &= (v_2)_f^0 e^{-\gamma k_x y}
    + \frac{p_f^0}{\rho k_x A (\gamma^2 - 1)}\left( e^{-k_x y} - e^{-\gamma k_x y} \right), \\
\tilde{p}(y) &= p_f^0 e^{-k_x y},
\end{align}
% \begin{align}
% \tilde{v}_1(y) &= \left((v_1)_f + \frac{i p_f}{z_\mu s^* (\gamma^2 - 1)} \right) e^{-k_x \gamma y}
% - \frac{i p_f}{z_\mu s^* (\gamma^2 - 1)} e^{-k_x y}, \\
% \tilde{v}_2(y) &= \left((v_2)_f - \frac{p_f}{z_\mu s^*(\gamma^2 - 1)} \right) e^{-k_x \gamma y}
% + \frac{p_f}{z_\mu s^* (\gamma^2 - 1)} e^{-k_x y}, \\
% \tilde{p}(y) &= p_f e^{-k_x y},
% \end{align}
\ese
%
where
\begin{align}
\gamma = \sqrt{\frac{1}{\Lambda}\frac{A-1}{A} + 1}, \qquad
\Lambda = \nu k_x^2 \dt.
\end{align}
%
Here, $\Lambda$ represents the viscous CFL number.
The constants, $(v_1)_f^0, (v_2)_f^0$, and $p_f^0$ are obtained by
enforcing the three fluid boundary conditions (ie.
equations~\eqref{eq:fracTangential}--\eqref{eq:fracProject}, and~\eqref{eq:fracPressure} 
for the AMP scheme,
equations~\eqref{eq:TPTangential}--\eqref{eq:TPNormal}, and~\eqref{eq:TPPressure} 
for the TP scheme, or
equations~\eqref{eq:ATPV1} and \eqref{eq:ATPDiv}--\eqref{eq:ATPP} for the ATP scheme).


% \begin{align}
% (v_1)_f &= -\frac{(\gamma^2+\gamma) z_\mu + \zb}{ \zb E} b_1 
%           + \frac{i z_\mu (\gamma-1)}{ \zb E} b_2 \\
% (v_2)_f &= -\frac{i z_\mu (\gamma - 1)}{ \zb E} b_1 
%           - \frac{(\gamma+1) z_\mu + \zb}{\zb E} b_2 \\
% p_f &= \frac{i (2 \gamma Z + 1) (\gamma + 1) Z}{E} b_1
%       - \frac{(\gamma+1) (\gamma^2 Z + \gamma + Z) Z}{E} b_2
% \end{align}

% \begin{align}
% E = (\gamma^3 + \gamma^2 + 3 \gamma - 1) Z^2 + (\gamma+1)^2 Z + 1
% \end{align}

We now search for solutions to the solid discretization. 
Let $\av_j^n = [(\aone)_j^n$,$ (\bone)_j^n$, $(\atwo)_j^n$, $(\btwo)_j^n$,$ (d)_j^n]^T.$
Solutions are sought of the form, $\av_j^n =  \phi^j A^n \tilde{\rv},$
where $\phi$ is a spacial eigenvalue and $\tilde{\rv}$ is a constant eigenvector.
The scheme is said to be weakly stable if there are no non-trivial solutions with $|A| > 1$.  
Our strategy for determining regions of stability will be to search for unstable modes with 
$|A| > 1$, and then identify regions of the parameter space where no non-trivial solution exist.  
To do this, we begin by finding the general solution for the spatial grid functions satisfying 
the discrete equations and regularity condition as $j\rightarrow-\infty$, assuming $|A| > 1$.  
We then apply the conditions at the interface to determine whether non-trivial solutions exist.
When the normal mode ansatz is substituted into the numerical scheme for the solid in 
equations \eqref{eq:schemeA1}--\eqref{eq:schemeD}, a homogeneous system arises of the form
% what should we call this matrix?
\newcommand{\SolidMatrixB}{Q}
\begin{align}
\SolidMatrixB(\phi) \tilde{\rv} = 0.
\end{align}
The matrix $\SolidMatrixB(\phi)$ is given by
\begin{align*}
\SolidMatrixB(\phi) = \left[\begin{array}{ccccc}
\eta(\phi) & 0 &  0& -i A \lx & i A \lx  \\
0 & \eta(1/\phi) & i A \lx & 0 & -i A \lx \\
0 & i A \lx & \eta(\phi) & 0 & 0 \\
-i A \lx & 0 & 0 & \eta(1/\phi) & 0 \\
0 & 0 & 0 & 0 & 1-A
\end{array}\right],
\end{align*}
%
where
\begin{align}
\eta(\phi) = 1-A+\ly (\phi-1).
\end{align}
%
This system is singular when $f(\phi) \defeq \det (\SolidMatrixB(\phi)) = 0.$
The function $f(\phi)$ can be written as 
\begin{align}
f(\phi) = (1-A) \left(\eta(\phi) \eta(1/\phi) + (A \lx)^2\right)^2,
\label{eq:SolidDetCond}
\end{align}
%
which is zero when $A=1$ or when $\eta(\phi) \eta(1/\phi) + (A \lx)^2 = 0.$
Since we are interested in searching for unstable modes, we are interested in the latter 
case. Roots of $f(\phi)$ can be written in the form
\newcommand{\bParam}{\theta}
\begin{align}
\phi_\pm = \bParam \pm \sqrt{\bParam^2 - 1}, \qquad 
\bParam = 1 - \frac{(A \lx)^2 + (1-A)^2}{2 \ly (1-A-\ly)}.
\end{align}
%
The product of the roots is equal to one ($\phi_+ \phi_- = 1$).
Since we are searching for solutions that are bounded as $j\rightarrow -\infty,$ 
we are only interested in the root with modulus greater than 1.

\medskip
\noindent\textbf{Lemma}: \textit{If $|A|>1$ and if $\lx$ and $\ly$ are chosen to satisfy a CFL 
condition, then there is precisely one root (either $\phi_+$ or $\phi_-$), denoted by 
$\phi_*$ that has magnitude strictly greater than one, $|\phi_*| > 1.$}
\medskip

\noindent This result follows from a similar argument to that given 
in~\cite{DifferenceApproximationsForTheInitialBoundary}.  
We first consider the scheme applied to the pure initial-value problem (Cauchy problem).  
Setting $\phi=e\sp{i\vartheta}$ in~\eqref{eq:SolidDetCond}, we determine a region of 
the $\lx$-$\ly$ plane for which $\vert A\vert\le1$ for all $\vartheta\in[0,2\pi]$.  
This region is found numerically as discussed in~\ref{sec:CFLRegionCauchy}
and shown in Figure~\ref{fig:viscousCFL}, and it corresponds 
to a region where the Cauchy problem is (Fourier) stable.  It is also shown that this stability 
region includes a region of $(\lx,\ly)$ satisfying a reasonable CFL restriction, 
namely $\lx\sp2+\ly\sp2\le1$.
Next, since $|A| \le 1$ when $|\phi| = 1$, we have that $|\phi| \ne 1$ when $|A| > 1$.  
Thus, if $|A| > 1$ and if $(\lx,\ly)$ remains within the CFL restriction, then $\phi$ cannot 
cross the unit circle, $|\phi|=1$, as $(\lx,\ly)$ vary.  
It is therefore only necessary to prove that the lemma holds for one set of parameters.  
For $\lx=0$, the discretization reduces to four uncoupled upwind schemes for linear advection. 
In this case, equation~\eqref{eq:SolidDetCond} is equivalent to 
$\eta(\phi) \eta(1/\phi) = 0,$
%
which has solutions
$\phi_+ = (A-1+\ly)/\ly$ and $\phi_- = 1/\phi_+$.
%
When $|A|>1$ and $\ly \in (0,1]$, $|\phi_+|>1$ and therefore $\phi_* = \phi_+.$ 
Thus, the condition holds for all $(\lx,\ly)$ provided the CFL condition is satisfied.

%
When $\phi=\phi_*,$ there are two eigenvectors, namely
\begin{align}
\tilde{\rv}_1 = 
\left[
\frac{\eta(1/\phi_*)}{i A\lx},\, 0,\, 0,\, 1,\, 0
\right]^T, \qquad 
\tilde{\rv}_2 = 
\left[
0,\, -\frac{\eta(\phi_*)}{i A\lx},\, 1,\, 0,\, 0
\right]^T
.
\end{align}
%
The solution which remains bounded as $j \rightarrow -\infty$ is given by
\begin{align*}
(\aone)_j^{n} = k_1 \frac{ \eta(1/\phi_*) }{i A \lx} \phi_*^{j} A^n, \quad
(\bone)_j^{n} = -k_2 \frac{ \eta(\phi_*) }{i A \lx} \phi_*^{j} A^n, \quad
(\atwo)_j^{n} = k_2 \phi_*^{j} A^n, \quad
(\btwo)_j^{n} = k_1 \phi_*^{j} A^n,
% (\aone)_j^{n} = k_1 \frac{ \eta(1/\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
% (\bone)_j^{n} = -k_2 \frac{ \eta(\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
% (\atwo)_j^{n} = k_2 \phi_*^{j-1} A^n, \quad
% (\btwo)_j^{n} = k_1 \phi_*^{j-1} A^n,
\end{align*}
%
where $k_1$ and $k_2$ are free constants to be determined by the interface conditions.
The discrete solutions are plugged into the boundary conditions, equations
\eqref{eq:a1CharBoundary}--\eqref{eq:a2CharBoundary},
to form another homogeneous system of equations, given by
\begin{align}
\dMat(A) \kv = \left[\begin{array}{cc}
g_{11} & g_{12} \\ 
g_{21} & g_{22}
\end{array}\right]
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right]
= 0.
\label{eq:StabilitySystemViscous}
\end{align}
%
The coefficients of the matrix $\dMat$
are provided in~\ref{sec:ComponentsOfDmatViscous} for the AMP, TP, and
ATP schemes.
Solutions for the amplification factor are roots of 
\begin{align}
\dMat(A) = \det(\dMat(A)) = g_{11} g_{22} - g_{12} g_{21} = 0.
\label{eq:ViscousDet}
\end{align}
%


Solutions for the amplification factor are the roots of the transcendental 
equation~\eqref{eq:ViscousDet}, which is dependent on the choice of interface coupling and 
four dimensionless parameters ($\Lambda, Z, \lx, \ly$). Here, $Z$ is a ratio of the
viscous fluid impedance to the solid impedance given by
\begin{align}
Z = \frac{\mu k_x}{\zb}.
\end{align}
%
Given the interface coupling and dimensional parameters, proving stability is equivalent to 
showing that there exist no roots of equation~\eqref{eq:ViscousDet} such that $|A|>1$.
The argument principle is applied to determine the number of unstable roots to the 
complex function $h(z) \defeq g(z^{-1}).$
\begin{align}
\mathcal{P} = \frac{1}{2 \pi i}\oint_C \frac{h'(z)}{h(z)} \; dz,
\qquad
C = \{z : z = e^{i \theta}, \theta = [0,2 \pi] \} 
\end{align}
%
It can be shown that the only branch cuts of $h(A)$ are located in the region $|A|>1$. 
In the region $|A|\le 1,$ there is a pole of order $2$ at the origin.
Therefore $\mathcal{P} = N-2$ where $N$ is the number of roots of $g(A)$ 
with $|A|>1$~\cite{carrier05}. 
By making the substitutions $h(z) = g(z^{-1}),$
$h'(z) = -z^{-2} g'(z^{-1}),$ 
$z = e^{i \theta},$ 
and $dz = i e^{i \theta} d \theta,$ it can be shown that $\mathcal{P}$ is equivalent to 
\begin{align}
\mathcal{P} &= -\frac{1}{2 \pi} \int_{0}^{2 \pi} \frac{g'(e^{-i\theta})}{  g(e^{-i\theta})} e^{- i \theta} \; d\theta. \label{eq:argPrinciple}
\end{align}
%
The number $\mathcal{P}$ was computed for a 31$\times$31$\times$20$\times$20
array of parameter values in the ($Z$,$\Lambda$,$\lx$,$\ly$) parameter space.
The parameters $Z$ and $\Lambda$ are logarithmically spaced in the 
interval $[10^{-3}, 10^{3}]$ 
while $\lx$ and $\ly$ are chosen to be equally spaced in the interval
$[0.05, 0.95]$.
A stable problem corresponds to $N=0$ and therefore $\mathcal{P}=-2$.
Results of this computation are shown in Figure~\ref{fig:argPrinciple}.
For each point $(\Lambda,Z)$, the computation of $\mathcal{P}$ is repeated for
all $\lx$ and $\ly$ in the search region. If any point in this search region is unstable,
then the point $(\Lambda,Z)$ is added to the region of instability.
The parameter search resulted in no unstable roots found for the AMP scheme. 
However, there are significant regions where The TP and ATP schemes are unstable.

\medskip
\noindent\textbf{Theorem}: \textit{By numerical evaluation of $\mathcal{P},$ we have found that
the AMP algorithm is weakly stable $(|A| \le 1)$ provided that $\lx^2 + \ly^2 \le 1,$ i.e.}
\begin{align}
\dt \le \frac{1}{\cb} \left[ \frac{1}{\dy^2} + k_x^2\right]^{1/2}.
\end{align}
\textit{This is a sufficient but not a necessary condition.}

% \das{finish me}

% \begin{figure}[h]
% \centering
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi0_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi1_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi2_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi0_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi1_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi2_theta0_lxp1_lyp1.png}
% \caption{
%   I fixed $\lx=\ly=.1$ and varied the scheme (non-fractional-step: \texttt{iBC=1}, 
%   fractional-step: \texttt{iBC=2}) and choice of projection weights ($\psi=0,1,2$).
%   The only case that goes unstable is the bottom right, when the fluid values are used
%   instead of a projection in equations~\eqref{eq:project1}--\eqref{eq:project4}.
%   \label{fig:argPrinciple}
% }
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=.4\textwidth]{fig/iBC3_psi2_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC4_psi2_theta0_lxp1_lyp1.png}
% \caption{
%   Left: traditional. Right: anti-traditional.
%   \label{fig:argPrinciple}
% }
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=.4\textwidth]{fig/iBC3_psi2_theta0_lxp1_lyp1.png}
\includegraphics[width=.48\textwidth]{fig/AMPstabilityViscousAnalysis}
\includegraphics[width=.48\textwidth]{fig/TPandATPstabilityViscousAnalysis}
\caption{
  Left: Green circles represent points for which 
  the AMP algorithm is stable in the CFL region $\lx^2+\ly^2\le 1$.
  Right: stability regions for the TP (red) and ATP (blue) schemes.
  \label{fig:argPrinciple}
}
\end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=\textwidth]{fig/ViscousContinuation_NL200_NZ50_nonfrac}
% \caption{Magnitude of maximum amplification factor for non-fractional-step scheme.
%   \das{Looks OK except for a point in the middle...}}
% \end{figure}



==> texFiles/viscousAnalysisOld.tex <==

\section{Viscous analysis old} \label{sec:viscousAnalysis}

In this section, the stability of the AMP algorithm applied to a simplified viscous model problem 
is analyzed. This model problem exposes an instability which motivates the use of new solid 
projection steps. For simplicity, we consider a first-order accurate algorithm 
which exposes the key issues for stability.

\subsection{FSI model problem}
The geometry of the viscous model problem is the same as the inviscid model problem 
and is shown in Figure~\ref{fig:rectangularModelProblem}.  
The fluid is assumed to be steady and incompressible with uniform pressure.
The solid is taken to be an ``acoustic'' solid. 
This case is obtained by taking $\lambdas=-\mus$ in the equations for linear elasticity
and corresponds to pressure and shear waves traveling at the same speed.
As in the inviscid analysis, 
the fluid-solid interface $\Gamma$ is linearized about the flat surface, $y=0$, and it is assumed that the velocity and traction between the fluid and solid match along $\Gamma$.  
The fluid velocity is taken to be zero along the top boundary, $y=H$, and the solutions for the fluid and solid are assumed to be periodic in the $x$-direction with period equal to~$L$.  
The governing equations for the FSI model problem are
\begin{align}
\text{Fluid: } &\begin{cases}
\Delta \vv = 0, & \xv\in\OmegaF \\
\vv = 0, & x\in(0,L), \quad y=H
\end{cases} \label{eq:fluidModel} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsv = \grad \cdot \sigmasv, & \xv\in\OmegaS \\
\partial_t \sigmasv = -\mus (\grad \cdot \vv) \Iv 
+ \mus (\grad \vv + (\grad \vv)^T), & \xv\in\OmegaS \\
\bar{z} |\vsv|^2+|\sigmasv|^2 < \infty, & y\rightarrow - \infty
\end{cases} \label{eq:solidModel} \\
\text{Interface: } &\begin{cases}
\vv = \vsv, & x\in(0,L), \quad y = 0 \\
\sigmav \nv = \sigmasv \nv, & x\in(0,L), \quad y = 0.
\end{cases}
\end{align}
%
Here, the unit normal to the fluid interface is $\nv = [0,-1]^T.$
Similar to the inviscid analysis, the solid equations are rewritten in terms of characteristic 
variables given by
\begin{align}
\aone = \sigmas_{12} + \bar{z} \vs_1 , \quad
\bone = \sigmas_{12} - \bar{z} \vs_1, \quad
\atwo = \sigmas_{22} + \bar{z} \vs_2, \quad
\btwo = \sigmas_{22} - \bar{z} \vs_2, \quad
d = \sigmas_{11} + \sigmas_{22},
\end{align}
%
where
\begin{align}
\bar{z} = \rhos \bar{c}, \quad \bar{c} = \sqrt{\mus \over \rhos}. 
\end{align}
%
The solid equations reduce to
\begin{alignat}{2}
\partial_t \aone - \bar{c} \partial_y \aone &= \bar{c} (\partial_x d - \partial_x \btwo),
\quad & y \in (-\infty,0) \label{eq:advA1}\\
\partial_t \bone + \bar{c} \partial_y \bone &= \bar{c} (\partial_x \atwo - \partial_x d),
\quad & y \in (-\infty,0) \label{eq:advB1}\\
\partial_t \atwo - \bar{c} \partial_y \atwo &= \bar{c} \partial_x \bone, 
\quad & y \in (-\infty,0) \label{eq:advA2}\\
\partial_t \btwo + \bar{c} \partial_y \btwo &= - \bar{c} \partial_x \aone,
\quad & y \in (-\infty,0) \label{eq:advB2}\\
\partial_t d &= 0,
\quad & y \in (-\infty,0) \label{eq:advD}
\end{alignat}
%
Equations~\eqref{eq:advA1}--\eqref{eq:advB2} are advection equations for the incoming 
characteristic variables, $\aone$ and $\atwo$,
and the outgoing characteristic variables $\bone$ and $\btwo$, corresponding to the variables defined in equations~\eqref{eq:ACharacteristic}--\eqref{eq:BmCharacteristic} for $\nv=[0,-1]^T$. 
\das{To be consistent with the notation above, we can instead use $a, a_1, b,$ and $b_1$.}
Equation~\eqref{eq:advD} describes the evolution of the steady characteristic.

\subsection{Discretization}

As in the inviscid analysis, the solution is represented as a discrete Fourier series
(ie. equation~\eqref{eq:discreteFourier}) in the transverse direction. 
The normalized wave number is $k_x = 2 \pi k /L.$
The solid characteristic variables are discretized in the $y$-direction using a
uniform staggered grid, defined by $y_j = \left(j-\frac{1}{2}\right) \dy$ for
$j = 1,0,-1,\dots$ with grid spacing $\dy$.
The solid equations in~\eqref{eq:advA1}--\eqref{eq:advD} are approximated using a 
first-order accurate upwind-type scheme given by
\begin{align}
(\aone)_j^{n+1} &= (\aone)_j^n + \ly ((\aone)_{j+1}^n-(\aone)_{j}^n) + i \lx ((d)_{j}^{n+1} - (\btwo)_{j}^{n+1}) \label{eq:schemeA1}\\
(\bone)_j^{n+1} &= (\bone)_j^n - \ly ((\bone)_{j}^n-(\bone)_{j-1}^n) + i \lx ((\atwo)_{j}^{n+1} - (d)_{j}^{n+1}) \label{eq:schemeB1}\\
(\atwo)_j^{n+1} &= (\atwo)_j^n + \ly ((\atwo)_{j+1}^n-(\atwo)_{j}^n) + i \lx (\bone)_{j}^{n+1} \label{eq:schemeA2}\\
(\btwo)_j^{n+1} &= (\btwo)_j^n - \ly ((\btwo)_{j}^n-(\btwo)_{j-1}^n) - i \lx (\aone)_{j}^{n+1} \label{eq:schemeB2}\\
(d)_j^{n+1} &= (d)_j^n, \label{eq:schemeD}
\end{align}
% \begin{align} % this was the original...
% a_{2,j}^{n+1} &= a_{2,j}^n + \ly (a_{2,j+1}^n-a_{2,j}^n) + i \lx b_{1,j}^{n+1} \\
% b_{2,j}^{n+1} &= b_{2,j}^n - \ly (b_{2,j}^n-b_{2,j-1}^n) - i \lx a_{1,j}^{n+1} \\
% a_{1,j}^{n+1} &= a_{1,j}^n + \ly (a_{1,j+1}^n-a_{1,j}^n) + i \lx (d_{j}^{n+1} - b_{2,j}^{n+1}) \\
% b_{1,j}^{n+1} &= b_{1,j}^n - \ly (b_{1,j}^n-b_{1,j-1}^n) + i \lx (a_{2,j}^{n+1} - d_{j}^{n+1}) \\
% d_j^{n+1} &= d_j^n
% \end{align}
%
where $\lx = \kx \bar{c} \dt$ and $\ly = \bar{c} \dt / \dy.$ 
The terms involving transverse derivatives are treated implicitly to stabilize the 
pseudo-spectral approximation. For reference, the solid velocity and stress 
are related to the characteristic variables by
\begin{align}
(\vs_1)_j^n = \frac{1}{2 \bar{z}} \left( (\aone)_j^n - (\bone)_j^n \right), \quad
(\vs_2)_j^n = \frac{1}{2 \bar{z}} \left( (\atwo)_j^n - (\btwo)_j^n \right), \label{eq:solidGridVelocity}\\
(\sigmas_{12})_j^n = \frac{1}{2 } \left( (\aone)_j^n + (\bone)_j^n \right), \quad 
(\sigmas_{22})_j^n = \frac{1}{2 } \left( (\atwo)_j^n + (\btwo)_j^n \right). \label{eq:solidGridStress}
\end{align}
%
We enforce that the solid solution remains bounded as $y\rightarrow -\infty$.
This implies
\begin{align}
|(\aone)_j^n|^2 +  |(\bone)_j^n|^2 + |(\atwo)_j^n|^2 + |(\btwo)_j^n|^2 < \infty,
\quad \text{ as } j \rightarrow -\infty.
\end{align}

The Laplace equation for the velocity, with the 
no-slip boundary condition at $y=H$, is solved exactly at time $t^n$ to give
\begin{align}
\vv^n(y) = \vv_f^n \frac{\sinh(k_x (H - y))}{\sinh(k_x H)}, \label{eq:velocitySolution}
\end{align}
%
where $\vv_f^n$ is an interface velocity which is specified later by the 
interface boundary conditions. 
The fluid stress involves the derivative of the velocity at the interface, which is
given by
\begin{align}
\partial_y \vv^n(0) = -\frac{\vv_f^n}{\Heff}, 
\quad 
\Heff = \frac{\tanh(k_x H )}{k_x}.
\end{align}
%
We note that the effective fluid height, $\Heff$, takes the same definition in the inviscid 
analysis.

The evolution of the solid requires boundary conditions for the two incoming characteristics
at $y=0.$ Similarly, the fluid requires boundary conditions for the two components of 
velocity. Since the fluid solution is determined by the solution of an elliptic equation
for the velocity, the fluid-solid coupling reduces to a modified boundary condition for the 
solid.

Assume that the solid characteristic variables, 
$(\aone)_j^n, (\bone)_j^n, (\atwo)_j^n, (\btwo)_j^n, (d)_j^n$,
are known at time level $t^n$ for all grid points, $y_j = \left(j-\frac{1}{2}\right) \dy,$
$j = 0,-1, \dots,$ including a ghost point at $j=1.$
The numerical scheme defined by~\eqref{eq:schemeA1}--\eqref{eq:schemeD} is used to 
advance the variables to $t^{n+1}.$
The interface solid velocity and stress are computed at grid point $j=0$ using 
equations~\eqref{eq:solidGridVelocity}--\eqref{eq:solidGridStress}.

\subsection{Interface coupling}

The fluid interface conditions are the following Robin conditions.
\begin{alignat}{3}
\mu \left(\partial_y (v_1)^{n+1} 
  + \partial_x (v_2)^{n+1} \right) - \bar{z} (v_1)^{n+1} &= (\bone)_{0}^{n+1}, \quad &&y=0,\\
2 \mu \partial_y (v_2)^{n+1} - \bar{z} (v_2)^{n+1} &= (\btwo)_0^{n+1}, \quad &&y=0.
\end{alignat}
%
Using the solution for the fluid velocity in equation \eqref{eq:velocitySolution}, the 
Robin conditions turn into algebraic conditions for $(v_1)_f^{n+1}$ and $(v_2)_f^{n+1}$,
given by
\begin{align}
\mu \left(-\frac{(v_{1})_f^{n+1}}{\Heff} + i k_x (v_2)_f^{n+1} \right) - \bar{z} (v_1)_f^{n+1} &= (\bone)_{0}^{n+1},\\
-2 \mu \frac{(v_{2})_f^{n+1}}{\Heff} - \bar{z} (v_2)_f^{n+1} &= (\btwo)_0^{n+1}.
\end{align}
%
The solution for $(v_1)_f^{n+1}$ and $(v_2)_f^{n+1}$ is
\begin{align}
(v_1)_f^{n+1} &= - \frac{1}{\bar{z} (Z_y + 1)} (\bone)_{0}^{n+1}
          - \frac{i Z_x}{\bar{z} (Z_y + 1) (2 Z_y + 1)} (\btwo)_{0}^{n+1}, 
\label{eq:v1fSol}\\
(v_2)_f^{n+1} &= - \frac{1}{\bar{z} (2 Z_y + 1)} (\btwo)_{0}^{n+1},
\label{eq:v2fSol}
\end{align}
%
where
\begin{align}
Z_x = \frac{\rho \nu k_x}{\rhos \bar{c}},
\quad
Z_y = \frac{\rho \nu}{\rhos \bar{c} \Heff}.
\end{align}
%
We note that $Z_x$ and $Z_y$ are ratios of fluid impedances to the solid impedance.
It is here where we find suitable measures for the fluid impedance for the viscous model problem.
The fluid impedance is of the form $\rho \nu / l,$ where $l$ is some characteristic length scale.

The interface velocity and stress are projected using the following.
\begin{align}
(v_1)_I^{n+1} &= \alpha_1 (v_{1})_f^{n+1} 
+ (1-\alpha_1) (\vs_1)_0^{n+1}
+ \gamma_1 \bar{z}^{-1} ( (\sigmas_{12})_0^{n+1} - (\sigma_{12})_f^{n+1}  ), \label{eq:project1}\\
(v_2)_I^{n+1} &= \alpha_2 (v_{2})_f^{n+1}
+ (1-\alpha_2) (\vs_2)_0^{n+1}
+ \gamma_2 \bar{z}^{-1} ( (\sigmas_{22})_0^{n+1} - (\sigma_{22})_f^{n+1}  ), \label{eq:project2}\\
(\sigma_{12})_I^{n+1} &= \beta_1 (\sigma_{12})_f^{n+1}
+ (1-\beta_1) (\sigmas_{12})_0^{n+1}
+ \delta_1 \bar{z} ( (\vs_1)_0^{n+1} - (v_1)_f^{n+1} ), \label{eq:project3}\\
(\sigma_{22})_I^{n+1} &= \beta_2 (\sigma_{22})_f^{n+1}
+ (1-\beta_2) (\sigmas_{22})_0^{n+1}
+ \delta_2 \bar{z} ( (\vs_2)_0^{n+1} - (v_2)_f^{n+1} )\label{eq:project4}
\end{align}
%
Here, the fluid stress components are given by
\begin{align}
(\sigma_{12})_f^{n+1} = \mu \left( - \frac{(v_1)_f^{n+1}}{\Heff} + i k_x (v_2)_f^{n+1}\right),
\quad (\sigma_{22})_f^{n+1} = -2 \mu \frac{(v_2)_f^{n+1}}{\Heff}.
\end{align}
%
% \begin{align}
% (v_1)_I^{n+1} &= \alpha_1 (v_{1})_f^{n+1} 
% + (1-\alpha_1) (\vs_1)_0^{n+1}, \\
% (v_2)_I^{n+1} &= \alpha_2 (v_{2})_f^{n+1}
% + (1-\alpha_2) (\vs_2)_0^{n+1}, \\
% (\sigma_{12})_I^{n+1} &= \beta_1 
% \mu \left( - \frac{(v_1)_f^{n+1}}{\Heff} + i k_x (v_2)_f^{n+1}\right)
% + (1-\beta_1) (\sigmas_{12})_0^{n+1}, \\
% (\sigma_{22})_I^{n+1} &= -2 \mu \beta_2 \frac{(v_2)_f^{n+1}}{\Heff}
% + (1-\beta_2) (\sigmas_{22})_0^{n+1}.
% \end{align}
%
These projections are used as conditions for obtaining the ghost point value 
for the incoming characteristic variables, $\aone$ and $\atwo.$
\begin{align}
(a_1)_1^{n+1} &= (\sigma_{12})_I^{n+1} + \bar{z} (v_1)_I^{n+1}, \label{eq:solidBC1}\\
(a_2)_1^{n+1} &= (\sigma_{22})_I^{n+1} + \bar{z} (v_2)_I^{n+1} \label{eq:solidBC2}.
\end{align}
%
We are interested in choosing the projection coefficients, $(\alpha_i,\beta_i,\gamma_i,\delta_i)$ 
for $i=1,2,$ so the scheme is stable for all possible physical and numerical parameters.
These projections include jump terms scaled by the positive coefficients 
$(\gamma_i,\delta_i).$ These terms introduce dissipation which may 
stabilize a typically unstable problem. However, the coefficients
$(\alpha_i,\beta_i)$ can be chosen to stabilize the scheme 
even when the jump terms are absent (ie. $\gamma_i = \delta_i = 0$).  
Natural choices for these coefficients appear in the normal mode analysis.

\subsection{Stability analysis}
Next, we search for normal mode solutions to the discretization. 
Let $\av_j^n = [(\aone)_j^n, (\bone)_j^n, (\atwo)_j^n, (\btwo)_j^n, (d)_j^n]^T.$
Solutions are sought of the form, $\av_j^n =  \phi^j A^n \rv,$
where $A$ is the amplification factor, $\phi$ is a spacial eigenvalue, and $\rv$ is
a constant vector. As in the inviscid analysis, our approach for determining 
regions of instability is to search for unstable modes assuming $|A|>1$ and 
find regions of the parameter space where non-trivial solutions exist.
When the normal mode ansatz is substituted into the numerical scheme for the solid in 
equations \eqref{eq:schemeA1}--\eqref{eq:schemeD}, a homogeneous system arises of the form
% what should we call this matrix?
% \newcommand{\SolidMatrixB}{Q}
\begin{align}
\SolidMatrixB(\phi) \rv = 0.
\end{align}
The matrix $\SolidMatrixB(\phi)$ is given by
\begin{align*}
\SolidMatrixB(\phi) = \left[\begin{array}{ccccc}
\eta(\phi) & 0 &  0& -i A \lx & i A \lx  \\
0 & \eta(1/\phi) & i A \lx & 0 & -i A \lx \\
0 & i A \lx & \eta(\phi) & 0 & 0 \\
-i A \lx & 0 & 0 & \eta(1/\phi) & 0 \\
0 & 0 & 0 & 0 & 1-A
\end{array}\right],
\end{align*}
%
where
\begin{align}
\eta(\phi) = 1-A+\ly (\phi-1).
\end{align}
%
This system is singular when $f(\phi) \defeq \det (\SolidMatrixB(\phi)) = 0.$
The function $f(\phi)$ can be written as 
\begin{align}
f(\phi) = (1-A) \left(\eta(\phi) \eta(1/\phi) + (A \lx)^2\right)^2,
\label{eq:SolidDetCond}
\end{align}
%
which is zero when $A=1$ or when $\eta(\phi) \eta(1/\phi) + (A \lx)^2 = 0.$
Since we are interested in searching for unstable modes, we are interested in the latter 
case. Roots of $f(\phi)$ can be written in the form
% \newcommand{\bParam}{\theta}
\begin{align}
\phi_\pm = \bParam \pm \sqrt{\bParam^2 - 1}, \qquad 
\bParam = 1 - \frac{(A \lx)^2 + (1-A)^2}{2 \ly (1-A-\ly)}.
\end{align}
%
We note that the product of the roots is one ($\phi_+ \phi_- = 1$).
Under the assumption $|A|>1,$ there will always be one root 
$\phi = \phi_*$ such that $|\phi_*| > 1.$ Assuming the principal branch of the square root,
$\phi_*$ can be written as
\begin{align}
\phi_* = 
\begin{cases}
\phi_+, & \text{if }\Re(A) \ge 1-\ly \\
\phi_-, & \text{if }\Re(A) < 1-\ly \\
\end{cases}.
\end{align}
%
When $\phi=\phi_*,$ there are two eigenvectors, namely
\begin{align}
\rv_1 = 
\left[
\frac{\eta(1/\phi_*)}{i A\lx},\, 0,\, 0,\, 1,\, 0
\right]^T, \qquad 
\rv_2 = 
\left[
0,\, -\frac{\eta(\phi_*)}{i A\lx},\, 1,\, 0,\, 0
\right]^T
.
\end{align}
%
The solution which remains bounded as $j \rightarrow -\infty$ is given by
\begin{align*}
(\aone)_j^{n} = k_1 \frac{ \eta(1/\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
(\bone)_j^{n} = -k_2 \frac{ \eta(\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
(\atwo)_j^{n} = k_1 \phi_*^{j-1} A^n, \quad
(\btwo)_j^{n} = k_2 \phi_*^{j-1} A^n,
\end{align*}
%
where $k_1$ and $k_2$ are free constants to be determined by the interface conditions.
The discrete solutions are plugged into the boundary conditions 
\eqref{eq:solidBC1}--\eqref{eq:solidBC2}
to form another homogeneous system of equations, given by
\begin{align}
G \kv = \left[\begin{array}{cc}
g_{11} & g_{12} \\ 
g_{21} & g_{22}
\end{array}\right]
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right]
= 0.
\end{align}
%
Solutions for the amplification factor are roots of 
\begin{align}
\det(G) = g_{11} g_{22} - g_{12} g_{21} = 0.
\label{eq:ViscousDet}
\end{align}
%
Let $\hat{\alpha}_i = \alpha_i-\delta_i$ and $\hat{\beta}_i = \beta_i-\gamma_i$
for $i=1,2.$
Then the components of $G$ are
\begin{align}
g_{11} &= 
\eta(1/\phi_*) \left(\hat{\alpha}_1 + \hat{\beta}_1 + 2 \phi_* - 2 \right)
- \frac{ 2 \lx A  Z_x \phi_* (\hat{\alpha}_1 + \hat{\beta}_1) }
  {(Z_y+1)(2 Z_y+1)} \\
g_{12} &= 
\eta(\phi_*) \left( 2 \phi_*\frac{\hat{\beta}_1 Z_y - \hat{\alpha}_1}{Z_y+1} 
         + \hat{\alpha}_1 - \hat{\beta}_1 \right) \\
g_{21} &= 2 \phi_* \frac{2 \hat{\beta}_2 Z_y - \hat{\alpha}_2}{2 Z_y+1}
         + \hat{\alpha}_2 - \hat{\beta}_2 \\
g_{22} &= 2 - 2 \phi_* - \hat{\alpha}_2 - \hat{\beta}_2
\end{align}
%
We explore different choices for the projection coefficients. In the first option,
we show that the jump term coefficients, $\gamma_i$ and $\delta_i,$
can be chosen to stabilize the scheme for any choice of $\alpha_i$ and $\beta_i$. 
When jump terms are absent (ie. $\gamma_i = \delta_i = 0$), 
we show both stable and unstable choices of coefficients.
In all cases, it is informative to consider choices of coefficients which lead to 
significant simplification of the matrix, $G$. 
For the case with jump terms, if we choose $\alpha_i=\delta_i$ and $\beta_i=\gamma_i,$
then $\hat{\alpha}_i = \hat{\beta}_i = 0$ and the determinant condition in equation~\eqref{eq:ViscousDet} becomes
\begin{align}
\det(G) = 4 \eta(1/\phi_*) (\phi - 1)^2.
\label{eq:DissipationDetCond}
\end{align}
%
Equations~\eqref{eq:SolidDetCond} and~\eqref{eq:DissipationDetCond} can be solved to show that
either $A=0$ and $A=1$. Since this violates the assumption that $|A|>1,$ the scheme is stable 
under this choice of coefficients.

Next, we consider the case when $\gamma_i = \delta_i = 0.$
In order to simplify the components of the matrix $G,$ we choose the coefficients to satisfy
\begin{align}
\beta_1 Z_y - \alpha_1 = 0, 
\quad
2 \beta_2 Z_y - \alpha_2 = 0.
\end{align}
%
Additionally we would like to apply the constraints
$\alpha_1 + \beta_1 = \alpha_2 + \beta_2 = 1.$ 
When these constraints are satisfied, 
the interface velocity and traction come from 
the solid velocity and fluid traction in the heavy solid limit
and the fluid velocity and solid traction in the light solid limit.
The constraints imply the following choice of coefficients.
%- \wdh{wdh: do you mean?
%- \ba
%- \alpha_1 - \delta_1 = \frac{Z_y}{Z_y+1}, 
%- \quad 
%- \beta_1 - \gamma_1 = \frac{1}{Z_y+1},
%- \quad
%- \alpha_2 - \delta_2 = \frac{2 Z_y}{2 Z_y + 1},
%- \quad
%- \beta_2 - \gamma_2 = \frac{1}{2 Z_y+1},
%- \ea  
%- }  
\begin{align}
\text{AMP}: \quad
\alpha_1 = \frac{Z_y}{Z_y+1}, 
\quad 
\beta_1 = \frac{1}{Z_y+1},
\quad
\alpha_2 = \frac{2 Z_y}{2 Z_y + 1},
\quad
\beta_2 = \frac{1}{2 Z_y+1}
\end{align}
%
Additionally, we can consider the choice of coefficients obtained 
by using the fluid interface values for the projection, given by
\begin{align}
\text{Unstable}: \quad
\alpha_1 = 1
\quad 
\beta_1 = 1
\quad
\alpha_2 = 1
\quad
\beta_2 = 1.
\end{align}
%
After substitution of these choices of coefficients into equation~\eqref{eq:ViscousDet},
the determinant can be manipulated into a single polynomial in $A$ of degree 6 whose 
coefficients depend on $\lx, \ly, Z_x,$ and $Z_y$. Due to the complexity of the coefficients,
Maple is used to generate the polynomial and compute roots.
%
The maximum amplification factor was computed for an array of points in 
the $(\lx, \ly, Z_x, Z_y)$ parameter space. 
A 200 x 200 logarithmically spaced array was used for $Z_x$ and $Z_y.$
For each pair $(Z_x, Z_y),$ 
the maximum amplification factor in the CFL region, $\lx^2+\ly^2 \le 1,$
was found. A 40 x 40 cylindrically spaced array was used for $\lx$ and $\ly.$
Shaded contours of the maximum amplification factor for both parameter sets
are shown in \ref{fig:viscousStability}. The AMP coefficients are stable for the entire 
search region, while the unstable coefficients are unstable for a significant area of the 
search region.
\begin{figure}[h]
\centering
\includegraphics[width=.49\textwidth]{fig/ViscousStability200}
\includegraphics[width=.49\textwidth]{fig/ViscousInstabilitySingleParameters}
% \includegraphics[width=.49\textwidth]{fig/ViscousInstability}
\caption{
Top left: new projection is stable for entire parameter search.
Top right: stability region for old projection conditions. 
Bottom left: stability region for single set of parameters.
\label{fig:viscousStability}
}
\end{figure}

\subsection{Changes for discrete fluid model}

In this section, we wish to derive projection coefficients when the fluid is discretized 
and governed by a Stokes model. Examine equations \eqref{eq:v1fSol}--\eqref{eq:v2fSol}. 
In general, the solution is given by
\begin{align}
(v_1)_f^{n+1} = - \frac{1}{z_{f,1} + \zp} (\bone)_0^{n+1} + C_1 (\btwo)_0^{n+1}, \qquad
(v_2)_f^{n+1} = - \frac{1}{z_{f,2} + \zp} (\btwo)_0^{n+1} + C_2 (\bone)_0^{n+1},
\label{eq:vSolutionForZf}
\end{align}
%
where $z_{f,1}$ and $z_{f,2}$ are measures of fluid impedances and 
$C_1$ and $C_2$ are constants. If the fluid impedances are known,
we can choose the projection weights in equations \eqref{eq:project1}--\eqref{eq:project4}
according to 
\begin{align}
\alpha_1 = \frac{z_{f,1}}{z_{f,1}+\zp}, \quad
\alpha_2 = \frac{z_{f,2}}{z_{f,2}+\zp}, \quad
\beta_1 = 1-\alpha_1, \quad
\beta_2 = 1-\alpha_2.
\end{align}

Consider a Stokes fluid in a semi-infinite domain defined by 
$\Omega = \{\xv : x \in (0,L), y > 0\}.$ The new governing equations are
given by the following.
\begin{align*}
\begin{cases}
\rho \vv_t + \grad p = \mu \Delta \vv, & \xv \in \Omega \\
\Delta p = 0,  & \xv \in \Omega \\
\grad \cdot \vv = 0,  & x \in (0,L), \quad y = 0 \\
\vv  \rightarrow 0, & x \in (0,L), \quad y \rightarrow \infty 
\end{cases}
\end{align*}
%
We discretize the equations in time and space using $t_n = n \dt$ and $y_j = j \dy$
for $n = 0,1,2,\dots$ and $j=-1,0,1,\dots.$
As before, the solution is represented as a discrete Fourier series in the transverse direction
with wave number $k_x = 2 \pi k / L.$
A backward-Euler scheme used to advance the fluid velocity in time and central
second-order accurate finite differences are used to discretize in space.
\begin{align}
(v_1)_j^{n+1} &= (v_1)_j^n 
- \frac{i r_x}{z_x} p_j^{n+1}
- r_x (v_1)_j^{n+1}
 + r_y \left( (v_1)_j^{n+1} - 2 (v_1)_j^{n+1} + (v_1)_j^{n+1} \right), \\
(v_2)_j^{n+1} &= (v_2)_j^n 
- \frac{r_y}{2 z_y}  \left(p_{j+1}^{n+1} - p_{j-1}^{n+1} \right)
- r_x (v_2)_j^{n+1}
 + r_y \left( (v_2)_j^{n+1} - 2 (v_2)_j^{n+1} + (v_2)_j^{n+1} \right), \\
0 &= -r_x p_j^{n+1} + r_y \left( p_{j+1}^{n+1} - 2 p_{j}^{n+1} + p_{j-1}^{n+1} \right),
\end{align}
%
for $j = 0,1,2,\dots.$ Here,
\begin{align}
r_x = \nu \dt k^2, \quad 
r_y = \frac{\nu \dt}{\dy^2}, \quad
z_x = \nu k, \quad
z_y = \frac{\nu}{\dy}.
\end{align}
%
$r_x$ and $r_y$ are viscous CFL numbers and $z_x$ and $z_y$ are fluid impedances.
Consider perturbing the solution at the new time by a small amount,
$\vv^{n+1}_j = \hat{\vv}^{n+1}_j + \delta \vv_j$ and $p^{n+1}_j = \hat{p}^{n+1}_j + \delta p_j.$
The variational equations for the perturbations are 
\begin{align}
(v_1)_j &= 
- \frac{i r_x}{z_x} p_j
- r_x (v_1)_j
 + r_y \left( (v_1)_j - 2 (v_1)_j + (v_1)_j \right), \label{eq:v1Eqn}\\
(v_2)_j &= 
- \frac{r_y}{2 z_y}  \left(p_{j+1} - p_{j-1} \right)
- r_x (v_2)_j
 + r_y \left( (v_2)_j - 2 (v_2)_j + (v_2)_j \right), \label{eq:v2Eqn}\\
0 &= -r_x p_j + r_y \left( p_{j+1} - 2 p_{j} + p_{j-1}\right), \label{eq:pressureEqn}
\end{align}
% 
Here, the $\delta$ has been dropped for simplicity. The solution of
equation \eqref{eq:pressureEqn} which satisfies the boundary conditions is
\begin{align}
p_j = p_f \kappa_-^j,
\end{align}
%
where $p_f$ is the interface fluid pressure and
\begin{align}
\kappa_\pm = 1 + \frac{\eta}{2} \pm \frac{1}{2} \sqrt{\eta^2 + 4 \eta},
\qquad  \eta = \frac{r_x}{r_y}.
\end{align}
%
The solutions to equations \eqref{eq:v1Eqn}--\eqref{eq:v2Eqn} are
\begin{align}
(v_1)_j &= 
\left(u_f + \frac{i r_x}{z_x} p_f\right) \psi_-^j - \frac{i r_x}{z_x} p_f \kappa_-^j, \\
(v_2)_j &= 
\left(v_f - \frac{r_y}{2z_y} \left(\frac{1}{\kappa_-} - \kappa_-\right) p_f \right) \psi_-^j 
+ \frac{r_y}{2z_y} \left(\frac{1}{\kappa_-} - \kappa_-\right) p_f \kappa_-^j.
\end{align}
%
Here, $u_f$ and $v_f$  are the interface horizontal and vertical components of velocity
and $p_f$ is the interface pressure. Let
\begin{align}
\psi_\pm = 1 + \frac{\xi}{2} 
\pm \frac{1}{2} \sqrt{
\xi^2 + 4 \xi
}, \qquad \xi = \frac{1}{r_y} + \eta.
\end{align}
%
We note that $\kappa_+ \kappa_- = \psi_+ \psi_- = 1$. Since $\eta$ and $\xi$ are real
and positive constants, $\kappa$ and $\psi$ are always real and we have
$|\kappa_-| < 1 < |\kappa_+|$ and $|\psi_-| < 1 < |\psi_+|.$
Therefore, $|\kappa_-|^j+|\psi_-|^j \rightarrow 0$ as $j\rightarrow\infty.$ 
We are interested in solving for $u_f, v_f,$ and $p_f$ in terms of the incoming characteristics, 
$(\bone)_0$ and $(\btwo)_0.$ The two characteristic boundary conditions are given by
\begin{align}
- p_0 + \frac{\mu}{\dy} \left((v_2)_{1} - (v_2)_{-1} \right)
- \zb (v_2)_0 &= (\btwo)_0, \\
\frac{\mu}{2\dy} \left((v_1)_{1} - (v_1)_{-1} \right)
+ i k \mu (v_2)_0
- \zb (v_1)_0 &= (\bone)_0. 
\end{align}
%
Additionally, we enforce that the discrete divergence of the velocity is zero at the boundary.
\begin{align}
i k (v_1)_0 + \frac{1}{2 \dy} \left((v_2)_{1} - (v_2)_{-1} \right) = 0
\end{align}
%
These three conditions form the following system of equations for $u_f, v_f,$ and $p_f$,
% \newcommand{\dpsi}{\left(\frac{1}{\psi}-\psi \right)}
% \newcommand{\dkappa}{\left(\frac{1}{\kappa}-\kappa \right)}
\newcommand{\dpsi}{ D_{\psi}}
\newcommand{\dkappa}{ D_{\kappa}}
% \begin{align}
% \left(-z_y \dpsi - \zb\right) v_f
% - \left(1+\frac{r_y}{2} \dkappa \left(\dkappa - \dpsi\right)
% \right) p_f &= (\btwo)_0 \\
% i \sqrt{\eta} z_y v_f
% - \left(\frac{1}{2} z_y \dpsi + \zb \right)u_f
% + i \sqrt{\eta} r_y \left(\dkappa - \dpsi \right) p_f &= (\bone)_0 \\
% \frac{1}{2} \dpsi v_f
% + i \sqrt{\eta} u_f
% - \frac{r_y}{ 4 z_y} \dkappa \left(\dkappa - \dpsi\right) p_f &= 0
% \end{align}
\begin{align}
A \left[\begin{array}{c}
v_f \\ u_f \\ p_f
\end{array}\right]
= 
\left[\begin{array}{c}
(\btwo)_0 \\ (\bone)_0 \\ 0
\end{array}\right]
\end{align}
%
where
\begin{align}
A = \left[\begin{array}{ccc}
-z_y \dpsi - \zb & 0 & -1-\frac{r_y}{2} \dkappa \left(\dkappa - \dpsi\right) \\
i \sqrt{\eta} z_y &
- \frac{1}{2} z_y \dpsi - \zb &
i \sqrt{\eta} r_y \left(\dkappa - \dpsi \right) \\
-\frac{1}{2} \dpsi  & i \sqrt{\eta}  &
- \frac{r_y}{ 4 z_y} \dkappa \left(\dkappa - \dpsi\right)
\end{array}\right].
\end{align}
%
Here,
\begin{align}
D_{\kappa} = \frac{1}{\kappa} - \kappa
= \sqrt{\eta^2 + 4 \eta}, 
\qquad D_{\psi} = \frac{1}{\psi} - \psi
= \sqrt{\xi^2 + 4 \xi}.
\end{align}
%
Let $e_k$ be the vector where the $k$th element is one and the rest of the elements are zero.
Let $A^{(kl)}$ be the matrix formed by replacing the $l$th column by $e_k$.
By Cramer's rule, the solution to the system is
\begin{align}
v_f &= \frac{\det(A^{(11)}) (\btwo)_0 + \det(A^{(21)}) (\bone)_0}{\det(A)}, \\
u_f &= \frac{\det(A^{(12)}) (\btwo)_0 + \det(A^{(22)}) (\bone)_0}{\det(A)}, \\
p_f &= \frac{\det(A^{(13)}) (\btwo)_0 + \det(A^{(23)}) (\bone)_0}{\det(A)}.
\end{align}
%
We compare this solution to equation \eqref{eq:vSolutionForZf}. We are interested in the 
coefficient of $(\btwo)_0$ in $v_f$ and $(\bone)_0$ in $u_f.$ By equating these coefficients,
we obtain
\begin{align}
z_{f,2} = -\zb -\frac{\det(A)}{\det(A^{(11)})}, \qquad
z_{f,1} = -\zb -\frac{\det(A)}{\det(A^{(22)})},
\end{align}
%
We can write $z_{f,2}$ and $z_{f,1}$ as scale factors multiplying $z_y$. Therefore,
\begin{align}
z_{f,2} = f_2 z_y, \qquad
z_{f,1} = f_1 z_y,
\end{align}
%
where 
\begin{align}
f_2 &= 
\dpsi
+\frac{
(\dkappa^2 r_y - \dkappa \dpsi r_y + 2)
(Z_y \dpsi^2 + 4 Z_y \eta + 2 \dpsi )
}{
r_y (\dpsi - \dkappa) (Z_y \dkappa \dpsi + 8 Z_y \eta + 2 \dkappa)
}.
\\
f_1 &= 
\frac{1}{2} \dpsi
+\frac{
4 \eta \left(\left(\dpsi Z_y - \frac{1}{2} Z_y \dkappa + 1\right) 
(\dpsi - \dkappa) r_y + Z_y\right)
}{
\dkappa (\dpsi - \dkappa) r_y + 2 \dpsi Z_y
}.
\end{align}
%
and $Z_y = z_y/\zb.$ See figure \ref{fig:scaleFactor}.
 
\begin{figure}[h]
\includegraphics[width=.5\textwidth]{fig/ZfScaleFactorDiscrete}
\includegraphics[width=.5\textwidth]{fig/ZfScaleFactorContinuous}
\caption{$f_2$ when $\eta=1$ for
discrete model problem (left) and continuous model problem (right).
\das{The right plot is the same plot as in the notes.pdf document but with a 
factor of two to account for the different definitions of $z_\mu$ and $z_y$.}
\label{fig:scaleFactor}}
\end{figure}


% \subsection{Changes for discrete fluid model}
% \das{OLD...}:
% How would the analysis change if the fluid were discrete and time dependent?
% Consider a heat equation for the fluid, given by
% \begin{align}
% \vv_t = \nu \Delta \vv.
% \end{align}
% %
% A backward Euler scheme is used to advance the velocity.
% \begin{align}
% \vv^{n+1}_j = \vv^n_j + (- r_x \vv_j^{n+1} + r_y (\vv_{j+1}^{n+1} - 2 \vv_{j}^{n+1} + \vv_{j-1}^{n+1}))
% \end{align}
% %
% The general solution is 
% \begin{align}
% \vv_j^n = \vv_f A^n \frac{\kappa^j - \kappa^{2N-j}}{1-\kappa^{2N}},
% \end{align}
% %
% where $\kappa$ and $A$ obey the following characteristic equation.
% \begin{align}
% \frac{1-A}{A} - r_x + r_y \left(\kappa -2 + \frac{1}{\kappa} \right) = 0,
% \quad r_x = \nu \dt k_x^2, \quad r_y = \frac{\nu \dt}{\dy^2}
% \end{align}
% %
% The boundary conditions for the fluid are
% \begin{align}
% -\frac{\mu}{\bar{z} \dy} \frac{1/\kappa - \kappa}{2} \frac{1+\kappa^{2N}}{1-\kappa^{2N}} v_{1,f}  
%   + i \frac{\mu k_x}{\bar{z}} v_{2,f}
% - v_{1,f} &= \frac{1}{\bar{z}} \bone^{(p)}, \\
% -\frac{\mu}{\bar{z} \dy} \frac{1/\kappa - \kappa}{2} \frac{1+\kappa^{2N}}{1-\kappa^{2N}} v_{2,f}  
% - v_{2,f} &= \frac{1}{\bar{z}} \btwo^{(p)}.
% \end{align}
% %
% This can be rewritten as
% \begin{align}
% -\tilde{Z}_y v_{1,f}  
%   + i Z_x v_{2,f}
% - v_{1,f} &= \frac{1}{\bar{z}} \bone^{(p)}, \\
% -2 \tilde{Z}_y v_{2,f}  
% - v_{2,f} &= \frac{1}{\bar{z}} \btwo^{(p)},
% \end{align}
% %
% where
% \begin{align}
% \tilde{Z}_y = Z_y \frac{1/\kappa - \kappa}{2} \frac{1+\kappa^{2N}}{1-\kappa^{2N}},
% \end{align}
% %
% When $N$ is large, the effect of the no slip boundary is negligible.
% \begin{align}
% \frac{1+\kappa^{2N}}{1-\kappa^{2N}} \sim 1
% \end{align}
% %
% The effect from the difference term can be computed in terms of $r_x,r_y,$ and $A.$
% \begin{align}
% 1/\kappa - \kappa = \frac{1}{r_y} 
% \sqrt{\left(r_x + 4 r_y + \frac{A-1}{A}\right) 
%   \left( r_x + \frac{A-1}{A} \right)}.
% \end{align}
% %
% When $r_x,r_y \gg 1,$ then \wdh{wdh: if $r_x=r_y$ doesn't this lead to $1/\kappa - \kappa \sim \sqrt{5}$?
% with $\tilde{Z}_y = Z_y \sqrt{5}/2$ ? }
% \begin{align}
% 1/\kappa - \kappa 
% \sim
%  \frac{1}{r_y} 
% \sqrt{r_x \left(r_x + 4 r_y \right) }.
% \end{align}
% %
% This corresponds to the steady limit ($\Delta \vv = 0$).
% If we can choose
% \begin{align}
% \alpha_1 = \frac{\tilde{Z}_y}{\tilde{Z}_y+1},
% \quad 
% \alpha_2 = \frac{2 \tilde{Z}_y}{2 \tilde{Z}_y+1},
% \quad 
% \beta_1 = 1-\alpha_1, 
% \quad 
% \beta_2 = 1-\alpha_2,
% \end{align}
% %
% then the above analysis still holds and the problem is stable. 


==> texFiles/viscousAnalysisOld2.tex <==
\section{Viscous analysis} \label{sec:viscousAnalysis}

In this section, the stability of the AMP, TP, and ATP algorithms 
are explored for model problem MP-VA.
This extends the analysis of the inviscid model problem in~\cite{fib2014} to 
a viscous model problem. 
When viscosity is involved, stability is more challenging since instabilities 
arise from both added mass and added damping effects.
Due to this, both horizontal and vertical motions in the solid must be considered.
This relaxes the assumption in~\cite{fib2014} where the model problem was constrained 
to vertical motions only.
Another difficulty is the introduction of the viscous CFL number in the fluid as a 
new dimensionless parameter. 
In Section~\ref{sec:monolithic}, a fluid impedance was derived which is a function of 
the viscous CFL number. This impedance is used in the interface projection step of the 
AMP algorithm and is critical to achieving stability.

\subsection{FSI model problem}

Consider model problem MP-VA. 
The geometry of this model problem is shown in Figure \ref{fig:rectangularModelProblemCartoon}
and discussed in Section~\ref{sec:FSIModelProblems}.
The fluid is taken to be semi-infinite ($H \rightarrow \infty$).
and is shown in Figure~\ref{fig:rectangularModelProblem}. The fluid is semi-infinite
and exists in the domain defined by $x \in (0,L)$ and $y>0.$ The solid domain is 
also semi-infinite and is defined by $x \in [0,L]$ and $y < 0.$
the fluid-solid interface $\Gamma$ is linearized about the flat surface, $y=0$, and it is 
assumed that the velocity and traction between the fluid and solid match along $\Gamma$.  
The fluid is governed by the Stokes equations and the solid is taken to be an 
``acoustic'' solid, which is the case obtained by taking $\lambdas=-\mus$ in the equations 
for linear elasticity and corresponds to pressure and shear waves traveling at the same speed.
The fluid velocity vanishes to zero as $y\rightarrow \infty$ and the solid solution remains
bounded as $y\rightarrow -\infty.$
The solutions for the fluid and solid are assumed to be periodic in the $x$-direction with 
period equal to~$L$.  
The governing equations for the FSI model problem are
\begin{align}
\text{Fluid: } &\begin{cases}
\rho \partial_t\vv + \grad p = \mu \Delta \vv, & \xv\in\OmegaF \\
\Delta p = 0, & \xv \in \OmegaF \\
|\vv| \rightarrow 0, & x\in (0,L), \quad y \rightarrow \infty \\
\grad \cdot \vv = 0, & x\in (0,L), \quad y=0
\end{cases} \label{eq:fluidModel} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsv = \grad \cdot \sigmasv, & \xv\in\OmegaS \\
\partial_t \sigmasv = -\mus (\grad \cdot \vv) \Iv 
+ \mus (\grad \vv + (\grad \vv)^T), & \xv\in\OmegaS \\
\bar{z} |\vsv|^2+|\sigmasv|^2 < \infty, & x\in (0,L), \quad y\rightarrow - \infty
\end{cases} \label{eq:solidModel} \\
\text{Interface: } &\begin{cases}
\vv = \vsv, & x\in(0,L), \quad y = 0 \\
\sigmav \nv = \sigmasv \nv, & x\in(0,L), \quad y = 0
\end{cases}
\end{align}
%
Here, the unit normal to the fluid interface is $\nv = [0,-1]^T.$
Similar to the inviscid analysis, the solid equations are rewritten in terms of characteristic 
variables given by
\begin{align}
\aone = \sigmas_{12} + \bar{z} \vs_1 , \quad
\bone = \sigmas_{12} - \bar{z} \vs_1, \quad
\atwo = \sigmas_{22} + \bar{z} \vs_2, \quad
\btwo = \sigmas_{22} - \bar{z} \vs_2, \quad
d = \sigmas_{11} + \sigmas_{22},
\end{align}
%
where
\begin{align}
\bar{z} = \rhos \bar{c}, \quad \bar{c} = \sqrt{\mus \over \rhos}. 
\end{align}
%
The solid equations reduce to
\begin{alignat}{2}
\partial_t \aone - \bar{c} \partial_y \aone &= \bar{c} (\partial_x d - \partial_x \btwo),
\quad & y \in (-\infty,0) \label{eq:advA1}\\
\partial_t \bone + \bar{c} \partial_y \bone &= \bar{c} (\partial_x \atwo - \partial_x d),
\quad & y \in (-\infty,0) \label{eq:advB1}\\
\partial_t \atwo - \bar{c} \partial_y \atwo &= \bar{c} \partial_x \bone, 
\quad & y \in (-\infty,0) \label{eq:advA2}\\
\partial_t \btwo + \bar{c} \partial_y \btwo &= - \bar{c} \partial_x \aone,
\quad & y \in (-\infty,0) \label{eq:advB2}\\
\partial_t d &= 0,
\quad & y \in (-\infty,0) \label{eq:advD}
\end{alignat}
%
Equations~\eqref{eq:advA1}--\eqref{eq:advB2} are advection equations for the incoming 
characteristic variables, $\aone$ and $\atwo$,
and the outgoing characteristic variables $\bone$ and $\btwo$, corresponding to the variables defined in equations~\eqref{eq:ACharacteristic}--\eqref{eq:BmCharacteristic} for $\nv=[0,-1]^T$. 
\das{To be consistent with the notation above, we can instead use $a, a_1, b,$ and $b_1$.}
Equation~\eqref{eq:advD} describes the evolution of the steady characteristic.

\subsection{Discretization}

As in the inviscid analysis, the solution is represented as a discrete Fourier series
(ie. equation~\eqref{eq:discreteFourier}) in the transverse direction. 
The normalized wave number is $k_x = 2 \pi k /L.$
The fluid is discretized in time and kept continuous in space. 
The temporal discretization is defined by $t_n = n \dt,$ with time step $\dt.$
A backward-Euler scheme is used to advance the fluid velocity.
\das{For the fractional-step scheme, I'm using FE for the pressure. For the non-fractional-step
scheme, I'm using BE for the pressure.}
\begin{align}
(v_1)^{n+1} &= (v_1)^n 
- \frac{i k_x \dt}{\rho} p^{n+1}
+ \nu \dt \left( - k_x^2 + \partial_y^2  \right) (v_1)^{n+1} \\
(v_2)^{n+1} &= (v_2)^n 
- \frac{\dt}{\rho} \partial_y p^{n+1}
+ \nu \dt \left( - k_x^2 + \partial_y^2\right) (v_2)^{n+1} \\
\left(-k_x^2 + \partial_y^2\right) p^{n+1} &= 0 
\end{align}
%
We enforce that the fluid velocity decays to zero ($|\vv^n| \rightarrow 0$)
as $y\rightarrow\infty$.
%

The solid characteristic variables are discretized in the $y$-direction using a
uniform staggered grid, defined by $y_j = \left(j-\frac{1}{2}\right) \dy$ for
$j = 1,0,-1,\dots$ with grid spacing $\dy$.
The solid equations in~\eqref{eq:advA1}--\eqref{eq:advD} are approximated using a 
first-order accurate upwind-type scheme given by
\begin{align}
(\aone)_j^{n+1} &= (\aone)_j^n + \ly ((\aone)_{j+1}^n-(\aone)_{j}^n) + i \lx ((d)_{j}^{n+1} - (\btwo)_{j}^{n+1}) \label{eq:schemeA1}\\
(\bone)_j^{n+1} &= (\bone)_j^n - \ly ((\bone)_{j}^n-(\bone)_{j-1}^n) + i \lx ((\atwo)_{j}^{n+1} - (d)_{j}^{n+1}) \label{eq:schemeB1}\\
(\atwo)_j^{n+1} &= (\atwo)_j^n + \ly ((\atwo)_{j+1}^n-(\atwo)_{j}^n) + i \lx (\bone)_{j}^{n+1} \label{eq:schemeA2}\\
(\btwo)_j^{n+1} &= (\btwo)_j^n - \ly ((\btwo)_{j}^n-(\btwo)_{j-1}^n) - i \lx (\aone)_{j}^{n+1} \label{eq:schemeB2}\\
(d)_j^{n+1} &= (d)_j^n, \label{eq:schemeD}
\end{align}
%
where $\lx = \kx \bar{c} \dt$ and $\ly = \bar{c} \dt / \dy.$ 
The terms involving transverse derivatives are treated implicitly to stabilize the 
pseudo-spectral approximation. For reference, the solid velocity and stress 
are related to the characteristic variables by
\begin{align}
(\vs_1)_j^n = \frac{1}{2 \bar{z}} \left( (\aone)_j^n - (\bone)_j^n \right), \quad
(\vs_2)_j^n = \frac{1}{2 \bar{z}} \left( (\atwo)_j^n - (\btwo)_j^n \right), \label{eq:solidGridVelocity}\\
(\sigmas_{12})_j^n = \frac{1}{2 } \left( (\aone)_j^n + (\bone)_j^n \right), \quad 
(\sigmas_{22})_j^n = \frac{1}{2 } \left( (\atwo)_j^n + (\btwo)_j^n \right). \label{eq:solidGridStress}
\end{align}
%
We enforce that the solid solution remains bounded as $y\rightarrow -\infty$.
This implies
\begin{align}
|(\aone)_j^n|^2 +  |(\bone)_j^n|^2 + |(\atwo)_j^n|^2 + |(\btwo)_j^n|^2 < \infty,
\quad \text{ as } j \rightarrow -\infty.
\end{align}

\subsection{Interface coupling}
The fluid requires three boundary conditions at $y=0.$ We consider two cases. 
The first case applied equations \eqref{eq:BCharacteristic}--\eqref{eq:BmCharacteristic}
directly to obtain coupled conditions for the velocity and pressure.
The third condition is setting the velocity to be divergence-free on the interface.

\bigskip
\noindent \textbf{Coupled boundary conditions}: 
\textit{ 
The following conditions are applied at $y=0$.
}
\begin{align}
\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right) - \zb (v_1)^{n+1} 
&= (\sigmas_{12})^{n+1}_0 - \zb (\vs_1)^{n+1}_0, \label{eq:v1ConditionCoupled} \\
-p^{n+1} + 2 \mu \partial_y (v_2)^{n+1} - \zb (v_2)^{n+1} 
&= (\sigmas_{22})^{n+1}_0 - \zb (\vs_2)^{n+1}_0, \label{eq:v2ConditionCoupled}\\
i k_x (v_1)^{n+1} + \partial_y (v_2)^{n+1} 
&= 0. \label{eq:divConditionCoupled}
\end{align}

The second case considers fractional-step boundary conditions which decouple 
the fluid velocity and pressure at the boundary. 
Equation~\eqref{eq:v2ConditionCoupled} sets the fluid velocity in the heavy solid limit
and the pressure in the light solid limit. From this condition and 
equation~\eqref{eq:divConditionCoupled}, we will derive 
separate conditions for velocity and pressure.
The first condition can be derived by eliminating $(v_2)^{n+1}$ and
$(\vs_2)^{n+1}_0$ in equation~\eqref{eq:v2ConditionCoupled} by a backward-Euler scheme.
\begin{align}
(v_2)^{n+1} &= (v_2)^* 
- \frac{\dt }{\rho} \partial_y p^{n+1} 
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}),\\
(\vs_2)^{n+1}_0 &= (v_2)^*
+ \dt (\dot{\vs}_2)^{n+1}_0.
\end{align}
%
Here, equation~\eqref{eq:divConditionCoupled} was used to replace
$\partial_y^2 (v_2)^{n+1} = -i k_x \partial_y (v_1)^{n+1}$ and 
$(\dot{\vs}_2)$ represents the solid interface acceleration. 
After substitution, a mixed pressure condition is derived.
\begin{align}
-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} 
=\;& (\sigmas_{22})^{n+1}_0 + 2 i k_x \mu  (v_1)^{n+1} 
- \zb \dt (\dot{\vs}_2)^{n+1}_0 \nonumber \\
&
+\nu \zb \dt \left( -k_x^2 (v_2)^{n+1} + i k_x \partial_y (v_1)^{n+1} \right)
\label{eq:pressureConditionFractional}
\end{align}
%
Again, equation~\eqref{eq:divConditionCoupled} was used to replace
$\partial_y (v_2)^{n+1} = -i k_x v_1^{n+1}.$
This condition replaces equation~\eqref{eq:v2ConditionCoupled}. 
Since the fluid velocity is no longer set in the heavy solid limit, 
we introduce the following projection condition for the fluid velocity.
\begin{align}
(v_2)^{n+1} = \alpha_F \left((v_2)^{n} 
- \frac{\dt }{\rho} \partial_y p^{n+1} 
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}) 
\right)
+ (1-\alpha_F) (\vs_2)^{n+1}_0.
\label{eq:velocityConditionFractional}
\end{align}
%
Here, $\alpha_F$ is chosen based on the fluid and solid impedances and is given by
\begin{align}
\alpha_F = \frac{\zf}{\zf+\zb}.
\end{align}
%
The fluid impedance is defined as $\zf = \rho c_f$ where $c_f$ is taken to be 
the sum of the viscous and inviscid contributions.
\begin{align}
c_f =  2 \mu k_x + \frac{1}{k_x \dt}
\end{align}
We can now summarize the fractional-step conditions.

\bigskip
\noindent \textbf{Fractional-step}:
\textit{ 
The following conditions are applied at $y=0$.
}
\begin{align}
&\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right) - \zb (v_1)^{n+1} 
= (\sigmas_{12})^{n+1}_0 - \zb (\vs_1)^{n+1}_0, \label{eq:fracTangential} \\
&-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} 
= (\sigmas_{22})^{n+1}_0 + 2 i k_x \mu  (v_1)^{n+1} 
- \zb \dt (\dot{\vs}_2)^{n+1}_0 
+\nu \zb \dt \left( -k_x^2 (v_2)^{n+1} + i k_x \partial_y (v_1)^{n+1} \right), 
\label{eq:fracPressure} \\
&(v_2)^{n+1} = \alpha_F \bigg{(} (v_2)^{n} 
- \frac{\dt }{\rho} \partial_y p^{n+1}
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}) 
\bigg{)} 
+ (1-\alpha_F) (\vs_2)^{n+1}_0.
\label{eq:fracProject}
\end{align}

The evolution of the solid requires boundary conditions for the two incoming 
characteristics at $y=0,$ namely 
\begin{align}
(\aone)_1^{n+1} &= (\sigma_{12})_I^{n+1}+ \zb (v_1)_I^{n+1}, \label{eq:a1CharBoundary}\\
(\atwo)_1^{n+1} &= (\sigma_{22})_I^{n+1}+ \zb (v_2)_I^{n+1}, \label{eq:a2CharBoundary}
\end{align}
%
where $(v_1)_I^{n+1}, (v_2)_I^{n+1}, (\sigma_{12})_I^{n+1}$, and $(\sigma_{22})_I^{n+1}$
are interface velocities and stresses projected from fluid and solid values, given by
\begin{align}
(v_1)_I^{n+1} &= \alpha_1 (v_{1})_f^{n+1} 
+ (1-\alpha_1) (\vs_1)_0^{n+1}
+ \gamma_1 \bar{z}^{-1} ( (\sigmas_{12})_0^{n+1} - (\sigma_{12})_f^{n+1}  ), \label{eq:project1}\\
(v_2)_I^{n+1} &= \alpha_2 (v_{2})_f^{n+1}
+ (1-\alpha_2) (\vs_2)_0^{n+1}
+ \gamma_2 \bar{z}^{-1} ( (\sigmas_{22})_0^{n+1} - (\sigma_{22})_f^{n+1}  ), \label{eq:project2}\\
(\sigma_{12})_I^{n+1} &= \beta_1 (\sigma_{12})_f^{n+1}
+ (1-\beta_1) (\sigmas_{12})_0^{n+1}
+ \delta_1 \bar{z} ( (\vs_1)_0^{n+1} - (v_1)_f^{n+1} ), \label{eq:project3}\\
(\sigma_{22})_I^{n+1} &= \beta_2 (\sigma_{22})_f^{n+1}
+ (1-\beta_2) (\sigmas_{22})_0^{n+1}
+ \delta_2 \bar{z} ( (\vs_2)_0^{n+1} - (v_2)_f^{n+1} ).\label{eq:project4}
\end{align}
%
Here, $(v_1)_f, (v_2)_f, (\sigma_{12})_f,$ and $(\sigma_{22})_f$ are fluid interface values
at $y=0.$
We are interested in choosing the projection coefficients
$(\alpha_i,\beta_i,\gamma_i,\delta_i)$ 
for $i=1,2,$ so the scheme is stable for all possible physical and numerical parameters.
These projections include jump terms scaled by the positive coefficients 
$(\gamma_i,\delta_i)$ which introduce dissipation that may 
stabilize a typically unstable problem. However, the coefficients
$(\alpha_i,\beta_i)$ can be chosen to stabilize the scheme 
even when the jump terms are absent (ie. $\gamma_i = \delta_i = 0$).  
Natural choices for these coefficients appear in the normal mode analysis.

\subsection{Stability analysis}

Next, we search for normal mode solutions to the discretization. In the fluid,
solutions are of the form,
\begin{align}
(v_1)^n(y) = A^n \hat{v}_1(y), \quad 
(v_2)^n(y) = A^n \hat{v}_2(y), \quad
p^n(y) = A^n \hat{p}(y),
\end{align}
%
where $A$ is the amplification factor and $\hat{v}_1(y), \hat{v}_2(y),$ and $\hat{p}$
are functions of space given by
\begin{align}
\hat{v}_1(y) &= \left((v_1)_f + \frac{i p_f}{z_\mu (\Gamma^2 - 1)} \right) e^{-k_x \Gamma y}
- \frac{i p_f}{z_\mu (\Gamma^2 - 1)} e^{-k_x y}, \\
\hat{v}_2(y) &= \left((v_2)_f - \frac{p_f}{z_\mu (\Gamma^2 - 1)} \right) e^{-k_x \Gamma y}
+ \frac{p_f}{z_\mu (\Gamma^2 - 1)} e^{-k_x y}, \\
\hat{p}(y) &= p_f e^{-k_x y}.
\end{align}
%
Here,
\begin{align}
z_\mu = \mu k, \qquad
\Gamma = \sqrt{\frac{1}{\Lambda}\frac{A-1}{A} + 1}, \qquad
\Lambda = \nu k^2 \dt.
\end{align}
%
$z_\mu$ is a measure of the fluid impedance and $\Lambda$ is a viscous CFL number.
The constants, $(v_1)_f, (v_2)_f$, and $p_f$ are obtained by
enforcing the three fluid boundary conditions (ie.
equations~\eqref{eq:v1ConditionCoupled}--\eqref{eq:divConditionCoupled} for the coupled scheme
or equations~\eqref{eq:fracTangential}--\eqref{eq:fracProject} for the fractional-step scheme)
 for each set of boundary conditions.
% \begin{align}
% (v_1)_f &= -\frac{(\Gamma^2+\Gamma) z_\mu + \zb}{ \zb E} b_1 
%           + \frac{i z_\mu (\Gamma-1)}{ \zb E} b_2 \\
% (v_2)_f &= -\frac{i z_\mu (\Gamma - 1)}{ \zb E} b_1 
%           - \frac{(\Gamma+1) z_\mu + \zb}{\zb E} b_2 \\
% p_f &= \frac{i (2 \Gamma Z + 1) (\Gamma + 1) Z}{E} b_1
%       - \frac{(\Gamma+1) (\Gamma^2 Z + \Gamma + Z) Z}{E} b_2
% \end{align}

% \begin{align}
% E = (\Gamma^3 + \Gamma^2 + 3 \Gamma - 1) Z^2 + (\Gamma+1)^2 Z + 1
% \end{align}

We now search for solutions to the solid discretization. 
Let $\av_j^n = [(\aone)_j^n, (\bone)_j^n, (\atwo)_j^n, (\btwo)_j^n, (d)_j^n]^T.$
Solutions are sought of the form, $\av_j^n =  \phi^j A^n \rv,$
where $\phi$ is a spacial eigenvalue and $\rv$ is
a constant vector. As in the inviscid analysis, our approach for determining 
regions of instability is to search for unstable modes assuming $|A|>1$ and 
find regions of the parameter space where non-trivial solutions exist.
When the normal mode ansatz is substituted into the numerical scheme for the solid in 
equations \eqref{eq:schemeA1}--\eqref{eq:schemeD}, a homogeneous system arises of the form
% what should we call this matrix?
\newcommand{\SolidMatrixB}{Q}
\begin{align}
\SolidMatrixB(\phi) \rv = 0.
\end{align}
The matrix $\SolidMatrixB(\phi)$ is given by
\begin{align*}
\SolidMatrixB(\phi) = \left[\begin{array}{ccccc}
\eta(\phi) & 0 &  0& -i A \lx & i A \lx  \\
0 & \eta(1/\phi) & i A \lx & 0 & -i A \lx \\
0 & i A \lx & \eta(\phi) & 0 & 0 \\
-i A \lx & 0 & 0 & \eta(1/\phi) & 0 \\
0 & 0 & 0 & 0 & 1-A
\end{array}\right],
\end{align*}
%
where
\begin{align}
\eta(\phi) = 1-A+\ly (\phi-1).
\end{align}
%
This system is singular when $f(\phi) \defeq \det (\SolidMatrixB(\phi)) = 0.$
The function $f(\phi)$ can be written as 
\begin{align}
f(\phi) = (1-A) \left(\eta(\phi) \eta(1/\phi) + (A \lx)^2\right)^2,
\label{eq:SolidDetCond}
\end{align}
%
which is zero when $A=1$ or when $\eta(\phi) \eta(1/\phi) + (A \lx)^2 = 0.$
Since we are interested in searching for unstable modes, we are interested in the latter 
case. Roots of $f(\phi)$ can be written in the form
\newcommand{\bParam}{\theta}
\begin{align}
\phi_\pm = \bParam \pm \sqrt{\bParam^2 - 1}, \qquad 
\bParam = 1 - \frac{(A \lx)^2 + (1-A)^2}{2 \ly (1-A-\ly)}.
\end{align}
%
We note that the product of the roots is one ($\phi_+ \phi_- = 1$).
Under the assumption $|A|>1,$ there will always be one root 
$\phi = \phi_*$ such that $|\phi_*| > 1.$ 
%
When $\phi=\phi_*,$ there are two eigenvectors, namely
\begin{align}
\rv_1 = 
\left[
\frac{\eta(1/\phi_*)}{i A\lx},\, 0,\, 0,\, 1,\, 0
\right]^T, \qquad 
\rv_2 = 
\left[
0,\, -\frac{\eta(\phi_*)}{i A\lx},\, 1,\, 0,\, 0
\right]^T
.
\end{align}
%
The solution which remains bounded as $j \rightarrow -\infty$ is given by
\begin{align*}
(\aone)_j^{n} = k_1 \frac{ \eta(1/\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
(\bone)_j^{n} = -k_2 \frac{ \eta(\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
(\atwo)_j^{n} = k_2 \phi_*^{j-1} A^n, \quad
(\btwo)_j^{n} = k_1 \phi_*^{j-1} A^n,
\end{align*}
%
where $k_1$ and $k_2$ are free constants to be determined by the interface conditions.
The discrete solutions are plugged into the boundary conditions, equations
\eqref{eq:a1CharBoundary}--\eqref{eq:a2CharBoundary},
to form another homogeneous system of equations, given by
\begin{align}
G(A) \kv = \left[\begin{array}{cc}
g_{11} & g_{12} \\ 
g_{21} & g_{22}
\end{array}\right]
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right]
= 0.
\end{align}
%
Solutions for the amplification factor are roots of 
\begin{align}
g(A) = \det(G(A)) = g_{11} g_{22} - g_{12} g_{21} = 0.
\label{eq:ViscousDet}
\end{align}
%
Although there are eight total projection coefficients 
$(\alpha_i,\beta_i,\gamma_i,\delta_i)$ for $i=1,2,$ the coefficients of $G$ only depend on three 
combinations of these coefficients, given by
\begin{align}
\psi_1 = \alpha_1 + \beta_1 - \gamma_1 - \delta_1, \qquad
\psi_2 = \alpha_2 + \beta_2 - \gamma_2 - \delta_2, \qquad
\psi_3 = \alpha_2-\delta_2.
\end{align}
%
In fact, when the coefficients are chosen so that $\psi_1=\psi_2=\psi_3=0,$ the matrix $G$
is diagonal. Here are four possible configurations.
\begin{align*}
\{\text{match jump terms: }  \alpha_j=\delta_j,\; \beta_j=\gamma_j,\; j=1,2 \} , 
\quad&\Rightarrow\quad \psi_1=\psi_2=\psi_3=0\\
\{\text{use solid, no jump: }  \alpha_j=\beta_j=\delta_j=\gamma_j=0,\; j=1,2  \},
\quad&\Rightarrow\quad \psi_1=\psi_2=\psi_3=0\\
\{\text{IWA, no jump: }  \alpha_j+\beta_j=1,\; \alpha_2=\alpha_F,\; \delta_j=\gamma_j=0,\; j=1,2  \}
\quad&\Rightarrow\quad \psi_1=\psi_2=1, \psi_3=\alpha_F\\
\{\text{use fluid, no jump: }  \alpha_j=\beta_j=1,\; \delta_j=\gamma_j=0,\; j=1,2  \}
\quad&\Rightarrow\quad \psi_1=\psi_2=2, \psi_3=1
\end{align*}
%
``Use solid'' and ``use fluid'' refer to using only the solid or fluid interface values in 
equations~\eqref{eq:project1}--\eqref{eq:project2}. ``IWA'' stands for impedance-weighted average.
By matching the coefficients of the jump terms, the FSI stability problem is equivalent to the
uncoupled solid problem. However, when jump terms are not used, the projection weights can
be chosen to produce a stable scheme.

Solutions for the amplification factor are the roots of the transcendental equation $g(A) = 0.$
The argument principle can be used to determine the number of unstable roots.
\begin{align}
\int_C \frac{g'(z)}{g(z)} \; dz
= 2 \pi i \left( n_{\text{roots}} - n_{\text{poles}} \right)
\end{align}
%
To determine the number of stable roots $|A| \le 1$, 
we integrate over the unit circle given by
\begin{alignat}{2}
z(\theta) &= e^{i \theta},\quad && \theta \in [0, 2 \pi].
\end{alignat}
%
In order to determine the total number of roots,
we integrate around a large circle of radius, $R$,
\begin{align}
z = R e^{i \theta}.
\end{align}
%
We take $R=?.$
If the total number of roots is equivalent to the number of stable roots, then the scheme is 
stable. Otherwise the scheme is unstable. 
Stability was assessed for 20 logarithmically spaced points in parameter space 
for $\Lambda$ and $Z$ 
in the interval $[10^{-3}, 10^{3}].$
For each pair of parameters, we take the max over the CFL region.
Figure \ref{fig:argPrinciple} shows the results of this computation.  
There will be results for fractional and non-fractional-step schemes with different 
choices of projection coefficients.
\das{finish me}

\begin{figure}[h]
\centering
\includegraphics[width=.4\textwidth]{fig/iBC1_psi0_theta1_lxp1_lyp1.png}
\includegraphics[width=.4\textwidth]{fig/iBC1_psi1_theta1_lxp1_lyp1.png}
\includegraphics[width=.4\textwidth]{fig/iBC1_psi2_theta1_lxp1_lyp1.png}
\includegraphics[width=.4\textwidth]{fig/iBC2_psi0_theta0_lxp1_lyp1.png}
\includegraphics[width=.4\textwidth]{fig/iBC2_psi1_theta0_lxp1_lyp1.png}
\includegraphics[width=.4\textwidth]{fig/iBC2_psi2_theta0_lxp1_lyp1.png}
\caption{
  I fixed $\lx=\ly=.1$ and varied the scheme (non-fractional-step: \texttt{iBC=1}, 
  fractional-step: \texttt{iBC=2}) and choice of projection weights ($\psi=0,1,2$).
  The only case that goes unstable is the bottom right, when the fluid values are used
  instead of a projection in equations~\eqref{eq:project1}--\eqref{eq:project4}.
  \label{fig:argPrinciple}
}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=.4\textwidth]{fig/iBC3_psi2_theta0_lxp1_lyp1.png}
\includegraphics[width=.4\textwidth]{fig/iBC4_psi2_theta0_lxp1_lyp1.png}
\caption{
  Left: traditional. Right: anti-traditional.
  \label{fig:argPrinciple}
}
\end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=\textwidth]{fig/ViscousContinuation_NL200_NZ50_nonfrac}
% \caption{Magnitude of maximum amplification factor for non-fractional-step scheme.
%   \das{Looks OK except for a point in the middle...}}
% \end{figure}



==> texFiles/viscousAnalysisOld3.tex <==
\section{Viscous analysis} \label{sec:viscousAnalysis}

In this section, the stability of the AMP, TP, and ATP algorithms 
are explored for model problem MP-VA.
This extends the analysis of the inviscid model problem in~\cite{fib2014} to 
a viscous model problem. 
When viscosity is involved, stability is more challenging since instabilities 
arise from both added mass and added damping effects.
Due to this, both horizontal and vertical motions in the solid must be considered.
This relaxes the assumption in~\cite{fib2014} where the model problem was constrained 
to vertical motions only.
Another difficulty is the introduction of the viscous CFL number in the fluid as a 
new dimensionless parameter. 
In Section~\ref{sec:monolithic}, a fluid impedance was derived which is a function of 
the viscous CFL number. This impedance is used in the interface projection step of the 
AMP algorithm and is critical to achieving stability.

Consider model problem MP-VA. 
The geometry of this model problem is shown in Figure \ref{fig:rectangularModelProblemCartoon}
and discussed in Section~\ref{sec:FSIModelProblems}.
The fluid is taken to be semi-infinite ($H \rightarrow \infty$).
The governing equations for the fluid solid are given by \eqref{eq:mpvaEquations}.
For the solid, these equations are considered in characteristic form by taking the
transformations in \eqref{eq:CharDef} to obtain \eqref{eq:advA1}--\eqref{eq:advB2}.

\subsection{Discretization}

As in Section~\ref{sec:monolithic}, the solution is represented as a discrete Fourier series
in the transverse direction (ie. equation~\eqref{eq:discreteFourier}).
The equations for the fluid Fourier coefficients are given by 
\eqref{eq:fourierV1}--\eqref{eq:fourierV2}. The equations for the solid Fourier coefficients are
given by
\begin{alignat}{2}
\partial_t \aone - \bar{c} \partial_y \aone &= \bar{c} i k_x ( d - \btwo),
\label{eq:advA1Fourier}\\
\partial_t \bone + \bar{c} \partial_y \bone &= \bar{c} i k_x ( \atwo -  d),
\\
\partial_t \atwo - \bar{c} \partial_y \atwo &= \bar{c} i k_x \bone, 
\\
\partial_t \btwo + \bar{c} \partial_y \btwo &= - \bar{c} i k_x \aone,
\\
\partial_t d &= 0.
\label{eq:advDFourier}
\end{alignat}
%
Here, the normalized wave number is $k_x = 2 \pi k /L.$
The fluid is discretized in time and kept continuous in space. 
The temporal grid spacing is defined by $t_n = n \dt,$ with time step $\dt.$
The fluid scheme is a first-order Euler type scheme given by
\begin{align}
(v_1)^{n+1} &= (v_1)^n 
- \frac{i k_x \dt}{\rho} p^{*}
+ \nu \dt \left( - k_x^2 + \partial_y^2  \right) (v_1)^{n+1}, \label{eq:viscousV1}\\
(v_2)^{n+1} &= (v_2)^n 
- \frac{\dt}{\rho} \partial_y p^{*}
+ \nu \dt \left( - k_x^2 + \partial_y^2\right) (v_2)^{n+1}, \label{eq:viscousV2}\\
\left(-k_x^2 + \partial_y^2\right) p^{n+1} &= 0 .\label{eq:viscousP}
\end{align}
%
The viscous terms are treated implicitly and the pressure gradient terms 
can either be treated implicitly ($p^*=p^{n+1}$) or explicitly ($p^*=p^n$).
The latter case corresponds to an IMEX discretization.
As in Section~\ref{sec:monolithic}, this is a system of differential-difference equations.
We enforce that the fluid velocity is bounded as $y\rightarrow\infty$.
Additionally, three conditions at the interface are required to close the system.

The solid characteristic variables are discretized in the $y$-direction using a
uniform staggered grid, defined by $y_j = \left(j-\frac{1}{2}\right) \dy$ for
$j = 1,0,-1,\dots$ with grid spacing $\dy$.
The solid equations in~\eqref{eq:advA1Fourier}--\eqref{eq:advDFourier} are approximated using a 
first-order accurate upwind-type scheme given by
\begin{align}
(\aone)_j^{n+1} &= (\aone)_j^n + \ly ((\aone)_{j+1}^n-(\aone)_{j}^n) + i \lx ((d)_{j}^{n+1} - (\btwo)_{j}^{n+1}) \label{eq:schemeA1}\\
(\bone)_j^{n+1} &= (\bone)_j^n - \ly ((\bone)_{j}^n-(\bone)_{j-1}^n) + i \lx ((\atwo)_{j}^{n+1} - (d)_{j}^{n+1}) \label{eq:schemeB1}\\
(\atwo)_j^{n+1} &= (\atwo)_j^n + \ly ((\atwo)_{j+1}^n-(\atwo)_{j}^n) + i \lx (\bone)_{j}^{n+1} \label{eq:schemeA2}\\
(\btwo)_j^{n+1} &= (\btwo)_j^n - \ly ((\btwo)_{j}^n-(\btwo)_{j-1}^n) - i \lx (\aone)_{j}^{n+1} \label{eq:schemeB2}\\
(d)_j^{n+1} &= (d)_j^n, \label{eq:schemeD}
\end{align}
%
where $\lx = \kx \bar{c} \dt$ and $\ly = \bar{c} \dt / \dy.$ 
The terms involving transverse derivatives are treated implicitly to stabilize the 
pseudo-spectral approximation. For reference, the solid velocity and stress 
are related to the characteristic variables by
\begin{align}
(\vs_1)_j^n = \frac{1}{2 \bar{z}} \left( (\aone)_j^n - (\bone)_j^n \right), \quad
(\vs_2)_j^n = \frac{1}{2 \bar{z}} \left( (\atwo)_j^n - (\btwo)_j^n \right), \label{eq:solidGridVelocity}\\
(\sigmas_{12})_j^n = \frac{1}{2 } \left( (\aone)_j^n + (\bone)_j^n \right), \quad 
(\sigmas_{22})_j^n = \frac{1}{2 } \left( (\atwo)_j^n + (\btwo)_j^n \right). \label{eq:solidGridStress}
\end{align}
%
We enforce that the solid solution remains bounded as $y\rightarrow -\infty$.
This implies
\begin{align}
|(\aone)_j^n|^2 +  |(\bone)_j^n|^2 + |(\atwo)_j^n|^2 + |(\btwo)_j^n|^2 < \infty,
\quad \text{ as } j \rightarrow -\infty.
\end{align}

\subsection{Interface coupling}

We explore different choices of interface coupling for the AMP, TP, and ATP schemes.
Furthermore in the fluid we distinguish between a 
\textit{fully-coupled scheme}, where the velocity and 
pressure are solved in the same step, and a 
\textit{fractional-step scheme}, where the velocity and pressure are solved separately.
For the fully-coupled scheme, the pressure gradient terms are treated implicitly ($p^*=p^{n+1}$)  
in equations \eqref{eq:viscousV1}--\eqref{eq:viscousV2}.
On the other hand for the fractional-step scheme, the pressure gradient terms are
treated explicitly ($p^*=p^{n}$).

First consider the AMP interface conditions for the fully-coupled scheme.
The first two conditions are formed by equating the two outgoing solid characteristic
to the analogous fluid quantities using equations
\eqref{eq:BCharacteristic}--\eqref{eq:BmCharacteristic}.
The third condition is obtained by setting the velocity to be divergence-free on the interface.

\bigskip
\noindent \textbf{Fully-coupled AMP conditions}: 
\textit{The pressure gradient terms are treated implicitly ($p^*=p^{n+1}$)
  and the following conditions are applied at $y=0$.}
\begin{align}
\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right) - \zb (v_1)^{n+1} 
&= (\sigmas_{12})^{n+1}_0 - \zb (\vs_1)^{n+1}_0, \label{eq:v1ConditionCoupled} \\
-p^{n+1} + 2 \mu \partial_y (v_2)^{n+1} - \zb (v_2)^{n+1} 
&= (\sigmas_{22})^{n+1}_0 - \zb (\vs_2)^{n+1}_0, \label{eq:v2ConditionCoupled}\\
i k_x (v_1)^{n+1} + \partial_y (v_2)^{n+1} 
&= 0. \label{eq:divConditionCoupled}
\end{align}

Next we derive fractional-step boundary conditions which decouple 
the fluid velocity and pressure at the interface. 
Equation~\eqref{eq:v2ConditionCoupled} sets the fluid velocity in the heavy solid limit
and the pressure in the light solid limit. 
A decoupled pressure condition can be derived from 
equation~\eqref{eq:v2ConditionCoupled} and 
equation~\eqref{eq:divConditionCoupled}.
The first condition can be derived by eliminating $(v_2)^{n+1}$ and
$(\vs_2)^{n+1}_0$ in equation~\eqref{eq:v2ConditionCoupled} using a backward-Euler type scheme.
\begin{align}
(v_2)^{n+1} &= \tilde{v}_2
- \frac{\dt }{\rho} \partial_y p^{n+1} 
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}),\\
(\vs_2)^{n+1}_0 &= \tilde{v}_2
+ \dt (\dot{\vs}_2)^{n+1}_0
\end{align}
%
Here, 
equation~\eqref{eq:divConditionCoupled} was used to make the substitution
$\partial_y^2 (v_2)^{n+1} = -i k_x \partial_y (v_1)^{n+1}$ and 
$(\dot{\vs}_2)$ represents the solid interface acceleration. 
The scheme is centered around $\tilde{v}_2,$ which is taken to be an 
interface velocity at time $t^{n}.$
After substitution, a mixed condition for the pressure is derived.
\begin{align}
-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} 
=\;& (\sigmas_{22})^{n+1}_0 + 2 i k_x \mu  (v_1)^{n+1} 
- \zb \dt (\dot{\vs}_2)^{n+1}_0 \nonumber \\
&
+\nu \zb \dt \left( -k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1} \right)
\label{eq:pressureConditionFractional}
\end{align}
%
Again, equation~\eqref{eq:divConditionCoupled} was used to replace
$\partial_y (v_2)^{n+1} = -i k_x v_1^{n+1}.$
This condition replaces equation~\eqref{eq:v2ConditionCoupled}. 
Since the fluid velocity is no longer set in the heavy solid limit, 
we introduce the following projection condition for the fluid velocity.
\begin{align}
(v_2)^{n+1} = \alpha_F \left((v_2)^{n} 
- \frac{\dt }{\rho} \partial_y p^{n} 
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}) 
\right)
+ (1-\alpha_F) (\vs_2)^{n+1}_0.
\label{eq:velocityConditionFractional}
\end{align}
%
That is, the fluid velocity on the interface is set to be a weighted average of the 
velocity predicted from the fluid scheme and the predicted solid velocity.
Here, $\alpha_F$ is chosen based on the fluid and solid impedances and is given by
\begin{align}
\alpha_F = \frac{\zf}{\zf+\zb},
\end{align}
%
where the fluid impedance $\zf$ is taken to be
\begin{align}
\zf = \rho v_f, \qquad v_f = 2\nu k_x + \frac{1}{k_x \dt},
\end{align}
%
as derived in Section~\ref{sec:monolithic}.
We can now summarize the fractional-step conditions.

\bigskip
\noindent \textbf{Fractional-step AMP conditions}: \textit{The pressure gradient terms are treated explicitly ($p^* = p^{n}$)
and the following conditions are applied at $y=0$.
}
\begin{align}
&\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right) - \zb (v_1)^{n+1} 
= (\sigmas_{12})^{n+1}_0 - \zb (\vs_1)^{n+1}_0, \label{eq:fracTangential} \\
&(v_2)^{n+1} = \alpha_F \bigg{(} (v_2)^{n} 
- \frac{\dt }{\rho} \partial_y p^{n+1}
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}) 
\bigg{)} \nonumber \\
&\phantom{(v_2)^{n+1} =\;}
+ (1-\alpha_F) (\vs_2)^{n+1}_0.
\label{eq:fracProject}\\
&-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} 
= (\sigmas_{22})^{n+1}_0 + 2 i k_x \mu  (v_1)^{n+1} 
- \zb \dt (\dot{\vs}_2)^{n+1}_0 \nonumber \\
&
\phantom{-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} =\;}
+\nu \zb \dt \left( -k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1} \right)
\label{eq:fracPressure} 
\end{align}
%
Analogous conditions for the TP and ATP scheme can be formed by taking the proper 
limits of equations~\eqref{eq:fracTangential}--\eqref{eq:fracProject}.
In the heavy solid limit, equations~\eqref{eq:fracTangential}--\eqref{eq:fracProject}
become Dirichlet conditions for the velocity and equation~\eqref{eq:fracPressure}
becomes a Neumann compatibility condition for the pressure.

\bigskip
\noindent \textbf{Fractional-step TP conditions}: \textit{The pressure gradient terms are treated explicitly ($p^* = p^{n}$)
and the following conditions are applied at $y=0$.
}
\begin{align}
(v_1)^{n+1} 
&=  (\vs_1)^{n+1}_0, \label{eq:TPTangential} \\
(v_2)^{n+1} &= (\vs_2)^{n+1}_0.
\label{eq:TPNormal} \\
\partial_y p^{n+1} 
&= 
- (\dot{\vs}_2)^{n+1}_0 
+\nu \left( -k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1} \right)
\label{eq:TPPressure} 
\end{align}

In the light solid limit, equation~\eqref{eq:fracTangential}
becomes a condition on the tangential stress.
Equation~\eqref{eq:fracProject} reduces to the numerical scheme for 
$(v_2)^{n+1}$ with the modification $\partial_y^2(v_2)^{n+1} = - i k_x \partial_y (v_1)^{n+1}$.
In the ATP scheme, the divergence free condition is enforced,
$\partial_y(v_2)^{n+1} = - i k_x (v_1)^{n+1}.$
Equation~\eqref{eq:fracPressure}
simplifies to a Dirichlet condition for the pressure.

\bigskip
\noindent \textbf{Fractional-step ATP conditions}: \textit{The pressure gradient terms are treated explicitly ($p^* = p^{n}$) and the following conditions are applied at $y=0$.
}
\begin{align}
\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right)
&= (\sigmas_{12})^{n+1}_0, \label{eq:ATPV1} \\
i k_x (v_1)^{n+1} + \partial_y (v_2)^{n+1} 
&= 0. \label{eq:ATPDiv}\\
-p^{n+1} + 2 \mu \partial_y (v_2)^{n+1} 
&= (\sigmas_{22})^{n+1}_0, \label{eq:ATPP}
\end{align}



The evolution of the solid requires boundary conditions for the two incoming 
characteristics at $y=0,$ namely 
\begin{align}
(\aone)_1^{n+1} &= (\sigma_{12})_I^{n+1}+ \zb (v_1)_I^{n+1}, \label{eq:a1CharBoundary}\\
(\atwo)_1^{n+1} &= (\sigma_{22})_I^{n+1}+ \zb (v_2)_I^{n+1}, \label{eq:a2CharBoundary}
\end{align}
%
where $(v_1)_I^{n+1}, (v_2)_I^{n+1}, (\sigma_{12})_I^{n+1}$, and $(\sigma_{22})_I^{n+1}$
are interface velocities and stresses projected from fluid and solid values, given by
\begin{align}
(v_1)_I^{n+1} &= \alpha (v_{1})_f^{n+1} 
+ (1-\alpha) (\vs_1)_0^{n+1}
+ \gamma_1 \bar{z}^{-1} ( (\sigmas_{12})_0^{n+1} - (\sigma_{12})_f^{n+1}  ), \label{eq:project1}\\
(v_2)_I^{n+1} &= \alpha (v_{2})_f^{n+1}
+ (1-\alpha) (\vs_2)_0^{n+1}
+ \gamma \bar{z}^{-1} ( (\sigmas_{22})_0^{n+1} - (\sigma_{22})_f^{n+1}  ), \label{eq:project2}\\
(\sigma_{12})_I^{n+1} &= \beta (\sigma_{12})_f^{n+1}
+ (1-\beta) (\sigmas_{12})_0^{n+1}
+ \delta \bar{z} ( (\vs_1)_0^{n+1} - (v_1)_f^{n+1} ), \label{eq:project3}\\
(\sigma_{22})_I^{n+1} &= \beta (\sigma_{22})_f^{n+1}
+ (1-\beta) (\sigmas_{22})_0^{n+1}
+ \delta \bar{z} ( (\vs_2)_0^{n+1} - (v_2)_f^{n+1} ).\label{eq:project4}
\end{align}
% \begin{align}
% (v_1)_I^{n+1} &= \alpha_1 (v_{1})_f^{n+1} 
% + (1-\alpha_1) (\vs_1)_0^{n+1}
% + \gamma_1 \bar{z}^{-1} ( (\sigmas_{12})_0^{n+1} - (\sigma_{12})_f^{n+1}  ), \label{eq:project1}\\
% (v_2)_I^{n+1} &= \alpha_2 (v_{2})_f^{n+1}
% + (1-\alpha_2) (\vs_2)_0^{n+1}
% + \gamma_2 \bar{z}^{-1} ( (\sigmas_{22})_0^{n+1} - (\sigma_{22})_f^{n+1}  ), \label{eq:project2}\\
% (\sigma_{12})_I^{n+1} &= \beta_1 (\sigma_{12})_f^{n+1}
% + (1-\beta_1) (\sigmas_{12})_0^{n+1}
% + \delta_1 \bar{z} ( (\vs_1)_0^{n+1} - (v_1)_f^{n+1} ), \label{eq:project3}\\
% (\sigma_{22})_I^{n+1} &= \beta_2 (\sigma_{22})_f^{n+1}
% + (1-\beta_2) (\sigmas_{22})_0^{n+1}
% + \delta_2 \bar{z} ( (\vs_2)_0^{n+1} - (v_2)_f^{n+1} ).\label{eq:project4}
% \end{align}
%
Here, $(v_1)_f, (v_2)_f, (\sigma_{12})_f,$ and $(\sigma_{22})_f$ are fluid interface values at $y=0.$
The choice of projection coefficients $(\alpha,\beta,\gamma,\delta)$ 
is determined by the choice of interface coupling and is shown in 
Table~\ref{tab:projectionCoeffs}.
For the AMP scheme, coefficients are chosen according to the impedance weighted average formula. 
For the TP scheme, coefficients are chosen so the interface velocity is taken to be the
solid velocity and the interface traction is taken to be the fluid traction.
For the ATP scheme, coefficients are chosen so the interface velocity is taken to be the
fluid velocity and the interface traction is taken to be the solid traction.

{
\begin{table}[h]
\centering
\caption{Choice of projection coefficients for the AMP, TP, and ATP schemes.
\label{tab:projectionCoeffs}}
\begin{tabular}{c|cccc}
scheme & $\alpha$ & $\beta$ & $\gamma$ & $\delta$ \\
\hline
AMP & $\frac{\zf}{\zf+\zb}$ & $\frac{\zf^{-1}}{\zf^{-1}+\zb^{-1}}$ & $\frac{\zf^{-1}}{\zf^{-1}+\zb^{-1}}$ & $\frac{\zf}{\zf+\zb}$\\
TP & $0$ & $1$ & $0$ & $0$ \\
ATP & $1$ & $0$ & $0$ & $0$
\end{tabular}
\end{table}
}


\subsection{Stability analysis}

Next, we search for normal mode solutions to the discretization. In the fluid,
solutions are of the form,
\begin{align}
(v_1)^n(y) = A^n \hat{v}_1(y), \quad 
(v_2)^n(y) = A^n \hat{v}_2(y), \quad
p^n(y) = A^n \hat{p}(y),
\end{align}
%
where $A$ is the amplification factor and $\hat{v}_1(y), \hat{v}_2(y),$ and $\hat{p}$
are functions of space given by
\begin{align}
\hat{v}_1(y) &= \left((v_1)_f + \frac{i p_f}{z_\mu A (\gamma^2 - 1)} \right) e^{-k_x \gamma y}
- \frac{i p_f}{z_\mu A(\gamma^2 - 1)} e^{-k_x y}, \\
\hat{v}_2(y) &= \left((v_2)_f - \frac{p_f}{z_\mu A(\gamma^2 - 1)} \right) e^{-k_x \gamma y}
+ \frac{p_f}{z_\mu A (\gamma^2 - 1)} e^{-k_x y}, \\
\hat{p}(y) &= p_f e^{-k_x y}.
\end{align}
%
Here, $\zm,\, \Lambda,$ and $\gamma$ take on similar definitions in 
Section~\ref{sec:monolithic} and are given by
\begin{align}
z_\mu = \mu k, \qquad
\Lambda = \nu k^2 \dt, \qquad
\gamma = \sqrt{\frac{1}{\Lambda}\frac{A-1}{A} + 1}.
\end{align}
%
As before, $z_\mu$ is a viscous impedance and $\Lambda$ is a viscous CFL number.
The constants, $(v_1)_f, (v_2)_f$, and $p_f$ are obtained by
enforcing the three fluid boundary conditions (ie.
equations~\eqref{eq:v1ConditionCoupled}--\eqref{eq:divConditionCoupled} for the fully-coupled 
AMP scheme,
equations~\eqref{eq:fracTangential}--\eqref{eq:fracPressure} for the fractional-step AMP scheme,
equations~\eqref{eq:TPTangential}--\eqref{eq:TPPressure} for the fractional-step TP scheme,
or
equations~\eqref{eq:ATPV1}--\eqref{eq:ATPP} for the fractional-step ATP scheme)
for each set of boundary conditions.

% \begin{align}
% (v_1)_f &= -\frac{(\gamma^2+\gamma) z_\mu + \zb}{ \zb E} b_1 
%           + \frac{i z_\mu (\gamma-1)}{ \zb E} b_2 \\
% (v_2)_f &= -\frac{i z_\mu (\gamma - 1)}{ \zb E} b_1 
%           - \frac{(\gamma+1) z_\mu + \zb}{\zb E} b_2 \\
% p_f &= \frac{i (2 \gamma Z + 1) (\gamma + 1) Z}{E} b_1
%       - \frac{(\gamma+1) (\gamma^2 Z + \gamma + Z) Z}{E} b_2
% \end{align}

% \begin{align}
% E = (\gamma^3 + \gamma^2 + 3 \gamma - 1) Z^2 + (\gamma+1)^2 Z + 1
% \end{align}

We now search for solutions to the solid discretization. 
Let $\av_j^n = [(\aone)_j^n$,$ (\bone)_j^n$, $(\atwo)_j^n$, $(\btwo)_j^n$,$ (d)_j^n]^T.$
Solutions are sought of the form, $\av_j^n =  \phi^j A^n \rv,$
where $\phi$ is a spacial eigenvalue, $\rv$ is a constant vector, and $A$ is an amplification 
factor. 
The scheme is said to be weakly stable if there are no non-trivial solutions with $|A| > 1$.  
Our strategy for determining regions of stability will be to search for unstable modes with 
$|A| > 1$, and then identify regions of the parameter space where no non-trivial solution exist.  
To do this, we begin by finding the general solution for the spatial grid functions satisfying 
the discrete equations and regularity condition as $j\rightarrow-\infty$, assuming $|A| > 1$.  
We then apply the conditions at the interface to determine whether non-trivial solutions exist.
When the normal mode ansatz is substituted into the numerical scheme for the solid in 
equations \eqref{eq:schemeA1}--\eqref{eq:schemeD}, a homogeneous system arises of the form
% what should we call this matrix?
\newcommand{\SolidMatrixB}{Q}
\begin{align}
\SolidMatrixB(\phi) \rv = 0.
\end{align}
The matrix $\SolidMatrixB(\phi)$ is given by
\begin{align*}
\SolidMatrixB(\phi) = \left[\begin{array}{ccccc}
\eta(\phi) & 0 &  0& -i A \lx & i A \lx  \\
0 & \eta(1/\phi) & i A \lx & 0 & -i A \lx \\
0 & i A \lx & \eta(\phi) & 0 & 0 \\
-i A \lx & 0 & 0 & \eta(1/\phi) & 0 \\
0 & 0 & 0 & 0 & 1-A
\end{array}\right],
\end{align*}
%
where
\begin{align}
\eta(\phi) = 1-A+\ly (\phi-1).
\end{align}
%
This system is singular when $f(\phi) \defeq \det (\SolidMatrixB(\phi)) = 0.$
The function $f(\phi)$ can be written as 
\begin{align}
f(\phi) = (1-A) \left(\eta(\phi) \eta(1/\phi) + (A \lx)^2\right)^2,
\label{eq:SolidDetCond}
\end{align}
%
which is zero when $A=1$ or when $\eta(\phi) \eta(1/\phi) + (A \lx)^2 = 0.$
Since we are interested in searching for unstable modes, we are interested in the latter 
case. Roots of $f(\phi)$ can be written in the form
\newcommand{\bParam}{\theta}
\begin{align}
\phi_\pm = \bParam \pm \sqrt{\bParam^2 - 1}, \qquad 
\bParam = 1 - \frac{(A \lx)^2 + (1-A)^2}{2 \ly (1-A-\ly)}.
\end{align}
%
The product of the roots is equal to one ($\phi_+ \phi_- = 1$).
Since we are searching for solutions that are bounded as $j\rightarrow -\infty,$ 
we are only interested in the root with modulus greater than 1.

\medskip
\noindent\textbf{Lemma}: \textit{If $|A|>1$ and if $\lx$ and $\ly$ are chosen to satisfy a CFL 
condition, then there is precisely one root (either $\phi_+$ or $\phi_-$), denoted by 
$\phi_*$ that has magnitude strictly greater than one, $|\phi_*| > 1.$}
\medskip

This result follows from a similar argument to that given 
in~\cite{DifferenceApproximationsForTheInitialBoundary}.  
We first consider the scheme applied to the pure initial-value problem (Cauchy problem).  
Setting $\phi=e\sp{i\vartheta}$ in~\eqref{eq:quarticPhi}, we determine a region of 
the $\lx$-$\ly$ plane for which $\vert A\vert\le1$ for all $\vartheta\in[0,2\pi]$.  
This region is found numerically as discussed in~\ref{sec:CFLRegionCauchy}, and it corresponds 
to a region where the Cauchy problem is (Fourier) stable.  It is also shown that this stability 
region includes a region of $(\lx,\ly)$ satisfying a reasonable CFL restriction, 
namely $\lx\sp2+\ly\sp2\le1$.
Next, since $|A| \le 1$ when $|\phi| = 1$, we have that $|\phi| \ne 1$ when $|A| > 1$.  
Thus, if $|A| > 1$ and if $(\lx,\ly)$ remains within the CFL restriction, then $\phi$ cannot 
cross the unit circle, $|\phi|=1$, as $(\lx,\ly)$ vary.  It is therefore only necessary to 
prove that the conditions on the roots in~\eqref{eq:SizeOfEigenvalues} hold for one set of 
parameters.  
For $\lx=0$, the discretization reduces to four uncoupled upwind schemes for linear advection. 
In this case, equation~\eqref{eq:SolidDetCond} is equivalent to 
$\eta(\phi) \eta(1/\phi) = 0,$
%
which has solutions
$\phi_+ = (A-1+\ly)/\ly$ and $\phi_- = 1/\phi_+$.
%
When $|A|>1$ and $\ly \in (0,1]$, $|\phi_+|>1$ and therefore $\phi_* = \phi_+.$ 
Thus, the condition holds for all $(\lx,\ly)$ provided the CFL condition is satisfied.

%
When $\phi=\phi_*,$ there are two eigenvectors, namely
\begin{align}
\rv_1 = 
\left[
\frac{\eta(1/\phi_*)}{i A\lx},\, 0,\, 0,\, 1,\, 0
\right]^T, \qquad 
\rv_2 = 
\left[
0,\, -\frac{\eta(\phi_*)}{i A\lx},\, 1,\, 0,\, 0
\right]^T
.
\end{align}
%
The solution which remains bounded as $j \rightarrow -\infty$ is given by
\begin{align*}
(\aone)_j^{n} = k_1 \frac{ \eta(1/\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
(\bone)_j^{n} = -k_2 \frac{ \eta(\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
(\atwo)_j^{n} = k_2 \phi_*^{j-1} A^n, \quad
(\btwo)_j^{n} = k_1 \phi_*^{j-1} A^n,
\end{align*}
%
where $k_1$ and $k_2$ are free constants to be determined by the interface conditions.
The discrete solutions are plugged into the boundary conditions, equations
\eqref{eq:a1CharBoundary}--\eqref{eq:a2CharBoundary},
to form another homogeneous system of equations, given by
\begin{align}
G(A) \kv = \left[\begin{array}{cc}
g_{11} & g_{12} \\ 
g_{21} & g_{22}
\end{array}\right]
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right]
= 0.
\end{align}
%
Solutions for the amplification factor are roots of 
\begin{align}
g(A) = \det(G(A)) = g_{11} g_{22} - g_{12} g_{21} = 0.
\label{eq:ViscousDet}
\end{align}
%
\das{These coefficients are provided in ...}
\das{Clean this up...}
Although there are eight total projection coefficients 
$(\alpha_i,\beta_i,\gamma_i,\delta_i)$ for $i=1,2,$ the coefficients of $G$ only depend on three 
combinations of these coefficients, given by
\begin{align}
\psi_1 = \alpha_1 + \beta_1 - \gamma_1 - \delta_1, \qquad
\psi_2 = \alpha_2 + \beta_2 - \gamma_2 - \delta_2, \qquad
\psi_3 = \alpha_2-\delta_2.
\end{align}
%
In fact, when the coefficients are chosen so that $\psi_1=\psi_2=\psi_3=0,$ the matrix $G$
is diagonal. Here are four possible configurations.
\begin{align*}
\{\text{match jump terms: }  \alpha_j=\delta_j,\; \beta_j=\gamma_j,\; j=1,2 \} , 
\quad&\Rightarrow\quad \psi_1=\psi_2=\psi_3=0\\
\{\text{use solid, no jump: }  \alpha_j=\beta_j=\delta_j=\gamma_j=0,\; j=1,2  \},
\quad&\Rightarrow\quad \psi_1=\psi_2=\psi_3=0\\
\{\text{IWA, no jump: }  \alpha_j+\beta_j=1,\; \alpha_2=\alpha_F,\; \delta_j=\gamma_j=0,\; j=1,2  \}
\quad&\Rightarrow\quad \psi_1=\psi_2=1, \psi_3=\alpha_F\\
\{\text{use fluid, no jump: }  \alpha_j=\beta_j=1,\; \delta_j=\gamma_j=0,\; j=1,2  \}
\quad&\Rightarrow\quad \psi_1=\psi_2=2, \psi_3=1
\end{align*}
%
``Use solid'' and ``use fluid'' refer to using only the solid or fluid interface values in 
equations~\eqref{eq:project1}--\eqref{eq:project2}. ``IWA'' stands for impedance-weighted average.
By matching the coefficients of the jump terms, the FSI stability problem is equivalent to the
uncoupled solid problem. However, when jump terms are not used, the projection weights can
be chosen to produce a stable scheme.

Solutions for the amplification factor are the roots of the transcendental equation $g(A) = 0.$
The argument principle can be used to determine the number of unstable roots.
\begin{align}
\int_C \frac{g'(z)}{g(z)} \; dz
= 2 \pi i \left( n_{\text{roots}} - n_{\text{poles}} \right)
\end{align}
%
To determine the number of stable roots $|A| \le 1$, 
we integrate over the unit circle given by
\begin{alignat}{2}
z(\theta) &= e^{i \theta},\quad && \theta \in [0, 2 \pi].
\end{alignat}
%
In order to determine the total number of roots,
we integrate around a large circle of radius, $R$,
\begin{align}
z = R e^{i \theta}.
\end{align}
%
We take $R=?.$
If the total number of roots is equivalent to the number of stable roots, then the scheme is 
stable. Otherwise the scheme is unstable. 
Stability was assessed for 20 logarithmically spaced points in parameter space 
for $\Lambda$ and $Z$ 
in the interval $[10^{-3}, 10^{3}].$
For each pair of parameters, we take the max over the CFL region.
Figure \ref{fig:argPrinciple} shows the results of this computation.  
% \das{finish me}

% \begin{figure}[h]
% \centering
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi0_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi1_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi2_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi0_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi1_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi2_theta0_lxp1_lyp1.png}
% \caption{
%   I fixed $\lx=\ly=.1$ and varied the scheme (non-fractional-step: \texttt{iBC=1}, 
%   fractional-step: \texttt{iBC=2}) and choice of projection weights ($\psi=0,1,2$).
%   The only case that goes unstable is the bottom right, when the fluid values are used
%   instead of a projection in equations~\eqref{eq:project1}--\eqref{eq:project4}.
%   \label{fig:argPrinciple}
% }
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=.4\textwidth]{fig/iBC3_psi2_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC4_psi2_theta0_lxp1_lyp1.png}
% \caption{
%   Left: traditional. Right: anti-traditional.
%   \label{fig:argPrinciple}
% }
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=.4\textwidth]{fig/iBC3_psi2_theta0_lxp1_lyp1.png}
\includegraphics[width=.48\textwidth]{fig/iBC1_psi1_theta1_lxp1_lyp1.png}
\includegraphics[width=.48\textwidth]{fig/TPandATPstability}
\caption{
  Left: stability for AMP scheme. Right: stability regions for the TP and ATP schemes.
  \das{Eventually will run for more points in parameter space so region is less jagged.}
  \label{fig:argPrinciple}
}
\end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=\textwidth]{fig/ViscousContinuation_NL200_NZ50_nonfrac}
% \caption{Magnitude of maximum amplification factor for non-fractional-step scheme.
%   \das{Looks OK except for a point in the middle...}}
% \end{figure}



==> texFiles/viscousAnalysisOld4.tex <==
\section{Viscous analysis} \label{sec:viscousAnalysis}

In this section, the stability of the AMP, TP, and ATP algorithms 
are explored for a viscous model problem.
This extends the analysis of the inviscid model problem in~\cite{fib2014} to 
a viscous model problem. 
When viscosity is involved, stability is more challenging since instabilities 
arise from both added mass and added damping effects.
Due to this, both horizontal and vertical motions in the solid must be considered.
This relaxes the assumption in~\cite{fib2014} where the model problem was constrained 
to vertical motions only.
Another difficulty is the introduction of the viscous CFL number in the fluid as a 
new dimensionless parameter. 
In Section~\ref{sec:monolithic}, a fluid impedance was derived which is a function of 
the viscous CFL number. This impedance is used in the interface projection step of the 
AMP algorithm and is critical to achieving stability.

\subsection{Viscous model problem}

% \dws{Consider model problem MP-VA described in Section~\ref{sec:FSIModelProblems} and illustrated in Figure~\ref{fig:rectangularModelProblemCartoon} with $H \rightarrow \infty$.}
% \old{Consider model problem MP-VA described in Section~\ref{sec:FSIModelProblems}. }

The geometry of the model problem is shown in Figure
\ref{fig:rectangularModelProblemCartoon}. The fluid 
occupies the region $\Omega$ given by $0 < x < L$
and $0 < y < H$ and the solid occupies the semi-infinite region $\OmegaS$ given by 
$0 < x < L$ and $-\infty < y < 0.$ 
The fluid-solid interface $\Gamma$ is linearized about the flat surface, $y=0$,
and it is assumed that the vertical components of the velocity and stress between the
fluid and solid match along $\Gamma$. 
The solutions for the fluid and solid are assumed to be periodic in the $x$-direction 
with period equal to $L$. 

\input texFiles/rectangularModelProblemCartoon

\medskip
\noindent \textbf{Model Problem MP-VA}. \textit{Model problem MP-VA defines a 
  viscous incompressible fluid and an acoustic solid, where the pressure and shear waves
  propagate at the same speed. It is also assumed that $H\rightarrow \infty.$}
\bse
\begin{align}
&\text{Fluid: } \begin{cases}
\rho \partial_t\vv + \grad p = \mu \Delta \vv, & \xv\in\OmegaF \\
\Delta p = 0, & \xv \in \OmegaF \\
|\vv| \rightarrow 0, & y \rightarrow \infty \\
\grad \cdot \vv = 0, & \xv \in \Gamma
\end{cases},
\qquad
\text{Solid: } \begin{cases}
\rhos \partial_t \vsv = \grad \cdot \sigmasv, & \xv\in\OmegaS \\
\partial_t \sigmasv = -\mus (\grad \cdot \vv) \Iv \\
\phantom{\partial_t \sigmasv =}
+ \mus (\grad \vv + (\grad \vv)^T), & \xv\in\OmegaS \\
\bar{z} |\vsv|^2+|\sigmasv|^2 < \infty, & y\rightarrow - \infty
\end{cases}  \label{eq:mpvaEquations}\\
&\text{Interface: } \begin{cases}
\vv = \vsv, & \xv \in \Gamma\\
\sigmav \nv = \sigmasv \nv, & \xv \in \Gamma
\label{eq:mpvaInterface}
\end{cases}
\end{align}
\ese

We note here that the acoustic solid corresponds to the case of linear elasticity 
when $\lambdas = - \mus$. For this choice, it can be shown that both components of
the displacement satisfy the canonical wave equation with speed $\cb=\sqrt{\mus/\rho}.$
It is useful to write the equations in terms of characteristic variables given by
\begin{align}
\aone = \sigmas_{12} + \bar{z} \vs_1 , \quad
\bone = \sigmas_{12} - \bar{z} \vs_1, \quad
\atwo = \sigmas_{22} + \bar{z} \vs_2, \quad
\btwo = \sigmas_{22} - \bar{z} \vs_2, \quad
d = \sigmas_{11} + \sigmas_{22},
\label{eq:CharDef}
\end{align}
%
where
\begin{align}
\bar{z} = \rhos \bar{c}, \qquad \bar{c} = \sqrt{\mus \over \rhos}. 
\label{eq:solidImpedance}
\end{align}
%
The solid equations reduce to
\bse
\label{eq:advFull}
\begin{alignat}{2}
\partial_t \aone - \bar{c} \partial_y \aone &= \bar{c} (\partial_x d - \partial_x \btwo),
\quad & \xv \in \OmegaS \label{eq:advA1}\\
\partial_t \bone + \bar{c} \partial_y \bone &= \bar{c} (\partial_x \atwo - \partial_x d),
\quad & \xv \in \OmegaS \label{eq:advB1}\\
\partial_t \atwo - \bar{c} \partial_y \atwo &= \bar{c} \partial_x \bone, 
\quad & \xv \in \OmegaS \label{eq:advA2}\\
\partial_t \btwo + \bar{c} \partial_y \btwo &= - \bar{c} \partial_x \aone,
\quad & \xv \in \OmegaS \label{eq:advB2}\\
\partial_t d &= 0,
\quad & \xv \in \OmegaS \label{eq:advD}
\end{alignat}
\ese
%
Equations~\eqref{eq:advA1}--\eqref{eq:advB2} are advection equations for the incoming 
characteristic variables, $\aone$ and $\atwo$,
and the outgoing characteristic variables $\bone$ and $\btwo$, corresponding to the variables defined in equations~\eqref{eq:ACharacteristic}--\eqref{eq:BmCharacteristic} for $\nv=[0,-1]^T$. 
Equation~\eqref{eq:advD} states that that the characteristic $d$ will remain constant 
in time.

% The geometry of this model problem is shown in Figure \ref{fig:rectangularModelProblemCartoon}
% and discussed in Section~\ref{sec:FSIModelProblems}.
% The fluid is taken to be semi-infinite ($H \rightarrow \infty$).
% The governing equations for the fluid and solid are given in~\eqref{eq:mpvaEquations}
% while the interface conditions are given in~\eqref{eq:mpvaInterface}.
% The hyperbolic equations for the solid are considered in characteristic form by taking the
% transformations in~\eqref{eq:CharDef} to obtain the set in~\eqref{eq:advFull}.

\subsection{Discretization}

As in Section~\ref{sec:monolithic}, the solution is represented as a discrete Fourier series in the transverse direction following~\eqref{eq:discreteFourier}.  The Fourier coefficients of the fluid variables (with the hats and $k$ subscripts dropped) are governed by the system in~\eqref{eq:fourierFull}.  These equations are discretized in time using
\bse
\begin{align}
(v_1)^{n+1} &= (v_1)^n 
- \frac{i k_x \dt}{\rho} p^{*}
+ \nu \dt \left( - k_x^2 + \partial_y^2  \right) (v_1)^{n+1}, \label{eq:viscousV1}\\
(v_2)^{n+1} &= (v_2)^n 
- \frac{\dt}{\rho} \partial_y p^{*}
+ \nu \dt \left( - k_x^2 + \partial_y^2\right) (v_2)^{n+1}, \label{eq:viscousV2}\\
\left(-k_x^2 + \partial_y^2\right) p^{n+1} &= 0 .\label{eq:viscousP}
\end{align}
\ese
%
In this discretization, the viscous terms in~\eqref{eq:viscousV1} and~\eqref{eq:viscousV2} are treated implicitly, while the pressure gradient terms can be treated implicitly by setting $p^*=p^{n+1}$ or explicitly if $p^*=p^n$.  The latter case corresponds to an IMEX discretization.  As before, we enforce that the Fourier coefficents of the fluid are bounded as $y\rightarrow\infty$.

The equations for the Fourier coefficients of the solid variables corresponding to the characteristic form in~\eqref{eq:advFull} are discretized in both time and space using an upwind-type scheme given by
\bse
\begin{align}
(\aone)_j^{n+1} &= (\aone)_j^n + \ly ((\aone)_{j+1}^n-(\aone)_{j}^n) + i \lx ((d)_{j}^{n+1} - (\btwo)_{j}^{n+1}) \label{eq:schemeA1}\\
(\bone)_j^{n+1} &= (\bone)_j^n - \ly ((\bone)_{j}^n-(\bone)_{j-1}^n) + i \lx ((\atwo)_{j}^{n+1} - (d)_{j}^{n+1}) \label{eq:schemeB1}\\
(\atwo)_j^{n+1} &= (\atwo)_j^n + \ly ((\atwo)_{j+1}^n-(\atwo)_{j}^n) + i \lx (\bone)_{j}^{n+1} \label{eq:schemeA2}\\
(\btwo)_j^{n+1} &= (\btwo)_j^n - \ly ((\btwo)_{j}^n-(\btwo)_{j-1}^n) - i \lx (\aone)_{j}^{n+1} \label{eq:schemeB2}\\
(d)_j^{n+1} &= (d)_j^n, \label{eq:schemeD}
\end{align}
\ese
%
where, for example, $(\aone)_j^{n+1}\approx \aone(y_j,t_n)$ with $y_j = \left(j-\frac{1}{2}\right)\dy$, and where $\lx = \bar{c}\kx \dt$ and $\ly = \bar{c} \dt / \dy$.  The grid in the $y$-direction staggers the interface at $y=0$, which is done for later convenience.  The terms involving transverse derivatives are treated implicitly to stabilize the pseudo-spectral approximation. For reference, the solid velocity and stress are related to the characteristic variables by
\bse
\begin{align}
(\vs_1)_j^n = \frac{1}{2 \bar{z}} \left( (\aone)_j^n - (\bone)_j^n \right), \qquad
(\vs_2)_j^n = \frac{1}{2 \bar{z}} \left( (\atwo)_j^n - (\btwo)_j^n \right), \label{eq:solidGridVelocity}\\
(\sigmas_{12})_j^n = \frac{1}{2 } \left( (\aone)_j^n + (\bone)_j^n \right), \qquad 
(\sigmas_{22})_j^n = \frac{1}{2 } \left( (\atwo)_j^n + (\btwo)_j^n \right). \label{eq:solidGridStress}
\end{align}
\ese
%
We enforce that the solid solution remains bounded as $y\rightarrow -\infty$, which implies
\begin{align}
|(\aone)_j^n|^2 +  |(\bone)_j^n|^2 + |(\atwo)_j^n|^2 + |(\btwo)_j^n|^2 < \infty,
\quad \text{ as } j \rightarrow -\infty.
\end{align}

\old{
As in Section~\ref{sec:monolithic}, the solution is represented as a discrete Fourier series
in the transverse direction following~\eqref{eq:discreteFourier}.
The Fourier coefficients of the fluid variables (with the hats and $k$ subscripts dropped) are governed by the system
in~\eqref{eq:fourierFull}, while the equations for the solid variables are
\bse
\begin{alignat}{2}
\partial_t \aone - \bar{c} \partial_y \aone &= \bar{c} i k_x ( d - \btwo),
\label{eq:advA1Fouriero}\\
\partial_t \bone + \bar{c} \partial_y \bone &= \bar{c} i k_x ( \atwo -  d),
\\
\partial_t \atwo - \bar{c} \partial_y \atwo &= \bar{c} i k_x \bone, 
\\
\partial_t \btwo + \bar{c} \partial_y \btwo &= - \bar{c} i k_x \aone,
\\
\partial_t d &= 0.
\label{eq:advDFouriero}
\end{alignat}
\ese
The fluid is discretized in time and kept continuous in space. 
The temporal grid spacing is defined by $t_n = n \dt,$ with time step $\dt.$
The fluid scheme is a first-order Euler type scheme given by
\bse
\begin{align}
(v_1)^{n+1} &= (v_1)^n 
- \frac{i k_x \dt}{\rho} p^{*}
+ \nu \dt \left( - k_x^2 + \partial_y^2  \right) (v_1)^{n+1}, \label{eq:viscousV1o}\\
(v_2)^{n+1} &= (v_2)^n 
- \frac{\dt}{\rho} \partial_y p^{*}
+ \nu \dt \left( - k_x^2 + \partial_y^2\right) (v_2)^{n+1}, \label{eq:viscousV2o}\\
\left(-k_x^2 + \partial_y^2\right) p^{n+1} &= 0 .\label{eq:viscousPo}
\end{align}
\ese
%
The viscous terms are treated implicitly and the pressure gradient terms 
can either be treated implicitly ($p^*=p^{n+1}$) or explicitly ($p^*=p^n$).
The latter case corresponds to an IMEX discretization.
As in Section~\ref{sec:monolithic}, this is a system of differential-difference equations.
We enforce that the fluid velocity is bounded as $y\rightarrow\infty$.
Additionally, three conditions at the interface are required to close the system.

The solid characteristic variables are discretized in the $y$-direction using a
uniform staggered grid, defined by $y_j = \left(j-\frac{1}{2}\right) \dy$ for
$j = 1,0,-1,\dots$ with grid spacing $\dy$.
A staggered has been used previously in~\cite{fib2014} in the analysis of a first order upwind
scheme.
The solid equations in~\eqref{eq:advA1Fourier}--\eqref{eq:advDFourier} are approximated using a 
first-order accurate upwind-type scheme given by
\bse
\begin{align}
(\aone)_j^{n+1} &= (\aone)_j^n + \ly ((\aone)_{j+1}^n-(\aone)_{j}^n) + i \lx ((d)_{j}^{n+1} - (\btwo)_{j}^{n+1}) \label{eq:schemeA1o}\\
(\bone)_j^{n+1} &= (\bone)_j^n - \ly ((\bone)_{j}^n-(\bone)_{j-1}^n) + i \lx ((\atwo)_{j}^{n+1} - (d)_{j}^{n+1}) \label{eq:schemeB1o}\\
(\atwo)_j^{n+1} &= (\atwo)_j^n + \ly ((\atwo)_{j+1}^n-(\atwo)_{j}^n) + i \lx (\bone)_{j}^{n+1} \label{eq:schemeA2o}\\
(\btwo)_j^{n+1} &= (\btwo)_j^n - \ly ((\btwo)_{j}^n-(\btwo)_{j-1}^n) - i \lx (\aone)_{j}^{n+1} \label{eq:schemeB2o}\\
(d)_j^{n+1} &= (d)_j^n, \label{eq:schemeDo}
\end{align}
\ese
%
where $\lx = \kx \bar{c} \dt$ and $\ly = \bar{c} \dt / \dy.$ 
The terms involving transverse derivatives are treated implicitly to stabilize the 
pseudo-spectral approximation. For reference, the solid velocity and stress 
are related to the characteristic variables by
\bse
\begin{align}
(\vs_1)_j^n = \frac{1}{2 \bar{z}} \left( (\aone)_j^n - (\bone)_j^n \right), \quad
(\vs_2)_j^n = \frac{1}{2 \bar{z}} \left( (\atwo)_j^n - (\btwo)_j^n \right), \label{eq:solidGridVelocityo}\\
(\sigmas_{12})_j^n = \frac{1}{2 } \left( (\aone)_j^n + (\bone)_j^n \right), \quad 
(\sigmas_{22})_j^n = \frac{1}{2 } \left( (\atwo)_j^n + (\btwo)_j^n \right). \label{eq:solidGridStresso}
\end{align}
\ese
%
We enforce that the solid solution remains bounded as $y\rightarrow -\infty$.
This implies
\begin{align}
|(\aone)_j^n|^2 +  |(\bone)_j^n|^2 + |(\atwo)_j^n|^2 + |(\btwo)_j^n|^2 < \infty,
\quad \text{ as } j \rightarrow -\infty.
\end{align}
}

\subsection{Interface coupling}

We explore different choices of interface coupling for the AMP, TP, and ATP schemes.
We also distinguish between a 
{\em fully-coupled scheme} for the fluid, where the velocity and 
pressure are solved in the same step, and a 
{\em fractional-step scheme}, where the velocity and pressure are solved separately.
For the fully-coupled scheme, the pressure gradient terms are treated implicitly so that $p^*=p^{n+1}$
is taken in~\eqref{eq:viscousV1} and~\eqref{eq:viscousV2}.
On the other hand, we set $p^*=p^{n}$ for the fractional-step scheme. 

We first consider the AMP interface conditions for the fully-coupled scheme.
The first two conditions are formed by equating the two outgoing characteristic variables of the solid
to the analogous quantities of the fluid following~\eqref{eq:BCharacteristic} and~\eqref{eq:BmCharacteristic}.
The third condition is obtained by setting the velocity to be divergence-free on the interface.  These
three conditions are summarized as follows:

\medskip
\noindent \textbf{Fully-coupled AMP conditions}: 
\textit{The interface conditions for the fully-coupled scheme (with $p^*=p^{n+1}$) are given by}
\bse
\begin{alignat}{2}
\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right) - \zb (v_1)^{n+1} 
&= (\sigmas_{12})^{n+1}_{\das{0}} - \zb (\vs_1)^{n+1}_{\das{0}}, \qquad && y=0, \label{eq:v1ConditionCoupled} \\
-p^{n+1} + 2 \mu \partial_y (v_2)^{n+1} - \zb (v_2)^{n+1} 
&= (\sigmas_{22})^{n+1}_{\das{0}} - \zb (\vs_2)^{n+1}_{\das{0}}, \qquad && y=0, \label{eq:v2ConditionCoupled}\\
i k_x (v_1)^{n+1} + \partial_y (v_2)^{n+1} 
&= 0,  \qquad && y=0. \label{eq:divConditionCoupled}
\end{alignat}
\ese
\textcolor{red}{What is done about the staggered grid here???  Previously, it had been $j=0$ which corresponds to $y=-1/2$???} 
\das{das: $j=0$ is the `boundary' point and $j=1$ is the `ghost' point. The above condition
  is using constant-order extrapolation. (This was done in FIB)}

\dws{Stopping edits for now until I have a chance to consult with Dan...}
We now derive suitable interface conditions for the fractional-step scheme. 
Equation~\eqref{eq:v2ConditionCoupled} sets the fluid velocity in the heavy solid limit
and the pressure in the light solid limit. 
A decoupled pressure condition can be derived from 
equation~\eqref{eq:v2ConditionCoupled} and 
equation~\eqref{eq:divConditionCoupled}.
The first condition can be derived by eliminating $(v_2)^{n+1}$ and
$(\vs_2)^{n+1}_0$ in equation~\eqref{eq:v2ConditionCoupled} using a backward-Euler type scheme.
\bse
\begin{align}
(v_2)^{n+1} &= \tilde{v}_2
- \frac{\dt }{\rho} \partial_y p^{n+1} 
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}),\\
(\vs_2)^{n+1}_0 &= \tilde{v}_2
+ \dt (\dot{\vs}_2)^{n+1}_0
\end{align}
\ese
%
Here, 
equation~\eqref{eq:divConditionCoupled} was used to make the substitution
$\partial_y^2 (v_2)^{n+1} = -i k_x \partial_y (v_1)^{n+1}$ and 
$(\dot{\vs}_2)$ represents the solid interface acceleration. 
The scheme is centered around $\tilde{v}_2,$ which is taken to be an 
interface velocity at time $t^{n}.$
After substitution, a mixed condition for the pressure is derived.
\begin{align}
-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} 
=\;& (\sigmas_{22})^{n+1}_0 + 2 i k_x \mu  (v_1)^{n+1} 
- \zb \dt (\dot{\vs}_2)^{n+1}_0 \nonumber \\
&
+\nu \zb \dt \left( -k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1} \right)
\label{eq:pressureConditionFractional}
\end{align}
%
Again, equation~\eqref{eq:divConditionCoupled} was used to replace
$\partial_y (v_2)^{n+1} = -i k_x v_1^{n+1}.$
This condition replaces equation~\eqref{eq:v2ConditionCoupled}. 
Since the fluid velocity is no longer set in the heavy solid limit, 
we introduce the following projection condition for the fluid velocity.
\begin{align}
(v_2)^{n+1} = \alpha_F \left((v_2)^{n} 
- \frac{\dt }{\rho} \partial_y p^{n} 
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}) 
\right)
+ (1-\alpha_F) (\vs_2)^{n+1}_0.
\label{eq:velocityConditionFractional}
\end{align}
%
That is, the fluid velocity on the interface is set to be a weighted average of the 
velocity predicted from the fluid scheme and the predicted solid velocity.
Here, $\alpha_F$ is chosen based on the fluid and solid impedances and is given by
\begin{align}
\alpha_F = \frac{\zf}{\zf+\zb},
\end{align}
%
where the fluid impedance $\zf$ is taken to be
\begin{align}
\zf = \rho v_f, \qquad v_f = 2\nu k_x + \frac{1}{k_x \dt},
\end{align}
%
as derived in Section~\ref{sec:monolithic}.
We can now summarize the fractional-step conditions.

\bigskip
\noindent \textbf{Fractional-step AMP conditions}: \textit{The pressure gradient terms are treated explicitly ($p^* = p^{n}$)
and the following conditions are applied at $y=0$.
}
\bse
\begin{align}
&\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right) - \zb (v_1)^{n+1} 
= (\sigmas_{12})^{n+1}_0 - \zb (\vs_1)^{n+1}_0, \label{eq:fracTangential} \\
&(v_2)^{n+1} = \alpha_F \bigg{(} (v_2)^{n} 
- \frac{\dt }{\rho} \partial_y p^{n+1}
+ \nu \dt (-k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1}) 
\bigg{)} \nonumber \\
&\phantom{(v_2)^{n+1} =\;}
+ (1-\alpha_F) (\vs_2)^{n+1}_0.
\label{eq:fracProject}\\
&-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} 
= (\sigmas_{22})^{n+1}_0 + 2 i k_x \mu  (v_1)^{n+1} 
- \zb \dt (\dot{\vs}_2)^{n+1}_0 \nonumber \\
&
\phantom{-p^{n+1}  + \frac{\zb \dt}{\rho} \partial_y p^{n+1} =\;}
+\nu \zb \dt \left( -k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1} \right)
\label{eq:fracPressure} 
\end{align}
\ese
%
Analogous conditions for the TP and ATP scheme can be formed by taking the proper 
limits of equations~\eqref{eq:fracTangential}--\eqref{eq:fracProject}.
In the heavy solid limit, equations~\eqref{eq:fracTangential}--\eqref{eq:fracProject}
become Dirichlet conditions for the velocity and equation~\eqref{eq:fracPressure}
becomes a Neumann compatibility condition for the pressure.

\bigskip
\noindent \textbf{Fractional-step TP conditions}: \textit{The pressure gradient terms are treated explicitly ($p^* = p^{n}$)
and the following conditions are applied at $y=0$.
}
\bse
\begin{align}
(v_1)^{n+1} 
&=  (\vs_1)^{n+1}_0, \label{eq:TPTangential} \\
(v_2)^{n+1} &= (\vs_2)^{n+1}_0.
\label{eq:TPNormal} \\
\partial_y p^{n+1} 
&= 
- (\dot{\vs}_2)^{n+1}_0 
+\nu \left( -k_x^2 (v_2)^{n+1} - i k_x \partial_y (v_1)^{n+1} \right)
\label{eq:TPPressure} 
\end{align}
\ese

In the light solid limit, equation~\eqref{eq:fracTangential}
becomes a condition on the tangential stress.
Equation~\eqref{eq:fracProject} reduces to the numerical scheme for 
$(v_2)^{n+1}$ with the modification $\partial_y^2(v_2)^{n+1} = - i k_x \partial_y (v_1)^{n+1}$.
In the ATP scheme, the divergence free condition is enforced,
$\partial_y(v_2)^{n+1} = - i k_x (v_1)^{n+1}.$
Equation~\eqref{eq:fracPressure}
simplifies to a Dirichlet condition for the pressure.

\bigskip
\noindent \textbf{Fractional-step ATP conditions}: \textit{The pressure gradient terms are treated explicitly ($p^* = p^{n}$) and the following conditions are applied at $y=0$.
}
\bse
\begin{align}
\mu \left( i k_x (v_2)^{n+1} + \partial_y (v_1)^{n+1} \right)
&= (\sigmas_{12})^{n+1}_0, \label{eq:ATPV1} \\
i k_x (v_1)^{n+1} + \partial_y (v_2)^{n+1} 
&= 0. \label{eq:ATPDiv}\\
-p^{n+1} + 2 \mu \partial_y (v_2)^{n+1} 
&= (\sigmas_{22})^{n+1}_0, \label{eq:ATPP}
\end{align}
\ese

\dws{Still confused about the staggered grid.}
The evolution of the solid requires boundary conditions for the two incoming 
characteristics at $y=0,$ namely 
\bse
\begin{align}
(\aone)_1^{n+1} &= (\sigma_{12})_I^{n+1}+ \zb (v_1)_I^{n+1}, \label{eq:a1CharBoundary}\\
(\atwo)_1^{n+1} &= (\sigma_{22})_I^{n+1}+ \zb (v_2)_I^{n+1}, \label{eq:a2CharBoundary}
\end{align}
\ese
%
where $(v_1)_I^{n+1}, (v_2)_I^{n+1}, (\sigma_{12})_I^{n+1}$, and $(\sigma_{22})_I^{n+1}$
are interface velocities and stresses projected from fluid and solid values, given by
\bse
\begin{align}
(v_1)_I^{n+1} &= \alpha (v_{1})_f^{n+1} 
+ (1-\alpha) (\vs_1)_0^{n+1}
+ \gamma_1 \bar{z}^{-1} ( (\sigmas_{12})_0^{n+1} - (\sigma_{12})_f^{n+1}  ), \label{eq:project1}\\
(v_2)_I^{n+1} &= \alpha (v_{2})_f^{n+1}
+ (1-\alpha) (\vs_2)_0^{n+1}
+ \gamma \bar{z}^{-1} ( (\sigmas_{22})_0^{n+1} - (\sigma_{22})_f^{n+1}  ), \label{eq:project2}\\
(\sigma_{12})_I^{n+1} &= \beta (\sigma_{12})_f^{n+1}
+ (1-\beta) (\sigmas_{12})_0^{n+1}
+ \delta \bar{z} ( (\vs_1)_0^{n+1} - (v_1)_f^{n+1} ), \label{eq:project3}\\
(\sigma_{22})_I^{n+1} &= \beta (\sigma_{22})_f^{n+1}
+ (1-\beta) (\sigmas_{22})_0^{n+1}
+ \delta \bar{z} ( (\vs_2)_0^{n+1} - (v_2)_f^{n+1} ).\label{eq:project4}
\end{align}
\ese
% \begin{align}
% (v_1)_I^{n+1} &= \alpha_1 (v_{1})_f^{n+1} 
% + (1-\alpha_1) (\vs_1)_0^{n+1}
% + \gamma_1 \bar{z}^{-1} ( (\sigmas_{12})_0^{n+1} - (\sigma_{12})_f^{n+1}  ), \label{eq:project1}\\
% (v_2)_I^{n+1} &= \alpha_2 (v_{2})_f^{n+1}
% + (1-\alpha_2) (\vs_2)_0^{n+1}
% + \gamma_2 \bar{z}^{-1} ( (\sigmas_{22})_0^{n+1} - (\sigma_{22})_f^{n+1}  ), \label{eq:project2}\\
% (\sigma_{12})_I^{n+1} &= \beta_1 (\sigma_{12})_f^{n+1}
% + (1-\beta_1) (\sigmas_{12})_0^{n+1}
% + \delta_1 \bar{z} ( (\vs_1)_0^{n+1} - (v_1)_f^{n+1} ), \label{eq:project3}\\
% (\sigma_{22})_I^{n+1} &= \beta_2 (\sigma_{22})_f^{n+1}
% + (1-\beta_2) (\sigmas_{22})_0^{n+1}
% + \delta_2 \bar{z} ( (\vs_2)_0^{n+1} - (v_2)_f^{n+1} ).\label{eq:project4}
% \end{align}
%
Here, $(v_1)_f, (v_2)_f, (\sigma_{12})_f,$ and $(\sigma_{22})_f$ are fluid interface values at $y=0.$
The choice of projection coefficients $(\alpha,\beta,\gamma,\delta)$ 
is determined by the choice of interface coupling and is shown in 
Table~\ref{tab:projectionCoeffs}.
For the AMP scheme, coefficients are chosen according to the impedance weighted average formula. 
For the TP scheme, coefficients are chosen so the interface velocity is taken to be the
solid velocity and the interface traction is taken to be the fluid traction.
For the ATP scheme, coefficients are chosen so the interface velocity is taken to be the
fluid velocity and the interface traction is taken to be the solid traction.

{
\begin{table}[h]
\centering
\caption{Choice of projection coefficients for the AMP, TP, and ATP schemes.
\label{tab:projectionCoeffs}}
\begin{tabular}{c|cccc}
scheme & $\alpha$ & $\beta$ & $\gamma$ & $\delta$ \\
\hline
AMP & $\frac{\zf}{\zf+\zb}$ & $\frac{\zf^{-1}}{\zf^{-1}+\zb^{-1}}$ & $\frac{\zf^{-1}}{\zf^{-1}+\zb^{-1}}$ & $\frac{\zf}{\zf+\zb}$\\
TP & $0$ & $1$ & $0$ & $0$ \\
ATP & $1$ & $0$ & $0$ & $0$
\end{tabular}
\end{table}
}


\subsection{Stability analysis}

\dws{As I am looking through this I am wondering if we ever actually consider the \lq\lq fully-coupled'' scheme...}
In order to assess the stability of the AMP, TP and ATP schemes, 
we search for normal mode solutions to the discretization. In the fluid,
solutions are of the form,
\begin{align}
(v_1)^n(y) = A^n \tilde{v}_1(y), \quad 
(v_2)^n(y) = A^n \tilde{v}_2(y), \quad
p^n(y) = A^n \tilde{p}(y),
\end{align}
%
where $A$ is the amplification factor and $(\tilde{v}_1(y), \tilde{v}_2(y),\tilde{p})$
are functions of space given by
\bse
\begin{align}
\tilde{v}_1(y) &= \left((v_1)_f + \frac{i p_f}{z_\mu s^* (\gamma^2 - 1)} \right) e^{-k_x \gamma y}
- \frac{i p_f}{z_\mu s^* (\gamma^2 - 1)} e^{-k_x y}, \\
\tilde{v}_2(y) &= \left((v_2)_f - \frac{p_f}{z_\mu s^*(\gamma^2 - 1)} \right) e^{-k_x \gamma y}
+ \frac{p_f}{z_\mu s^* (\gamma^2 - 1)} e^{-k_x y}, \\
\tilde{p}(y) &= p_f e^{-k_x y},
\end{align}
\ese
%
where $\zm$, $\Lambda$ and $\gamma$ take on similar definitions in 
Section~\ref{sec:monolithic} and are given by
\begin{align}
z_\mu = \mu \das{k_x}, \qquad
\Lambda = \nu \das{k_x^2} \dt, \qquad
\gamma = \sqrt{\frac{1}{\Lambda}\frac{A-1}{A} + 1}.
\end{align}
%
\dws{Should $k$ really be $k_x$ and is it that helpful to define $z_\mu$?  Maybe we can avoid defining another $z$???}
\das{new:}
\begin{align}
\das{\Lambda = \nu \das{k_x^2} \dt, \qquad
\gamma = \sqrt{\frac{1}{\Lambda}\frac{A-1}{A} + 1}, \qquad
\theta= \frac{\zb}{\mu \kx}}
\end{align}
\das{The above definitions look like the current definitions in Section~\ref{sec:monolithic}.
  Do we want to use $\theta$ for the impedance ratio?}
Additionally, $s^* = A$ when $p^* = p^n$ and $s^* = 1$ when $p^*=p^{n+1}.$
As before, $z_\mu$ is a viscous impedance and $\Lambda$ is a viscous CFL number.
The constants, $(v_1)_f, (v_2)_f$, and $p_f$ are obtained by
enforcing the three fluid boundary conditions (ie.
equations~\eqref{eq:v1ConditionCoupled}--\eqref{eq:divConditionCoupled} for the fully-coupled 
AMP scheme,
equations~\eqref{eq:fracTangential}--\eqref{eq:fracPressure} for the fractional-step AMP scheme,
equations~\eqref{eq:TPTangential}--\eqref{eq:TPPressure} for the fractional-step TP scheme,
or
equations~\eqref{eq:ATPV1}--\eqref{eq:ATPP} for the fractional-step ATP scheme)
for each set of boundary conditions.

% \begin{align}
% (v_1)_f &= -\frac{(\gamma^2+\gamma) z_\mu + \zb}{ \zb E} b_1 
%           + \frac{i z_\mu (\gamma-1)}{ \zb E} b_2 \\
% (v_2)_f &= -\frac{i z_\mu (\gamma - 1)}{ \zb E} b_1 
%           - \frac{(\gamma+1) z_\mu + \zb}{\zb E} b_2 \\
% p_f &= \frac{i (2 \gamma Z + 1) (\gamma + 1) Z}{E} b_1
%       - \frac{(\gamma+1) (\gamma^2 Z + \gamma + Z) Z}{E} b_2
% \end{align}

% \begin{align}
% E = (\gamma^3 + \gamma^2 + 3 \gamma - 1) Z^2 + (\gamma+1)^2 Z + 1
% \end{align}

We now search for solutions to the solid discretization. 
Let $\av_j^n = [(\aone)_j^n$,$ (\bone)_j^n$, $(\atwo)_j^n$, $(\btwo)_j^n$,$ (d)_j^n]^T.$
Solutions are sought of the form, $\av_j^n =  \phi^j A^n \tilde{\rv},$
where $\phi$ is a spacial eigenvalue and $\tilde{\rv}$ is a constant eigenvector.
The scheme is said to be weakly stable if there are no non-trivial solutions with $|A| > 1$.  
Our strategy for determining regions of stability will be to search for unstable modes with 
$|A| > 1$, and then identify regions of the parameter space where no non-trivial solution exist.  
To do this, we begin by finding the general solution for the spatial grid functions satisfying 
the discrete equations and regularity condition as $j\rightarrow-\infty$, assuming $|A| > 1$.  
We then apply the conditions at the interface to determine whether non-trivial solutions exist.
When the normal mode ansatz is substituted into the numerical scheme for the solid in 
equations \eqref{eq:schemeA1}--\eqref{eq:schemeD}, a homogeneous system arises of the form
% what should we call this matrix?
\newcommand{\SolidMatrixB}{Q}
\begin{align}
\SolidMatrixB(\phi) \tilde{\rv} = 0.
\end{align}
The matrix $\SolidMatrixB(\phi)$ is given by
\begin{align*}
\SolidMatrixB(\phi) = \left[\begin{array}{ccccc}
\eta(\phi) & 0 &  0& -i A \lx & i A \lx  \\
0 & \eta(1/\phi) & i A \lx & 0 & -i A \lx \\
0 & i A \lx & \eta(\phi) & 0 & 0 \\
-i A \lx & 0 & 0 & \eta(1/\phi) & 0 \\
0 & 0 & 0 & 0 & 1-A
\end{array}\right],
\end{align*}
%
where
\begin{align}
\eta(\phi) = 1-A+\ly (\phi-1).
\end{align}
%
This system is singular when $f(\phi) \defeq \det (\SolidMatrixB(\phi)) = 0.$
The function $f(\phi)$ can be written as 
\begin{align}
f(\phi) = (1-A) \left(\eta(\phi) \eta(1/\phi) + (A \lx)^2\right)^2,
\label{eq:SolidDetCond}
\end{align}
%
which is zero when $A=1$ or when $\eta(\phi) \eta(1/\phi) + (A \lx)^2 = 0.$
Since we are interested in searching for unstable modes, we are interested in the latter 
case. Roots of $f(\phi)$ can be written in the form
\newcommand{\bParam}{\theta}
\begin{align}
\phi_\pm = \bParam \pm \sqrt{\bParam^2 - 1}, \qquad 
\bParam = 1 - \frac{(A \lx)^2 + (1-A)^2}{2 \ly (1-A-\ly)}.
\end{align}
%
The product of the roots is equal to one ($\phi_+ \phi_- = 1$).
Since we are searching for solutions that are bounded as $j\rightarrow -\infty,$ 
we are only interested in the root with modulus greater than 1.

\medskip
\noindent\textbf{Lemma}: \textit{If $|A|>1$ and if $\lx$ and $\ly$ are chosen to satisfy a CFL 
condition, then there is precisely one root (either $\phi_+$ or $\phi_-$), denoted by 
$\phi_*$ that has magnitude strictly greater than one, $|\phi_*| > 1.$}
\medskip

\noindent This result follows from a similar argument to that given 
in~\cite{DifferenceApproximationsForTheInitialBoundary}.  
We first consider the scheme applied to the pure initial-value problem (Cauchy problem).  
Setting $\phi=e\sp{i\vartheta}$ in~\eqref{eq:SolidDetCond}, we determine a region of 
the $\lx$-$\ly$ plane for which $\vert A\vert\le1$ for all $\vartheta\in[0,2\pi]$.  
This region is found numerically as discussed in~\ref{sec:CFLRegionCauchy}
and shown in Figure~\ref{fig:viscousCFL}, and it corresponds 
to a region where the Cauchy problem is (Fourier) stable.  It is also shown that this stability 
region includes a region of $(\lx,\ly)$ satisfying a reasonable CFL restriction, 
namely $\lx\sp2+\ly\sp2\le1$.
Next, since $|A| \le 1$ when $|\phi| = 1$, we have that $|\phi| \ne 1$ when $|A| > 1$.  
Thus, if $|A| > 1$ and if $(\lx,\ly)$ remains within the CFL restriction, then $\phi$ cannot 
cross the unit circle, $|\phi|=1$, as $(\lx,\ly)$ vary.  
It is therefore only necessary to prove that the lemma holds for one set of parameters.  
For $\lx=0$, the discretization reduces to four uncoupled upwind schemes for linear advection. 
In this case, equation~\eqref{eq:SolidDetCond} is equivalent to 
$\eta(\phi) \eta(1/\phi) = 0,$
%
which has solutions
$\phi_+ = (A-1+\ly)/\ly$ and $\phi_- = 1/\phi_+$.
%
When $|A|>1$ and $\ly \in (0,1]$, $|\phi_+|>1$ and therefore $\phi_* = \phi_+.$ 
Thus, the condition holds for all $(\lx,\ly)$ provided the CFL condition is satisfied.

%
When $\phi=\phi_*,$ there are two eigenvectors, namely
\begin{align}
\tilde{\rv}_1 = 
\left[
\frac{\eta(1/\phi_*)}{i A\lx},\, 0,\, 0,\, 1,\, 0
\right]^T, \qquad 
\tilde{\rv}_2 = 
\left[
0,\, -\frac{\eta(\phi_*)}{i A\lx},\, 1,\, 0,\, 0
\right]^T
.
\end{align}
%
The solution which remains bounded as $j \rightarrow -\infty$ is given by
\begin{align*}
(\aone)_j^{n} = k_1 \frac{ \eta(1/\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
(\bone)_j^{n} = -k_2 \frac{ \eta(\phi_*) }{i A \lx} \phi_*^{j-1} A^n, \quad
(\atwo)_j^{n} = k_2 \phi_*^{j-1} A^n, \quad
(\btwo)_j^{n} = k_1 \phi_*^{j-1} A^n,
\end{align*}
%
where $k_1$ and $k_2$ are free constants to be determined by the interface conditions.
The discrete solutions are plugged into the boundary conditions, equations
\eqref{eq:a1CharBoundary}--\eqref{eq:a2CharBoundary},
to form another homogeneous system of equations, given by
\begin{align}
\dMat(A) \kv = \left[\begin{array}{cc}
g_{11} & g_{12} \\ 
g_{21} & g_{22}
\end{array}\right]
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right]
= 0.
\label{eq:StabilitySystemViscous}
\end{align}
%
The coefficients of the matrix $\dMat$
are provided in~\ref{sec:ComponentsOfDmatViscous} for the AMP, TP, and
ATP schemes.
Solutions for the amplification factor are roots of 
\begin{align}
\dMat(A) = \det(\dMat(A)) = g_{11} g_{22} - g_{12} g_{21} = 0.
\label{eq:ViscousDet}
\end{align}
%


Solutions for the amplification factor are the roots of the transcendental 
equation~\eqref{eq:ViscousDet}, which is dependent on the choice of interface coupling and the 
four dimensionless parameters ($\Lambda, Z, \lx, \ly$).
Given the interface coupling and dimensional parameters, proving stability is equivalent to 
showing that there exist no roots of equation~\eqref{eq:ViscousDet} such that $|A|>1$.
The argument principle is applied to determine the number of unstable roots to the 
complex function $h(z) \defeq g(z^{-1}).$
\begin{align}
\mathcal{P} = \frac{1}{2 \pi i}\oint_C \frac{h'(z)}{h(z)} \; dz,
\qquad
C = \{z : z = e^{i \theta}, \theta = [0,2 \pi] \} 
\end{align}
%
It can be shown that the only branch cuts of $h(A)$ are located in the region $|A|>1$. 
In the region $|A|\le 1,$ there is a pole of order $2$ at the origin.
Therefore $\mathcal{P} = N-2$ where $N$ is the number of roots of $g(A)$ 
with $|A|>1$~\cite{carrier05}. 
By making the substitutions $h(z) = g(z^{-1}),$
$h'(z) = -z^{-2} g'(z^{-1}),$ 
$z = e^{i \theta},$ 
and $dz = i e^{i \theta} d \theta,$ it can be shown that $\mathcal{P}$ is equivalent to 
\begin{align}
\mathcal{P} &= -\frac{1}{2 \pi} \int_{0}^{2 \pi} \frac{g'(e^{-i\theta})}{  g(e^{-i\theta})} e^{- i \theta} \; d\theta. \label{eq:argPrinciple}
\end{align}
%
The number $\mathcal{P}$ was computed for a 31$\times$31$\times$20$\times$20
array of parameter values in the ($Z$,$\Lambda$,$\lx$,$\ly$) parameter space.
The parameters $Z$ and $\Lambda$ are logarithmically spaced in the 
interval $[10^{-3}, 10^{3}]$ 
while $\lx$ and $\ly$ are chosen to be equally spaced in the interval
$[0.05, 0.95]$.
A stable problem corresponds to $N=0$ and therefore $\mathcal{P}=-2$.
Results of this computation are shown in Figure~\ref{fig:argPrinciple}.
For each point $(\Lambda,Z)$, the computation of $\mathcal{P}$ is repeated for
all $\lx$ and $\ly$ in the search region. If any point in this search region is unstable,
then the point $(\Lambda,Z)$ is added to the region of instability.
The parameter search resulted in no unstable roots found for the AMP scheme. 
However, there are significant regions where The TP and ATP schemes are unstable.

\medskip
\noindent\textbf{Theorem}: \textit{By numerical evaluation of $\mathcal{P},$ we have found that
the AMP algorithm is weakly stable $(|A| \le 1)$ provided that $\lx^2 + \ly^2 \le 1,$ i.e.}
\begin{align}
\dt \le \frac{1}{\cb} \left[ \frac{1}{\dy^2} + k_x^2\right]^{1/2}.
\end{align}
\textit{This is a sufficient but not a necessary condition.}

% \das{finish me}

% \begin{figure}[h]
% \centering
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi0_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi1_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC1_psi2_theta1_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi0_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi1_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC2_psi2_theta0_lxp1_lyp1.png}
% \caption{
%   I fixed $\lx=\ly=.1$ and varied the scheme (non-fractional-step: \texttt{iBC=1}, 
%   fractional-step: \texttt{iBC=2}) and choice of projection weights ($\psi=0,1,2$).
%   The only case that goes unstable is the bottom right, when the fluid values are used
%   instead of a projection in equations~\eqref{eq:project1}--\eqref{eq:project4}.
%   \label{fig:argPrinciple}
% }
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=.4\textwidth]{fig/iBC3_psi2_theta0_lxp1_lyp1.png}
% \includegraphics[width=.4\textwidth]{fig/iBC4_psi2_theta0_lxp1_lyp1.png}
% \caption{
%   Left: traditional. Right: anti-traditional.
%   \label{fig:argPrinciple}
% }
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=.4\textwidth]{fig/iBC3_psi2_theta0_lxp1_lyp1.png}
\includegraphics[width=.48\textwidth]{fig/AMPstabilityViscousAnalysis}
\includegraphics[width=.48\textwidth]{fig/TPandATPstabilityViscousAnalysis}
\caption{
  Left: Green circles represent points for which 
  the fully-coupled AMP algorithm and fractional-step AMP algorithm
  are stable in the CFL region $\lx^2+\ly^2\le 1$.
  Right: stability regions for the TP (red) and ATP (blue) schemes.
  \label{fig:argPrinciple}
}
\end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=\textwidth]{fig/ViscousContinuation_NL200_NZ50_nonfrac}
% \caption{Magnitude of maximum amplification factor for non-fractional-step scheme.
%   \das{Looks OK except for a point in the middle...}}
% \end{figure}


